Stochastic Analysis in Problems, part 1 (in Russian)

This book contains a large number of exercises related to different stochastic disciplines. Difficulty of the problems varies from the basic level in the first chapter up to the analysis of articles in Probability, Statistics and Computer Science. Range of the given exercises covers most of the significant classical results of the area including techniques that arise in modern stochastic disciplines. The book is recommended for the course "Stochastic Analysis in problems" which is held by the Department of Mathematical Foundations of Control in Moscow Institute of Physics and Technology. Content of the book may be used for practical classes, exams and for self-education reasons in various stochastic disciplines.

==> 123.tex <==
\section{Метод Монте-Карло}
\label{MK}

\begin{problem}
На плоскости дано ограниченное измеримое по Лебегу множество $S$. Требуется найти площадь (меру Лебега) этого множества с заданной точностью 
$\varepsilon$. 

Поскольку по условию множество ограничено, то вокруг него можно описать квадрат со стороной $a$. Выберем декартову систему координат 
в одной из вершин квадрата с осями, параллельными сторонам квадрата. Рассмотрим $n$  независимых с.в. $\{ X_k\}_{k=1}^{n}$,  имеющих 
одинаковое равномерное распределение в этом квадрате, т.е. $X_k\in R([0,a]^2)$. Введем с.в. 
$$
Y_k=I(X_k\in S)=\begin{cases}
1,\quad X_k\in S,\\
0, \quad X_k\notin S.
\end{cases} 
$$
Тогда $\{ Y_k\}_{k=1}^{n}$ --- независимые одинаково распределенные с.в.. Ясно, что $Y_k\in\Be(p(S))$. Следовательно, по УЗБЧ 
$$
\frac{Y_1+\ldots+Y_n}{n} \xrightarrow{\text{ п.н. }} {\mathbb E}(Y_1)=p(S)=\frac{\mu(S)}{a^2} \quad \text{ при  } n\to\infty . 
$$
Оцените сверху следующую вероятность:
$$
{\mathbb P}\Bigl( \Bigl| \frac{Y_1+\ldots+Y_n}{n}-\frac{\mu(S)}{a^2}\Bigr|>\delta \Bigr) . 
$$
\end{problem}

\begin{ordre}
См. раздел 5, а также часть 2.
\end{ordre}


\begin{problem}(Вычисление значения интеграла.) а) Требуется вычислить с заданной точностью $\varepsilon $ и с заданной доверительной вероятностью $\gamma $ абсолютно сходящийся интеграл 
\[
J=\int _{\left[0,\; 1\right]^{m} }f\left({x}\right)d{x}.
\] Считайте, что $\forall \; \; {x}\in \left[0,\; 1\right]^{m}$  выполнено $\left|f\left({x}\right)\right|\le 1$.

\begin{remark}
Введем случайный $m$-вектор ${X}\in R\left(\left[0,\; 1\right]^{m} \right)$ и с.в. $\xi =f\left({X}\right)$. Тогда $\Exp\xi =\int _{\left[0,\; 1\right]^{m} }f\left({x}\right)d{x} =J$. Поэтому получаем оценку интеграла $\bar{J}_{n} =\frac{1}{n} \sum _{k=1}^{n}f\left(\tilde{X}_{k} \right) $, где $\tilde{X}_{k} $, $k=1,...,n$ --- повторная выборка значений случайного вектора ${X}$ (т.е. все $\tilde{x}_{k} $, $k=\overline{1,n}$,  независимы и одинаково распределены: так же, как и вектор $X$). В задаче требуется оценить сверху число $n$ ($n\gg m$), начиная с которого $\mathbb{P}\left(\left|J-\bar{J}_{n} \right|\le \varepsilon \right)\ge \gamma $.
\end{remark}



\indent б) Решите задачу из п. а) при дополнительном предположении липшецевости функции $f\left({x}\right)$, разбив единичный куб на $n=N^{m} $ одинаковых кубиков со стороной ${1\mathord{\left/ {\vphantom {1 N}} \right. \kern-\nulldelimiterspace} N} $ и используя оценку $\bar{J}_{n} =$\linebreak $=\frac{1}{n} \sum _{k=1}^{n}f\left(\tilde{X}_{k} \right) $, где $\tilde{X}_{k} $ --- имеет равномерное распределение в \textit{k}-м кубике.

\indent в) (Метод включения особенности в плотность.) Решите задачу \linebreak п. а), не предполагая, что $f\left({x}\right)$ --- ограниченная функция на единичном кубе. Предложите способы уменьшения дисперсии полученной оценки интеграла. Как можно использовать информацию об особенностях функции $f\left({x}\right)$?
\end{problem}
\begin{ordre}
См. книгу Соболь И.М. Численный метод Монте-Карло. -- М.: Наука, 1973, а также \cite{24}.
\end{ordre}

\begin{problem}Стандартный способ моделирования с.в. --- {\it метод обратной функции}. Покажите, что если с.в. $\eta $ равномерно распределена на отрезке $\left[0,1\right]$, то с.в. $\xi =F^{-1} \left(\eta \right)$ имеет функцию распределения $F\left(x\right)$. Предполагается, что $F\left(x\right)$ непрерывна и строго монотонна. Как выглядит формула для моделирования с.в. из показательного распределения с функцией распределения $F\left(x\right)=\left(1-e^{-\lambda x} \right)I\left(x\geq 0\right)$?
\end{problem}

\begin{problem}
Пусть с.в. $\eta _{1} $, $\eta _{2}$ независимы и имеют равномерное распределение на отрезке $\left[0,1\right]$. Докажите, что с.в. $X$ и $Y$, где $X=\sqrt{-2\ln \eta _{1} } \cos \left(2\pi \eta _{2} \right)$, $Y=\sqrt{-2\ln \eta _{1} } \sin \left(2\pi \eta _{2} \right)$ -- независимые и одинаково распределенные: стандартно нормально ${\rm {\mathcal N}}\left(0,1\right)$.

\begin{ordre}
Покажите, что
\[f_{XY} (x,y)=\frac{1}{\sqrt{2\pi } } e^{-\frac{x^{2} }{2} } \frac{1}{\sqrt{2\pi } } e^{-\frac{y^{2} }{2} } =\frac{1}{2\pi } e^{-\frac{x^{2} +y^{2} }{2} } .\] 
Перейдите к полярным координатам, не забыв о якобиане замены переменных.
\end{ordre}

\end{problem}


\begin{problem}

Если $X$ --- с.в., имеющая стандартное нормальное распределение, то $X^{-2} $ имеет устойчивую плотность (см. замечание к задаче \ref{bluzd_ust} раздела 5):
\[\frac{1}{\sqrt{2\pi } } e^{-\frac{1}{2x} } x^{-\frac{3}{2} }, \quad x>0.\] 
Используя это, покажите, что если $X$ и $Y$ --- независимые нормально распределенные с.в. с нулевым математическим ожиданием и дисперсиями $\sigma _{1}^{2} $ и $\sigma _{2}^{2} $, то величина $Z=\frac{XY}{\sqrt{X^{2} +Y^{2} } } $ нормально распределена с дисперсией $\sigma _{3}^{2} $, такой, что $\frac{1}{\sigma _{3}^{2} } =\frac{1}{\sigma _{1}^{2} } +\frac{1}{\sigma _{2}^{2} } $.

\end{problem}


\begin{problem}(Теорема Бернштейна \cite{28}, \cite{21} Т.~2.) а) С помощью неравенства Чебышёва установите следующий результат из анализа: 

\[
\forall \; \; f\in C\left[0,1\right]\Rightarrow \left\| f_{n} -f\right\| _{C\left[0,1\right]}
\to 0, \, n\to \infty
\] 

\[
f_{n} \left(x\right)=\sum_{k=0}^{n}f\left(\frac{k}{n} \right) C_{n}^{k} x^{k} \left(1-x\right)^{n-k}. 
\]

\indent б) Исходя из предыдущей задачи и п. а) предложите способ генерирования распределения с.в. $\xi $, имеющей плотность $f_{\xi } \left(x\right)$ с финитным носителем. Пусть, для определенности,  носителем будет отрезок $\left[0,1\right]$.

\end{problem}

\begin{problem}(Метод фон Неймана.) 
Пусть с.в. $\xi $ распределена на отрезке $\left[a,b\right]$, причем ее плотность распределения ограничена: $\mathop{\max }\limits_{x\in \left[a,b\right]} f_{\xi } (x) < C$.\linebreak Пусть с.в. $\eta _{1} $, $\eta _{2} $, \dots \ независимы и равномерно распределены на $\left[0,1\right]$, $X_{i} =a+\left(b-a\right)\eta _{2i-1} $, $Y_{i} =C\eta _{2i} $, $i=1,2,...$, т.е. пары $\left(X_{i} ,Y_{i} \right)$ независимы и равномерно распределены в прямоугольнике $\left[a,b\right]\times \left[0,C\right]$. Обозначим через $\nu $ номер первой точки с координатами $\left(X_{i} ,Y_{i} \right)$, попавшей под график плотности $f_{\xi } (x)$, т.е.\linebreak $\nu =\min \left\{i:\: Y_{i} \le f_{\xi } (X_{i} )\right\}$. Положим $X_{\nu } =\sum _{n=1}^{\infty }X_{n} I\left(\nu =n\right) $.

\begin{enumerate}
\item Покажите, что с.в. $X_{\nu } $ распределена так же, как $\xi $.

\item Сколько в среднем точек $\left(X_{i} ,Y_{i} \right)$ потребуется «вбросить» в прямоугольник $\left[a,b\right]\times \left[0,C\right]$ для получения одного значения $\xi $?

\item Предложите модификацию рассмотренного метода для генерации дискретной случайной величины, принимающей значения $\lbrace 1, 2, ... , k \rbrace$ с одинаковой вероятностью, имея в распоряжении монету (генератор бинарной случайной величины).   
\end{enumerate}
\end{problem}

\begin{problem}
Как с помощью с.в. $\xi $, равномерно распределенной на отрезке $\left[0,1\right]$ ($\xi \in R\left[0,1\right]$), и симметричной монетки построить с.в. $X$, имеющую плотность распределения $f_{X} (x)=\frac{1}{4} \left(\frac{1}{\sqrt{x} } +\frac{1}{\sqrt{1-x} } \right)$, $x\in \left(0,1\right)$?
\end{problem}

\begin{problem}

Пусть $\xi $ распределена на $\left[0,1\right]$ с плотностью $f_{\xi } (x)$, представимой в виде степенного ряда $\sum _{k=0}^{\infty }a_{k} x^{k}  $ с $a_{k} \ge 0$. Положим $p_{k} ={a_{k} \mathord{\left/ {\vphantom {a_{k}  (k+1)}} \right. \kern-\nulldelimiterspace} (k+1)} $. Тогда $f_{\xi } (x)=\sum _{k=0}^{\infty }p_{k} \cdot (k+1)x^{k}  $. Примените \textit{метод суперпозиции} для моделирования с.в. $\xi $.

\begin{ordre}
\textit{Метод суперпозиции}:

\indent а) Разыгрывается значение дискретной с.в., принимающей значения $k=0,1,2,...$ с вероятностями $p_{k}, \, k = 0,1,2\dots$.

\indent б) Для каждого $k$ моделируется с.в. с функцией распределения $F_{k} (x) = x^{k+1}$, $x\in [0,1]$ (например, методом обратной функции).

\end{ordre}

\end{problem}


\begin{problem}
Покажите, что в случае общего положения невозможно построить генератор дискретной с.в., принимающей $n$ значений, быстрее чем за $O(n)$. Однако, существуют процедуры построения генератора такие, что можно, начиная со второго раза, генерировать распределение этой с.в. за $O(\log n)$. Более того, если потребуется сгенерировать распределение немного отличной с.в. (например, в которой поменялось несколько вероятностей исходов и, как следствие, нормировочный множитель всего распределения), то это также можно сделать за $O(\log n)$. Покажите, что если случайная величина принимает разные значения с одинаковыми вероятностями, то  построить генератор такой с.в. можно и за $O(\log n)$. 
\end{problem}

\begin{problem}(Алгоритм Кнута–Яо.)
С помощью бросаний симметричной монетки требуется сгенерировать распределение заданной дискретной с.в., принимающей конечное число значений. Обобщите описанную ниже схему на общий случай. Предположим, что нам нужно сгенерировать распределение с.в., принимающей три значения 1, 2, 3 с равными вероятностями 1/3. Действуем таким образом. Два раза кидаем монетку: если выпало 00, то считаем, что выпало значение 1, если 01, то 2, если 11, то 3. Если 10, то еще два раза кидаем монетку и повторяем рассуждения. Покажите, что в среднем с помощью не более чем $\log_2 (n - 1) + 2$ подбрасываний симметричной монетки можно сгенерировать распределение дискретной с.в., принимающей, вообще говоря, с разными вероятностями $n$ значений.
\end{problem}
\begin{remark}
См. Ермаков С.М. Метод Монте-Карло в вычислительной математике. -- М.: Бином, 2009.
\end{remark}

\begin{problem}(Метод Уокера.)
Пусть с.в. $\xi$ принимает значения $1, \ldots, n$ с вероятностями $p_1, \ldots, p_n$. Докажите, что 
с.в. $\xi$ можно сгенерировать при помощи смеси дискретных распределений с двумя исходами и с.в. $\xi'$, принимающей значения $1, \ldots, n$ с одинаковыми вероятностями. 
\end{problem}

\begin{ordre}

\begin{enumerate}
\item Покажите, что $\exists i, j \neq i: \;  p_i \leq 1/n, \; p_i + p_j > 1/n$.
\item Зафиксируем пару $i, j$ с указанным свойством и определим с.в. $\eta^{(1)}$ с двумя исходами:
\[
\mathbb{P}(\eta^{(1)}=i)=q_i^{(1)} = n p_i, \; \mathbb{P}(\eta^{(1)}=j)=q_j^{(1)} = 1 - n p_i, \; q_k^{(1)} = 0.   
\]
Покажите, что $\xi$ может быть представлена в виде смеси $\eta^{(1)}$ и случайной величины $\zeta^{(1)}$, принимающей значения из множества $\{1, \ldots, n\} \backslash i$. 
\item Повторите рассуждения пункта б) для с.в. $\zeta^{(1)}$ и таким образом получите, что %, выразите $p_1, \ldots, p_n$ через  $ \{q_i^{(j)}\}$: 
\[
p_l = \frac{1}{n} \sum \limits_{j=1}^n q_l^{(j)}.
\]
\end{enumerate}

См. также  Ермаков С.М. Метод Монте-Карло в вычислительной математике. -- М.: Бином, 2009.
\end{ordre}

\begin{problem}(Теорема Пайка.) \label{paika} 
Пусть ${X}_{k} ,\; k=1,...,n$ --- независимые равномерно распределенные на отрезке $\left[0,1\right]$ с.в. Упорядочим эти с.в., введя обозначения
\[\mathop{\min }\limits_{k=1,...,n} {X}_{\left(k\right)} ={X}_{\left(1\right)} \le ...\le {X}_{\left(n\right)} =\mathop{\max }\limits_{k=1,...,n} {X}_{\left(k\right)} .\] 
Пусть ${\eta}_{k} ,\; k=1,...,n+1$ --- независимые показательно распределенные с.в.: 
\[\mathbb{P}\left({\eta}_{k} >t\right)=e^{-t} ,\; t\ge 0.\] 
Покажите, что
\[\left({X}_{\left(1\right)} {\rm ,}\; {X}_{\left(2\right)} {\rm ,...,}\; {X}_{\left(n\right)} \right) \mathop{=}\limits^{d} \left(\frac{{\eta}_{1} }{\sum _{k=1}^{n+1}{\eta}_{k}  } {\rm ,}\; \frac{{\eta}_{1} +{\eta}_{2} }{\sum _{k=1}^{n+1}{\eta}_{k}  } {\rm ...,}\; \frac{\sum _{k=1}^{n}{\eta}_{k}  }{\sum _{k=1}^{n+1}{\eta}_{k}  } \right). \] 
\end{problem}

\begin{remark}
См. Лагутин М.Б. Наглядная математическая статистика. -- М.: Бином, 2009 и Кендалл М., Моран П. Геометрические вероятности. – М.: Наука, 1972.
\end{remark}

\begin{problem}(Генерация точек из равномерного распределения.) а) Пусть ${X}$ ---  $n$-мерный вектор с независимыми одинаково распределенными компонентами с распределением $\mathcal{N}(0,1)$. Покажите, что ${\xi} = \frac{{X}}{\|{X}\|_2}$ имеет  равномерное распределение на единичной сфере в $\mathbb{R}^n$. 

\indent б) Пусть ${X}$ --- вектор с независимыми компонентами, каждая с распределением Лапласа (т.е. с плотностью $p(x)=\frac{1}{2}\exp(-|x|)$). Какое распределение имеет вектор  ${\xi} = \frac{{X}}{\|{X}\|_1}$?
\end{problem}




\begin{problem}\Star (Сдвиг Бернулли.)
Рассмотрим динамическую систему (ДС): $x\to\{2x\}$ ($\{\cdot \}$ --- дробная часть числа), преобразования отрезка $X = [0,1]$ в себя. Покажите, что для почти всех (по равномерной мере Лебега на отрезке $X$) точек старт, полученная c помощью ДС последовательность точек будет ``квазислучайной'' (схожей с последовательностью независимых одинаково распределенных на отрезке $X$ с.в.), то есть для неё, например, справедливы ЗБЧ и ЦПТ.
\begin{ordre}
B.B. Pokhodzei. "Niederreiter H. Random number generation and quasi-Monte Carlo methods.(CBMS-NSF regional conference series in applied mathematics, V. 63.) Philadelphia, Penn.: SIAM, 1992.
\end{ordre}
\begin{remark}
В контексте этой задачи рекомендуется ознакомиться также с понятиями непредсказуемой последовательности, типичной последовательности, случайной (сложной) по Колмогорову последовательности, например, по книге Верещагин Н.К., Успенский В.А., Шень А. Колмогоровская сложность и алгоритмическая случайность. -- М.: МЦНМО, 2013. Задача отражает то обстоятельство, что случайность ``переносится'' из начальных данных (даже простым в смысле Колмогорова алгоритмом). Рассматриваемая динамическая система последовательно считывает числа после запятой в двоичной записи начальной точки. Почти все числа из отрезка $[0,1]$ сложны (несжимаемы) в смысле Колмогорова, правда для подавлющего большинства конкретных чисел это утверждение не может быть доказано. Студенты ФУПМ имеют возможность познакомиться с колмогоровской сложностью и алгоритмическими вопросами теории вероятностей по курсу (книги) Вьюгин В.В. Колмогоровская сложность и алгоритмическая случайность. -- М.: МФТИ, 2012. В частности, рекомендуется ознакомиться со сложностным доказательством закона повторного логарифма и эргодической теоремы Биркгофа\linebreak(--Хинчина), а также с  вопросами эффективности эргодической теоремы. 

Другая причина появления случайности --- это поведение динамических систем (например, рассмотренной) в условиях небольших внешних возмущений. По данной тематике стоит отметить книгу Опойцева В.И. Нелинейная системостатика. -- М.: Наука, 1986 и в цикле недавних работ В.А. Малышева и А.А.~Лыкова. Вообще между динамическими системами и случайными (марковскими) процессами имеется глубокая взаимообогащающая связь. См., например, конструкцию Улама в книге Бланк~М.Л. Устойчивость и локализация в хаотической динамике. -- М.: \mbox{МЦНМО}, 2001 и Синай~Я.Г. Как математики изучают хаос // Математическое просвещение, 2001. Вып. 5. С.~32--46. Интересные взгляды на эту науку также имеются в книгах Вент\-цель~А.Д., Фрейд\-лин~М.И. Флуктуации в динамических системах под воздействием малых случайных возмущений. -- М.: Наука, 1979, \cite{333}, \cite{101}, см.~также 
blogs.princeton.edu/imabandit/2014/12/22/guest-post-by-sasho-nikolov-beating-monte-carlo.

Ну а самое главное, что в приложениях нам нужна не ``природная случайность''. Нам нужно лишь выполнение для полученной квазислучайной последовательности неких тестов типа ЗБЧ., ЦПТ с такими же оценками скорости сходимости (или не сильно худшими). Однако оказывается, что псевдослучайная последовательность может даже увеличить скорость сходимости по сравнению с настоящими случайными данными. Обнаружено это было более 40 лет назад (сюда можно отнести метод выбора узлов Холтона--Соболя, обобщающий идею задачи 2 п. б) настоящего раздела), но по-прежнему активно используется на практике (см. Соболь И.М. Численные методы Монте-Карло. -- \linebreak М.: Наука, 1973) и позволяет вместо $~1/\sqrt{n}$ получать точность $~n^{\varepsilon - 1}$ cо сколь угодно малым $\varepsilon > 0$.


В заключение хочется отметить, что в последние десятилетия очень бурно развивается область Theoretical Computer Sсience, связанная с изучением генераторов псевдослучайных чисел (в том числе в связи с проблемой $P \ne NP$), см.  
Разборов А.А. Theoretical Computer Sсience: взгляд математика. 2013. См. также ссылку:\\ www.people.cs.uchicago.edu/razborov/files/computerra.pdf.


\end{remark}
\end{problem}

\begin{comment}
\begin{problem}[MCMC]
\label{mcmc}
Для оценки статистик распределения с неизвестной нормировочной константой (см. задачу \ref{varinf} из раздела \ref{CS}) 
\[
p(X) = \frac{1}{S_p} \tilde{p}(X)
\]   
методы Монте Карло требуют возможность генерации выборки из этого распределения
\[
X_1,\ldots,X_N \sim p(X).
\]
Впоследствии, выборка может быть использована для оценки статистик
\[
\Exp_p T(X) \approx \frac{1}{N} \sum_{i = 1}^N T(X_i).
\]
Принцип работы метода MCMC  состоит в использовании некоторой марковской цепи с априорным распределением $p_0(X)$ и вероятностями перехода в момент времени $n:$ $q_n(X_{n+1}|X_n)$. Генерация выборки происходит таким образом:
\[
X_1 \sim p_0(X),  X_2 \sim q_1(X|X_1), \ldots, X_N \sim q_{N-1}(X|X_{N-1}). 
\]
Заметим, что при таком подходе генерируемая выборка не является набором независимых случайных величин, который может быть получен за счет прореживания $X_1,\ldots,X_N $, взяв каждый $m$-й $X$.

Рассмотрим вопрос выбора однородной вероятности перехода $q_n(X_{n+1}|X_n) = q(X_{n+1}|X_n)$, требуя принадлежность генерируемой выборки интересующему нас распределению $p(T)$. Необходимым требованием в таком случае является инвариантность $p(T)$ относительно переходов марковской цепи, т.е.
\[
p(X)=\int q(X|Y) p(Y)dY \Leftarrow q(X|Y) p(Y) = q(Y|X) p(X).
\]
Марковская цепь может иметь более одного инвариантного распределения. 
Пусть $\pi(X)$ –-- ее инвариантное распределение. Тогда марковская цепь называется \textit{эргодичной}, если
\[
\forall p_0(X): \; p_n(X) = \int q(X|Y) p_{n-1}(Y)dY \to \pi(X). 
\]
Очевидно, что эргодичная марковская цепь имеет только одно инвариантное распределение. Докажите, что достаточным условием эргодичности однородной марковской цепи является  свойство:
\[
\forall X, \forall Y: \pi(Y) > 0 \Rightarrow q(Y|X) > 0. 
\]

\end{problem}
\end{comment}

\begin{problem}(PageRank.)
Ориентированный граф $G=\left\langle {V,E} \right\rangle$  сети Интернет представляется в виде набора web-страниц $V$ и ссылок между ними: запись $\left( {i,j} \right)\in E$ означает, что на $i$-й странице имеется ссылка на $j$-ю страницу. 

\begin{enumerate}

\item По web-графу случайно блуждает пользователь. За один такт 
времени пользователь, находящийся на web-странице с номером $i$, с вероятностью $p_{ij} $ переходит по ссылке на web-страницу $j$. 
Пусть из любой web-страницы можно по ссылкам перейти на любую другую 
web-страницу (условие неразложимости) графа $G$. Проверьте, что при бесконечно долгом блуждании доля времени, которую пользователь проведет на web-странице с номером $k$, есть $p_k $, где $ 
{p} =\left( {p_1 ,...,p_n } \right)^T $, ${p}^T = {p}^T P$, 
$P=\left\| {p_{ij} } \right\|_{i,j=1}^{n,n} $ -- стохастическая матрица, $\sum_k p_k = 1$ (решение единственно  ввиду неразложимости $P$). Обратим внимание, что ответ не зависит от того, с какой вершины стартует пользователь.

\item В условиях предыдущего пункта пустим независимо блуждать по web-графу $N$ 
пользователей ($N\gg \left| V \right| \gg 1)$. Пусть $n_i \left( t \right)$ -- число посетителей web-страницы $i$ в момент времени $t$. Считая стохастическую матрицу $P$ неразложимой и апериодической, покажите, 
что
\[
\exists \;\;\lambda _{0.99} >0,\;T_G>0:\;\;\;\forall \;\;t\ge 
T_G,
\]
\[
\PR\left( {\left. {\left| {\frac{n_k \left( t \right)}{N}-p_k } \right|\le 
\frac{\lambda _{0.99} }{\sqrt N }} \right)\ge 0.99} \right.,
\]
где $ {p}^T= {p}^T P$ (решение единственно). Как и в п. а), и здесь ответ не зависит от того, с каких вершин стартуют пользователи.

\end{enumerate}

\end{problem}

\begin{remark}
\begin{comment}
Матрица $P^n = \Vert p_{ij}^{(n)} \Vert$ является матрицей переходных вероятностей за $n$ шагов. Число
\[
    d(j) = \text{НОД} \left\{n : p_{jj}^{(n)} > 0 \right\},
\]
где $\gcd$ обозначает наибольший общий делитель, называется \textit{периодом} вершины $j$. Если $d(j) = 1$, то  вершина называется апериодической. Для неразложимой $P$ периоды у всех вершин совпадают. Соответственно,  стохастическая матрица $P$ называется апериодической, если $\forall j: \; d(j) = 1$.
\end{comment}
Если организовать случайные блуждая, следуя п. б) 
(отметим, что эти блуждания хорошо распараллеливаются по числу 
блуждающих пользователей), то при определенных условиях можно получить решение задачи  ${p}^T = {p}^TP$ значительно быстрее, чем, скажем, ${\it O}\left( {n^2} \right)$. Такой способ численного поиска вектора $ {p}$ основан на методе Markov 
chain Monte Carlo. %(см. задачу \ref{mcmc})%. 
Детали и ссылки см., например, в работе Гасников А.В., Дмитриев Д.Ю. Об эффективных рандомизированных алгоритмах поиска вектора PageRank // ЖВМиМФ, 2015 Т. 55:3.  -- arXiv:1410.3120. Упомянем также недавнюю работу Belloni~A., Chernozhukov V. On the Computational Complexity of MCMC-based Estimators in Large Samples. 2012 -- arXiv:0704.2167,  содержащую строгие результаты об эффективной вычислимости байесовских оценок. Если 
использовать неравенства концентрации меры и иметь оценки на спектральную 
щель матрицы $P$ (см. \cite{44,240}), то приведенный в п. 
б) результат можно также сделать  более строгим, а именно точнее 
оценивать скорость сходимости и плотность концентрации (см.  задачу 19 раздела \ref{macrosystems}).
\end{remark}

\begin{comment}

\begin{problem}

В руки опытных криптографов попалось закодированное письмо (10 000 символов). Чтобы это письмо прочитать нужно его декодировать. Для этого берется стохастическая матрица переходных вероятностей $P$
(линейный размер которой определяется числом возможных символов (букв, знаков препинания и т.п.) в языке на котором до шифрования было написано письмо – этот язык известен и далее будет называться базовым). $P_{ij}$ отвечает за вероятность появления символа с номером $j$ сразу после символа под номером $i$. Такая матрица может быть идентифицирована с помощью статистического анализа  большого текста, скажем,  Войны и мира Л.Н. Толстого.

Пусть способ (де)шифрования определяется некоторой неизвестной функцией $\overline{f}$ – преобразование (перестановка) множества кодовых букв во множество символов базового языка.
В качестве, “начального приближения” выбирается какая-то функция $f$, например,
полученная исходя из легко осуществимого частотного анализа. Далее рассчитывается вероятность выпадения полученного закодированного текста, сгенерированного при заданной функции $f$  (правдоподобие выборки).

Случайно  выбираются два аргумента у функции $f$ и значения функции при этих аргументах меняются местами. Если в результате правдоподобие возрастает, то замена аргументов фиксируется, иначе бросается монетка с вероятностью выпадения орла равной отношению правдоподобий. 

Объясните, почему предложенный алгоритм ``сходится'' именно к $\overline{f}$ ? Оцените скорость сходимости.


\end{problem}



\subsection{ Markov chain Monte Carlo }

\begin{problem}
Чтобы построить однородный дискретный марковский процесс с конечным числом состояний, имеющий заданную инвариантную (стационарную) меру $\pi$ , переходные вероятности ищутся в следующим виде: $p_{ij} = p_{ij}^0 a_{ij}$ , 
$i \neq j$; $p_{ii} = 1 - \sum p_{ij}$ , где $p^0$ – некоторая затравочная матрица, которую будем далее предполагать симметричной. Покажите, что матрица $p$ имеет инвариантную (стационарную) меру  $\pi$, если
\[
\frac{a_{ij}}{a_{ji}} = \frac{\pi_{j} p^0_{ji}}{\pi_{i} p^0_{ij}} = \frac{\pi_{j}}{\pi_{i}} 
\]

Чтобы найти  $a_{ij}$ достаточно найти функцию F: $\mathbb{R_+} \rightarrow [0,1]$ такую, что

\[
\frac{F(z)}{F(1/z)} = z; a_{ij}  \leftarrow F( \frac{\pi_{j}}{\pi_{i}} )
\]

Пример функции $F(z) = \min(z,1)$ определяет алгоритм Метрополиса. 

\end{problem}

\begin{problem}

В руки опытных криптографов попалось закодированное письмо (10 000 символов). Чтобы это письмо прочитать нужно его декодировать. Для этого берется стохастическая матрица переходных вероятностей $P$
(линейный размер которой определяется числом возможных символов (букв, знаков препинания и т.п.) в языке на котором до шифрования было написано письмо – этот язык известен и далее будет называться базовым). $P_{ij}$ отвечает за вероятность появления символа с номером j сразу после символа под номером i . Такая матрица может быть идентифицирована с помощью статистического анализ  большого текста, скажем,  Войны и мира Л.Н. Толстого.

Пусть способ (де)шифрования определяется некоторой неизвестной функцией $\overline{f}$ – преобразование (перестановка) множества кодовых букв во множество символов базового языка.
В качестве, “начального приближения” выбирается какая-то функция f , например,
полученная исходя из легко осуществимого частотного анализа. Далее рассчитывается вероятность выпадения полученного закодированного текста, сгенерированного при заданной функции f  (правдоподобие выборки).

Случайно  выбираются два аргумента у функции f и значения функции при этих аргументах меняются местами. Если в результате правдоподобие возрастает, то замена аргументов фиксируется, иначе бросается монетка с вероятность выпадения орла равной отношению правдоподобий. 

Объясните, почему предложенный алгоритм “сходится” именно к $\overline{f}$ ? Почему сходимость оказывается такой быстрой (0.01 сек. на современном PC)?


\end{problem}

\subsection{Gibbs Sampler}

\subsection{Variational Inference}

\end{comment}




\begin{problem}\Star\,\,\Star (Markov Chain Monte Carlo Revolution и состоятельность
оценок максимального правдоподобия; P. Diaconis.)
\label{cript}
В руки опытных криптографов попалось закодированное письмо (10~000 символов). Чтобы это 
письмо прочитать, нужно его декодировать. Для этого берется стохастическая 
матрица переходных вероятностей $P=\left\| {p_{ij} } \right\|$ (линейный 
размер которой определяется числом возможных символов (букв, знаков 
препинания и т.п.) в языке, на котором до шифрования было написано письмо, --- 
этот язык известен и далее будет называться базовым), в которой $p_{ij} $ -- это вероятность появления символа с номером $j$ сразу после символа 
под номером $i$. Такая матрица может быть идентифицирована с помощью 
статистического анализ какого-нибудь большого текста, скажем, ``Войны и 
мира'' Л.Н.~Толстого.

Пускай способ (де)шифрования (подстановочный шифр) определяется некоторой 
неизвестной дешифрующей функцией $\bar {f}$ --- преобразование 
(перестановка) множества кодовых букв во множество символов базового языка.

В качестве ``начального приближения'' выбирается какая-то функция $f$, 
например, полученная исходя из легко осуществимого частотного анализа. Далее 
рассчитывается вероятность выпадения полученного закодированного текста 
$ {x}$, сгенерированного при заданной функции $f$ (функция 
правдоподобия):

\[%\tag{*}
L\left( {{x};f} \right)=\prod\limits_k {p_{f\left( {x_k } 
\right),f\left( {x_{k+1} } \right)} } . 
\]

Случайно выбираются два аргумента у функции $f$ и значения функции при этих 
аргументах меняются местами. Если в результате получилась такая $f^\ast $, 
что $L\left( { {x};f^\ast } \right)\ge L\left( { {x};f} \right)$, то 
$f:=f^\ast $, иначе независимо бросается монетка с вероятностью выпадения 
орла $p={L\left( { {x};f^\ast } \right)} \mathord{\left/ {\vphantom 
{{L\left( { {x};f^\ast } \right)} {L\left( { {x};f} \right)}}} 
\right. \kern-\nulldelimiterspace} {L\left( { {x};f} \right)}$, и если 
выпадает орёл, то $f:=f^\ast $, иначе $f:=f$. Далее процедура повторяется (в 
качестве $f$ выбирается функция, полученная на предыдущем шаге).

Объясните, почему предложенный алгоритм после некоторого числа итераций с 
большой вероятностью и с хорошей точностью восстанавливает дешифрующую 
функцию $\bar {f}$? Почему сходимость оказывается такой быстрой (0.01 с на современном PC)?

\end{problem}

\begin{ordre}
Описанный в задаче пример взят из обзора Diaconis P. The Markov 
chain Monte Carlo revolution // Bulletin (New Series) of the AMS. 2009. V. 
49:2. P. 179--205. Детали того, что будет написано далее, можно найти в работах Jerrum M., Sinclair A. The Markov chain Monte Carlo method: an approach to 
approximate counting and integration // Approximation Algorithms for NP-hard 
Problems / D.S.~Hochbaum ed. Boston: PWS Publishing, 1996. P. 482--520; Joulin~A., Ollivier Y. Curvature, concentration and 
error estimates for Markov chain Monte Carlo // Ann. Prob. 2010. V. 38:6. 
P. 2418--2442; Paulin~D. Concentration inequalities for Markov chains by 
Marton couplings. 2013  (arXiv:1212.2015v2). См. также \cite{240}.

Для того чтобы построить однородный дискретный марковский процесс с конечным 
числом состояний, имеющий наперед заданную инвариантную (стационарную) меру 
$\pi $, переходные вероятности ищутся в следующем виде: $p_{ij} =p_{ij}^0 
b_{ij} $, $i\ne j$; $p_{ii} =1-\sum\limits_{j:\;\;j\ne i} {p_{ij} } $, где 
$p_{ij}^0 $ -- некоторая ``затравочная'' матрица, которую будем далее 
предполагать симметричной. Легко проверить, что матрица $p_{ij} $ имеет 
инвариантную (стационарную) меру $\pi $, если при $p_{ij}^0 >0$
\[
\frac{b_{ij} }{b_{ji} }=\frac{\pi _j p_{ji}^0 }{\pi _i p_{ij}^0 }=\frac{\pi 
_j }{\pi _i }.
\]
Чтобы найти $b_{ij} $, достаточно найти функцию $F:\;{\mathbb{R}}_+ \to \left[ 
{0,1} \right]$ такую, что

$$\frac{F\left( z \right)}{F\left( {1 \mathord{\left/ {\vphantom {1 z}} 
\right. \kern-\nulldelimiterspace} z} \right)}=z\quad \text{и}\quad b_{ij} =F\left( 
{\frac{\pi _j p_{ji}^0 }{\pi _i p_{ij}^0 }} \right)=F\left( {\frac{\pi _j 
}{\pi _i }} \right).$$

Пожалуй, самый известный пример (именно он и использовался в задаче) такой 
функции $\tilde {F}\left( z \right)=\min \left\{ {z,1} \right\}$ --- алгоритм 
Хастингса--Метрополиса. Заметим, что для любой такой функции $F\left( z 
\right)$ имеем $F\left( z \right)\le \tilde {F}\left( z \right)$. Другой 
пример дает функция $F\left( z \right)=z \mathord{\left/ {\vphantom {z 
{\left( {1+z} \right)}}} \right. \kern-\nulldelimiterspace} {\left( {1+z} 
\right)}$. Заметим также, что $p_{ij}^0 $ обычно выбирается равным $p_{ij}^0 
=1 \mathord{\left/ {\vphantom {1 M}} \right. \kern-\nulldelimiterspace} M_i 
$, где $M_i $ --- число ``соседних'' состояний у $i$, или
\[
p_{ij}^0 =1 \mathord{\left/ {\vphantom {1 {\left( {2M} \right)}}} \right. 
\kern-\nulldelimiterspace} {\left( {2M} \right)},
\quad
i\ne j;
\quad
p_{ii}^0 =1 \mathord{\left/ {\vphantom {1 2}} \right. 
\kern-\nulldelimiterspace} 2,
\quad
i\ne j.
\]
При больших значениях времени $t$, согласно эргодической теореме, имеем, что 
распределение вероятностей близко к стационарному $\pi $. Действительно, при 
описанных выше условиях имеет место условие детального баланса (марковские 
цепи, для которых это условие выполняется, иногда называют обратимыми):
\[
\pi _i p_{ij} =\pi _j p_{ji} ,\;i,j=1,...,n,
\]
из которого сразу следует инвариантность меры $\pi $, т.е.
\[
\sum\limits_i {\pi _i p_{ij} } =\pi _j \sum\limits_i {p_{ji} } =\pi _j 
,\;j=1,...,n.
\]
Основное применение замеченного факта состоит в наблюдении, что время выхода 
марковского процесса на стационарную меру (mixing time) во многих случаях 
оказывается удивительно малым. Притом что 
выполнение одного шага по времени случайного блуждания по графу, отвечающему 
рассматриваемой марковской цепи, как следует из алгоритма Кнута--Яо (см. задачу 11), также 
может быть быстро сделано. Таким образом, довольно часто можно получать 
эффективный способ генерирования распределения дискретной случайной величины 
с распределением вероятностей $\pi $ за время, полиномиальное от логарифма 
числа компонент вектора $\pi $.

Для лучшего понимания происходящего в условиях задачи отметим, что одним из 
самых универсальных способов получения асимптотически наилучших оценок 
неизвестных параметров по выборке является метод наибольшего правдоподобия 
(И.А. Ибрагимов -- Р.З. Хасьминский, В.Г. Спокойный). Напомним вкратце, в чем он 
заключается. Пусть имеется выборка из распределения, зависящего от 
неизвестного параметра --- в нашем случае выборкой $ {x}$ из 10~000 
элементов будет письмо, а неизвестным\; ``параметром''\; будет функция~$f$. 
Далее считается вероятность (или плотность вероятности в случае непрерывных 
распределений) $L\left( { {x};f} \right)$ того, что выпадет данный $
{x}$ при условии, что значение параметра $f$. Если посмотреть на $L\left( { {x};f} \right)$ 
как на распределение в 
пространстве параметров ($ {x}$  зафиксирован), то при большом объеме 
выборки (размерности~${x}$) при естественных условиях это распределение 
концентрируется в малой окрестности наиболее вероятного значения
\[
f\left( {{x}} \right)=\arg \mathop {\max }\limits_f L\left( { 
{x};f} \right),
\]
которое ``асимптотически'' совпадает с неизвестным истинным значением $\bar 
{f}$.

\end{ordre}

\begin{remark}
Для оценки mixing time нужно оценить спектральную щель 
стохастической матрицы переходных вероятностей, задающей исследуемую 
марковскую динамику, то есть нужно оценить расстояние от максимального 
собственного значения этой матрицы, равного единице (теорема 
Фробениуса--Перрона), до следующего по величине модуля. Именно это число 
определяет основание геометрической прогрессии, мажорирующей исследуемую 
последовательность норм разностей расстояний (по вариации) между 
распределением в данный момент времени и стационарным (финальным) 
распределением. Для оценки спектральной щели разработано довольно много 
методов, из которых мы упомянем лишь некоторые: неравенство Пуанкаре 
(канонический путь), изопериметрическое неравенство Чигера (проводимость), с 
помощью техники каплинга (получаются простые, но, как правило, довольно 
грубые оценки), с помощью каплинга Мертона, с помощью дискретной кривизны 
Риччи и теорем о концентрации меры (Мильмана--Громова). Приведем некоторые 
примеры применения MCMC: тасование $n$ карт разбиением приблизительно на 
две равные кучи и перемешиванием этих куч (mixing time$\sim \log _2 
n)$;\footnote{ Здесь контраст проявляется, пожалуй, наиболее ярко. Скажем, 
для колоды из 52 карт пространство состояний марковской цепи будет иметь 
мощность 52! (если сложить времена жизней в наносекундах каждого человека, 
когда либо жившего на Земле, то это число на много порядков меньше 52!). В 
то время как такое тасование: взять сверху колоды карту и случайно 
поместить ее во внутрь колоды, отвечающее определенному случайному 
блужданию, с очень хорошей точностью выйдет на равномерную меру, отвечающую 
перемешанной колоде, через каких-то 200--300 шагов. Если брать тасование 
разбиением на кучки, то и того меньше --- за 8--10 шагов. Это обнаружил P. Diaconis.} Hit and Run 
(mixing time $\sim n^3)$; модель Изинга --- $n$ спинов на отрезке, 
стационарное распределение = распределеню Гиббса, глауберова динамика 
(mixing time $\sim n^{{2\log _2 e} \mathord{\left/ {\vphantom {{2\log _2 e} 
T}} \right. \kern-\nulldelimiterspace} T}$, $0<T\ll 1$ (см. задачу 18)); проблема поиска 
кратчайших гамильтоновых путей; имитация отжига (см. задачу 20) для решения 
задач комбинаторной оптимизации, MCMC для решения задач перечислительной 
комбинаторики. Но, пожалуй, самым известным примером (Dyer--Frieze--Kannan) 
является полиномиальный вероятностный алгоритм (работающий быстрее известных 
``экспоненциальных'' детерминированных) приближенного поиска центра тяжести 
выпуклого множества и вычисления его объема. Одна из работ в этом 
направлении была удостоена премии Фалкерсона -- аналога Нобелевской премии в 
области Computer Science. Близкие идеи используются и при применении 
экспандеров в Computer Science. В 2010 году премия Неванлинны 
была вручена Д. Спилману, в частности, за сублинейное (по числу элементов 
матрицы, отличных от нуля) решение системы линейных уравнений с помощью 
экспандеров (см. часть 2). 

%Полезно сравнить эту задачу с задачей 7 и с задачей 19 раздела [ССЫЛКА].
\end{remark}

\begin{problem} (Одномерная модель Изинга \cite{44}.) 
Рассмотрим конечный отрезок одномерной целочисленной решетки $\{0,1,\dots,n\}$, в каждой вершине $k$ которой находится спин, принимающий два значения $\sigma(k)=\pm1$. При этом считаем, что $\sigma(0)=\sigma(n)=1$. Определим гамильтониан системы $H(\sigma) = \sum_{k=0}^{n-2}(1-\sigma(k)\sigma(k+1))/2$. Определим расстояние Больцмана--Гиббса по формуле $\pi(\sigma) = Z^{-1}\exp(-\beta H(\sigma))$, $\beta = T^{-1}>0$~--- величина, обратная <<температуре>>, а $Z$~--- нормирующий множитель (статсумма). Одним из способов построения однородной дискретной марковской цепи с заданным стационарным распределением $\pi(\sigma)$ является использование распределение Глаубера:
\begin{enumerate}
\item Выбираем $k\in\{1,\dots,n-1\}$ согласно равномерному распределению.
\item С вероятностью $$p=\exp(\beta H(\sigma_{k,+1}))/\left(\exp(\beta H(\sigma_{k,+1}))+\exp(\beta H(\sigma_{k,-1}))\right)$$ новым состоянием будет $\sigma_{k,+1}$, а с вероятностью $1-p$ состояние  $\sigma_{k,-1}$,
где $$\sigma_{k,+1} = \sigma_{k}(i),\,i\not=k,\,\sigma_{k,+1} = 1;$$
$$\sigma_{k,-1} = \sigma_{k}(i),\,i\not=k,\,\sigma_{k,-1} = -1.$$
Покажите, что характерное время выхода на стационарное распределение (mixing time) 
этой марковской цепи оценивается сверху как $n^{2\log_2(\beta\exp(1))}$ в предположении $\beta \gg 1$.
\end{enumerate}
\end{problem}


\begin{problem}\Star (Hit and Run.)
Ряд задач, в которых используется метод Монте-Карло, предполагает возможность случайно равномерно набрасывать точки в некоторое наперед заданное множество (не обязательно выпуклое и связное). Например, при вычислении интеграла с помощью метода
Монте-Карло или при численном решении задач оптимизации, в которых нужно уметь
приближенно находить центр тяжести множества. Исходя из MCMC подхода (см. \cite{240}) обоснуйте,
аккуратно оговорив детали, следующий способ генерации точек.

Берем любую точку внутри множества и проводим случайно направление через эту точку, далее с помощью
граничного оракула случайно генерируем (с помощью равномерного распределения) на
этом направлении внутреннюю точку рассматриваемого множества. Через эту точку снова
проводим случайное направление и т.д. Хорошо ли будет работать Hit and Run для вытянутых множеств или для множеств, имеющих достаточно острые углы? Предложите модификацию (например, с помощью эллипсоидов Дикина) алгоритма Hit and Run для таких “плохих” множеств. Предложите другие способы случайно равномерно набрасывать точки в некоторое наперед заданное множество (например, Shake and Bake). Хорошо ли будет работать метод Shake and Bake для множеств в пространствах большой размерности? Как следует действовать, если рассматриваемое множество имеет простую структуру: $n$-мерный куб, $n$-мерный шар, $n$-мерный симплекс, многогранник?
\end{problem}

\begin{remark}
См. Lov?sz, L?szl?, and Santosh Vempala. ``Hit-and-run from a corner.''  // SIAM Journal on Computing 35.4 (2006): 985-1005.
\end{remark}

\begin{problem}\DStar(Глобальная оптимизация и монотонный симметричный 
марковский поиск; Некруткин--Тихомиров.) 
Рассматривается задача глобальной оптимизации $f\left( x \right)\to \mathop {\min }\limits_{x\in 
\mathbb{R}^n} $. Считаем, что глобальный минимум достигается в единственной 
точке $x^\ast $ (причем для любых $\varepsilon >0$ выполняется 
условие\footnote{$B_\varepsilon ^c \left( {x } \right)$ --- дополнение 
шара $B_\varepsilon { \left( x \right)}$ радиуса $\varepsilon $ с 
центром в точке $x $.} $\inf \left\{ {f\left( x \right):\;\;x\in B_\varepsilon^c \left( {x^* } \right)} \right\}>f\left( {x^* } \right))$, где 
$f\left( x \right)$ --- непрерывная функция, дважды гладка в точке 
$x^\ast $, причем матрица Гессе $G$ функции $f\left( x \right)$ в этой точке 
положительно определена. Опишем алгоритм (с точностью до выбора функции 
плотности распределения $g\left( r \right)$, $r\in \left[ {0,\infty } 
\right))$:

\begin{enumerate}
\item (начальный шаг) выбираем точку старта $x_0 =x$;
\item (шаг $k<N$) независимо генерируем с.в. $\xi _k $ из центрально симметричного распределения с заданной плотностью $g\left( r \right)$. Если
	\begin{itemize}
	\item $f\left( {x_k +\xi _k } \right)\le f\left( {x_k } \right),$ то $x_{k+1} =x_k +\xi _k $,
	\item иначе $x_{k+1} =x_k $;
	\end{itemize}

\end{enumerate}
Введем обозначения
\[
M_r =\inf \left\{ {x\in B_r{\left( {x^* } \right)}:\;\;f\left( x 
\right)<f\left( y \right)\;\mbox{для всех }y\in B_r^{c} \left( {x^* } 
\right)} \right\},
\]
\[
\tau _\varepsilon =\min \left\{ {n\in {\rm N}:\quad x_n \in M_\varepsilon } 
\right\},
\quad
\delta \left( x \right)=\inf \left\{ {r\ge 0:\;\;x\in M_r } \right\},
\quad
\]
\[
\Gamma =\prod\limits_{i=1}^n {\left( {\frac{\lambda _i }{\lambda _{\min } }} 
\right)^{1 \mathord{\left/ {\vphantom {1 2}} \right. 
\kern-\nulldelimiterspace} 2}} ,
\]
где $\lambda _i $ --- собственные числа $G$. Покажите, что, как бы 
мы не выбирали функцию плотности $g\left( r \right)$, всегда при 
$\varepsilon <\rho \left( {x,x^\ast } \right)$ имеет место следующая оценка 
снизу:
\[
\Exp\left[ {\left. {\tau _\varepsilon } \right|x_0 =x} \right]\ge \ln \left( 
{{\rho \left( {x,x^\ast } \right)} \mathord{\left/ {\vphantom {{\rho \left( 
{x,x^\ast } \right)} \varepsilon }} \right. \kern-\nulldelimiterspace} 
\varepsilon } \right)+2.
\]
Покажите, что метод с плотностью (есть много других вариантов)
\[
g\left( r \right)=\nu \left( r \right)r^{-d},
\quad
\nu \left( r \right)=\frac{c}{\left( {e+n\left| {\ln r} \right|} \right)\ln 
^2\left( {e+n\left| {\ln r} \right|} \right)},
\]
где $c$  находится из условия нормировки, дает оценку ($\varepsilon 
<{\delta \left( x \right)} \mathord{\left/ {\vphantom {{\delta \left( x 
\right)} 2}} \right. \kern-\nulldelimiterspace} 2)$

\[\tag{1}
\Exp\left[ {\left. {\tau _\varepsilon } \right|x_0 =x} \right]\le b^n\Gamma \ln 
^2\left( \varepsilon \right)\ln ^2\left( {\ln \left( \varepsilon \right)} 
\right)\left| {\ln \left( {\delta \left( x \right)} \right)} \right|, 
\]
где $b\in \left( {2,3} \right)$ (для простоты восприятия мы привели здесь 
огрубленный вариант). 

\end{problem}

\begin{remark}
Если отказаться от гладкости и(или) положительной 
определенности матрицы $G$, то вместо $\Gamma $, которое в типичных 
ситуациях растет с размерностью пространства экспоненциально быстро, в (*) 
можно использовать $F_{\varepsilon ,x}^{-1} $, где
\[
F_{\varepsilon ,x}  = \mathop {\inf }\limits_{\varepsilon \le r<\delta 
\left( x \right)} \left\{ {{\mbox{vol}\left( {M_r } \right)} \mathord{\left/ 
{\vphantom {{\mbox{vol}\left( {M_r } \right)} {\mbox{vol}\left( {B_r \left( 
{x^\ast } \right)} \right)}}} \right. \kern-\nulldelimiterspace} 
{\mbox{vol}\left( {B_r \left( {x^\ast } \right)} \right)}} \right\}.
\]
Отметим, что все приведенные результаты сохраняются с небольшими поправками 
и для оценок вероятностей больших уклонений, т.е. для
\[
n\left( {x,\varepsilon ,\gamma } \right)=\min \left\{ {n:\;\;\PR\left( {x_n 
\in M_\varepsilon \left| {x_0 =x} \right.} \right)\ge \gamma } \right\}=
\]
\[=\min 
\left\{ {n:\;\;\PR\left( {\tau _\varepsilon \le n\left| {x_0 =x} \right.} 
\right)\ge \gamma } \right\}.
\]
Детали имеются в работах А.С. Тихомирова, опубликованных за последние 20 лет 
в ЖВМ и МФ. 

Изложенные в этой задаче результаты могут вызвать на первых порах удивление. 
И, действительно, как такое возможно, чтобы в задачах глобальной оптимизации 
зависимость числа итераций от точности была логарифмическая, в то время как 
известны нижние оценки, в которых эта точность входит в степени размерности 
пространства (в случае равномерной гладкости высокого порядка степень можно 
понижать) в знаменателе, см., например, A. Zhigljavsky. A. Zilinskas. Stochastic global optimization //
 Optimization and Its Applications. Springer, 2008. -- V. 9. P. 262. Тут стоит отметить, что, 
во-первых, нижние оценки получаются для детерминированных методов, ну и 
самое главное, что ``проклятие размерности'' здесь также никуда не делось. 
Даже при самом благоприятном раскладе в оценку (1) входит фактор $2^n$, 
экспоненциально растущий с ростом размерности пространства. В отличие от 
глобальной оптимизации, в выпуклой оптимизации такие проблемы можно решать (см. Часть 2).

\end{remark}

 \begin{problem}(Глобальная оптимизация и simulated annealing.)
 \label{annealing}
 Пожалуй, самым популярным сейчас методом глобальной оптимизации (правда, с очень 
плохими на данный момент теоретическими оценками скорости сходимости) 
является simulated annealing (имитация затвердевания или отжига), 
представляющий собой дискретное приближение решения стохастического 
дифференциального уравнения\footnote{ Детально изученного в статье S.~German., C.P.~Hwang. 
Diffusions for global optimization // SIAM J. Control and Optimization. --
1986. V. 24:5. P. 1031--1043.}
\[
dx_t =-\nabla f\left( {x_t } \right)dt+\sqrt {2T\left( t \right)} dw_t ,
\]
где $w_t $ --- винеровский процесс. Покажите, что при неограничительных 
условиях и $T\left( t \right)\equiv T$ траектория $x_t $ имеет при $t\to 
\infty $ стационарное распределение с плотностью Гиббса:
\[
\frac{\exp \left( {-{f\left( x \right)} \mathord{\left/ {\vphantom {{f\left( 
x \right)} T}} \right. \kern-\nulldelimiterspace} T} \right)}{\int {\exp 
\left( {-{f\left( z \right)} \mathord{\left/ {\vphantom {{f\left( z \right)} 
T}} \right. \kern-\nulldelimiterspace} T} \right)dz} },
\]
экспоненциально концентрирующееся в окрестности единственной точки 
глобального минимума $x^\ast $ дважды гладкой функции $f\left( x \right)$ 
при $T\to 0+$. Однако при $T\to 0+$ и время выхода на это стационарное 
распределение неограниченно возрастает, что создает проблемы для 
практического применения. Более правильно брать $T\left( t \right)=$\linebreak $=c 
\mathord{\left/ {\vphantom {c {\ln \left( {2+t} \right)}}} \right. 
\kern-\nulldelimiterspace} {\ln \left( {2+t} \right)}$, где $c$ --- 
достаточно большое число. Покажите, что тогда для любой начальной точки $x_0 
$ траектория процесса $x_t $ имеет в пределе $t\to \infty $ (который 
фактически с хорошей точностью проявляется уже на конечных временах) 
распределение, сосредоточенное в точке~$x^\ast$. 

\end{problem}

\begin{remark} 
Детали и способы дискретизации можно почерпнуть из 
работы H.~Kushner.  Asymptotic global behavior for stochastic approximation and 
diffusion with slowly decreasing noise effects: global minimization via 
Monte Carlo // SIAM J. Appl. Math. 1987. V. 47:1. P. 169--183.
\end{remark}

\begin{problem} (Multilevel Monte\;Carlo; M.\;Giles.) 
Некоторый диффузионный процесс описывается стохастическим дифференциальным урав\-нением
\[
dS\left( t \right)=a\left( {S(t),t} \right)dt+b\left( {S(t),t} \right)dW\left( t 
\right),
\quad
0\le t\le T,
\quad
S\left( 0 \right)=S_0 ,
\]
где $W\left( t \right)$ --- винеровский процесс. Задана липшицева функция 
$f\left( S \right)$. Требуется предложить численный способ оценивания 
\[
Y=\Exp\left[ {f\left( {S\left( T \right)} \right)} \right].
\]

а)* Дискретизируем задачу по схеме Эйлера:
\[
\hat {S}_{n+1} =\hat {S}_n +a\left( {\hat {S}_n ,t_n } \right) \Delta t +b\left( 
{\hat {S}_n ,t_n } \right)\Delta W_n,
\quad \Delta t = h.
\]
возьмем $N$ независимых реализаций $\left\{ {\hat {S}_n^{\left( i \right)} } 
\right\}$ и положим
\[
\overline {Y}=\frac{1}{N}\sum\limits_{i=1}^N {f\left( {\hat {S}_{T 
\mathord{\left/ {\vphantom {T h}} \right. \kern-\nulldelimiterspace} 
h}^{\left( i \right)} } \right)} .
\]
Покажите, что найдутся такие $C_1 ,C_2 >0$, что
\[
\mbox{MSE}=\mathbb{E}\left[ {\left( {\overline {Y}-Y} \right)^2} \right]\approx C_1 
N^{-1}+C_2 h^2.
\]
Покажите, что если от оценки требуется точность $\varepsilon $ ($\sqrt 
{\mbox{MSE}} ={\it O}\left( \varepsilon \right))$, то оптимально (с точки 
зрения $\mbox{Total}\left( \varepsilon \right)$ -- общего числа 
арифметических операций / генерирования нормальных с.в. $\Delta W_n )$ 
выбирать
\[
h={\it O}\left( \varepsilon \right),
\quad
N={\it O}\left( {\varepsilon ^{-2}} \right),
\quad
\mbox{Total}\left( \varepsilon \right)={\it O}\left( {\varepsilon ^{-3}} 
\right).
\]

б)** Предложим другой (более эффективный) способ оценивания. Для 
этого введем константу $M>1$ и положим
\[
h_l =M^{-l}T,
\quad
\overline {Y}_l =\frac{1}{N_l }\sum\limits_{i=1}^{N_l } {\left( {f\left( {\hat 
{S}_{T \mathord{\left/ {\vphantom {T {h_l }}} \right. 
\kern-\nulldelimiterspace} {h_l }}^{\left( i \right)} } \right)-f\left( 
{\hat {S}_{T \mathord{\left/ {\vphantom {T {h_{l-1} }}} \right. 
\kern-\nulldelimiterspace} {h_{l-1} }}^{\left( i \right)} } \right)} 
\right)} ,
\]
\[
\overline {Y}_0 =\frac{1}{N_0 }\sum\limits_{i=1}^{N_0 } {f\left( {\hat {S}_{T 
\mathord{\left/ {\vphantom {T {h_0 }}} \right. \kern-\nulldelimiterspace} 
{h_0 }}^{\left( i \right)} } \right)} ,
\quad
\overline {Y}=\sum\limits_{l=0}^L {\overline {Y}_l } .
\]
Покажите, что
\[
\mbox{Bias}=\mathbb{E}\left[ {\overline {Y}-Y} \right]={\it O}\left( {h_L } \right),
\]
\[
V_l =D\left[ {f\left( {\hat {S}_{T \mathord{\left/ {\vphantom {T {h_l }}} 
\right. \kern-\nulldelimiterspace} {h_l }}^{\left( i \right)} } 
\right)-f\left( {\hat {S}_{T \mathord{\left/ {\vphantom {T {h_{l-1} }}} 
\right. \kern-\nulldelimiterspace} {h_{l-1} }}^{\left( i \right)} } \right)} 
\right]={\it O}\left( {h_l } \right),
\]
Мы хотим, чтобы
\[
\sqrt {\mbox{MSE}} =\sqrt {\mbox{Bias}^2+\Var\left[ {\overline {Y}} \right]} \le 
\mbox{Bias}+\sqrt {\Var\left[ {\overline {Y}} \right]} \sim \varepsilon ,
\]
что достигается, если положить
\[
L={\log \left( {\varepsilon ^{-1}} \right)} \mathord{\left/ {\vphantom 
{{\log \left( {\varepsilon ^{-1}} \right)} {\log M}}} \right. 
\kern-\nulldelimiterspace} {\log M}+{\it O}\left( 1 \right),
\quad
\Var\left[ {\overline {Y}} \right]=\sum\limits_{l=0}^L {N_l^{-1} V_l } \sim 
\sum\limits_{l=0}^L {N_l^{-1} h_l } \sim \varepsilon ^2.
\]
Учитывая это, покажите, что решение задачи $$\mbox{Total}\left( \varepsilon 
\right)=\sum\limits_{l=0}^L {N_l h_l } \to \mathop {\min }\limits_{\left\{ 
{N_l } \right\}\ge 0}$$ 
при ограничении $\sum\limits_{l=0}^L {N_l^{-1} h_l } 
={\it O}\left( {\varepsilon ^2} \right)$ имеет вид $N_l ={\it O}\left( 
{\varepsilon ^{-2}Lh_l } \right)$. Таким образом, $\mbox{Total}\left( 
\varepsilon \right)={\it O}\left( {\varepsilon ^{-2}\left( {\log \varepsilon 
} \right)^2} \right)$.

\end{problem}

\begin{remark}
Описанный в п. б) метод был предложен относительно 
недавно в контексте разработки эффективных численных методов оценки 
финансовых инструментов на рынке, поэтому он попал далеко не во все 
классические монографии на эту тему: P.~Glasserman Monte Carlo methods in financial 
engineering // Springer, 2005; C.~Graham, D.~Talay Mathematical foundation of stochastic 
simulation // Series ``Stochastic modelling and applied probability''. 2013, V.~68. 
 Тем не менее, мы рекомендуем эти книги для погружения в~область 
численных методов финансовой математики.

\end{remark}


==> abstract.tex <==
\thispagestyle{empty} 

УДК 519.21
 
 $ $ \\ $ $ \\
 
%\premierAuthors, \autresAuthors. 
Н.О. Бузун, А.В. Гасников, Ф.О. Гончаров, О.Г. Горбачев, С.А. Гуз, Е.А. Крымова, А.А. Натан, Е.О. Черноусова. Стохастический анализ в задачах: Учебно-методическое пособие. Под ред. А.В. Гасникова. Часть 1 / МФТИ. М.--Д., 2015, изд. 3-е, доп.

$ $ \\ 
 
\begin{abstract}

Содержит программу, список литературы и задачи одноименного курса, читаемого сотрудниками кафедры Математических основ управления студентам факультета управления и прикладной математики Московского физико-технического института. Задачи могут быть использованы в качестве упражнений на семинарских занятиях, сдачах заданий, экзаменах, а также при самостоятельном освоении курса. В новое издание добавлен ряд задач, отражающих также опыт преподавания вероятностных дисциплин в Независимом московском университете и опыт наших коллег из ПреМоЛаб МФТИ, преподающих вероятностные дисциплины в ведущих научных центрах Германии и Франции. Данный сборник задач разрабатывался с учетом направлений подготовки: студентов МФТИ, студентов НМУ, магистров факультета Компьютерных наук ВШЭ и магистров факультета Прикладной математики и информационных технологий БФУ им. И.~Канта.  

 $ $ \\ $ $ \\ $ $ \\ $ $ \\ $ $ 

\noindent рецензенты: д.ф.-м.н. А.В. Колесников \\
\noindent проф. Факультета математики НИУ ВШЭ \\
\noindent д.ф.-м.н. А.Н. Соболевский \\ 
\noindent проф. Независимого московского университета, \\ зам. директора ИППИ РАН 

\end{abstract}


  
 \newpage 

==> additions.tex <==
\section{Вспомогательные материалы}

\subsection*{Метод зеркального спуска}

Рассмотрим задачу стохастической онлайн оптимизации\footnote{ Запись $\Exp_{\xi 
^k} \left[ {f_k \left( {x;\xi ^k} \right)} \right]$ означает, что 
математическое ожидание берется по $\xi^k$, то есть $x$ и $f_k $ понимаются 
в такой записи не случайными. Отметим, что $\xi ^k$ может зависеть от $\xi 
^1$, {\ldots}, $\xi ^{k-1}$, а распределение $\xi^k$ может зависеть от $x$.}
\begin{equation}
\label{eq1}
\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi ^k} \left[ {f_k \left( {x;\xi ^k} 
\right)} \right]} \to \mathop {\min }\limits_{x\in S_n \left( 1 \right)} 
,
\end{equation}
\[
S_n \left( 1 \right)=\left\{ {x\ge 0: \; \sum\limits_{i=1}^n {x_i =1} } 
\right\}
\]
при следующих условиях:

\begin{enumerate}
\item $\Exp_{\xi^k} \left[ {f_k \left( {x;\xi ^k} \right)} \right]\quad -$ выпуклые функции (по $x)$, для этого достаточно выпуклости по $x$ функций $f_k \left( {x;\xi ^k} \right)$;
\item Существует такой вектор $\nabla _x f_k \left( {x;\xi ^k} \right)$, который для компактности будем называть субградиентом, хотя последнее верно не всегда, что
\[
\Exp_{\xi ^k} \left( {\left. {\nabla _x f_k \left( {x;\xi ^k} \right)-\nabla _x 
\Exp_{\xi ^k} \left[ {f_k \left( {x;\xi ^k} \right)} \right]} \right|\Xi 
^{k-1}} \right)\equiv 0,
\]
где $\Xi ^{k-1}$ -- $\sigma $-алгебра, порожденная с.в. 
$\xi ^1, \ldots ,\xi ^{k-1}$. Далее мы будем использовать 
обозначения обычного градиента для векторов, которые мы назвали здесь 
субградиентами. 
%В частности, если мы имеем дело с обычным субградиентом, то 
%запись $\nabla _x f_k \left( {x;\xi ^k} \right)$ в вычислительном контексте 
%(например, в итерационной процедуре МЗС, описанной ниже) означает какой-то 
%его элемент (не важно какой именно), а если в контексте проверки условий 
%(например, в условии 3 ниже), то $\nabla _x f_k \left( {x;\xi ^k} \right)$ 
%пробегает все элементы субградиента (говорят также, субдифференциала);

\item $\left\| {\nabla _x f_k \left( {x;\xi ^k} \right)} \right\|_\infty \le M\quad -$ (равномерно, с вероятностью 1) ограниченный субградиент. Для справедливости части утверждений достаточно требовать одно из следующих (более слабых) условий:
\end{enumerate}
\begin{center}
 $1) \Exp_{\xi ^k} \left[ {\left\| {\nabla _x f_k \left( {x;\xi ^k} \right)} 
\right\|_\infty ^2 } \right]\le M^2$; $2) \Exp_{\xi ^k} \left[ {\left. {\exp 
\left( {\frac{\left\| {\nabla _x f_k \left( {x;\xi ^k} \right)} 
\right\|_\infty ^2 }{M^2}} \right)} \right|\Xi ^{k-1}} \right]\le \exp 
\left( 1 \right)$.
\end{center}

Онлайновость постановки задачи допускает, что на каждом шаге $k$ функция 
$f_k $ может подбираться из рассматриваемого класса функций враждебно по 
отношению к используемому нами методу генерации последовательности $\left\{ 
{x^k} \right\}$. В частности, $f_k $ может зависеть от $\left\{ {x^1,\xi 
^1;...;x^{k-1},\xi ^{k-1};x^k} \right\}$, если выбор $x^k$ осуществляется 
исходя только из информации $\left\{ {x^1,\xi ^1;...;x^{k-1},\xi ^{k-1}} 
\right\}$, т.е. без дополнительной рандомизации. Ситуация с дополнительной 
рандомизацией при выборе $x^k$ рассматривается в следующем пункте.

Для решения задачи (\ref{eq1}) воспользуемся адаптивным методом зеркального спуска (точнее двойственных усреднений). Положим $x_i^1 =1 \mathord{\left/ 
{\vphantom {1 n}} \right. \kern-\nulldelimiterspace} n$, $i=1,...,n$. Пусть 
$t=1,...,N-1$.

\underline {Алгоритм МЗС1-адаптивный}

\[
x_i^{t+1} \propto \exp \left( {-\frac{1}{\beta _{t+1} }\sum\limits_{k=1}^t 
{\frac{\partial f_k \left( {x^k;\xi ^k} \right)}{\partial x_i }} } 
\right),\quad i=\overline{1,n},\; \beta _t 
=\frac{M\sqrt t }{\sqrt {\ln n} }.
\]

\begin{theorem}
Пусть справедливы условия а, б, в.1, тогда
\[
\mbox{ }\frac{1}{N}\sum\limits_{k=1}^N {\Exp\left[ {f_k \left( {x^k;\xi ^k} 
\right)} \right]} -\mathop {\min }\limits_{x\in S_n \left( 1 \right)} 
\frac{1}{N}\sum\limits_{k=1}^N {\Exp \left[ {f_k \left( {x;\xi ^k} 
\right)} \right]} \le 2M\sqrt {\frac{\ln n}{N}} .
\]
Если $f_k = f$, а $\left\{ {\xi ^k} \right\}$ -- независимы и одинаково распределены, как $\xi$, то
\[
\Exp\left[ {f\left( {\frac{1}{N}\sum\limits_{k=1}^N {x^k} ;\xi } \right)} 
\right]-\mathop {\min }\limits_{x\in S_n \left( 1 \right)} \Exp \left[ 
{f\left( {x;\xi } \right)} \right]\le 2M\sqrt {\frac{\ln n}{N}} .
\]
Пусть справедливы условия а, б, в, тогда\footnote{ Запись\par ``$\PR_{x^1,...,x^N} \left\{ 
{\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi ^k} \left[ {f_k \left( {x^k;\xi ^k} 
\right)} \right]} -...} \right.$''\par означает, что внутри фигурных скобок мы 
считаем математическое ожидание по $\xi ^k$ при фиксированных $x^k$.} при $\Omega \ge 0$
\[
\PR_{x^1,...,x^N} \left\{ {\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi ^k} \left[ 
{f_k \left( {x^k;\xi ^k} \right)} \right]} -\mathop {\min }\limits_{x\in S_n 
\left( 1 \right)} \frac{1}{N}\sum\limits_{k=1}^N {\Exp \left[ {f_k 
\left( {x;\xi ^k} \right)} \right]} \ge } \right.
\]
\[
\left. {\frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {8\Omega } } 
\right)} \right\} \le \exp \left( {-\Omega } \right).
\]
Если $f_k = f$, а $\left\{ {\xi ^k} \right\}$ -- независимы и одинаково распределены, как $\xi$, то
\[
\PR_{x^1,...,x^N} \left\{ {\Exp_\xi \left[ {f\left( 
{\frac{1}{N}\sum\limits_{k=1}^N {x^k} ;\xi } \right)} \right]-\mathop {\min 
}\limits_{x\in S_n \left( 1 \right)} \Exp \left[ {f\left( {x;\xi } \right)} 
\right]} \right.
\]
\[
\left. {\ge \frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {8\Omega } } 
\right)} \right\} \le \exp \left( {-\Omega } \right).
\]
\end{theorem}

\textbf{Замечание.} Для задач стохастической выпуклой оптимизации (см., 
например, Shapiro A., Dentcheva D., Ruszczynski A. Lecture on stochastic programming. Modeling and theory. MPS-SIAM series on Optimization, 2009), в которых $\left\{ {\xi ^k} \right\}$ -- 
независимые случайные величины, можно привести оценку вероятностей больших 
уклонений с точностью до констант аналогичную оценке, приведенной в теореме 
и для случая, когда вместо условия в) предполагается условие в.2 при этом в 
правой части неравенства под вероятностью вместо $\sqrt \Omega $ необходимо 
писать $\Omega $ (с точностью до констант).

Снова рассмотрим постановку задачи стохастической онлайн оптимизации (\ref{eq1}). Но на этот раз будем допускать, что метод генерирования последовательности 
$\left\{ {x^k} \right\}$ может допускать (внешнюю, дополнительную) 
рандомизацию. Т.е.  вместо   Также как и раньше онлайновость постановки задачи допускает, 
что на каждом шаге $k$ функция $f_k $ может подбираться из рассматриваемого 
класса функций враждебно по отношению к используемому нами методу генерации 
последовательности $\left\{ {x^k} \right\}$. В частности, $f_k $ и $\xi ^k$ 
могут зависеть от $\left\{ {x^1,\xi ^1;...;x^{k-1},\xi ^{k-1}} \right\}$, и 
даже от распределения вероятностей $p^k$ (многорукие бандиты), согласно 
которому осуществляется выбор $x^k$. Чтобы можно было работать с таким 
классом задач, нам придется наложить дополнительное условие:


г) На каждом шаге генерирование случайной величины $x^k$ согласно распределению вероятностей $p^k$ осуществляется независимо ни от чего.

Положим $p_i^1 =x_i^1 =1 \mathord{\left/ {\vphantom {1 n}} \right. 
\kern-\nulldelimiterspace} n$, $i=1,...,n$. Пусть $t=1,...,N-1$.

$ $

\underline {Алгоритм МЗС2-адаптивный}

\noindent Согласно распределению вероятностей

\[
p_i^{t+1} \propto \exp \left( {-\frac{1}{\beta _{t+1} }\sum\limits_{k=1}^t 
{\frac{\partial f_k \left( {x^k;\xi ^k} \right)}{\partial x_i }} } 
\right), \quad i=\overline{1,n},\;
\beta _t =\frac{M\sqrt t }{\sqrt {\ln n} },
\]
получаем случайную величину 
$i\left( {t+1} \right)$, т.е. \\ $x_{i\left( {t+1} \right)}^{t+1} =1,\;\;x_j^{t+1} 
=0,\;j\ne i\left( {t+1} \right).$



\underline {Алгоритм МЗС2-неадаптивный (заранее известно $N$)}

\noindent Согласно распределению вероятностей

\[
p_i^{t+1} \propto \exp \left( {-\frac{1}{\beta _{t+1} }\sum\limits_{k=1}^t 
{\gamma _k \frac{\partial f_k \left( {x^k;\xi ^k} \right)}{\partial x_i }} } 
\right),\quad i=\overline{1,n},
\]
\[
\gamma _k \equiv M^{-1}\sqrt {{2\ln n} \mathord{\left/ {\vphantom {{2\ln n} 
N}} \right. \kern-\nulldelimiterspace} N} ,
\quad
\beta _t \equiv 1,
\]
получаем случайную величину 
$i\left( {t+1} \right)$, т.е. \\ $x_{i\left( {t+1} \right)}^{t+1} =1,\;\;x_j^{t+1} 
=0,\;j\ne i\left( {t+1} \right).$

Аппроксимируя
\[
\mathop {\min }
\limits_{x\in S_n \left( 1 \right)} 
\frac{1}{N}
\sum_{k=1}^t 
f_k \left( x \right) \approx \mathop {\min} \limits_{x\in S_n \left( 1 \right)}  
\frac{1}{N}\sum\limits_{k=1}^t 
\left\{ 
  f_k \left( x^k  \right)+
  \left\langle \nabla f_k \left( {x^k } 
   \right),x-x^k  \right\rangle  
\right\} ,
\]
получим
\[
\PR\left( {x_j^{t+1} =1;\;x_i^{t+1} =0,\;i\ne j} \right)\mathop =
\]
\[ 
= \PR_\varsigma \left( {j=\arg \mathop {\max }\limits_{i=1,...,n} \left\{ 
{\sum\limits_{k=1}^t {\left[ {-\nabla f_k \left( {x^k } \right)} \right]_i 
+\varsigma _{t,i} } } \right\}} \right),
\]
где $\varsigma _{t,i} $ -- независимые одинаково распределенные случайные 
величины по закону Гумбеля с параметром $\beta _{t+1} $, характеризующим 
среднеквадратичное отклонение $\varsigma _{t,i} $ (см. задачу \ref{gumbel} раздела 
\ref{hard}):\footnote{ Поскольку случайные величины $\varsigma _{t,i} $ получаются в 
результате суммирования $t$ слагаемых (невязок в аппроксимации выпуклой 
функции линейными минорантами), то можно ожидать, что среднеквадратичное 
отклонение $\varsigma _{t,i} $ имеет порядок $\sqrt t $. Условие одинаковой 
распределенности $\varsigma _{t,i} $, которое не понятно за счет чего может 
иметь место, в действительности, не очень здесь и нужно. Достаточно, чтобы 
$E\left[ {\varsigma _{t,i} -\varsigma _{t,j} } \right]=o\left( {\sqrt t } 
\right)$ и $\mbox{Var}\left[ {\varsigma _{t,i} } \right]\sim \sqrt t $. 
Более того, если, с некоторой натяжкой, наряду с независимостью $\left\{ 
{\varsigma _{t,i} } \right\}_{i=1}^n $ также считать, что при формировании 
$\varsigma _{t,i} $ суммируются независимые слагаемые, то можно ожидать, что 
$\varsigma _{t,i} $ нормальные случайные величины (центральная предельная 
теорема). Следовательно, в контексте последующих операций при $n\gg 1$, 
$\varsigma _{t,i} $ могут быть заменены на случайные величины, 
распределенные по закону Гумбеля с соответствующими среднеквадратичными 
отклонениями. }
\[
P\left( {\varsigma _{t,i} <\tau } \right)=\exp \left\{ {-e^{-\tau 
\mathord{\left/ {\vphantom {\tau {\beta _{t+1} }}} \right. 
\kern-\nulldelimiterspace} {\beta _{t+1} }}} \right\}.
\]
Тогда (см. задачу \ref{gibbs} раздела \ref{hard})
\[
E_\varsigma \left[ {x^{t+1}} \right]=\nabla W_{\beta _{t+1} } \left( 
{-\sum\limits_{k=1}^t {\nabla f_k \left( {x^k } \right)} } \right).
\]
Распределение Гумбеля возникает именно в таком контексте совсем не случайно, 
и связано это с тем, что оно max-устойчиво. 
Другими словами, при некоторых довольно общих предположениях (типа Крамера) 
$\varsigma _{t,i} $ могут быть распределенными произвольно, тем не менее, 
при $n\gg 1$ с хорошей точностью можно считать, что мы в итоге имеем дело с 
соответствующим распределением Гумбеля. Более того, если задаться вопросом: 
а какое распределение ``наиболее подходит'' для $\varsigma _{t,i} $, чтобы в 
случае ``враждебной Природы'' (то есть в минимаксном смысле) иметь наилучшие 
оценки, то ответом будет: симметричное показательное распределение 
(Лапласа), которое ведет себя в интересном для анализа диапазоне подобно 
распределению Гумбеля, но в отличие от распределения Лапласа, в случае 
Гумбеля мы явно можем посчитать интересующие нас вероятности. Как правило, 
такого рода задачи явно не решаются, и распределение Гумбеля является 
приятным исключением, для которого есть явные формулы. 

К сожалению, не делая относительно функций $f_k \left( {x;\xi ^k} \right)$ 
дополнительно никаких предположений, не удается доказать для МЗС2 аналог 
теоремы 1. Чтобы можно было сформулировать такой аналог, мы вынуждены будем 
предполагать, что $f_k \left( {x;\xi ^k} \right)$ -- линейные функции по $x$ 
(можно обобщить и на сублинейные). С одной стороны это существенно сужает 
класс задач, к которым применим МЗС2. С другой стороны, как будет 
продемонстрировано в следующем пункте, даже такой узкий класс функций за 
счет ``онлайновости'' позволяет применять МЗС2 к довольно широкому кругу 
задач. Для того чтобы лучше чувствовалась преемственность методов и 
доказательств их сходимости, далее мы по-прежнему будем использовать общие 
обозначения $f_k \left( {x;\xi ^k} \right)$, не подчеркивая в формулах 
линейность.

\begin{theorem}

Пусть справедливы условия а, б, в.1, г и $f_k \left( {x;\xi ^k} \right)$ -- линейные функции по $x$, тогда
\[
\frac{1}{N}\sum\limits_{k=1}^N {\Exp\left[ {f_k \left( {x^k;\xi ^k} \right)} 
\right]} -\mathop {\min }\limits_{x\in S_n \left( 1 \right)} 
\frac{1}{N}\sum\limits_{k=1}^N {\Exp\left[ {f_k \left( {x;\xi ^k} \right)} 
\right]} \le 2M\sqrt {\frac{\ln n}{N}} .
\]
Для неадаптивного метода ``2''-у перед $M$ можно занести под знак корня.
Кроме того если справедливы условия а, б, в, г, при  $\Omega \ge 0$
\[
\PR_{x^1,...,x^N} \left\{ {\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi ^k} \left[ 
{f_k \left( {x^k;\xi ^k} \right)} \right]} -\mathop {\min }\limits_{x\in S_n 
\left( 1 \right)} \frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi ^k} \left[ {f_k 
\left( {x;\xi ^k} \right)} \right]} \ge } 
\right.
\]
\[
\left. {\frac{2M}{\sqrt N 
}\left( {\sqrt {\ln n} +\sqrt {18\Omega } } \right)} \right\} \le \exp 
\left( {-\Omega } \right).
\]
Если $f_k \left( {x;\xi ^k} \right) = f_k \left( x \right)$ , то это неравенство можно уточнить
\[
\frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {18\Omega } } \right)\to 
\frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {2\Omega } } \right),
\]
при этом же условии для неадаптивного метода можно еще больше уточнить:
\[
\frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {2\Omega } } \right)\to 
\frac{\sqrt 2 M}{\sqrt N }\left( {\sqrt {\ln n} +2\sqrt \Omega } \right).
\]

\end{theorem}

==> algorithms.tex <==
\section{Вероятностные методы в Computer Science}
\label{CS}

%\subsection{Рандомизированные алгоритмы}

\begin{comment}
\begin{problem}

Пять философов сидят за круглым столом. В центре стола находится чаша со
спагетти. Между каждой парой соседних философов лежит вилка. Философы чередуют размышления с приемами пищи, не отвлекаясь на второстепенные занятия. Однако
для того, чтобы вытащить спагетти из чаши и донести их до рта философу требуются
две вилки. Каждый философ может взять вилку рядом с ним (если она доступна), или положить - если он уже держит её. Если требуемая вилка занята соседом, голодный философ вынужден ждать - он не может вернуться к размышлениям, не поев. После окончания еды философ кладет обе вилки на стол.

Время одного приема пищи одним философом равномерно распределено на отрезке [0, a]. 
Время одного размышления равномерно распределено на отрезке [0, b].

Данный процесс подвержен взаимной блокировке (Dead Lock): например, если каждый возьмет по левой вилке, то начнется вечное голодание. Для избежания блокировки каждый философ кладет первую вилку, если за время t после ее взятия вторая не освободилась.

Требуется определить распределение времени t, минимизирующее среднее время ожидания после размышления и перед приемом пищи.

\end{problem}
\end{comment}

\begin{problem}
\noindent Алгоритм быстрой сортировки основан на парадигме ``разделяй и властвуй''. Выбирается из элементов массива опорный элемент, относительно которого переупорядочиваются все остальные элементы. Желательно выбрать опорный элемент близким к значению медианы, чтобы он разбивал список на две примерно равные части. Переупорядочивание элементов относительно опорного происходит так, что все переставленные элементы, лежащие левее опорного, меньше его, а те, что правее -- больше или равны опорному. Далее процедура быстрой сортировки рекурсивно применяется к левому и правому списку для их упорядочивания по отдельности.

Наихудшие входные данные для описанного алгоритма быстрой сортировки (предполагается, что в качестве опорного элемента выбирается последний элемент обрабатываемого массива) -- элементы уже упорядоченные по возрастанию. 
Откуда следует, что асимптотика времени работы быстрой сортировки в худшем случае $\Theta (n^{2} )$.

Оценить время работы алгоритма быстрой сортировки в среднем. 


\begin{ordre}
Получить рекуррентное соотношение для математического ожидания времени работы, введя индикаторную функцию позиции опорного элемента. 
Воспользоваться соотношением:
\[\begin{array}{l} {\sum _{k=1}^{n-1}k\log k \le \log \frac{n}{2} \sum _{k=1}^{\left\lceil \frac{n}{2} \right\rceil -1}k +\log n\sum _{k=\left\lceil \frac{n}{2} \right\rceil }^{n-1}k =} \\ {=\frac{n(n-1)}{2} \log n-\frac{\left\lceil \frac{n}{2} \right\rceil \left(\left\lceil \frac{n}{2} \right\rceil -1\right)}{2} \le \frac{1}{2} n^{2} \log n-\frac{n^{2} }{8} } .\end{array}\]
 
\end{ordre}

Показать неулучшаемость оценки для произвольного алгоритма сортировки. Привести способ сортировки с асимптотикой $O(n \log n)$ в худшем случае.

\end{problem}


\begin{problem}[Задача поиска $k$-ой порядковой статистики]

Рекурсивное применение процедуры, основанной на методе быстрой сортировки, позволяет быстро (в среднем) находить $k$-ую порядковую статистику. Задача вычисления порядковых статистик состоит в следующем: дан список (массив) из $n$ чисел, необходимо найти значение, которое стоит в $k$-ой позиции в отсортированном в возрастающем порядке списке. 

Модифицируем алгоритм быстрой сортировки:


 Выбираем опорный элемент. Делим список на две группы. В первой --- элементы меньше опорного, во второй --- больше либо равны.
 Если размер (число элементов) первой группы больше либо равен $k$, то к ней снова применяется эта процедура. Иначе --- вызывается процедура для второй группы.
 
Покажите, используя ту же технику, что и при анализе в среднем алгоритма быстрой сортировки, что среднее время работы такого алгоритма линейно.

\begin{ordre}

\noindent Покажите, что выполняется оценка среднего времени работы алгоритма:

\[
\Exp [T(n)]\le \Exp\left\{\sum _{k=1}^{n}T\left(\max (k-1,n-k)\right)+O(n)\right\} 
\]
\[ \le \frac{2}{n} \sum _{k=\left\lfloor \frac{n}{2} \right\rfloor }^{n-1} \Exp[T(k)] + O(n).
\]



\end{ordre}
\end{problem}



\begin{problem}[Задача о рюкзаке] 

Рассмотрим  NP-трудную задачу
\[\sum _{j=1}^{n}x_{j}  \to \max , x_{j} \in \left\{0,\; 1\right\}, j=1,...,n;\] 
\[\sum _{j=1}^{n}a_{ij} x_{j}  \le 1, i=1,\ldots,m,                         (*)\] 
где $a_{ij} \in \left\{0,\; 1\right\}$, $i=1,\ldots,m$, $j=1,\ldots,n$.

Булев вектор $\vec{x}$ длины $n$ будем называть допустимыми, если он удовлетворяет системе (*). Обозначим через $T\left(j\right)$ множество всех допустимых булевых векторов для системы (*) с $(n-j)$ нулевыми последними компонентами и через $\vec{e}_{j} $ - вектор длины $n$ с единичной $j$--ой компонентой и с остальными нулевыми компонентами.

Рассмотрим алгоритм: 1) строим множество допустимых решений $T\left(j\right)$ на основе множества $T\left(j-1\right)$, пытаясь добавить вектор $\vec{e}_{j} $ ко всем булевым векторам $T\left(j-1\right)$; 2) среди $\left|T\left(n\right)\right|$ допустимых булевых векторов ищем ``наилучший''.
\begin{enumerate}
\item Покажите, что сложность описанного алгоритма составляет ${\rm O} \left(\left|T\left(n\right)mn\right|\right)$. При каких $a_{ij} \in \left\{0,\; 1\right\}$ алгоритм будет работать экспоненциально долго?

\item Оцените сложность в среднем (математическое ожидание времени работы алгоритма), т.е. ${\rm O} \left(\Exp\left(\left|T\left(n\right)\right|\right)mn\right)$, если с.в. $\left\{a_{ij} \right\}_{i,j=1}^{m,n} $ -- независимые и одинаково распределенные по закону Бернулли \\ $\mathrm{Be}\left(p\right)$ ($mp^{2} \ge \ln n$).
\end{enumerate}

\begin{ordre}
Пусть $k>0$. Положим: $\vec{x}_{j_{1} ,...,j_{k} } $ - вектор с $k$ единицами (на позициях $\left\{j_{1} ,...,j_{k} \right\}$) и $n-k$ нулями; $p_{ki} $ - вероятность выполнения $i$-го неравенства системы (*) для $\vec{x}_{j_{1} ,...,j_{k} } $; $P_{k} $ -- вероятность того, что $\vec{x}^{k} $ -- допустимое решение (покажите, что $p_{ki} $ и $P_{k} $ не зависят от набора $\left\{j_{1} ,...,j_{k} \right\}$). Докажите, что $p_{ki} \le \left(1-p^{2} \right)^{k-1} \le e^{-p^{2} \left(k-1\right)} $, $P_{k} \le e^{-mp^{2} \left(k-1\right)} $ и $\Exp\left(\left|T\left(n\right)\right|\right)=\sum _{k=0}^{n}C_{n}^{k}  P_{k} <1+n+n\sum _{k=2}^{n}e^{\left(k-1\right)\left(\ln n-mp^{2} \right)}  $.
\end{ordre}

\end{problem}

\begin{problem}

Даны три матрицы $A,B,C$ размера $n\times n$. Требуется проверить равенство $AB=C$.

Простой детерминированный алгоритм перемножает матрицы $A$, $B$ и сравнивает результат с $C$. Время работы такого алгоритма при использовании обычного перемножения матриц составляет $O(n^{3} )$, при использовании быстрого - $O(n^{2,376} )$. Вероятностный алгоритм Фрейвалда с односторонней ошибкой проверяет равенство за время $O(n^{2} )$.

Описание вероятностного алгоритма:

\begin{enumerate}
\item \textbf{ }взять случайный вектор $x\in \left\{0,1\right\}^{n}; $

\item  вычислить $y=Bx;$

\item  вычислить $z=Ay;$

\item  вычислить $t=Cx;$

\item  если $z=t$ вернуть «да», иначе «нет».
\end{enumerate}
Покажите, что для предъявленного алгоритма выполняется 
\[\begin{array}{l} {\PR\left\{z=t \vert AB=C\right\}=1,} \\ {\PR\left\{z \neq t \vert AB\ne C\right\}\ge 1/2.} \end{array}\] 

\begin{remark} (амплификация)
Оцените вероятность ошибочного ответа на одной ненулевой строке матрицы $D = AB - C$. Как можно добиться того, чтобы вероятность ошибочного ответа стала меньше 0.01?
\end{remark}

\end{problem}


\begin{problem}
\label{derandom}
Рассмотрим задачу из класса \textit{NP-трудных} задач -- \textit{максимальная выполнимость (MAX-SAT)}: даны $m$ скобок \textit{конъюнктивной нормальной формы }(КНФ) с $n$ переменными, нужно найти значения переменных, максимизирующее число выполненных скобок.

\begin{enumerate}

\item Для \textit{приближенного} решения задачи MAX-SAT воспользуемся простейшим вероятностным алгоритмом, выбирая значения каждой переменной (0 или 1) независимо и равновероятно. Покажите, что такой алгоритм гарантирует точность ${1\mathord{\left/ {\vphantom {1 2}} \right. \kern-\nulldelimiterspace} 2} $: для всех входов $I$

\[\frac{\Exp m_{A} (I)}{m_{0} (I)} \ge \frac{1}{2} ,\] 
где $m_{0} (I)$ - оптимум, $m_{A} (I)$ - случайное значение, найденное алгоритмом. 

\item Алгоритм с лучшими оценками точности строится на основе \textit{метода вероятностного округления}. Для начала переформулируем задачу MAX-SAT в терминах задачи целочисленного линейного программирования (ЦЛП). Каждой скобке $C_{j} $ поставим в соответствие булеву переменную $z_{j} \in \left\{0,1\right\}$, которая равна 1, если скобка $C_{j} $ выполнена; каждой входной переменной $x_{i} $ сопоставляем переменную $y_{i} $, которая равна 1, если $x_{i} =1$, и равна 0 в противном случае. Обозначим $C_{j}^{+} $ индексы переменных в скобке $C_{j} $, которые входят в нее без отрицания, а через $C_{j}^{-} $ - множество индексов переменных, которые входят в скобку с отрицанием. Тогда задача MAX-SAT эквивалентна следующей задаче ЦЛП:

\[\begin{array}{l} {\sum _{j=1}^{m}z_{j}  \to \mathop{\max }\limits_{z,y} } \\ {\sum _{i\in C_{j}^{+} }y_{i} +\sum _{i\in C_{j}^{+} }(1-y_{i} )  \ge z_{j} ,\quad j=1,...,m} \\ {y_{i} ,z_{j} \in \left\{0,1\right\},\quad i=1,...,n,j=1,...,m} \end{array}\] 

Рассмотрим и решим задачу \textit{линейной релаксации} целочисленной программы:

\[\begin{array}{l} {\sum _{j=1}^{m}\hat{z}_{j}  \to \mathop{\max }\limits_{\hat{y},\hat{z}} } \\ {\sum _{i\in C_{j}^{+} }\hat{y}_{i} +\sum _{i\in C_{j}^{+} }(1-\hat{y}_{i} )  \ge \hat{z}_{j} ,\quad j=1,...,m} \\ {\hat{y}_{i} ,\hat{z}_{j} \in \left\{0,1\right\},\quad i=1,...,n,j=1,...,m} \end{array}\] 

Пусть $\hat{y}_{i} ,\; \hat{z}_{j} $ - решения задачи линейной релаксации. Ясно, что $\sum _{j=1}^{m}\hat{z}_{j}  $ является верхней оценкой числа выполненных скобок для данной КНФ.

Рассмотрим вероятностный алгоритм решения задачи максимальной выполнимости, где каждая переменная $y_{i} $ независимо принимает значения 0 или 1 уже не с равными вероятностями, а с вероятностью $\hat{y}_{i} $ принимает значение 1 (и 0 с вероятностью $1-\hat{y}_{i} $). Такой метод называется \textit{вероятностным округлением}.

Докажите, что если в скобке $C_{j} $ имеется $k$ литералов, то вероятность того, что она выполнена при вероятностном округлении, не менее

\[\left(1-\left(1-\frac{1}{k} \right)^{k} \right)\hat{z}_{j} .\] 

\begin{remark}
Тогда из того, что

\[1-\left(1-\frac{1}{k} \right)^{k} \ge 1-\frac{1}{e} >0.63\] 
для всех положительных целых $k$, получаем, что для произвольной КНФ среднее число скобок, выполненное при вероятностном округлении, не меньше $1-\frac{1}{e} >0.63$ от максимально возможного числа выполненных скобок.
\end{remark}

\item Для получения детерминированного алгоритма приближенного решения задачи MAX-SAT воспользуемся один из способов\textit{ дерандомизации -- методом условных математических ожиданий. }Введем случайную величину\textit{ }$Z(x)$, где в булевом векторе $x=(x_{1} ,...,x_{n} )$ компоненты - суть значения переменных в КНФ, назначенных вероятностным алгоритмом - являются независимыми случайными величинами, причем $\PR\left\{x_{i} =1\right\}=p_{i} $, $\PR\left\{x_{i} =0\right\}=1-p_{i} $; $Z(x)$ - число невыполненных скобок. Требуется найти булев вектор $\hat{x}$, для которого выполнено неравенство $Z(\hat{x})\le \Exp Z$. Обозначим через $Z(x|x_{1} =d_{1} ,...,x_{k} =d_{k} )$ новую случайную величину, которая получена из $Z$ фиксированием значений первых $k$ булевых переменных.

Рассмотрим покомпонентную стратегию определения искомого вектора $\hat{x}$. Для определения его первой компоненты вычисляем значения $f_{0} =\Exp Z(x|x_{1} =0)$ и $f_{1} =\Exp Z(x|x_{1} =1)$. Если $f_{0} <f_{1} $ полагаем $x_{1} =0$, иначе полагаем $x_{1} =1$. При определенной таким образом первой компоненты (обозначим ее $d_{1} $) вычисляем значение функционала $f_{0} =\Exp Z(x|x_{1} =d_{1} ,x_{2} =0)$ и $f_{1} =\Exp Z(x|x_{1} =d_{1} ,x_{2} =1)$. Если $f_{0} <f_{1} $ полагаем $x_{2} =0$, иначе полагаем $x_{2} =1$. Фиксируем вторую координату (обозначая ее $d_{2} $) и продолжаем описанный процесс до тех пор, пока не определится последняя компонента решения.

Покажите, что найденный вектор $(x_{1} =d_{1} ,\ldots ,x_{n} =d_{n} )$ будет удовлетворять требованию минимизации оценки математического ожидания:

\begin{enumerate}
\item  для этого докажите неравенство $\Exp Z\ge \Exp Z(x|x_{1} =d_{1} )$;

\item  рекуррентно получите неравенство $\Exp Z\ge \Exp Z(x|x_{1} =d_{1} ,\ldots ,x_{n} =d_{n} )$;

\item  заметьте, что $\Exp Z(x|x_{1} =d_{1} ,\ldots ,x_{n} =d_{n} )=Z(x|x_{1} =d_{1} ,\ldots ,x_{n} =d_{n} )$.
\end{enumerate}

Покажите справедливость формул:
\begin{enumerate} 

\item $\Exp Z=\sum _{j=1}^{m}\PR_{j}$, где $\PR_{j} =\PR\left\{\sum _{i\in C_{j}^{+} }x_{i} +\sum _{i\in C_{j}^{-} }(1-x_{i} )  =0\right\};$
\item в предположении, что значения первых $k$ переменных уже определены и $I_{0} $ --- множество индексов тех переменных, значения которых равно 0, а $I_{1} $ --- множество индексов тех переменных, значения которых равно 1:
$$\Exp Z(x|x_{1} =d_{1} ,\ldots ,x_{k} =d_{k} )=\sum _{j=1}^{m}\PR_{j} ^{k},$$ 
\[ \text{где}\PR_{j} ^{k} = \PR\left\{\sum _{i\in C_{j}^{+} }x_{i} +\sum _{i\in C_{j}^{-} }(1-x_{i} )  =0|x_{1} =d_{1} ,\ldots,x_{k} =d_{k} \right\}=\] 
\[\left\{\begin{array}{cc} {0,} & { \text{при }  (I_{0} \cap C_{j}^{-} ) \cup ( I_{1} \cap C_{j}^{+} ) \ne \emptyset ;} \\ {\prod_{i\in C_{j}^{+} \backslash I_{0} }(1-p_{i} ) \prod _{i\in C_{j}^{-} \backslash I_{1} }p_{i}  ,} & \text{иначе} \end{array}\right. \] 
Здесь $C_{j}^{+} $ --- множество индексов переменных в скобке $C_{j} $, которые входят в нее без отрицания,  $C_{j}^{-} $ --- множество индексов переменных, которые входят в скобку с отрицанием.

\end{enumerate}

\end{enumerate}

\end{problem}

\begin{remark}
Детали см. в  Кузюрин Н.Н., Фомин~С.А. Эффективные алгоритмы и сложность вычислений: Учебное пособие. -- М.: МФТИ, 2007.
\end{remark}




%\begin{comment}

\begin{problem}[Коммуникационная сложность, хэширование]

Требуется сравнить ("достаточно достоверно") две битовые строки $a,b$,  осуществив как можно меньше по битовых сравнений. Основная идея -- сравнивать не сами строки, а функции от них. Так сравниваются $a\; \mod\; p$ и $b\; \mod\; p$, для некоторого простого числа $p$. Для этого требуется передать $2\log p$ бит информации.

Описание алгоритма сравнения строк:

\begin{enumerate}
\item  Пусть $\left|a\right|=\left|b\right|=n$, $N=n^{2} \log  n^{2}; $ 

\item  Выбираем случайное простое число $p$из интервала $\left[2..N\right]$ ;

\item  Выдать «да», если $a\; \mod\; p=b\; \mod\; p\Leftrightarrow (a-b)\equiv 0\; \mod\; p$, иначе выдать «нет».
\end{enumerate}

\noindent  Обоснуйте выбор именно простого числа на шаге 2 и предложите способ его генерации.  

\noindent Покажите что,

\[\begin{array}{l} {\PR\left\{(a-b)\equiv 0,\mod(p)|a=b\right\}=1,} \\ {\PR\left\{(a-b)\equiv 0,\mod(p)|a\ne b\right\}=O(1/n),} \end{array}\] 
 
При этом необходимое количество переданных бит равно $O\left(\log  n\right)$.

\begin{ordre}

Воспользоваться асимптотическим законом распределения простых чисел:
\[\mathop{\lim }\limits_{n\to \infty } \frac{\pi \left(n\right)}{n/\ln n}  =1,\] 
где $\pi \left(n\right)$ - функция распределения простых чисел, равная количеству простых чисел, не превосходящих $n$.

\end{ordre}

\end{problem}

\begin{remark}
В приведенной задаче требуется проверка простоты числа. Согласно малой теореме Ферма, если $N$ - простое число и целое $a$ не делится на $N$, то  
\[a^{N-1} \equiv 1\; \mod\; N.                         \; \; \;            \left(*\right)\] 

Отсюда следует, что если при каком-то $a$ сравнение $\left(*\right)$ нарушается, то можно утверждать, что $N$ - составное. 
К сожалению,  простой вариант подбора $a$ не всегда позволяет эффективно выявить составное число. Имеются составные числа $N$, обладающие свойством $\left(*\right)$ для любого целого $a$ с условием $\left(a,N\right)=1$ ($a$ и $N$ - взаимно простые). Такие числа называются числами Кармайкла.

В 1976 г. Миллер предложил заменить проверку $\left(*\right)$ проверкой несколько иного условия. Если $N$ - простое число, то $N-1=2^{s} t$, где $t$ нечетно, то согласно малой теоремы Ферма для каждого a с условием $\left(a,N\right)=1$ хотя бы одна из скобок в произведении 
\[\left(a^{t} -1\right)\left(a^{t} +1\right)\left(a^{2t} +1\right) \ldots  \left(a^{2^{s-1} t} +1\right)=a^{N-1} -1\] 
делится на $N$. 

Пусть $N$ - нечетное составное число, $N-1=2^{s} t$, где \textbf{$t$ }нечетно. Назовем целое число $a$, $1<a<N$ «выявляющим» для $N$, если нарушается одно из двух условий:

I) $N$ не делится на $a$

II) $a^{t} \equiv 1\; \mod\; N$ или существует целое $k$, $0\le k<s$ такое, что $a^{2^{k} t} \equiv -1\; \mod\; N$.

Если $N$ составное число, то согласно теореме Рабина  существует не менее $\frac{3}{4} \left(N-1\right)$  выявляющих чисел.

\end{remark}

\begin{comment}

\begin{problem}

Пусть $f(x_{1} ,...,x_{n} )=C_{1} \vee \cdots \vee C_{m} $ - булева формула в дизъюнктивной нормальной форме (ДНФ), где каждая скобка $C_{i} $ - есть конъюнкция $L_{1} \wedge \cdots \wedge L_{k_{i} } $ $k_{i} $ литералов (литерал есть либо переменная, либо ее отрицание). Набор значений переменных $a=(a_{1} ,...,a_{n} )$ называется выполняющим для $f$, если $f(a_{1} ,...,a_{n} )=1$. Требуется найти число выполняющих наборов для данной ДНФ.

\noindent $V$ - множество всех двоичных наборов длины $n$.

\noindent $G$ - множество выполняющих наборов.


\noindent  Проведем $N$ независимых испытаний:

\noindent Выбираем случайно $v_{i} \in V$ ( в соответствии с равномерным распределением).
\noindent $y_{i} =f(v_{i} )$. Заметим, что $P\left\{y_{i} =1\right\}=\frac{\left|G\right|}{\left|V\right|} =p$.
Рассмотрим сумму независимых случайных величин $Y=\sum _{i=1}^{N}y_{i}  $. В качестве аппроксимации $\left|G\right|$ возьмем величину $\frac{Y}{N} \left|V\right|$.

\noindent Оцените необходимое число испытаний $N$ как функцию от $|V|$, $|G|$ и точности аппроксимации $\varepsilon$. 

\begin{ordre}
Докажите следующее утверждение. Пусть $X_{1} ,...,X_{n} $ - независимые случайные величины, принимающие значения 0 или 1, при этом $P\left\{X_{i} =1\right\}=p,\quad P\left\{X_{i} =0\right\}=1-p$. Тогда для $X=\sum _{i=1}^{N}X_{i}  $ и для любого $0<\delta <1$, выполнены неравенства
\[\begin{array}{l} {P\left\{X>(1+\delta )EX\right\}\le e^{-\frac{\delta ^{2} }{3} EX} } \\ {P\left\{X<(1-\delta )EX\right\}\le e^{-\frac{\delta ^{2} }{2} EX} } \end{array}\] 
\end{ordre}

\end{problem}


\begin{problem}

(Задача о покрытии). Дано конечное множество из m элементов и система его подмножеств $S_{1} ,...,S_{n} $. Требуется найти минимальную по числу подмножеств подсистему $S_{1} ,...,S_{n} $, покрывающую все множество объектов. 

\noindent Сформулируем ее в терминах булевых матриц и целочисленного линейного программирования:
\[\left\{\begin{array}{l} {cx\to \min ,} \\ {Ax\ge b,} \\ {\forall j\; x_{j} \in \{ 0,1\} .} \end{array}\right. \] 
Здесь переменные $x_{1} ,...,x_{n} $ соответствуют включению подмножеств $S_{1} ,...,S_{n} $ в решение-покрытие, матрица $A$ - матрица инцидентности, $c=(1...1)^{T} \in {\mathbb R}^{n} ,\quad b=(1...1)^{T} \in {\mathbb R}^{m} $ - векторы стоимости и ограничений.

\noindent Пусть элементы матрицы инцидентности -- независимые случайные величины с бернулевским распределением:$P\{ a_{ij} =1\} =p,$ $P\{ a_{ij} =0\} =1-p$. 

\noindent Для решения задачи применяется жадный алгоритм: на каждом шаге выбирается подмножество, максимально покрывающее еще не покрытые объекты. 

Доказать следующее утверждение. Пусть для случайной матрицы $A$, определенной выше, выполнены соотношения:
\[\begin{array}{l} {\forall \gamma >0:} \\ {\frac{\ln n}{m^{\gamma } } \mathop{\to }\limits_{n\to \infty } 0,} \\ {\frac{\ln m}{n} \mathop{\to }\limits_{n\to \infty } 0.} \end{array}\] 
Тогда для $\forall \varepsilon >0:$ $P\left\{\frac{Z}{M} \le 1+\varepsilon \right\}\mathop{\to }\limits_{n\to \infty } 1$, где Z -- решение жадного алгоритма, M -- величина минимального покрытия. 

\begin{fixme}
Добавить указание.
\end{fixme}

\end{problem}

\end{comment}

\begin{comment}
\begin{problem}
А) Пусть имеется генератор случайных чисел, в 
результате обращения к которому появляется 0 или 1 с одинаковой вероятностью 
равной 1/2 (аналог подбрасывания симметричной монеты). Пусть задано 
вещественное число $0\le p\le 1$. С помощью имеющегося генератора определить 
генератор randp, в результате обращения к которому появляется 0 или 1 с 
вероятностями $p$ и $1-p$ соответственно (незначительные отклонения 
допустимы). Оцените сложность в среднем алгоритма получения одного 
случайного числа с помощью randp (затраты определяются числом обращений $к$ 
изначально имеющемуся генератору). 

Б) Пусть имеется генератор 
случайных чисел randp (описанный выше). Известно, что $p\ne 0,\quad p\ne 1$. 
Как с помощью него сконструировать генератор, в результате обращения 
которому появляется 0 или 1 с одинаковой вероятностью 1/2. 

В) Чему равно математическое ожидание числа обращений к изначально имеющемуся 
генератору случайных чисел при построении последовательности пар до 
появления 0,1 или 1,0? Найти сложность в среднем алгоритма получения k 
``равновероятных'' нулей и единиц с помощью сконструированного генератора 
(затраты определяются количеством обращений к изначально имеющемуся 
генератору). Можно ли указать значения $p$, для которых эта сложность имеет 
минимальное и, соответственно, максимальное значение?
\end{problem}
\end{comment}

\begin{problem}[Интерактивные доказательства] 

а) (изоморфизм графов). Авдотье известен изоморфизм $\phi$ графов $G_0$ и $G_1$. Но она посылает Евлампию граф $H =\psi(G_0)$, либо $H =\psi(G_1)$, где $\psi$ -- некоторый другой изоморфизм, не равный $\phi$. Евлампий бросает симметричную монетку и просит изоморфизм либо $H : G_0$, либо $H : G_1$. В первом случае Авдотья  посылает  $\psi$, во втором -- $\psi \phi^{-1}$. Таких партий разыгрывается $N$ штук. Заметим, что в каждой новой партии Авдотья придумывает новую перестановку $\psi$   вершин графа $G_0$. Если $\phi$  -- действительно изоморфизм $G_0 : G_1$, то все проверки Евлампия будут положительны.
Покажите, что если $\phi$ -- блеф, то с вероятностью  $1 - 2^{-N}$  хотя бы одна проверка обнаружит это (та проверка, в которой Евлампий попросил $H : G_1$).

\begin{remark}
Этот пример поучителен с точки зрения ``криптографического фокуса'' -- Авдотья  убедила Евлампия в $G_0 : G_1$ так и не огласив самого изоморфизма $\phi$. Если $\phi$ –- пароль, то диалог можно вести даже в открытую, что служит примером криптосистемы с нулевым разглашением.
\end{remark}

Обоснуйте справедливость данного замечания (Евлампий не получает никакой информации об изоморфизме $\phi$).

б) (неизоморфизм графов). Теперь наделим Авдотью сверхъестественными вычислительными способностями. Для удобства переименуем игроков: ``Prover'' и ``Verifier''. Verifier выбирает случайно (равновероятно) $ i \in \lbrace 0, 1 \rbrace$ и некоторую перестановку $\pi$ вершин графа $G_i$, затем посылает граф $H =\psi(G_i)$ и требует, чтобы Prover определил $i$. Таких партий разыгрывается $N$ штук. Аналогично предыдущему примеру, $\pi$ в каждой новой партии свое. Если графы неизоморфны, то Prover всегда верно определит индекс $i$. Все тесты будут пройдены. Покажите, что иначе с вероятностью $1-2^{-N}$  Prover ошибется хотя бы один раз (хотя бы в одной партии).
 
 \begin{remark}
Заинтересовавшимся в этой теме, можно также порекомендовать посмотреть про цифровую подпись (протокол аутентификации) и электронную систему голосвания в книге Введение в криптографию под ред. В.В. Ященко. М.: МЦНМО, 2013.
\end{remark}
\end{problem}

\begin{problem}[Хеш функции]
\label{hesh_func}
Для компактного хранения данных, индексированных, как правило, ключами целочисленного или строкового форматов, используются хеш-функции, при помощи которых вычисляются  номера ячеек в таблице в зависимости от значения ключа. Пусть хэш-функция задана на множестве ключей $K$ 
\[
h: K \to \{1,\ldots,m\}.
\]  
Заведем таблицу размера $m$, в которой элемент с ключом $k$ будет размещаться по адресу $h(k)$ (во многих случаях $m \ll |K|$). Ключи с одинаковым значением $h(\cdot)$ образуют список, начинающийся с ячейки таблицы. Если всего имеется $n$ элементов, то желательно чтобы количество ключей с одинаковым хеш-значением не  превышало значительно $\alpha = n/m$ (в таком случае длины списков будут ограничены $O(1+\alpha)$). Формально данное свойство может быть сформулировано в виде двух требований:
\begin{enumerate}
\item $h(k)$ является с.в. с равномерным распределением;
\item $\forall k_1, k_2 \in K$ $h(k_1)$ и  $h(k_2)$ независимы.  
\end{enumerate}    
Покажите, что в случае выполнения требований среднее время поиска отсутствующего ключа в таблице составляет $(1+ \alpha)$, а также среднее время поиска присутствующего ключа в таблице составляет $(1+ \alpha/2)$ (где усреднение ведется как по $h(k)$, так и по множеству других присутствующих в таблице ключей). 
\end{problem}

\begin{remark}
Так как хеш-функция является детерминированной, то случайность, присутствующая в требованиях, может быть реализована посредством выбора функции $h$ из некоторого семейства $H$. $H$ называется \textit{универсальным} для множества $K$, если $\forall k_1, k_2 \in K$ вероятность выбрать функцию из $H$, в которой возникает коллизия, не превышает $1/m$. Для универсального семейства справедливы приведенные в задаче оценки времени поиска ключа в таблице. 
Примером универсального семейства $H$ для целых чисел может служить
\[
\{h_{ab}: h_{ab}(k) = ((ak +b) \; \text{mod} \; p) \; \text{mod} \;   m, \; a,b \in \{1,\ldots, p-1\}\},
\]    
где $p$ -- простое число, большее $m$.

Другой пример универсального семейства, используемого при хешировании IP адресов вида $(x_1,x_2,x_3,x_4)$, $x_i \in \{0,\ldots,255\}$ представляет собой 
множество хеш-функций
\[
\{
h_a(x_1,x_2,x_3,x_4) = (a_1 x_1 + a_2 x_2 + a_3 x_3 + a_4 x_4) \; \text{mod} \; p
\}.
\]
где $p$ -- также простое число, большее $m$.
\end{remark}

\begin{problem}[Хеширование без коллизий]
При известном заранее множестве ключей $K, |K| = n$ хеширование без коллизий может быть реализовано при помощи двухуровневой схемы. На первом уровне используется таблица размера $m = n$, для которой хеш функция выбирается случайно из универсального семейства (см. замечание к задаче \ref{hesh_func}). На втором уровне осуществляется хеширование без коллизий (вместо создания списка ключей будем использeтся вторичная хеш-таблица $T_i$, хранящая все ключи, хешированные функцией $h$ в ячейку $i$, со своей функцией $h_i$).  Покажите, что при выборе  на втором уровне таблицы размером $n_i^2$ ($n_i$ -- количество ключей в $i$-й ячейке первого уровня) вероятность возникновения коллизий менее $1/2$ (поэтому для данной ячейки всегда найдется функция $h_i$ свободная от коллизий). Докажите, что существует хеш функция $h$ для первого уровня, при которой затраты памяти составят суммарно $O(n)$.    
\end{problem}

\begin{ordre}
Получите оценку $\Exp \left(\sum_i n_i^2\right) < 2n$, воспользуйтесь неравенством Маркова.
\end{ordre}


\begin{problem}[Bloom filter]
Вероятностная структура данных Bloom filter используется для проверки принадлежности элемента множеству $S$. Она представляет собой массив $A$ длиной $m$ бит и $k$ различных хэш-функций $h_1, \ldots, h_k$, равновероятно отображающих элементы множества  $D \supseteq S$ в позиции массива $A$ ($h_i: S \to \{1, \ldots, m\}$). 
Интерфейс данной структуры включает следующие операции:

\verb|add_element(s)|: устанавливает биты $A[h_1(s)], \ldots, A[h_k(s)]$ равными 1 (изначально все биты равны 0);

\verb|contains(s)|: если биты $A[h_1(s)], \ldots, A[h_k(s)]$ равны 1, то возвращает \verb|true|, иначе \verb|false|;

Последовательно добавив все элементы множества $S$ при помощи операции \verb|add_element|, получим объект структуры данных, который при вызове метода \verb|contains(s)| всегда возвращает \verb|true| при $s \in S$, но не всегда возвращает \verb|false| при  $s \notin S$, так как соответствующие биты могли быть установлены равными 1 за счет других элементов из $S$.     

\verb|approx_size|: возвращает приближенное количество добавленных элементов
 \[
 |S| \approx  - m \frac{\ln (1 - \mathbb{I}/m)}{k},
 \] 
где $\mathbb{I}$ -- сумма элементов $A$. 

\imgh{80mm}{bf.png}{Пример структуры данных Bloom filter ($k = 3$, $m=18$): x, y, z -- принадлежат множеству, w -- не принадлежит.}


Считая события $A[i] = 1$ и $A[j] = 1$ при добавлении $n$ элементов в пустой объект структуры Bloom filter  независимыми, ввиду независимости значений хэш-функций, покажите, что:
\[
\PR(\text{contains(s)} = \text{true} \; | \; s \text{ not in } S) \approx p =  \left( 1 - e^{k n / m} \right)^k.
\]   
Откуда следует, что оптимальные значения $m$ и $k$ могут быть вычислены по формулам:
\[
k = \frac{m}{n} \ln 2, \quad m = -n \frac{\ln p}{(\ln 2)^2}.
\]
\end{problem}

\begin{remark}
Bloom filter  обладает следующими отличительными характеристиками:
\begin{enumerate}
\item При вероятности ошибки $p = 0.01$ требуется всего лишь 9.6 бит на один элемент множества.
\item  Сложность операций \verb|contains| и \verb|add_element| составляет $O(k)$, вне зависимости от $|S|$. Стоит также учесть, что $k$ операций над элементами массива могут быть выполнены параллельно. 
\item Операции объединения и пересечения двух множеств выполняются побитно (за сравнительно короткое время): 
\[
 |S_1 \cup S_2| \approx  - m \frac{\ln (1 - \mathbb{I}_{12}/m)}{k},
 \]   
 \[
 |S_1 \cap S_2| = |S_1| + |S_2| -   |S_1 \cup S_2|,
 \]
где $\mathbb{I}_{12}$ -- скалярное произведение  $A_1 $ и $A_2$. 

\item Сборщик мусора, ровно как и сериализатор могут осуществлять сравнительно быстрые операции чтения/записи/удаления структуры данных Bloom filter, т. к.  $A$ представляет собой единичный объект, состоящий из элементарных типов данных.
\end{enumerate}

Области применения: снижение количества обращений к базе данных, хранящейся на диске в случае отсутствия запрашиваемых данных (Apache Cassandra);  локальная проверка url-адресов на принадлежность списку, хранящемуся на удаленном сервере (Google Chrome); 
выявление содержимого архива (Venti archival storage system);  
\end{remark}

\begin{problem}[Jaccard similarity]
Для измерения близости (веса связи) двух множеств часто используется коэффициент Жаккара:
\[
J(S_1, S_2) = \frac{|S_1 \cap S_2|}{|S_1 \cup S_2|}.
\]
Типичными представителями таких множеств являются списки смежных вершин в графе, изображения, профили пользователей социальных сетей и прочие web-страницы. Вычисление коэффициента Жаккара позволяет выявлять дубликаты, проводить кластеризацию, восстанавливать фрагменты перечисленных выше объектов. 

Для получения попарной близости $S_1, \ldots, S_N$   множеств больших размеров ($|S_i| = s > 500$, $i \in \overline{1,N}$) возникает потребность в приближенном вычислении коэффициента Жаккара, снижающем нагрузку на сеть вычислительного кластера и временную сложность вычислений. Для этой цели достаточно для каждого множества $|S_i|$ найти минимумы $k$ хэш-функций и далее при попарном сравнении оперировать только с набором подмножеств из минимумов. В итоге, временная сложность окажется равной $O(k N^2 + k s N \log N)$, в то время как в исходной задаче сравнения без аппроксимации меры $O(s \log s  N^2)$.

Рассмотрим два варианта приближенного вычисления, базирующиеся на следующем свойстве: пусть $h$ -- хэш-функция, иньективно и равновероятно отображающая элементы множества $\cup_i S_i$ в $\mathbb{N}$, тогда 
 \[
\PR( \min \limits_{s \in S_1} h(s) = \min \limits_{s \in S_2} h(s)) = J(S_1, S_2). 
 \]         
\begin{enumerate}
\item[\textit{1 вар.}] Задействуем $k$ различных хэш-функций. В этом случае оценкой $J$ будет являться доля функций, у которых совпадают минимальные значения на обоих множествах.    
\item[\textit{2 вар.}] Обозначим за $h_{(k)}(S)$ подмножество $S$  из $k$  элементов с наименьшими значениями $h$. Тогда  $J$ можно оценить как $h_{(k)}(S_1) \cap h_{(k)}(S_2) \cap h_{(k)}(S_1 \cup S_2)$.
\end{enumerate}

Сравните временные сложности двух вариантов. Используя метод Чернова  (см. задачу \ref{chernov_th} из раздела \ref{measure}), покажите, что порядок ошибки аппроксимации в обоих вариантах $O(1/ \sqrt{k})$.

\end{problem}


\begin{problem}[EM-алгоритм]
\label{em}

Рассмотрим задачу поиска неизвестных параметров распределения при помощи метода максимального правдоподобия. В ряде случаев, где функция правдоподобия имеет вид, не допускающий удобных аналитических методов исследования, для ее упрощения удобно ввести дополнительные ``скрытые'' (латентные) переменные и воспользоваться EM-алгоритмом.
Пусть требуется найти максимум правдоподобия $L(X,\theta) = \log p(X | \theta)$ в вероятностной модели со скрытыми переменными $Z$
\[
p(X | \theta) = \int p(X, Z | \theta) dZ.
\]
Покажите, что $L(X,\theta)$ можно представить как
\[
L(X,\theta) = \int \log \frac{p(X, Z | \theta)}{q(Z)} q(Z) dZ - \int \log \frac{p(Z | X, \theta)}{q(Z)} q(Z) dZ = 
\]
\[
 = l(X, \theta, q) + \mathcal{KL}(q \Vert p(Z | X, \theta)),
\]
где $q(Z)$ -- произвольное распределение над скрытыми переменными.

Итерационная схема EM-флгоритма состоит в фиксации на шаге $t$ некоторого значения $\theta^{(t)}$ и аппроксимации в этой точке правдоподобия с помощью его нижней оценки $l(\cdot)$:
\[
q(Z) = p(Z | X, \theta^{(t)}), \quad l(X, \theta, q) \to \max_{\theta}.
\]
Expectation step: фиксируется значение параметров $\theta^{(t)}$. Оценивается распределение на скрытые переменные
\[
q(Z) = p(Z |X, \theta^{(t)}) = \frac{p(X, Z | \theta^{(t)})} {p(X|\theta^{(t)})};
\]
Maximization step: фиксируется распределение $p(Z|X, \theta)$ и выполняется поиск новых параметров
\[
\theta^{(t+1)} = \arg\max_{\theta} \Exp_q \log p(X,Z|\theta).
\]
Покажите, что 
\[
L(X,\theta^{(t+1)}) \geq L(X,\theta^{(t)}),
\]
а также при гладкости $L$
\[
\frac{\partial L}{\partial \theta} \bigg|_{\theta^{(\infty)}} = 0.
\]
\end{problem}

\begin{ordre}
Воспользуйтесь конструкцией
\[
\theta^{(t+1)} = \arg \max \limits_{\theta} \{ Q(\theta)  - b_t \mathcal{R} (\theta, \theta^{(t)})\},
\]
где $\mathcal{R} (\theta, \theta^{(t)}) \geq 0$ -- регуляризатор, в нашем случае равный $\mathcal{KL}(\cdot\Vert\cdot) $.
\end{ordre}


\begin{problem}[Pазделение смеси распределений]


%Рассмотрим задачу поиска неизвестных параметров распределения при помощи метода максимального правдоподобия. В ряде случаев, где функция правдоподобия имеет вид, не допускающий удобных аналитических методов исследования, но допускающий серьезные упрощения, если в задачу ввести дополнительные ``скрытые'' (латентные) переменные, удобно воспользоваться EM-алгоритмом.

%В общем случае ЕМ-алгоритм может быть представлен в следующем виде. Пусть $X$ -- наблюдаемые переменные (выборка), $Z$ -- скрытые переменные с вариационным распределением $q$, $\theta$ -- искомые параметры,  $L(\theta, X, Z) = p(X,Z | \theta)$, $L(\theta, X) = \int p(X,z | \theta) p(z | \theta) dz$,
%\[
%\mathcal{F}(q, \theta) = \Exp_q[\log L(\theta, X, Z)] + H_q(q)  = L
%(\theta, X) - \mathcal{KL}(q \Vert p(Z | X, \theta)) 
%\]

%\begin{enumerate}
%\item[1)] Expectation step:
%\[
%q^{(t)} = \arg \max \limits_q \mathcal{F}(q, \theta^{(t)})
%\]
%\item[2)] Maximization step:
%\[
%\theta^{(t+1)} = \arg \max \limits_{\theta} \mathcal{F}(q^{(t)}, \theta)
%\]

%\end{enumerate}

Целью разделения смеси является как восстановление плотности наблюдаемых данных $X$, так и покомпонентная их категоризация (каждый элемент выборки  $X$ принадлежит одному из распределений, входящих в осотав смеси).
Допустим, что плотность распределения в $z$-й компоненте смеси равна $p (x | z) = p (x | z, \alpha_z)$, т.е. известна с точностью до параметра $\alpha_z$. Тогда плотность $x \in X$ можно аппроксимировать смесью 
\[
p_{\theta}(x) = \sum \limits_{z = 1}^K w_i \; p (x | z),
\]
где $\theta = (w_1, \ldots, w_K, z_1, \ldots, z_K)$, $w_i \geq 0$, $\sum_i w_i = 1$, $K$ -- количество компонент смеси. Правдоподобие $X$ задается формулой 
\[
\log L(\theta, X) = \sum \limits_{j=1}^{n} \left(\log  \sum \limits_{z = 1}^K w_i p (x_j | z) \right). 
\]
Непосредственный поиск точки максимума данной функции весьма затруднителен. Для упрощения вычислений применим EM-алгоритм (см. задачу \ref{em}),  сопоставив каждому $x_j$  скрытую переменную $z_j$ -- номер компоненты смеси, породившей  $x_j$, т. е.  $x_j \sim p(x | z_j)$. 
Проверьте, что при такой модификации данных, функция правдоподобия примет вид

\[
\log L(\theta, X, Z) = \sum \limits_{j=1}^{n} \log w_{z_j} + \sum \limits_{j=1}^{n} \log  p (x_j | z_j). 
\]
Покажите, что шагами  EM-алгоритма в этом случае будут 

\begin{enumerate}
\item[1)] Expectation step:
\[
q_{j}^{(t)}(z) \propto w_{z}^{(t)} \; p (x_j | z, \alpha_z^{(t)});
\]
\item[2)] Maximization step:
\[
w_z^{(t+1)} = \frac{1}{n}   \sum \limits_{j=1}^{n} q_{j}^{(t)}(z),
\]
\[
\alpha_z^{(t+1)} = \arg \max \limits_{\alpha}  \sum \limits_{j = 1}^n q_{j}^{(t)}(z) \; p (x_j | z, \alpha). 
\]
\end{enumerate}

\end{problem}

\begin{comment}
Приведем два важных обобщения EM-алгоритма:
\begin{enumerate}
\item PP-алгоритм (см. Васильев, Методы оптимизации – М.: Факториал Пресс, 2002): 
\[
Q(\theta) \to \max
\]
\[
\theta^{(t+1)} = \arg \max \limits_{\theta} \{ Q(\theta)  - b_t \mathcal{R} (\theta, \theta^{(t)})\},
\]
где $\mathcal{R} (\theta, \theta^{(t)}) \geq 0$ -- регуляризатор, в нашем случае равный $\mathcal{KL}(q \Vert p(Z | X, \theta)) $.

\item Variational EM: 
\[
\mathcal{F}(q, \theta)  = \mathcal{F}(q_z(z) \cdot q_\theta(\theta)) = \log p(X) - \mathcal{KL}(q_z  q_\theta \Vert p(Z, \theta | X)). 
\] 

\begin{enumerate}
\item[1)] Expectation step:
\[
q_z^{(t)}(z)  \propto \mathrm{exp} \left\{ \int \log p(X, z, \theta) q_\theta^{(t)}(\theta) d \theta \right\}
\]

В случае $p(X, Z | \theta) = h(X, Z) g(\theta) e^{\phi(\theta)^T u(X, z)}$
\[
q_z^{(t)}(z)  \propto h(X, Z) e^{\phi^T u(X, z)} , \quad \phi^{(t)} = \int  \phi(\theta) \; q_\theta^{(t)}(\theta) d \theta. 
\]
\item[2)] Maximization step:
\[
q_\theta^{(t+1)}(\theta)  \propto \mathrm{exp} \left\{ \int \log p(X, z, \theta) q_z^{(t)}(z) dz \right\}.
\]

\end{enumerate}

\end{enumerate}
\end{comment}

\begin{remark}

Для более глубокого ознакомления с модификациями EM алгоритма -- медианные модификации, SEM, CEM, MCEM, SAEM, выбор начального приближения, определение числа компонент и типа смеси -- рекомендуем ознакомится с работой  В.Ю. Королева ЕМ-алгоритм, его модификации и их применение к задаче разделения смесей вероятностных распределений.  

\end{remark}


\begin{problem}[Вариационный вывод]
\label{varinf}

Рассмотрим  задачу оценки некоторой статистики $T(X)$ для распределения с плотностью $p(X)$, т.е. величины 
\[
\Exp_p T(X) = \int  T(X)p(X)dX.
\] 
Предполагается, что  $p(X)$  известно с точностью до нормировочной константы ($S_p =  \int \tilde{p}(X)dX$ является недоступным):
\[
p ( X ) = \frac{1}{S_p} \tilde{p}( X ) \propto \tilde{p}( X ). 
\]
Например, для получения оценки скрытых параметров $Z$ распределения $p(X,Z)$ можно подсчитать  $\Exp_{p(Z|X)} Z$. В этом случае в качестве недоступной для вычисления нормировочной константы выступает $p(X)$. В задачах, решаемых при помощи ЕМ-алгоритма (см. задачу \ref{em}), в качестве ненормированного распределения $\tilde{p}$ выступает совместное распределение $p(X, Z |\theta)$, недоступной нормировочной константой является неполное правдоподобие $p(X |\theta)$, а искомой статистикой $T(X,Z)$ -- величина $\log p(X, Z | \theta)$.

Одним из вариантов решения задач такого рода является нахождение приближения $q(x)$ в некотором простом семействе распределений и последующая оценка статистики как $\Exp_p T(X) \approx \Exp_q T(X)$. Для нахождения $q(X)$ решается следующая оптимизационная задача  
\[
\mathcal{KL}(q \Vert p) \to \min_q
\Leftrightarrow
\int q(X) \log \frac{\tilde{p}(X)}{q(X)}dX \to \max_q.
\]
Получите для семейства полностью факторизованных распределений $q(X) = \prod_i q_i(x_i)$, $X = (x_1,\ldots,x_n)$ итерационный метод вычисления оптимальных $q_i$: 
\[
q_i(x_i) \propto \exp \left(\int \log \big[ \tilde{p}(X) \big] \prod_{j \neq i} q_j(x_j) dx_j \right), 
\quad i = \overline{1,n}.
\]
Рассмотрите случай экспоненциального распределения 
\[
p(x_i |X_{-i})=h(x_i) e^{ \langle \theta, f(x_i) \rangle - d(\theta) },\quad
\theta = \theta(X_{-i}).
\]
Докажите, что для этого случая справедливо упрощенное  соотношение для  $q_i$:
\[
q_i(x_i) = h(x_i) e^{ \langle \Exp\theta , f(x_i) \rangle - d(\Exp\theta) } , 
\quad i = \overline{1,n}.
\] 

\end{problem}

\begin{remark}
Сравним между собой два метода приближенной оценки статистик $T(X)$: вариационный вывод и методы MCMC. В методе MCMC оценка $\Exp_p T(X)$ является тем точнее, чем больше выборок $X$ генерируется, а в пределе является точной. В вариационном выводе нет никаких гарантий на близость между $\Exp_p T(X)$ и $\Exp_q T(X)$. В итерациях вариационного вывода происходит максимизация функционала $L(q)$, являющегося нижней оценкой для  $\log S_p$, что, как правило,  обеспечивает достаточно точную оценку на значение нормировочной константы даже при существенно ограниченном семействе распределений~$q$. Время работы одной итерации вариационного вывода и одной итерации схемы MCMC, обычно, очень близки. Однако, для сходимости вариационного вывода часто достаточно несколько десятков итераций, в то время как для надежной оценки статистик MCMC требует несколько тысяч итераций.
\end{remark}





Для того чтобы описать следующий цикл задач на метод \textit{зеркального спуска} 
А.С. Немировского, нам потребуется ввести ряд определений и сформулировать 
некоторые необходимые в дальнейшем результаты (см. раздел Вспомогательные материалы). Отметим, что одну задачу, 
которая может быть отнесена к задачам этого цикла мы уже встречали (см. 
задачу \ref{bandit} раздела \ref{information}).  Далее при изложении мы будем опираться в основном на работы

Lugosi G., Cesa-Bianchi N. Prediction, learning and games. -- New York: Cambridge University Press, 2006.

Вьюгин В.В. Математические основы теории машинного обучения и прогнозирования. -- М.: МЦНМО, 2013.

%\underline {http://www.iitp.ru/upload/publications/6256/vyugin1.pdf}

Гасников А.В., Нестеров Ю.Е., Спокойный В.Г. Об эффективности одного метода рандомизации зеркального спуска в задачах онлайн оптимизации. -- М.: Автоматика и телемеханика. 2014.



\begin{problem}
Рассмотрим задачу взвешивание экспертных решений. Имеется $n$ различных 
Экспертов. Каждый Эксперт играет на рынке. Игра повторяется $N\gg 1$ раз 
(это число может быть заранее неизвестно). Пусть $l_i^k $ -- проигрыш 
Эксперта $i$ на шаге $k$ ($\left| {l_i^k } \right|\le M)$. На каждом шаге 
$k$ мы распределяем один доллар между Экспертами, согласно вектору $x^k\in 
S_n \left( 1 \right)$. Потери, которые мы при этом несем, рассчитываются по 
потерям экспертов $\left\langle {l^k,x^k} \right\rangle $. Целью является 
таким образом организовать процедуру распределения доллара на каждом шаге, 
чтобы наши суммарные потери были бы минимальны. Допускается, что потери 
экспертов $l^k$ могут зависеть еще и от текущего хода $x^k$. Легко 
проверить, что для данной постановки применима теорема 1 в детерминированном 
варианте с функциями
\[
f_k \left( {x;\xi ^k} \right)\equiv f_k \left( x \right)=\left\langle 
{l^k,x} \right\rangle .
\]
Покажите, что оценка, даваемая теоремой 1, имеет вид
\[
{\rm O}\left( {M\sqrt {\frac{\ln n}{N}} } \right).
\]

Докажите, что данную оценку нельзя улучшить. 
\end{problem}

\begin{ordre} См. S. Bubeck, N. Cesa-Bianchi. Regret Analysis of Stochastic and Nonstochastic Multi-armed Bandit Problems. In Foundati- ons and Trends in Machine Learning, Vol 5, 2012. 
\end{ordre}

\begin{problem}
В условиях предыдущей задачи предположим, что на $k$-м шаге $i$-й эксперт 
использует стратегию $\zeta _i^k \in \Delta $ (множество $\Delta $ -- 
выпуклое), дающую потери $\lambda \left( {\omega ^k,\zeta _i^k } \right)$, 
где $\omega ^k$ -- ``ход'', возможно, враждебной ``Природы'', знающей, в том 
числе, и нашу текущую стратегию. Функция $\lambda \left( {\,\cdot \,} 
\right)$ -- выпуклая по второму аргументу и $\left| {\lambda \left( {\,\cdot 
\,} \right)} \right|\le M$. На каждом шаге мы должны выбирать свою стратегию
\[
x\mathop =\limits^{def} \sum\limits_{i=1}^n {x_i \cdot \zeta _i^k } \in 
\Delta ,
\]
дающую потери $\lambda \left( {\omega ^k,x} \right)$ так, чтобы наши 
суммарные потери были минимальны. Для данной постановки также применима 
теорема 1 в детерминированном варианте с
\[
f_k \left( {x;\xi ^k} \right)\equiv f_k \left( x \right)=\sum\limits_{i=1}^n 
{x_i \lambda \left( {\omega ^k,\zeta _i^k } \right)} \ge \lambda \left( 
{\omega ^k,x} \right).
\]
Покажите, что оценка, даваемая теоремой 1, имеет вид
\[
{\rm O}\left( {M\sqrt {\frac{\ln n}{N}} } \right).
\]
Отметим, что эта оценка для данного класса задач.

\end{problem}

\begin{ordre}
Чтобы применить теорему заметим, что функция $\lambda 
\left( {\omega ^k,\zeta } \right)$ -- выпуклая по $\zeta $ для любого 
$\omega ^k$, поэтому
\[
\sum\limits_{k=1}^N {\lambda \left( {\omega ^k,x^k} \right)} -\mathop {\min 
}\limits_{i=1,...,n} \sum\limits_{k=1}^N {\lambda \left( {\omega ^k,\zeta 
_i^k } \right)} \le \sum\limits_{k=1}^N {f_k \left( {x^k} \right)} -\mathop 
{\min }\limits_{x\in S_n \left( 1 \right)} \sum\limits_{k=1}^N {f_k \left( x 
\right)} .
\]
\end{ordre}

\begin{problem}
Предположим, что в условиях предыдущей задачи мы не можем 
гарантировать выпуклость $\lambda \left( {\,\cdot \,} \right)$ -- по второму 
аргументу. Тогда мы выбираем стратегию -- распределение вероятностей на 
множестве стратегий Экспертов, и разыгрываем случайную величину согласно 
этому распределению вероятностей. Другими словами мы просто пользуемся МЗС2 
c $f_k \left( {x;\xi ^k} \right)\equiv f_k \left( x 
\right)=\sum\limits_{i=1}^n {x_i \lambda \left( {\omega ^k,\zeta _i^k } 
\right)} $, применимость которого обосновывается теоремой 2. Получите оценки

${\rm O}\left( {M\sqrt {\frac{\ln n}{N}} } \right) $ -- в среднем;

${\rm 
O}\left( {M\sqrt {\frac{\ln \left( {n \mathord{\left/ {\vphantom {n \sigma 
}} \right. \kern-\nulldelimiterspace} \sigma } \right)}{N}} } \right)$ -- с 
вероятностью $\ge 1-\sigma $.

%Отметим, что эти оценки для данного класса задач. 
\end{problem}

\begin{problem}[Антагонистические матричные игры]

Пусть есть два игрока А и Б. Задана матрица игры $A=\left\| {a_{ij} } \right\|$, где $\left| 
{a_{ij} } \right|\le M$, $a_{ij} $ -- выигрыш игрока А (проигрыш игрока Б) в 
случае когда игрок А выбрал стратегию $i$, а игрок Б стратегию $j$. 
Отождествим себя с игроком Б. И предположим, что игра повторяется $N\gg 1$ 
раз (это число может быть заранее неизвестно). Мы находимся в условиях 
предыдущей задачи с $\lambda \left( {\omega ^k,\zeta _j^k } 
\right)=\sum\limits_{i=1}^n {\omega _i^k a_{ij} } $, то есть
\[
f_k \left( x \right)=\left\langle {\omega ^k,Ax} \right\rangle ,
\quad
x\in S_n \left( 1 \right),
\]
где $\omega ^k$ -- вектор\footnote{ Вообще говоря, зависящий от всей истории 
игры до текущего момента включительно, в частности, как-то зависящий и от 
текущей стратегии (не хода) игрока Б, заданной распределением вероятностей 
(результат текущего разыгрывания (ход Б) игроку А не известен).} со всеми 
компонентами равными 0, кроме одной компоненты, соответствующей ходу А на 
шаге $k$, равной 1. Хотя функция $f_k \left( x \right)$ определена на 
единичном симплексе, по ``правилам игры'' вектор $x^k$ имеет ровно одну 
единичную компоненту, соответствующую ходу Б на шаге $k$, остальные 
компоненты равны нулю. Обозначим цену игры

$C=\mathop {\max }\limits_{\omega \in S_n \left( 1 \right)} \mathop {\min 
}\limits_{x\in S_n \left( 1 \right)} \left\langle {\omega ,Ax} \right\rangle 
=\mathop {\min }\limits_{x\in S_n \left( 1 \right)} \mathop {\max 
}\limits_{\omega \in S_n \left( 1 \right)} \left\langle {\omega ,Ax} 
\right\rangle .$ (теорема фон Неймана о минимаксе)

Пару векторов $\left( {\omega ,x} \right)$, доставляющих решение этой 
минимаксной задачи, назовем равновесием Нэша. По определению (это 
неравенство восходит к Ханнану)
\[
\mathop {\min }\limits_{x\in S_n \left( 1 \right)} 
\frac{1}{N}\sum\limits_{k=1}^N {f_k \left( x \right)} \le C.
\]
Тогда, если мы (игрок Б) будем придерживаться рандомизированной стратегии 
МЗС2, то по теореме 2 с вероятностью $\ge 1-\sigma $ (в случае когда $N$ 
заранее известно оценку можно уточнить)
\[
\frac{1}{N}\sum\limits_{k=1}^N {f_k \left( {x^k} \right)} -\mathop {\min 
}\limits_{x\in S_n \left( 1 \right)} \frac{1}{N}\sum\limits_{k=1}^N {f_k 
\left( x \right)} \le \frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {2\ln 
\left( {\sigma ^{-1}} \right)} } \right),
\]
т.е. с вероятностью $\ge 1-\sigma $ наши потери ограничены
\[
\frac{1}{N}\sum\limits_{k=1}^N {f_k \left( {x^k} \right)} \le 
C+\frac{2M}{\sqrt N }\left( {\sqrt {\ln n} +\sqrt {2\ln \left( {\sigma 
^{-1}} \right)} } \right).
\]
Самый плохой для нас случай (с точки зрения такой оценки) -- это когда игрок 
А тоже ``знает'' теорему 2, и действует согласно МЗС2 (точнее версии МЗС2 
для максимизации вогнутых функций на симплексе). Очевидно, что если и А и Б 
будут придерживаться МЗС2, то они сойдутся к равновесию Нэша, причем 
чрезвычайно быстро:

$\frac{8M\left( {\ln n+2\ln \left( {\sigma ^{-1}} \right)} 
\right)}{\varepsilon ^2}$ -- итераций;

${\rm O}\left( {n+M\frac{s\ln n\left( {\ln n+\ln \left( {\sigma ^{-1}} 
\right)} \right)}{\varepsilon ^2}} \right)\quad $ -- общая сложность вычислений,
где $s\le n$ -- среднее число элементов в строках и столбцах матрицы $A$. 
Докажите эти оценки.

\end{problem}


















\begin{comment}
%refactorise%
\begin{problem} [Метод зеркального спуска Немировского--Юдина] ** Рассмотрим задачу стохастической оптимизации
\[
\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi_k} \left[ {f_k \left( {x,\xi_k } \right)} 
\right]} \to \mathop {\min }\limits_{x\in S_n \left( 1 \right)} ,\quad S_n 
\left( 1 \right)=\left\{ {x\ge 0: \; \sum\limits_{i=1}^n {x_i =1} } 
\right\},
\]
где $\xi _k $ -- независимые случайные величины, $f_k \left( {x,\xi _k } 
\right)$:

\begin{enumerate}
\item выпуклые по $x$; 
\item $\left\| {\nabla _x f_k\left( {x,\xi_k } \right)} \right\|_\infty \le M$; 
\item  $\Exp\left[ {\nabla_x f_k \left( {x; \xi_k} \right)} \right]=\nabla _x \Exp\left[ {f_k \left( {x;\xi_k} \right)} \right].$ 
\end{enumerate}

С целью получить адаптивный алгоритм поиска оптимального $x^t$ при известных $\xi_1 \ldots \xi_t$ и уже вычисленных $x^1 \ldots x^{t-1}$ выполним линейную аппроксимацию функций $f_k \left( {x,\xi _k } 
\right)$:  

\[
\min \limits_{x\in S_n \left( 1 \right)} \sum\limits_{k=1}^t 
f_k(x) \approx \min \limits_{x \in S_n(1)} 
\sum\limits_{k=1}^t \left\{ f_k (x^{k-1})+ \left\langle 
\sum\limits_{k=1}^t \nabla f_k(x^{k-1}) , x-x^{t-1}  
\right\rangle  \right\}.
\]
Полагая при этом, что невязка $i$-й компоненты $\nabla f_k \left( x^{k-1} \right)$ равна случайной величине $\varepsilon_{k,i}$:
\[
\PR(x_t = e_j) \mathop{=}
\PR_\varepsilon \left( 
  j=\arg \max \limits_{i=1,...,n} \sum \limits_{k=1}^t 
  \left( 
    \left[ 
        -\nabla f_k \left( x^{k-1} \right) 
    \right]_i + \varepsilon_{k,i}  
  \right) 
\right),
\]
получим, при довольно общих условиях относительно с.в. $\varepsilon _{k,i} $ 
(типа i.i.d.), что если $t\gg 1$, то
\[
\begin{array}{c}
 P_\varepsilon \left( {j=\arg \mathop {\max }\limits_{i=1,...,n} 
\sum\limits_{k=1}^t {\left\{ {\left[ {-\nabla f_k \left( {x^{k-1} } 
\right)} \right]_i +\varepsilon _{k,i} } \right\}} } \right)\approx \\ 
 \approx P_\varsigma \left( {j=\arg \mathop {\max }\limits_{i=1,...,n} 
\left\{ {\sum\limits_{k=1}^t {\left[ {-\nabla f_k \left( {x^{k-1} } 
\right)} \right]_i } } \right\}+\varsigma _{t,i} } \right), \\ 
 \end{array}
\]
где с.в. $\varsigma _{t,i} $ -- i.i.d. с распределением Гумбеля 
(max-устойчивым), с параметром, зависящим от $t$: $P\left( {\varsigma _{t,i} 
<\tau } \right)=\exp \left\{ {-e^{-\tau \mathord{\left/ {\vphantom {\tau 
{\beta _t }}} \right. \kern-\nulldelimiterspace} {\beta _t }}} \right\}$, $\beta _t =\frac{M}{\sqrt {\ln n} }\sqrt {t+1}$
(см. задачу \ref{gumbel}).

Тогда
\[
E_\varsigma \left[ {x^t} \right]=-W_{\beta _t } \left( {\sum\limits_{k=1}^t 
{\nabla f_k \left( {x^{k-1} } \right)} } \right),
\]
где \[W_\beta \left( y \right)=\beta \ln \left( 
{\frac{1}{n}\sum\limits_{i=1}^n {\exp \left( {-\frac{y_i }{\beta }} \right)} 
} \right).\]

Используя результат задачи \ref{gibbs}, получите конечную формулу для независимого вычисления каждой из компонент $x^t$:

\[
x_i^t \propto \exp \left( {-\frac{1}{\beta_t 
}\sum\limits_{k=1}^{t-1} {\frac{\partial f_k \left( {x^{k-1},\xi _k } 
\right)}{\partial x_i }} } \right).
\]

\begin{remark}
Полученный алгоритм является стохастическим вариантом метода 
зеркального спуска (экспоненциального взвешивания в наших условиях).

Стоит подчеркнуть, что независимость вычислений каждой из компонент $x^t$ позволяет использовать распределенные вычисления $x^t$, предварительно разослав (broadcast) $x^{t-1}$ на каждый из рабочих узлов кластера.  
\end{remark}

Известно (см., например, работу Юдицкий А.Б., Назин А.В., Цыбаков А.Б., 
Ваятис Н. Рекуррентное агрегирование оценок методом зеркального спуска с 
усреднением // Пробл. передачи информ., 2005. Т. 41:4. стр. 78--96), что

\[
\sum\limits_{k=1}^t {\gamma _k \left\{ {E_{\xi ,x} \left[ {f_k \left( 
{x^{k-1};\xi_k} \right)} \right]-E_{\xi} \left[ {f_k \left( {x;\xi_k} 
\right)} \right]} \right\}} \le 
\]
\begin{equation}
\label{terrible}
\begin{array}{c}
 \le \sum\limits_{k=1}^t {\gamma _k \left( {x^{k-1}-x} \right)^T} \nabla _x 
E_{\xi ,x} \left[ {f_k \left( {x^{k-1};\xi_k} \right)} \right]\le \beta _t 
V\left( x \right)- \\ 
 -\sum\limits_{k=1}^t {\gamma _k \left( {x^{k-1}-x} \right)^T} \left( 
{\nabla _x f_k \left( {x^{k-1};\xi_k} \right)-\nabla _x E_{\xi ,x} \left[ 
{f_k \left( {x^{k-1};\xi_k} \right)} \right]} \right)+ \\ 
 +\sum\limits_{k=1}^t {\frac{\gamma _k^2 }{2\beta _{k-1} }\left\| {\nabla _x 
f_k \left( {x^{k-1};\xi_k} \right)} \right\|_\infty ^2,} \\ 
 \end{array}
\end{equation}
где  $V\left( x \right)=\ln n+\sum\limits_{i=1}^n {x_i \ln x_i }$.

Введем компактное обозначение для минимума целевой функции
\[
{\rm F_{min}} = \mathop {\min }\limits_{x\in S_n \left( 1 \right)} 
\frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi_k} \left[ {f_k \left( {x,\xi _k } 
\right)} \right]}
\]

Получите следующие оценки для среднего отклонения от минимального значения 
целевой функции:

$$
\Exp_{x} \left( \frac{1}{N}\sum\limits_{k=1}^N {\Exp_{\xi_k} \left[ {f_k \left( {x^{k-1},\xi 
_k } \right)} \right]} \right) -\rm{F_{min}} \le 2M\sqrt {\frac{\ln n}{N}},
$$

a если все $f_k \equiv f$ и $\xi_k$ -- независимы и одинаково распределены, то

\[
\Exp_{x}  {\Exp_{\xi} \left[ {f\left( 
{\frac{1}{N}\sum\limits_{k=1}^N {x^{k-1}} ,\xi } \right)} \right] - {\rm F_{min}} } \le 2M\sqrt {\frac{\ln n}{N}}.  
\]

Также получите вероятностные оценки отклонения от минимального значения 
целевой функции на величину  
$\delta(\Omega) = \frac{2M}{\sqrt N } \left({\sqrt {\ln n} +\sqrt {3\Omega }  }\right)$:

\[
\PR_{x} 
\bigg[
    \frac{1}{N}\sum\limits_{k=1}^N \Exp_{\xi _k} 
    \left[ {
      f_k \left( {x^{k-1},\xi_k } \right)
    } \right] 
    - {\rm F_{min}}  \ge  
   \delta(\Omega)
\bigg] 
\le \exp \left( {-\Omega}  \right),
\]
\[
\PR_{x}
\Bigg[
  \Exp_\xi \left[{
     f\left({
        \frac{1}{N}\sum\limits_{k=1}^N {x^{k-1}} ,\xi 
     } \right)
  } \right]
- {\rm F_{min}} \ge
\delta(\Omega)
\Bigg]
\le \exp \left( {-\Omega } \right).
\]
\end{problem}

\begin{ordre}  
Для получения оценок вероятностей больших уклонений, 
воспользуйтесь п. б)  задачи \ref{sec:mirrorDescent} из раздела \ref{measure}. 
\end{ordre}  

\begin{remark} 
Важно отметить, что описанный в этой задаче адаптивный 
метод помимо приложений в статистике имеет широкие приложения в задачах 
оптимального взвешивания экспертных решений (см., например, Вьюгин В.В. Элементы 
математической теории машинного обучения. М.: МФТИ, 2010, глава 3) и в 
задачах о многоруких бандитах (см., например, \textit{Lugoshi G., Cesa-Bianchi N}. Prediction, learning and 
games. New York: Cambridge University Press, 2006, а также Juditsky A., 
Nazin A.V., Tsybakov A.B., Vayatis N. Gap-free Bounds for Stochastic 
Multi-Armed Bandit // IFAC World congress, 2008). Удивительно, что во всех 
случаях, описанный метод дает (с мультипликативной точностью до константы) 
не улучшаемые оценки (только в случае многоруких бандитов c 
мультипликативной точностью $\sim \sqrt {\ln n} )$.

Для того чтобы применять этот метод к многоруким бандитам: $f_k \left( 
{x,\xi _k } \right)=r_i^k $ с вероятностью $x_i $, $i=1,...,n$; а чтобы 
$\nabla _x \Exp\left[ {f_k \left( {x,\xi _k } \right)} \right]=a=\Exp\left[ {r^k} 
\right]$, выбирают $\nabla _x f_k \left( {x,\xi _k } \right)=(\underbrace 
{0,..,r_i^k}_i{} \mathord{\left/ {\vphantom {{r_i^k } {x_i }}} \right. 
\kern-\nulldelimiterspace} {x_i },...,0)^T$ с вероятностью $x_i $, 
$i=1,...,n$, где $r_i^k \ge 0$ -- потери (regret), которые выдает 
$i\mbox{-я}$ ручка, если её дернуть на шаге $k$. При этом вместо слагаемых

$\frac{\gamma _k^2 }{2\beta _{k-1} }\left\| {f_k \left( {x^{k-1};\xi ^k} 
\right)} \right\|_\infty ^2 $ в выражении (\ref{terrible}) необходимо писать точнее \[\gamma _k^2 
\frac{x_j^{k-1} \left( {1-x_j^{k-1} } \right)}{\beta _{k-1} }\left( {\frac{r_j^k 
}{x_j^{k-1} }} \right)^2,\]
где $j$ -- номер ручки, выбранной алгоритмом на $k$-м шаге.

Для задач оптимального рандомизированного взвешивания экспертных решений 
$\Exp_\xi \left[ {f_k \left( {x,\xi_k } \right)} \right]=\sum\limits_{i=1}^n 
{\lambda \left( {\omega _k ,\zeta _k^i } \right)x_i } $, где $\lambda \left( 
{\omega _k ,\zeta _k^i } \right)$ -- потери Эксперта $i$, выбравшего на шаге 
$k$ стратегию $\zeta _k^i $, при ходе ``сопротивляющейся Природы'' $\omega 
_k $ (на каждом шаге первым выбирают свои ходы Эксперты, потом мы, потом 
природа; но есть важный нюанс: наш ход заключается в выборе распределения 
вероятностей, которое становится известным Природе, но разыгрывание согласно 
этому распределению вероятностей происходит после того, как Природа выбрала 
свой ход.

Тонкая разница в постановке этих двух задача (``стоящая'' $\sqrt n )$, 
заключается в том, что в многоруких бандитах игрок имеет только свою историю 
дергания ручек (ему не известно, какой бы \textit{regret} принесли ему другие ручки, кабы 
он их выбрал), а в постановке взвешивания экспертных решений это все 
известно и называется потерями экспертов.

В случае решения детерминированных разреженных задач выпуклой оптимизации в 
пространствах огромных размеров, как, например, задачи о ранжировании 
web-страниц

\begin{center}
http://goo.gl/HLM6w
\end{center}
важную роль играет искусственное введение случайности (рандомизация), позволяющее найти $x.\mathrm{top}(\cdot)$, проводя вычисления с разреженным вектором $x$:

\[
x_{i\left( t \right)}^t =x_{i\left( t \right)}^{t-1} +1,\;\;x_j^t =x_j^{t-1} 
,\;j\ne i\left( t \right), 
\]
где
\[
p_i^t \propto \exp \left( {-\frac{1}{\beta _t }\sum\limits_{k=1}^{t-1} 
{\gamma _k \frac{\partial f_k \left( {x^{k-1},\xi _k } \right)}{\partial x_i }} 
} \right),\quad i=1,...,n,
\]

Для этого алгоритма $\beta _t $ и $\gamma _t $ разумнее брать постоянными:
\[
\beta _t \equiv 1,
\quad
\gamma _t \equiv M^{-1}\sqrt {{2\ln n} \mathord{\left/ {\vphantom {{2\ln n} 
N}} \right. \kern-\nulldelimiterspace} N} .
\]
При этом сохраняются все приведенные в задаче оценки, но, к сожалению, 
теряется адаптивность, то есть теперь мы должны знать заранее либо требуемую точность, либо число шагов.
\end{remark}

\end{comment}


==> geometric_probability.tex <==
\section{Геометрические вероятности}
\label{geom}

\begin{problem}

Три бабочки капустницы садятся на круглый кочан капусты радиуса 1 случайным образом (имеется в виду, что место положение каждой бабочки -- с.в., равномерно распределенная на сфере) и независимо друг от друга. Если между двумя бабочками (геодезическое) расстояние оказывается меньше ${\pi \mathord{\left/ {\vphantom {\pi  2}} \right. \kern-\nulldelimiterspace} 2} $, то обе улетают. Найдите вероятность того, что на капусте сидят все три бабочки.

\end{problem}

\begin{problem}

Выбирается случайно и равномерно $n$ точек $P_{1} ,\ldots ,P_{n} $ на единичной окружности. Какова вероятность того, что начало координат (цент окружности) окажется внутри выпуклой оболочки этих точек.

\end{problem}

\begin{ordre} 
Выберите $n$ случайных пар диаметрально противоположных точек $Q_{1} ,Q_{n+1} =-Q_{1} $, $Q_{2} ,Q_{n+2} =-Q_{2} $, \dots , $Q_{n} ,Q_{2n} =-Q_{n} $ в соответствии с равномерным распределением. Ясно, что с вероятность 1 все пары различны. В качестве точки $P_{i} $ равновероятно выбирается либо точка $Q_{i} $, либо диаметрально противоположная ей $Q_{n+i} =-Q_{i} $. Покажите, что такая процедура эквивалентна случайному выбору точек $P_{i} $. Покажите, что вероятность того, что начало координат не окажется внутри выпуклой оболочки точек $P_{1} ,\ldots ,P_{n} $, при заданных различных точках $Q_{1} ,\ldots ,Q_{n} ,Q_{n+1} ,\ldots ,Q_{2n} $ равна $\frac{2n}{2^{n} } $, так как нужные точки $P_{1} ,\ldots ,P_{n} $ могут давать только подмножества вида $\left\{\tilde{Q}_{i} ,\ldots ,\tilde{Q}_{i+n-1} \right\}$(суммирование в индексах берется по модулю $2n$), где $\tilde{Q}_{1} ,\ldots ,\tilde{Q}_{2n} $ перенумерованные, например по часовой стрелке, точки $Q_{1} ,\ldots ,Q_{2n} $.
\end{ordre}

\begin{problem}
Найти среднюю длину секущих трехмерного куба с единичной длиной.
\end{problem}

\begin{problem}[Парадокс Бертрана]
Рассмотрим окружность, описанную около равностороннего треугольника ABC. Какова вероятность того, что случайным образом проведенная хорда будет иметь длину большую, чем длина стороны треугольника ABC? 
\end{problem}

\begin{ordre}
Предложите разные способы генерации хорды (не менее трех). Зависит ли ответ на задачу от способа генерации?
\end{ordre}

\begin{problem}
Пусть в пространстве $\mathbb R^n$ с евклидовой нормой задан $n$-мерный шар единичного радиуса. Внутри него имеются две случайные точки с радиус-векторами ${\bf{r}}_1$ и ${\bf{r}}_2$ соответственно, имеющие равномерное пространственное распределение внутри шара. Найти распределение случайной величины, являющейся расстоянием между этими двумя точками $r = \left|{\bf r}_1 - {\bf r}_2\right|$.
\end{problem}




\begin{problem}
На плоскости проведены параллельные прямые на единичном расстоянии друг от друга, и на плоскость наугад бросается иголка длиной $L<1$. 
Угол между прямыми и иголкой и расстояние от середины иглы до ближайшей прямой являются независимыми с.в., равномерно распределенными 
на $(0,2\pi)$ и $(-1/2,1/2)$ соответственно. С помощью серии таких опытов вычислить число $\pi$ с заданной точностью 
$\delta=1\%$ и с вероятностью ошибки не больше $\varepsilon=5\%$. Решите аналогичную задачу для случая погнутой иглы длиной менее 1.
\end{problem}

\begin{ordre}

Рассмотрим окружность диаметра $1$, т.е. длины $\pi$. Такая окружность с вероятностью $1$ пересекает дважды одну из прямых. 
Тогда, исходя из линейности математического ожидания числа попаданий иглы на прямую относительно длины иглы, для иглы длиной $L<1$ 
имеем ${\mathbb E}\xi_L = 2L/\pi$. 

\end{ordre}



\begin{problem}
Покажите, что средняя площадь ортогональной проекции куба с ребром единица на случайную плоскость равна $3/2$. 
\end{problem}

\begin{ordre}
Покажите, что  средняя площадь  ортогональной проекции всякого измеримого тела 
линейно зависит от площади его границы. 
Рассмотрим вспомогательное (см. предыдущую задачу) тело, у которого легко вычисляется средняя площадь ортогональной проекции. 
\end{ordre}

\begin{remark}
Обозначим через $S_k$ $k$-мерный объем ортогональной 
проекции рассматриваемой области $V$ в ${\mathbb R}^n$ на случайную $k$-мерную 
плоскость. Имеет место следующая формула для объема $h$-окрестности данной области:
\[
V\left( h \right)=V_0 +V_1 h+V_2 h^2+...+V_n h^n,
\]
где $V_0 $ -- объем области; $V_1 $ -- $(n-1)$-мерный объем границы области, 
пропорциональный среднему значению от числа 1; число $V_k $ пропорционально 
$S_k $ и выражается через средние значения (усредненным по поверхности рассматриваемой области)  от произведений $k$ главных 
кривизн. 

В случае $n = 3$, из главных кривизн $k_1 $ и $k_2 $ в каждой точке 
можно составить \textit{среднюю кривизну} $k_1 +k_2 $ и \textit{гауссову кривизну} $K=k_1 k_2 $. В этом случае объем 
$h$-окрестности получается $V\left( h \right)=V_0 +V_1 h+V_2 h^2+V_3 h^3$, где 
$V_2 $ пропорционален интегралу от средней кривизны по всей поверхности, а $V_3 $ -- от гауссовской:
\[
V_3 =\frac{4}{3}\pi \int\!\!\!\int {KdS} .
\]
Например, для сферы радиуса $R$
\[
V\left( h \right)=\frac{4}{3}\pi \cdot \left( {R+h} \right)^3=\frac{4}{3}\pi 
R^3+h\cdot \left( {4\pi R^2} \right)+h^2\left( {4\pi R} 
\right)+\frac{4}{3}\pi h^3.
\]
Здесь $k_1 + k_2 = \frac{2}{R}$, $k_1 k_2 = \frac{1}{R^2}$,
\[
\int  (k_1 +k_2)   dS = 8\pi R,
\]
Формула Гаусса-Бонне:
 \[\int\!\!\!\int {\left( {k_1 k_2 } \right)dS} =4\pi. \] 


\end{remark}


\begin{problem}
Приведем геометрическую интерпретацию пуассоновского процесса (см. задачу \ref{sec:poisson}). Пуассоновским процессом $\text{П}$ в пространстве $S \subset \mathbb{R}^m$ называется  счетное множество точек, случайно разбросанных по $S$, но подчиняющихся следующему правилу: существует мера $\mu: S \to [0, \infty]$, соответствующая процессу $\text{П}$, такая что для любых непересекающихся 
измеримых множеств $A_1,\ldots,A_n \subset S$ случайные величины 
\[
N(A_i) = \# \{ A_i \cap \text{П}\} \sim  \Po(\mu(A_i)), \quad i = \overline{1,n},
\] 
порожденные случайным попаданием точек в множества $A_1,\ldots,A_n$, независимы и имеют распределение $\Po(\mu)$. 

К примеру стандартный пуассоновский процесс из задачи \ref{sec:poisson} раздела \ref{zb4} определен в пространстве $S = \mathbb{R}_{+}$, имеет меру $\mu \big( (t_1, t_2] \big) = \lambda ( t_2 - t_1)$, $N( (t_1, t_2] ) = K(t_2) - K(t_1) \sim \Po \big(\lambda (t_2 - t_1) \big)$.

Отметим, что определение $\text{П}$ требует, чтобы мера $\mu$ была \textit{неатомической} (значение на любом счетном множестве равно 0), а также представимой в следующем виде
\[
\mu = \sum_{k = 1}^{\infty} \mu_{k}, \quad \mu_k(S) < \infty.
\]
Пусть $X_1,\ldots,X_n$ -- независимые случайные величины, распределенные по $A \subset S$, $\mu(A) < \infty$ в соответствии с вероятностной мерой $p(\cdot) = \mu(\cdot) / \mu(A)$, Обозначим за $N(B)$ количество $X_i \in B$. Покажите, что для непересекающихся $A_1,\ldots,A_k  \subset A$, $A = A_1 \cup\ldots\cup A_k $ выполнено  
\[
\PR_n(N(A_1) = n_1,\ldots,N(A_k) = n_k) = \frac{n!}{n_1!,\ldots,n_k!} p(A_1)^{n_1} \ldots p(A_k)^{n_k}.
\]
Докажите, что если $X_1,\ldots,X_n$ -- точки пуассоновского процесса с мерой $\mu$ внутри множества $A$, то справедливо равенство
\[
\PR(\cdot | N(A) = n) = \PR_n(\cdot).
\]
\begin{remark}
Последнее выражение утверждает, что при фиксированном числе точек $N(A)$ внутри множества $A$, сами точки пуассоновского процесса выглядят как $N(A)$ независимых случайных величин с плотностью распределения $p(\cdot) = \mu(\cdot) / \mu(A)$. 
Таким образом, пуассоновский процесс является неизбежным следствием моделирования системы с большим числом независимых точек в пространстве~$\mathbb{R}^m$.
\end{remark} 


\begin{problem}
\label{poi_proj}
Однородный пуассоновский процесс $\text{П}$ определен в пространстве $S = \mathbb{R}^{2}$ и имеет интенсивность $\lambda$, т.е. $\mu (A)  = \int_{A} \lambda dxdy$. Осуществим переход к полярным координатам $(r, \theta)$ при помощи преобразования 
\[
f(x, y) = \left( 
(x^2 + y^2)^{1/2}, \; \arctan (y/x)
\right).
\]
Покажите, что образы точек $\text{П}$  образуют пуассоновский процесс в полосе
\[
\{(r,\theta): \; r > 0, \; 0 \leq \theta <  2 \pi \},
\]
который имеет интенсивность $\lambda^{*}(r) = \lambda r$.
Покажите, что значения $r$, соответствующие $\text{П}$, образуют пуассоновский процесс в $(0, \infty)$ с интенсивностью $2 \pi \lambda r$. 

\end{problem}

\begin{remark}
Сформулируем правило отображения $\text{П}$ при помощи произвольного правила преобразования координат $f: S \to T$: если мера $\mu$ процесса $\text{П}$ является $\sigma$-конечной ($S$ можно представить в виде $\cup_n S_n$, где $\mu(S_n) < \infty$), помимо того мера на множестве образов $T$ 
\[
\mu^{*}(B) = \mu( f^{-1} (B))
\]  
является неатомической, то $f(\text{П})$ -- пуассоновский процесс в пространстве $T$ c  мерой интенсивности $\mu^{*}$.
\end{remark}

\begin{problem}
Используя результат предыдущей задачи, покажите, что плотность распределения упорядоченных расстояний $r_{(1)}, r_{(2)}, \ldots$ имеет следующий вид
\[
f_{r_{(s)}} (r) = \frac{2 (\lambda \pi)^s r_{}^{2s - 1} e^{-\lambda \pi r_{}^2}}{ (s-1)! }. 
\]  
В таком случае, $2 \lambda \pi r_{(s)}^2$ распределено как $\chi_{2s}^{2}$. Данный результат может быть использован для оценки плотности точек на плоскости путем выбора случайных точек и измерения расстояния до 1-го ближайшего соседа. Пусть $X_1, \ldots, X_n$ -- $n$ реализаций $r_{(1)}^{2}$. Покажите, что $2\lambda \pi n \overline{X}$ распределено как $\chi_{2n}^{2}$, предложите оценку для $\lambda$ и вычислите ее дисперсию.
\end{problem}

\begin{remark}
Аналогичный подход с измерением переменной плотности точек $\lambda(\cdot)$ продемонстрирован в задаче $\ref{sort_dir}$ раздела $\ref{bayes}$  c использованием упорядоченного распределения Дирихле.
\end{remark}

\begin{problem}
Сопоставим каждой точке $X \in S$ случайного множества  $\text{П}$ (пуассоновский процесс) случайную величину $m_X$ (метку), принимающую значения из множества $M$.
Распределение $m_X \sim p(X, m)$ может зависеть от  $X$, но не зависит от других точек $\text{П}$ и их меток. Докажите, что случайное множество
\[
\text{П}^{*} = \{(X, m_X): \; X \in \text{П}\}
\]
является пуассоновским процессом на множестве $S \times M$ c мерой интенсивности
\[
\mu^{*}(C) = \mathop{\int\int} \limits_{(x,m) \in C} \mu(dx) p(x, m) dm.
\]
Используя замечание к задаче \ref{poi_proj}, убедитесь что метки  $m_X$ образуют пуассоновский процесс на $M$ с мерой интенсивности 
\[
\mu_m(B) = \int_{S}\int_{B}  \mu(dx) p(x, m) dm. 
\]
\end{problem}

\begin{ordre}
Докажем, что $\text{П}$ однозначно задается набором характеристических функционалов вида
\[
\Exp(e^{\Sigma_f}) = \exp \left( - \int_{S}(1 - e^{-f(x)}) \mu(dx)  \right),
\]
где 
\[
\Sigma_f = \sum_{X \in \text{П}} f(X), \quad f \in \mathcal{F},
\]
$\mathcal{F}$ -- класс функций, содержащий все индикаторные функции для измеримых множеств из $S$. Выбрав набор непересекающихся множеств $A_1,\ldots,A_k$, сопоставим 
каждому множеству свое значение $f_i$. Тогда
\[
\Sigma_f  = \sum_{i=1}^k f_i N(A_i), \quad
\Exp(e^{\Sigma_f}) = \exp \left( - \sum_{i=1}^k (1 - e^{-f_i}) \mu(A_i)  \right).
\]    
Сделав замену $z_i  = e^{-f_i}$, получаем
\[
\Exp \left(z_1^{N(A_i)} \ldots z_k^{N(A_k)} \right) = \prod_{i=1}^k e^{\mu (A_i) (z-1)},
\]  
что свидетельствует о независимости $N(A_i)$ и принадлежности распределению Пуассона.
\end{ordre}

\end{problem}

\begin{problem}
\label{subord}
Случайный процесс $\varphi(t)$ называется \textit{субординатором} (процесс Леви с положительными приращениями), если он удовлетворяет следующим свойствам: приращения  процесса независимы, положительны и зависят только от приращения аргумента $t$. Докажите, что  справедливо следующее представление субординатора 
\[
\varphi(t) = \beta t + \sum_{\tau} \{z: \; (\tau, z) \in  \text{П}, \; 0 < \tau < t  \},
\]
где суммируются значения второй координаты пуассоновского процесса $\text{П}$ с мерой интенсивности
\[
\mu(d\tau, dz) = d\tau \gamma(dz). 
\]
Мера $\gamma(dz)$ соответствует скачкам процесса  $\varphi(t)$, образующем пуассоновский процесс по координате $z$, и может быть найдена из выражения (представление Леви-Хинчина)
\[
\Exp  e^{ -s \varphi(t)} = \exp \left(
-t \left[ s\beta - \int_{0}^{\infty} (1 - e^{-s z}) \gamma(dz)  \right]
 \right). 
\] 
\end{problem}

\begin{ordre}
Используя результат предыдущей задачи, покажите, что для чисто атомической меры на $S$, определенной как  
\[
\Psi(A)  = \sum_{\tau} \{z: \; (\tau, z) \in  \text{П}, \;  \tau \in A\} 
\]  
характеристическая функция имеет вид
\[
\Exp  e^{ -s \Psi(A) } = \exp \left(
- \int_{0}^{\infty} (1 - e^{-s z}) \gamma(A, dz) 
 \right),
\]
где $\gamma(\cdot, \cdot)$ --  мера процесса $\text{П}$.

Покажите, что для случайной неатомической меры $\Phi$ с независимыми значениями на непересекающихся множествах $\Phi(A)$ есть безгранично делимая с.в. и для нее  справедливо представление  Леви-Хинчина: 
\[
\Exp  e^{ -s \Phi(A)} = \exp \left(
 - s\beta(A) + \int_{0}^{\infty} (1 - e^{-s z}) \gamma(A, dz) 
 \right). 
\]  
Далее, $\varphi(t)$ может быть представлен как случайная мера $\Phi(0,t]$ при значениях $t \geq 0$. Убедитесь, что такая мера является неатомической, используя свойство инвариантности $\Phi$ относительно сдвига. 
\end{ordre}

\begin{problem}
Рассмотрим звезды, находящиеся на расстоянии, не превышающем $R$ от наблюдателя. Для простоты будем считать, что все звезды имеют одинаковый диаметр $\delta$ и равномерное пространственное распределение с количеством звезд $\lambda$ на единицу объема. Показать, что при $R \rightarrow \infty$ любой участок неба будет полностью светящимся.   

\begin{remark}
В действительности такое явление не наблюдается. В связи с конечным возрастом вселенной ($14 \cdot 10^9$ лет) ее радиус ограничен величиной $ct$.
\end{remark}
\end{problem}

\begin{problem}[Формула Крофтона]
Пусть  $N$ точек независимо распределены в области $D$ $n$-мерного пространства, $P$ -- вероятность того, что фигура $F$, образованная $N$ точками, обладает определенным свойством,
зависящим только от взаимного расположения точек. Область $D$ является измеримой по Лебегу и ее мара равна $V$. Обозначим как $P_1$ вероятность того, что $F$ обладает требуемым свойством для случайных точек в области $D_1 \supset D$. Докажите следующее соотношение для малых приращений $\delta V$:
 \[
 \delta P = N (P_1 - P) V^{-1} \delta V .
 \]  

\end{problem}

\begin{problem}
Вычислите распределение  расстояния между точками, случайно взятыми внутри круга радиуса $R$, воспользовавшись формулой Крофтона.
\end{problem}
\begin{ordre}
Пусть $f(x,R)dx$ есть вероятность того, что расстояние между точками $A$ и $B$ принадлежит интервалу  $(x, x + dx)$. Для случая, когда $A$ лежит на границе
\[
f(x,R) = \frac{ 2 \theta x}{\pi R^2}, \quad \theta = \arccos (x/2R).
\]
Тогда уравнение Крофтона примет вид
\[
\frac{df}{d\theta} + 4 f \tg \theta = \frac{32 \theta}{\pi x} \sin \theta \cos \theta.
\]
\end{ordre}



\begin{problem}[Теорема Дворецкого]
\label{sec:dvor}
Доказать, что для любого $\epsilon > 0$ и $k \in \mathbb{N}$
существует $N = N(k, \epsilon) < \exp(C\frac{\log \epsilon}{\epsilon^2}k)$ такое, что любое конечномерное банахово пространство ($X, \Vert\cdot\Vert)$, где $\dim X > N$, содержит $k$-мерное подпространство $E$, являющееся $\epsilon$-евклидовым, т.е. в нем можно задать такую норму $\vert \cdot \vert$, что $\Vert x \Vert \leqslant \vert x \vert \leqslant (1 + \epsilon) \Vert x \Vert$ $\forall x \in E$.     

\begin{remark} См. работу В. Д. Мильман, “Новое доказательство теоремы А. Дворецкого о сечениях выпуклых тел”, Функц. анализ и его прил., 5:4 (1971), 28–37. 

\end{remark}

\begin{comment}
НАЗАР, СЮДА СТОИТ ВСТАВИТЬ ЗАМЕЧАНИЕ ИЗ СТАТЬИ GOWERS'а
И ДОБАВИТЬ В ВИДЕ ЗАДАЧИ ТЕОРЕМУ Б.С, Кашина - см. статью того же Gowers'a и ссылки в том моем письме
\end{comment}


\end{problem}

\begin{problem}
Выберем наугад (равновероятно) $k$ вершин $m$-мерного куба $[0,1]^m$. Обозначим как $X$ выпуклую оболочку выбранных вершин. Пусть $p_{km}$ - вероятность того, что все вершины многогранника попарно смежны. Докажите справедливость следующей оценки при $m > 3$:

\[
p_{km} > 1 - \frac{k^4 \cdot 5^m}{4 \cdot 8^m}
\]
    
\end{problem}
\begin{remark}
См. монографию Бондаренко В.А., Максименко А.Н. Геометрические конструкции, сложность в комбинаторной оптимизации. -- М.: УРСС, 2008.
\end{remark}


\begin{problem}
На плоскости нарисована выпуклая фигура, ограниченная кривой длины $L$. Докажите, что ее диаметр, т.е. максимальное расстояние между двумя ее точками, не меньше $\frac{L}{\pi }$.
\end{problem}
\begin{ordre}
Проведите в случайном направлении прямую. Покажите, что 
математическое ожидание длины проекции фигуры на случайное направление равно 
$\frac{L}{\pi }$.
\end{ordre}

\begin{problem}
В московском метро можно провозить коробки, у которых сумма измерений (длины, ширины и высоты) не превосходит некоторой границы. Можно ли перехитрить правила, поместив одну коробку в другую (сумма измерений внутренней коробки больше суммы измерений внешней)?
\end{problem}
\begin{ordre}
Спроектируйте коробку на случайно выбранное (в пространстве) 
направление. Длина проекции коробки складывается из проекций отрезков, 
идущих по ее высоте, длине и ширине. Проекция внутренней коробки не 
превосходит проекции внешней.
\end{ordre}

\begin{problem}
Несамопересекающаяся кривая длины 22 находится внутри круга радиуса 1. Докажите, что найдется прямая, имеющая с этой кривой по крайней мере 8 общих точек.
\end{problem}
\begin{problem}
Известно, что более половины поверхности Земли занимают океаны. Докажите, что можно найти две диаметрально противоположные точки, обе попавшие в океан.
\end{problem}


\begin{problem}
На плоскости расположено $2n$ векторов, выходящих из начала координат и длиной не более 1. Доказать, что существует угол $\alpha$ такой, что при повороте каждого из векторов на угол $\pm \alpha$, их векторная сумма окажется не большей 1.  
\end{problem}

\begin{problem}[случайный поворот куба, мера Хаара] 10{\%} поверхности 
шара (по площади) выкрашено в черный цвет, остальные 90{\%} -- белые. 
Докажите, что можно вписать в шар куб таким образом, чтобы все вершины куба 
попали в белые точки.
\end{problem}

\begin{problem}[Теорема Уилкса]
Для выборки $X \sim f(\theta, X)$, $\dim X = n$ осуществляется проверка гипотезы $H_0: \theta = \theta_0$, для чего используется обобщенный критерий отношения правдоподобия. 
Определим статистику для критерия как 
\[
W(\theta_0) = \log f(\widehat{\theta}, X) - \log f(\theta_0, X),
\quad  \widehat{\theta} = \arg\max_{\theta \in \Theta} f(\theta, X).
\] 
Теорема Уилкса утверждает, что в случае истинности гипотезы  $H_0$ и при асимптотической нормальности оценки $\widehat{\theta}$, статистика  
$2W(\theta_0)$ сходится по распределению к $\chi_{p}^2$, где $p = |\Theta|$. 
Тогда критерием отклонения гипотезы $H_0$ будет $[2W(\theta_0) > x]$, $\PR(\chi_{p}^2 > x) < \alpha$. 

Существует также обобщение теоремы Уилкса для случая, когда $\widehat{\theta}$ не является асимптотически нормальной. При довольно слабых дополнительных ограничениях для выполнения теоремы Уилкса достаточно, чтобы поверхности уровня  $S_w = \{\theta: W(\theta) = w\}$ в пределе при $n \to \infty$ имели форму
\[
S_w  \approx \widehat{\theta} + a_n w^r S
\]  
где $a_n \to 0 $ при $n \to \infty$, $S = \{\theta: h(\theta) = 1 \}$, $h(t\theta) = t^{1/r} h(\theta)$. В частности, при асимптотической нормальности оценки $\widehat{\theta}$ поверхности уровня являются эллиптическими:
\[
S_w  \approx \widehat{\theta} +  \sqrt{\frac{2w}{n}} \theta^T D \theta.
\]
Докажите при дополнительных ограничениях, $W(\widehat{\theta})$ строго локально вогнута и $\inf\{h(\theta): \Vert \theta \Vert = 1\} > 0$, что 
\[
W(\theta_0) \overset{d}{\longrightarrow} \text{Г}(rp, 1),
\]
где плотность гамма $\text{Г}(\alpha, \lambda)$ распределения задается как $\frac{x^{\alpha-1} e^{-x/\lambda}}{\lambda^\alpha\text{Г}(\alpha)}$.

\end{problem}

\begin{ordre}
См. работу Fan et al. Geometric Understanding of Likelihood Ratio Statistics. Department of Statistics, UCLA 1998.
\end{ordre}


==> information.tex <==
\section{Теория информации и кодирование}
\label{information}

\begin{comment}
\subsection{Основные определения}
Пусть $X$ - дискретная случайная величина, принимающая значения из конечного множества (алфавита) $A = \{a_1,..., a_{|A|}\}$. $P = \{\mathbb{P}\{X = a_i\} = p_{a_i}\}$ - вероятностное распределение $X$ на $A$.

\textit{Условной энтропией} двух с.в. $X \in P$ и $Y \in Q$ называется $H(P|Q) = \sum_{a \in A} \mathbb{P}(Y = a)H(P|Y=a)$, где $H(P|Y=a) = \sum_{a' \in A} \frac{\mathbb{P}(X = a', Y = a)}{\mathbb{P}(Y = a)} \log \frac{\mathbb{P}(X = a', Y = a)}{\mathbb{P}(Y = a)}$. Условная энтропия характеризует ту среднюю степень неопределнности, содержащейся в $X$, если имеется некоторая информация об $Y$.

\begin{definition} \textit{Словом} в алфавите $A$ будем называть реализацию последовательности случайных величин $X_1,...,X_n..$: $w = (x_1...x_n..)$, $x_i \in A$.
\end{definition}

\begin{definition} 
\textit{Энтропией} $H(X)$ случайной величины $X$ распределенной по закону $P$ называется:
\begin{center}
$H(X) = - \sum_{a \in A} p_a\log p_a$, где $\log = \log_2$.
\end{center}
Иногда вместо $H(X)$  используется запись $H(P)$.
Энтропия измеряется в битах и интерпретируется как мера неопределенности или информационного содержания случайной величины. Чем она больше, тем больше неопределенность. В качестве иллюстрации, читателю предлагается решить первую задачу.
\end{definition}
В случае нескольких случайных величин можно определить два тесно связанных понятия: \textit{условной энтропии} и \textit{совместной информации}.
\begin{definition}
\textit{Условной энтропией} двух с.в. $X$ и $Y$ называется $H(X|Y) = \sum_{a \in A} \mathbb{P}(Y = a)H(X|Y=a)$, где $H(X|Y=a) = \sum_{a' \in A} \frac{\mathbb{P}(X = a', Y = a)}{\mathbb{P}(Y = a)} \log \frac{\mathbb{P}(X = a', Y = a)}{\mathbb{P}(Y = a)}$. Условная энтропия характеризует ту среднюю степень неопределнности, содержащейся в $X$, если имеется некоторая информация об $Y$.
\end{definition}

\begin{definition}
\textit{Совместная информация} $I(X,Y) = H(X) - H(X|Y)$ определяет то, сколько информации об $X$ содержится в $Y$.
\end{definition}

\begin{definition}
\textit{Относительной энтропией} случайных величин $X \backsim P$ и $Y \backsim Q$ на множестве $A$ (или расстоянием Кульбака-Лейблера между ними) называется
\begin{center}
$KL(P||Q) = \sum_{a \in A} p_a \log \frac{p_a}{q_a}$. 
\end{center}
В статистике эта величина определяет то, насколько "неэффективно" использование распределения $Q$ для аппроксимации распределедния $P$, или как много дополнительных бит мы заплатим за такую аппроксимацию.
\end{definition}

\begin{definition}
\textit{Кодом} слова $w \in A^{len(w)}$ в алфавите $\Sigma$ называется отображение $C(w) : w \rightarrow \sigma$, $\sigma \in B^{len(\sigma)}$. $len(\sigma)$ - длина кодового слова.
\end{definition}

\subsection{Задачи}


ЧТО ТАКОЕ РЫЧАЖНЫЕ ВЕСЫ? ПОЧЕМУ В УСЛОВИИ ЗАДАЧИ СТОИТ СЛОВО ВОЗМОЖНО? В ЧЕМ ЗАКЛЮЧАЕТСЯ ВЗВЕШИВАНИЕ?

25 ПОТОМУ ЧТО ФАЛЬШИВОЙ МОНЕТЫ МОЖЕТ НЕ БЫТЬ?

"потому чтокаждый из 25-и исходов может быть закодирован двоичным словомуказанной длины." - и что?

см. две статьи в КВАНТе и то как об этом написано у Щепина в совместной книге с Верещагиным
\end{comment}

\begin{problem}
Имеется 12 монет, из них ровно одна фальшивая, которая может быть как легче, так и тяжелее настоящих.   Предложите алгоритм взвешиваний на чашечных весах без гирь, выявляющий за 3 взвешивания подделку, а также определяющий является ли фальшивая монетка тяжелее или легче настоящих.
\begin{ordre}
Любая из 12 монет может быть фальшивой, при этом быть легче, либо тяжелее настоящих. Для решения требуется с помощью взвешиваний  получить $\log_24$ бит информации (по Хартли), так как каждый  исходов может быть закодирован двоичным словом длины 24. С другой стороны, каждое взвешивание имеет три возможных исхода: выше левая чаша весов, выше правая или они в равновесии. То есть каждое взвешивание дает не более $\log3$ бит информации. Соответственно, требуемое число взвешеваний не может быть мееньше $\frac{\log24}{\log3} = 3$. 

Для решения этой задачи и последующих полезно ознакомиться с книгой Н.К. Верещагин, Е.В. Щепин Информация, кодирование и предсказание. -- М.:  МЦНМО, 2012, а также см. метод Дайсона в статье Г. Шестопала ``Как обнаружить фальшивую монетку'' в журнале Квант 1979, номер 10.
\end{ordre}
\end{problem}

\begin{problem}
Патриций решил устроить праздник и для этого приготовил 240 бочек вина. Однако к нему пробрался недоброжелатель, который подсыпал яд в одну из бочек. Про яд известно, что человек, его выпивший, умирает в течение (не «через»!) 24 часов. До праздника осталось два дня, то есть 48 часов. У патриция есть пять собак, которыми он готов пожертвовать, чтобы узнать в какой именно бочке яд.
Как патрицию вычислить отравленную бочку?
\end{problem}

\begin{problem}[Цена информации] Имеется неизвестное число от $1$ до $n$, $n \geq 2$. Разрешается задавать любые вопросы с ответами ДА/НЕТ. При этом при ответе ДА игрок платит 1 рубль, а при ответе НЕТ - 2 рубля. Сколько необходимо и достаточно заплатить для отгадывания числа?
\end{problem}


\begin{problem}[Аксиоматическое определение энтропии]
Рассмотрим множество функций, заданных на единичном симплексе. Докажите, что существует единственная (с точностью до множителя) функция, удовлетворяющая нижеперечисленным требованиям. Она имеет вид $H(P) = -\sum_{i=1}^n p_i \log p_i$ и используется в качестве количественной характеристики меры неопределенности.
\begin{enumerate}
\item Значение функции $H(P)$ не меняется при перестановке чисел ${p_{a_1},..., p_{a_n}}$,
\item $H(P)$ непрерывная функция,
\item выполняется равенство
\begin{center}
$H(p_1,...,p_n) = H(p_1 + p_2, p_3,..., p_n) + (p_1 + p_2) H(\frac{p_1}{p_1+p_2},\frac{p_2}{p_1+p_2} )$.
\end{center}
То есть неопределенность в исходе опыта не зависит от того, осуществляется ли выбор среди всех возможных альтернатив одномоментно или в несколько этапов.
\end{enumerate}
\end{problem}

\begin{problem}
\begin{enumerate}
\item Ф.М. Достоевский решил изменить своим привычкам и отправился на скачки. У него есть предварительные (априорные) данные о том, какие шансы на победу имеет каждая из восьми лошадей-участниц: $(\frac{1}{2}, \frac{1}{4}, \frac{1}{8}, \frac{1}{16}, \frac{1}{64}, \frac{1}{64}, \frac{1}{64}, \frac{1}{64})$. Оцените энтропию, которая содержится в таких данных. 
\item Сравните результат со случаем, когда все исходы равновероятны. Какое из двух респределений содержит больше информации?
\item Докажите в общем случае, что из всех дискретных распределений на конечном множестве $A$, наибольшей энтропией обладает равномерное.
\end{enumerate}
\end{problem}

\begin{comment}
\begin{problem}
ТО КАК СЕЙЧАС ПЛОХО, см. 

http://dcam.mipt.ru/students/study/stohanaliz-files/ Задание по теории вероятнсотей 2010

Эта таблица ничуть не помогает в восприятии:(

В таблице приведен прогноз погоды в г. Долгопрудный:
$p$ - вероятность наличия/отсутствия осадков, $q$ - вероятность того, что прогноз окажется верным.
\begin{table}[h]
\caption{Прогноз погоды}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
 &$p_{rain}$  &$p_{fine}$ & $q_{rain}$ & $q_{fine}$  \\
\hline
$15$ июня & $0.4$ & $0.6$ & $3/5$ & $4/5$\\
\hline
$15$ октября & $0.8$ & $0.2$ & $9/10$ & $1/2$\\
\hline
\end{tabular}
\end{center}
\end{table}
В какой из указанных двух дней прогноз дает нам больше информации о реальной погоде?
\end{problem}
\end{comment}
\begin{problem}
Пусть для некоторого населенного пункта вероятность того, что 15 июня будет дождь, равна 0.4, а вероятность того, что дождя не будет, равна 0.6. Для этого же пункта вероятность дождя 15 октября равна 0.8, а вероятность отсутствия осадков равна 0.2. Предположим, что определенный метод прогноза погоды 15 июня оказывается верным в $3/5$ всех тех случаев, когда предсказывается дождь и в $4/5$ тех случаев, в которых прогнозируется отсутствие осадков. Применительно к погоде на 15 октября этот метод оказывается правильным в 9 из 10 случаев, когда предсказывается дождь, и в половине случаев, когда предсказывается его отсутствие. В какой из указанных двух дней прогноз дает нам больше информации о реальной погоде?
\end{problem}


\begin{problem}[Задача о шляпах. Тодд Эберт, 1998]

Трех игроков отводят в комнату, где на них надевают (случайно и независимо) белые и черные шляпы. Каждый видит 
цвет других шляп и должен написать на бумажке одно из трех слов: <<белый>>, <<черный>>, <<пас>> 
(не советуясь с другими и не показывая им свою бумажку). Команда выигрывает, если хотя бы один из игроков назвал правильный 
цвет своей шляпы и ни один не назвал неправильного. Как им сговориться, чтобы увеличить шансы? Оптимальна ли предложенная Вами стратегия?
Решите эту же задачу, если игроков $n=2^m -1$ $( m\in {\mathbb N} )$. 
\end{problem}

\begin{ordre}
Воспользуйтесь кодом Хэмминга.
Докажем для случая трех игроков, что вероятность выигрыша не может превышать $3/4$. 

Единственная информация, которой владеет $i$-й игрок --- это цвета шляп двух других. Поэтому стратегия для $i$-го игрока должна зависеть 
только от этих двух цветов. В каждом случае имется три варианта ответа для игрока: $0$, $1$ или <<пас>>, т.е. всего $3^{12}$ различных 
стратегий. Поскольку есть $8$ вариантов расположения шляп на игроках, более выгодная стратегия должна обеспечивать выигрыш в $7$ вариантах. 
Тогда один из игроков должен угадать свой цвет в $3$ ситуациях. Значит, имеются для него ответы $\alpha_{i_1 j_1}$, 
$\alpha_{i_2 j_2}$, не являющиеся пасами. Но тогда в ситуациях $\overline{\alpha_{i_1 j_1}} i_1 j_1$ и 
$\overline{\alpha_{i_2 j_2}} i_2 j_2$ он ошибется, что противоречит предположению о $7$ выигрышных ситуациях. 

Таким образом, максимальная вероятность выигрыша не превышает $3/4$.
Обобщите это рассуждение на случай $n = 2^m - 1$.
\end{ordre}

\begin{problem}[Граница Эдгара Гилберта]
Для обеспечения помехоустойчивости кода при передачи информации, вместо исходного $k$-буквенного сообщения, передается $n$-буквенное ($n>k$). Возникает вопрос, при каких значениях параметров $q = |\Sigma|$ - размер алфавита, $k$, $n$, $l$ существует код $F: \Sigma^k \rightarrow \Sigma^n$, исправляющий  $l$ ошибок, и как его построить? 
Достаточное условие существования кода дает так называемая \textit{граница Гилберта}, которая описана ниже. 

Пространство кодовых слов содержит всего $q^n$ элементов. 
Назовем шаром радиуса $e$ с центром в слове $x\in \Sigma^n$ множество слов, отличающихся от $x$ не более чем в $l$ позициях.
Будем выбирать кодовые слова одно за другим произвольным образом, следя за тем, чтобы расстояния (по Хэммингу) между ними были больше $2l$. В какой-то момент пространство окажется полностью покрытым шарами, каждый из которых состоит из $V_q(2l, n)$ элементов, где $V_q(2l, n)$ - объем шара радиуса $2l$. Тогда при выполнении условия:
\[
(q^k - 1) V_q(2e, n) < q^n
\] 
существует код с параметрами  $q$, $k$, $n$, $l$.
Используя формулу Стирлинга ($k! \approx (k/е)^k$), оцените число элементов в шаре $V_q(2l, n)$. В случае $q=2$ последняя оценка легко получается применением оценок больших уклонений биномиальной случайно величины.

С помощью идеи {\it случайного кодирования} можно посторить код, с точностью до двух битов, реализующий границу Гилберта с большой вероятностью. Для этого случайно и независимо выбираются $N$ кодовых слов $\xi_1, \ldots, \xi_N$ в пространстве $\Sigma^n$. 

Найдите достаточное условие на параметры  $q$, $N$, $n$, $e$, при котором среди сгенерированных кодовых слов менее половины в среднем (усреднение по выбору случайного кода) будут иметь ``ближайшего соседа''  на расстоянии, не превышающем  $2l$.

\begin{remark}
В контексте это задачи полезно познакомиться с брошюрой Ромащенко А., Румянцев А., Шень А. Заметки по теории кодирования. -- М.: МЦНМО, 2011.
\end{remark}

\end{problem} 


\begin{problem}
Пусть $\{X_i\}_{i=1}^n$ -- независимые в совокупности одинаково распределенные случайные величины с распределением $P = \{p_{a}\}$, на конечном множестве $A = \{a\}$. Доказать, что 
\begin{center}
$-\frac{1}{n} \sum_{i = 1}^n \log \biggl ( P(X_i) \biggr ) \xrightarrow[n \to \infty]{\mathbb{P}} H(P)$
\end{center}
Или, другими словами, для любых $\delta, \varepsilon > 0$ найдется $n_0$ такое что для всех $n \geq n_0$:
\begin{center}
$\mathbb{P}(|-\frac{1}{n} \sum_{i = 1}^n \log P(X_i) - H(P)| < \delta) > 1-\varepsilon$
\end{center}

\begin{ordre}
Воспользутесь тем, что $-\mathbb{E} \log P(X) = H(P)$.
\end{ordre}
\end{problem}

\begin{remark} При достаточно больших значениях $n$ можно определить множество \textit{типичных последовательностей} или \textit{слов}, энтропия которых близка к истинной энтропии распределения $P$. Вероятность появления слова $w$
\begin{center}
$p_w = p_{x_1}...p_{x_n} = 2^{-n (-\frac{1}{n} \sum_{i = 1}^n \log P(X_i))}$.
\end{center}
\textit{Множеством $\delta$-типичных $n$-буквенных слов} в модели, где буквы появляются независимо, назовем $T_{\delta}^{(n)}$:
$$
T_{\delta}^{(n)} = \{w: 2^{-n(H(P) + \delta)} < p_w < 2^{-n(H(P) - \delta)} \}
$$
\end{remark}

\begin{problem}[Асимптотическая равнораспределенность]
Докажите, что:
\begin{enumerate}
\item мощность множества типичных слов ограничено: \[|T_{\delta}^{(n)}| \leq 2^{n(H(X) + \delta)};\]
\item $|T_{\delta}^{(n)}| \geq (1-\varepsilon)2^{n(H(X) + \delta)}$ для достаточно больших $n$;
\item вероятность нетипичности $w$: $\mathbb{P}\{w \not\in T_{\delta}^{(n)} \} \to 0, \; n\to\infty$.
\end{enumerate}
\end{problem}

\begin{remark} Идея о типичных последовательностях лежит в основе кодирования. Например, $\delta$-типичные $n$-буквенные слова кодируются при помощи двоичных последовательностей длины $n(H(X) + \delta)$, нетипичные отбрасываются или представляются одним и тем же добавочным символом. Очевидно, что при декодировании (восстановлении) вероятность ошибки не превысит $\varepsilon$.
\end{remark}
\begin{comment}
\begin{problem} Рассмотрите связь между доказательством принципа асимптотической равнораспределенности и эквивалентностью (для больших систем)энтропий Больцмана и Гиббса.
\end{problem}
\end{comment}

\begin{comment}
\begin{problem}
Всего существует $2^{n\log m}$ $n$-буквенных случайных текстов над алфавитом $(x_1,\ldots,x_m)$. Для их кодирования понадобиться $n\log m$ бит. Предполагая, что все буквы появляются независимо друг от друга по закону $(p_1,\ldots,p_m)$, который в общем случае не является равномерным, предложите лучший способ кодирования, основанный 
на законе больших чисел.
\begin{ordre}
Воспользуйтесь результатами, полученными в предыдущих задачах.
\end{ordre}
\end{problem}

\begin{remark}
Необходимым и достаточным условием существования префиксных кодов является неравенство Крафта -- Макмиллана. 
Пусть $n_1,..., n_k$ - длины кодовых слов, тогда $\sum_{i=1}^k 2^{-n_i} \leq 1$.
Тогда задача о построении кода минимальной средней длины может быть сформулирована следующим образом:
задан вектор $(p_1,...,p_k)$, $\sum p_i = 1$. Найти $n_1,..., n_k$, $n_i > 0$, для которых выполнено
неравенство Крафта -- Макмиллана, а $\sum_{i=1}^k p_in_i \rightarrow \min$, где минимум берется по всем возможным наборам
$n_1,..., n_k$.
Решением этой оптимизационной задачи является \textit{код Хаффмена}. 

\end{remark}
\end{comment}

\begin{problem}
Рассмотрим $n$-буквенные слова, порождаемые следующей моделью: появление каждой буквы $x_i \in A$ ($|A| = m$ - алфавит) не зависит от контекста и подчиняется закону распределения $P = \{p_a, a \in A\}$. Всего существует $2^{n\log m}$ таких слов, поэтому каждое из них может быть закодировано при помощи $n\log m$ бит информации. Если же предполагать, что распределение букв $P$ не является равномерным, то найдется лучший способ кодирования. Предложите такой способ.
\begin{comment}
\begin{ordre}
Воспользуйтесь результатами, полученными в предыдущих задачах.
\end{ordre}
\end{comment}
\end{problem}
\begin{comment}
НЕ ОЧЕНЬ УДАЧНОЕ ЗАМЕЧАНИЕ!

НУЖНО ПОЯСНИТЬ, ЧТО ТАКОЕ КОД?
В ЧЕМ РАЗЛИЧИЕ И ЧТО ТАКОЕ КОДЫ ХАФФМАНА И ШЕННОНА-ФАНО?
"Этот подход продемонстрирован в следующих задачах" - ЭТО НЕ ТАК!
\end{comment}
\begin{remark}
Во многих приложениях код должен быть не только однозначно декодируем, но и \textit{оптимален} в смысле минимальности средней длины. Необходимым (а в  случае префиксных кодов и достаточным) условием для выполнения первого требования является \textit{неравенство Крафта -- Макмиллана}: пусть $l(a)$ - длина кодового слова для буквы $a \in A$, тогда $\sum_{a \in A} 2^{-l(a)} \leq 1$.

Среди всех кодов, удовлетворяющих неравенству Крафта -- Макмиллана найдется код минимальной средней длины: $\sum_{a \in A} p_{a}l(a)\rightarrow \min$, при условии  $\sum_{a \in A} 2^{-l(a)} \leq 1$.  Для этого можно, например, воспользоваться методом множителей Лагранжа: $$
\sum_{a \in A} p_{a}l(a) + \lambda (\sum_{a \in A} 2^{-l(a)} - 1)\rightarrow \min.
$$ Решением является набор $\{l_{opt}(a) = -\log{p(a)}, a \in A\}$, а величина $-\log{p(a)}$ также называется \textit{собственной информацией}. Тогда минимальная средняя длина кода $-\sum_{a \in A}p(a)\log{p(a)} = H(P)$ это ни что иное, как энтропия.
\end{remark}

\begin{problem}[Оценка энтропии марковской цепи]
Приведем еще одну модель генерирования слов над алфавитом $A = \{a_1,...,a_m\}$. Текст моделируется стационарной конечной цепью Маркова, порождающей слова вида  $X_1,\ldots,X_n \in \{A\}^{n}$.   
Вероятность появления $j$-й буквы зависит только от того, какая буква стоит перед ней: $\PR(X_k = a_j| X_{k-1} = a_i) = p_{ij} > 0$. Стационарность означает, что $\forall k: \; P(X_k = a_j) = p_j$, причем, пользуясь формулой условной вероятности, $p_j$ можно представить как $p_j = \sum_{i=1}^m p_i p_{ij}$. 

Энтропия $X_k$ при фиксированной $(k-1)$-й букве определяется как $H(X_k|X_{k-1} = a_i) = -\sum_{j = 1}^m p_{ij}\log{p_{ij}}$, а условная энтропия $X_k$ при условии, что $X_{k-1}$ станет известным перед генерацией $X_{k-1}$, определяется  как $H = H(X_k|X_{k-1}) = -\sum_{i=1}^m p_i \sum_{j=1}^m p_{ij}\log{p_{ij}}$. Энтропия всей цепочки случайных величин в силу марковского свойства равна
\[
H(X_1,..., X_n) = H(X_1) + H(X_2|X_{1}) + \ldots + H(X_n|X_{n-1}) \sim n H.
\]

Пусть $W_n = (X_1,..., X_n)$ -- некоторое слово, порождаемое описанной моделью, докажите что:
\begin{enumerate}

\item $\frac{-\log \PR(W_n)}{n} \overset{p}{\longrightarrow} H$, т.е. все слова $W_n$  могут быть разбиты на два множества: для первого множества \textit{типичных} слов $|\frac{-\log P(W_n)}{n} - H| < \delta(n)$, для второго -- сумма вероятностей элементов сходится к 0 при $n\rightarrow \infty$;

\item Обозначим через $M_\alpha(n)$ максимальное количество значений $W_n$ с суммарной вероятностью не более $\alpha$. Докажите, что
\[
\forall \alpha: \;  \frac{M_\alpha(n)}{n} \to H, \quad n \to \infty.
\]

\end{enumerate}
\end{problem}

\begin{remark}
Пусть длина алфавита $m = 2^N$, а длина слова -- $n$. Пункт б) утверждает, что найдется код, с помощью которого с высокой вероятностью исходное сообщение $W_n$ может быть передано в $N/H \geq 1$ раз более коротким сообщением, чем при кодировании при помощи двоичных слов, когда каждому слову $W_n$ ставится в однозначное соответствие двоичная цепочка длины $2^n = 2^{nN}$.
\end{remark}


\begin{comment}
Написать о роли условной энтропии в оценке энтропии марковского источника. Эмпирические оценки распределения МЦ и "штраф" за аппроксимацию, равный расстояюни КЛ.

НАМНОГО ПОДРОБНЕЕ СТОИТ РАСПИСАТЬ ЗАДАЧУ про Оценка энтропии марковской цепи

ЕСЛИ ЧЕСТНО, Я ПЛОХО ПОНИМАЮ СМЫСЛ СЛЕДУЮЩЕЙ ЗАДАЧИ:(

\begin{problem}[Оценка энтропии русского языка]
Рассмотрим алфавит $A$ состоящий из $34$х букв: $33$ буквы русского алфавита и пробел. На каждом шаге игроку необходимо угадать следующую букву текста, которая будет открыта, при условии, что он видит все буквы, открытые ранее. За каждую правильную догадку игрок получает $34$ рубля. Предложите стратегию, позволяющую оценить снизу энтропию русского языка.
\begin{ordre} Необходимо на каждом шаге выбирать ту букву, появление которой наиболее вероятно с учетом предыдущей информации. Тогда на шаге $n$ выигрыш может быть записан как $S_n = (34)^n \hat{p}(X_1...X_n)$, где $\hat{p}(X_1,...,X_n) = \sum_{a \in A} \hat{p}(a|x_{n-1}...x_1)$. Показать, что $\mathbb{E}\frac{1}{n}S_n \leq \log(34) + H(X)$, $H(X)$ - энтропия русского языка.
\end{ordre}   
\end{problem}


\begin{problem}[Основная теорема теории кодирования Шеннона]
Пусть буква $X$ --- дискретная с.в., принимающая значения из алфавита $(x_1,\ldots,x_m)$ с вероятностями $(p_1,\ldots,p_m)$. 
Имеется случайный текст из $n$ букв $X$ (предполагается, что буквы в тексте независимы друг от друга). Общее количество таких 
текстов $2^{n\log m}$. Поэтому можно закодировать все эти слова, используя $n\log m$ бит. Однако, используя то обстоятельство, что 
$(p_1,\ldots,p_m)$ --- в общем случае неравномерное распределение, предложите лучший способ кодирования, основанный 
на усиленном законе больших чисел.
\end{problem}

\begin{ordre}
Пусть $\Omega=\{ \omega:\; \omega=(X_1,X_2,\ldots, X_n),\, X_i\in 1,2,\ldots,m\}$ --- пространство элементарных исходов. 
Вероятность появления слова $\omega=(X_1,X_2,\ldots, X_n)$ равна $p(\omega)=p_{X_1}\cdot\ldots\cdot p_{X_n}$. По теореме Колмогорова об 
у.з.б.ч. 
$$
-\frac{1}{n}\log p(\omega)=-\frac{1}{n}\sum\limits_{i=1}^{n}\log p_{X_i} \xrightarrow{\text{ п.н. }} 
-{\mathbb E}p(\omega)=-\sum\limits_{i=1}^{m}p_i\log p_i=H(p) 
$$
В частности, $\frac{S_n}{n}\xrightarrow{P}H(p)$, где $S_n=-\log p(\omega)=-\sum\limits_{i=1}^{n}\log p_{X_i}$. Это можно записать в виде 

$$
{\mathbb P}\Bigl( \Bigl| \frac{S_n-nH(p)}{n}\Bigr|>\delta \Bigr)  \xrightarrow{n\to\infty} 0 
$$
\end{ordre}
\end{comment}

\begin{comment}
\begin{remark}
О связи совместная информации $I(x,y)$ и пропускной способности канала.  
\end{remark}

\begin{problem} \textit{Случайные коды.}
\end{problem}


\begin{remark} Стоит ли писать что на этом подходе основывается построение кодов оптимальной длины?
\end{remark}

\end{comment}

\begin{problem}[Неравенство Пинскера] 
\label{KL}
\textit{Относительной энтропией} двух распределений $P$ и $Q$ на множестве $A$ (или \textit{расстоянием Кульбака--Лейблера} между ними) называется
$\mathcal{KL}(P||Q) = \sum_{a \in A} p_a \log \frac{p_a}{q_a}$. 
\textit{Расстоянием по вариации} между двумя распределениями называется $||\mathbb{P}_1 - \mathbb{P}_2||_1 = \sum_{a \in A} |\mathbb{P}_1(a) - \mathbb{P}_2(a)|$. Доказать, что между ним и расстоянием Кульбака--Лейблера справедливо следующее соотношение:
$$\mathcal{KL}(\mathbb{P}_1||\mathbb{P}_2) \geq \frac{1}{2\ln2} ||\mathbb{P}_1 - \mathbb{P}_2||_1^2.$$
\end{problem}

\begin{problem}
%[Критическая размерность] 

 В уездном городе \textit{M} хотят опросить население с целью восстановления матрицы трудовых корреспонденций. Город разделен на $l\gg 1$ районов. Таким образом, число различных пар (место жительство)--(место работы) равно $m = l^2$. Именно эти пропорции (какая доля людей в городе $p_k$ соответствует корреспонденции с номером $k$): $p_k$, $k = 1,...,m$ и нужно определить, опрашивая случайно выбранных жителей города о том где они живут и работают. Используя формулу Стирлинга (для мультиномиального распределения) и неравенство Пинскера, определите какое количество людей достаточно опросить (постарайтесь оценить это число как можно точнее -- опросы стоят денег), чтобы имело место неравенство 
 $$\PR\left(\sum _{k=1}^{m}\left|\frac{n_{k} }{n} -p_{k} \right| \ge 0.05\right) = \PR\left(\frac{1}{n}\|\vec {n} - n \vec{p} \|_{1} \ge 0.05\right)\le 0.05,$$
Покажите, что справедливо аналогичное неравенство для $l_2$ нормы:
 \[
 \PR\left(\frac{1}{n}\|\vec {n} - n \vec{p} \|_{2} \ge \sqrt{\frac{8x}{n}}\right)
\le e^{-x}. 
 \]
 \begin{ordre}
 В первом неравенстве воспользуйтесь неравенствами концентрации меры из раздела \ref{measure}. Для второго неравенства докажите неравенство Хефдинга в Гильбертовом пространстве: пусть $X_1,\ldots,X_n$ -- независимые случайные вектора, причем $\Exp X_i = 0$, $\Vert X_i \Vert_2 < c/2$, $v = nc^2/4$, тогда при $t \ge \sqrt{v}$
 \[
 \PR\left(\left\Vert \sum_{i=1}^{n} X_i \right\Vert > t
 \right)  \le e^{-(t - \sqrt{v}) / 2v}.
 \]    
 Воспользуйтесь неравенством МакДиармида  и следующим свойством нормы
 \[
 \Exp \left\Vert \sum_{i=1}^{n} X_i \right\Vert \le  \sqrt{  \sum_{i=1}^{n} \Exp \Vert X_i \Vert^2   }.
 \]
 \end{ordre}

\begin{comment}
б) (Спокойный--Клочков) * Решите эту же задачу используя другие нормы: $l_2$, $l_\infty$, расстояние $KL$, используя другую нормировку $\left|n_{k}/(p_{k}n) - 1 \right|$, используя другие неравенства: Бернштейна, Буске, Спокойного (см. раздел 6); используя многомерную ц.п.т. и оценки скорости сходимости в ней (В.В. Сенатов). Рассматрите разные случаи: когда все $p_k$ приблизительно одного порядка и когда это не так. Сравните ответы. Как зависит минимально возможное значение $n = \sum _{k=1}^{m}n_{k}$ от $m$? В каком случае достаточно, чтобы $n\gg m^{3/2}$, в каком случае этого условия не достаточно? Чем чревато нарушение этого условия и что можно сделать, если мы не можем его обеспечить? Всегда ли достаточно, чтобы $n \gg m^3$? 
\end{comment}
\end{problem}


\begin{problem}
Для двух монеток, симметричной ($p = \frac{1}{2}$) и неправильной ($q = \frac{1 +\varepsilon}{2}$), требуется выяснить какая из них является симметричной. Покажите, что для выявления симметричной монетки потребуется $\Omega (1 / \varepsilon^2)$ бросаний. Рассмотрите также случай $p = \varepsilon$, $q = 2 \varepsilon$. В каком случае потребуется больше бросаний? 

\end{problem}

\begin{ordre}
Пусть $f(X_1,\ldots, X_n) \in [0, M]$ является некоторой статистикой, которую можно подсчитать для каждой из монеток и по разности значений идентифицировать монетки. Покажите, что 
\[
\bigg\vert \Exp_{ \mathbb{Q} }[ f(X_1,\ldots, X_n) ] - \Exp_{ \mathbb{P} }[ f(Y_1,\ldots, Y_n) ]  \bigg\vert 
\leq  M \Vert \mathbb{Q} - \mathbb{P} \Vert_1,
\]   
где $(X_1,\ldots, X_n) \in \mathbb{Q}$, $(Y_1,\ldots, Y_n) \in \mathbb{P}$. Далее, для оценки $ \Vert \mathbb{Q} - \mathbb{P} \Vert_1$ можно воспользоваться неравенством Пинскера (см. задачу \ref{KL}), а также цепным правилом для $\mathcal{KL}$ дивергениции (см. указание к задаче \ref{bandit_lower}).
\end{ordre}



\begin{comment}
\begin{remark} Необходимость построения нижних оценок возникает тогда, когда случайная последовательность генерируется одним из распределений $\{P_i\}$ (неизвестно каким), а наилучшая стратегия игрока зависит от вида истинного $P_k \in \{P_i\}$, о котором нет никакой информации  . 
\end{remark}


\begin{problem}[Многорукие бандиты--1]
\end{problem}

ЗАДАЧА ПРО МНОГОРУКИХ БАНДИТОВ НА ОЦЕНКУ СНИЗУ ПО 5-й ЛЕКЦИИИ Yishay Mansour (в рамках курса Advanced Topics in Machine Learning and Algorithmic Game Theory), в которой в двух местах есть опечатка вместо + там стоит -
\end{comment}
\begin{problem}$^*$
Есть $N$ ручек, с каждой из которых связана вероятность успеха $p_k$ (дергая $k$-ю ручку с вероятностью $p_k$ мы получим 1, а с вероятностью $1-p_k$ ничего).
Таким образом, выигрыш игрока при выборе $k$-й ручки есть $r_k \in \text{Be}(p_k)$.    
Вероятности $p_k$ не известны игроку. Игрок намеревается выполнить $T \gg N$ дерганий ручек. При выборе ручки на новом шаге можно использовать всю предысторию. Предложите стратегию, ``максимально близкую'' в среднем по размеру выигрыша к величине $T \max \limits_k p_k$.

\begin{remark} См. монографию Lugoshi G., Cesa-Bianchi N. Prediction, learning and games. New York: Cambridge University Press, 2006, а также S. Bubeck, N. Cesa-Bianchi. Regret Analysis of Stochastic and Nonstochastic Multi-armed Bandit Problems. In Foundations and Trends in Machine Learning, Vol 5, 2012. 
\end{remark}
\end{problem}


\begin{problem}[Многорукие бандиты]
\label{bandit}
В модели \textit{стохастического многорукого бандита} имеется $K$ распределений $f_1, \ldots,f_K$ на множестве $\Omega = [0, 1]$, каждое из которых является распределением выигрыша в зависимости от выбора действия $a \in \{1,\ldots,K\}$. 
Игра повторяется $T \gg K$ раундов, причем на $t$-м раунде
\begin{enumerate}
\item игрок выбирает действие $A(t)$, исходя из результатов предыдущих раундов;
\item среда генерирует выигрыш $r_t$ из распределения  $f_{A(t)}$, независимо от предыдущих раундов.
\end{enumerate}   

Пусть $m_k = \Exp_{f_k} (r)$, $m^{*} = \max_{k} m_k$, $\triangle_k = m^{*} - m_k$  
Цель игрока состоит в минимизации следующей функции потерь
\[
\overline{R}_T = T m^{*} - \sum_{t=1}^{T} \Exp m_{A(t)} = \sum_{k=1}^{K} \triangle_k \Exp A_k(T),
\]
где $A_k(T)$ -- количество действий с номером $k$ за $T$ раундов.
Опишем используемую  стратегию игры (то есть алгоритм выбора действий~$A$).
В каждом раунде будем вычислять доверительные интервалы для оценок $\widehat{m}_1, \ldots, \widehat{m}_K$ и выбирать в следующем раунде действие, соответствующее максимальному значению верхней границы доверительного интервала.

Используя неравенство Маркова в экспоненциальной форме (метод Чернова), покажите 
что согласно описанной стратегии 
\[
A(t+1) \in \mathop{\arg\max} \limits_{k \in \{1,\ldots,K\}} \left[ 
\widehat{m}_{k, A_k(t)} + g^{-1} \left(\frac{\alpha \ln t}{ A(t)} \right)
\right],
\]  
при уровне значимости для доверительного интервала $1 / t^{\alpha}$, где $g$ определяется из условия 
\[
\Exp e^{\lambda |r - \Exp_{f_k} (r)|} \leq  \psi(\lambda), 
\quad
g(x) = \psi^{*}(x) = \sup_{\lambda} (\lambda x - \psi(\lambda)).  
\] 

\end{problem}


\begin{problem}
Докажите верхнюю оценку для стратегии, предложенной в задаче 
\ref{bandit}:
\[
\overline{R}_T \leq \sum_{k: \triangle_k > 0} \left(
\frac{\alpha \triangle_k}{ g(\triangle_k / 2) } \ln (T	) + \frac{\alpha}{\alpha - 2}
\right).
\]
Также установите для случая $f_k = \Be(p_k)$, что для любой стратегии $A$, при выполнении условия $\forall k: \triangle_k > 0 \to \Exp A_k(T) = o(T^{\gamma})$, $\gamma > 0$, справедлива нижняя оценка
\[
\mathop{\underline{\lim}}\limits_{T \to \infty} \frac{\overline{R}_T}{\ln(T)} \geq 
\sum_{k: \triangle_k > 0} 
\frac{\triangle_k}{\KL(m_k, m^{*}) }.
\]
\end{problem}

\begin{ordre} См. S. Bubeck, N. Cesa-Bianchi. Regret Analysis of Stochastic and Nonstochastic Multi-armed Bandit Problems. In Foundations and Trends in Machine Learning, Vol 5, 2012. 
\end{ordre}


\begin{remark}
Последняя оценка говорит об асимптотической неулучшаемости стратегии из задачи \ref{bandit}. Для сравнения приведенных оценок можно воспользоваться неравенством
\[
\KL(m_k, m^{*}) = \KL(p_k, p^{*})  \leq \frac{(p_k - p^{*})^2}{p^{*} (1- p^{*})} =   \frac{\triangle_k^2}{p^{*} (1- p^{*})}.
\] 
\end{remark}


\begin{problem}
\label{bandit_lower}
Пусть параметры распределений $f_k = \Be(p_k)$:  $p_1,\ldots,p_K$ в модели из задачи \ref{bandit} принадлежат распределению $F$. Докажите, что сушествует такое $F$, что для любого детерминированного алгоритма игрока $A$ выполнено неравенство
\[
T \max \limits_k p_k - \sum_{t = 1}^{T} \Exp(r_t | A) \geq \frac{1}{20} \min(\sqrt{KT}, T) = \Omega (\sqrt{KT}).
\]
\end{problem}

\begin{ordre}
В качестве $F$ возьмите следуюшее распределение: все $p_k = 0.5$, за исключением одного $p_i = 0.5 + \varepsilon$, $i$ выбрано случайно равновероятно из множества $\{1,\ldots,K\}$. Установите тождество
\[
\Exp(r_t | A) = \frac{1}{2} + \frac{\varepsilon}{K} \sum_{j=1}^K \sum_{r} \big[A(t,r) = j \big] \PR(r|A, j=i),
\]
где $r \in \{0,1\}^T$, $[\cdot]$ -- индикаторная функция. Далее, воспользуйтесь 
соотношением
\[
\sum_{r} \big[A(t,r) = j \big] \PR_i(r) \leq \sum_{r} \big[A(t,r) = j \big] \PR_u(r) + \Vert \PR_i - \PR_u \Vert_1,
\]
где $\PR_i(r) = \PR(r|A, j=i)$, $\PR_u(r)$ -- распределение выигрышей при $p_1 = \ldots = p_K = 0.5$. Воспользуйтесь неравенством Пинскера и цепным разложением величины 
\[
\mathcal{KL}(p(x,y),q(x,y)) = \mathcal{KL}(p(x),q(x)) + \sum_{x} p(x) \mathcal{KL}(p(y|x),q(y|x)). 
\]

\end{ordre}


\begin{problem}
Пусть казино делает $n$ бросаний, используя распределение вероятностей на бинарных словах длины $n$ -- $p\left(x\right)$, где $x \in \left\{0,1\right\}^{n} $, известное игроку. При этом казино производит выплаты так, как если бы оно использовало распределение $q\left(x\right)$ (то есть выигранная ставка на 0, после выпадения последовательности исходов $x$ увеличивается в $\frac{q\left(x\right)}{q\left(x :+ 0\right)} $ раз, выигранная ставка на 1 -- увеличивается в $\frac{q\left(x\right)}{q\left(x :+ 1\right)} $ раз). Докажите, что у игрока есть стратегия, логарифм значения капитала которой равен расстоянию Кульбака--Лейблера (см. задачу \ref{KL})  между распределениями $p$ и $q$.
\end{problem}

\begin{comment}
ЗАМЕЧАНИЕ ВЕРЕЩАГИН И ЩЕПИН
\begin{problem} \textit{Неравенство больших уклонений}
Рассмотрим последовательность незовисимых одинаково распределенных случайных величин $X_1, ..., X_n$, $X_i~Be(q)$. Доказать, что $-\frac{1}{n}\log \mathbb{P}(\frac{1}{n}\sum X_i \geq p) \rightarrow p\log \frac{p}{q} + (1-p)\log \frac{1-p}{1-q} = KL((p, 1-p)||(q, 1-q))$.
\begin{ordre}
\end{ordre}
\end{problem}

\begin{remark} 
Этот результат является следствием теоремы Санова, которая позволяет оценивать вероятности больших уклонений.. Приведем ниже её упрощенную формулировку.\\
\textit{Теорема Санова}
\end{remark}

\end{comment}


\begin{problem} [Теорема Шеннона о пропускной способности канала с шумом] 

Канал (поток) связи с шумом описывается матрицей переходных вероятностей $p(Y|X)$, где $X$ и $Y$ -- случайные величины с распределениями $P$ (на множестве $A$ -- входной алфавит) и $Q$ (на множестве $B$ -- выходной алфавит) соответственно. Другими словами, $p(y|x)$ -- вероятность прочитать  символ $y$ из потока при условии, что в него был записан символ $x$.
Определим \textit{Шенноновское количество информации} как $I(P, Q) = H(P) + H(Q) - H(P,Q)$. Пропускной способностью такого канала называется величина $C= \max_{\{p_x\}}I(P;Q)$.
Пусть по каналу передаются слова $w_1,...,w_N$ длины $n$.
Разобьем множество кодовых слов в алфавите $Y$ на непересекающиеся области $V_0,...,V_N$. Если принятое слово $y \in V_j$, $j = \overline{1,N}$, то принимается решение о том, что было послано слово $w_j$. Если $y \in V_0$ то никакое определенное решение не принято. Введем \textit{среднюю вероятность ошибки} $$\overline{P}_{\varepsilon}(W, V) = \frac{1}{N} \sum_{i=1}^n (1 - p(V_i|w_i)).$$
Пусть $p_{\varepsilon}(n, N) = \min_{W, V} \overline{P}_{\varepsilon}(W, V)$, докажите что:
\begin{enumerate}
\item[а)] $p_{\varepsilon}(n, 2^{nR}) \rightarrow 0$, $R < C$;
\item[б)] $p_{\varepsilon}(n, 2^{nR}) \not\rightarrow 0$, $R > C$;
\item[в)] $p_{\varepsilon}(n, 2^{nR}) \rightarrow 1$, $R > C$,
\end{enumerate}
где $R = \frac{\log N}{n}$ -- скорость передачи.
\begin{remark}
Величина $H(P,Q) = -\sum_{a\in A} p(a)\sum_{b \in B}p(a, b)\log p(a, b)$ называется \textit{совместной энтропией} двух случайных величин.
\end{remark}
\end{problem} 
\begin{comment}
В ЗАМЕЧАНИИ ХОТЕЛОСЬ БЫ ВИДЕТЬ И СВЯЗЬ С ЗАДАЧЕЙ ПРО ГРАНИЦУ ГИЛБЕРТА, ГДЕ ИСПОЛЬЗУЕТС ЯСЛУЧАЙНОЕ КОДИРОВАНИЕ
ПОЛЕЗНО ЗДЕСЬ ЖЕ ОБЫГРАТЬ СТР, 133 теорему 10.11 Верещагин Щепин

Вообще стоит подробнее в заадчах осветить главу 11 этой книги!
\end{comment}




==> measure_concentration.tex <==
\section{Неравенства концентрации меры \\ и вероятности больших уклонений}
\label{measure}


\begin{problem}[Концентрация площади сферы и объема шара]
\
\begin{enumerate}
\item Рассмотрим шар $B^{n}(r)$ радиуса $r$ в евклидовом пространстве $\mathbb{R}^n$ большой размерности, пусть в шаре задана равномерная мера. 
%Пусть $V\big[B^{n}(r)\bigl]$ ~--- объем шара.
 Необходимо убедиться в том, что мера сконцентрирована в малой окрестности  границы шара.
\item
Рассмотрим сферу $S^{n-1}(r)$ в евклидовом пространстве $\mathbb{R}^r$ с радиусом в начале координат. Необходимо убедиться в том, что выбранные наугад два единичных вектора в пространстве $\mathbb{R}^n$ большой размерности с большой вероятностью окажутся почти ортогональными, если на сфере задано равномерное распределение.  
%Зафиксируем координатную ось $x$.
%Необходимо убедиться в том, что подавляющая часть площади многомерной сферы $S^{n-1}$ сосредоточена в малой окрестности экватора, перпендикулярного выбранной оси $x$. Каково взаимное расположение двух выбранных наугад единичных векторов в простанстве $\mathbb{R}^n$, если концы векторов распределены на сфере равномерно?
\end{enumerate}
\end{problem}


\begin{remark}
Во втором пункте достаточно доказать, что для всякого сколь угодно малого $\delta>0$ проекция второго вектора на ось $x_1$ с вероятностью, близкой к 
единице, лежит в промежутке $[-\delta, \delta]$ при $n\to\infty$. Это равносильно тому, что доля от площади всей сферы $S^{n-1}(r)$, 
которую занимает сферический слой $S^{n-1}_{\delta}(r)$, проектирующийся в отрезок $[-\delta, \delta]$ оси $x_1$, 
может быть сделана сколь угодно близкой к $1$ при $n\to\infty$. 

Перейдя к $n$-мерным сферическим координатам и обратно, покажите, что мера сферического слоя $S^{n-1}_{\delta}(r)$ равна 
$$
\mu_{n-1} S_{\delta}^{n-1}(r) = Cr^{n-1} 
\int\limits_{-\delta}^{\delta} \Bigl( 1-(x/r)^2\Bigr)^{(n-3)/2} \, dx ,
$$
тогда вероятность попадания в данный слой $S_{\delta}^{n-1}(r)$ равна 
$$
{\mathbb P}[-\delta, \delta]=\frac{\int\limits_{-\delta}^{\delta} \Bigl( 1-(x/r)^2\Bigr)^{(n-3)/2} \, dx}
{\int\limits_{-r}^{r} \Bigl( 1-(x/r)^2\Bigr)^{(n-3)/2} \, dx} . 
$$
Данное отношение на зависит от $r$, поэтому можно считать $r=1$. 

Для нахождения асимптотики имеющихся интегралов ($n\to\infty$) используйте классические результаты относительно асимптотики интеграла 
Лапласа $F(\lambda)=\int_a^b f(x)e^{\lambda S(x)}\, dx$ при $\lambda\to +\infty$ (см. указание к задаче \ref{laplas} из раздела  \ref{genF}). %Если обе функции $f$ и $S$ определены и регулярны 
%на промежутке $I=[a,b]$ и функция $S$ имеет единственный глобальный максимум на $I$, который достигается в точке $x_0\in I$, 
%$f(x_0)\ne 0$, то асимптотика интеграла такая же, как в окрестности точки $x_0$ (принцип локализации). В зависимости от расположения 
%точки $x_0$ и свойств функции $S(x)$ возможны следующие тейлоровские разложения при $\lambda\to +\infty$: 
%$$
%F(\lambda)=\frac{f(x_0)}{-S'(x_0)}e^{\lambda S(x_0)} \lambda^{-1}\bigl( 1+O(\lambda^{-1})\bigr) , 
%$$
%если $x_0=a$ и $S'(x_0)\ne 0$ (т.е. $S'(x_0)<0$); 
%$$
%F(\lambda)=\sqrt{\frac{\pi}{-2S''(x_0)}} f(x_0) e^{\lambda S(x_0)} \lambda^{-1/2}\bigl( 1+O(\lambda^{-1/2})\bigr) , 
%$$
%если $x_0=a$, $S'(x_0)=0$, $S''(x_0)\ne 0$ (т.е. $S''(x_0)<0$); 
%$$
%F(\lambda)=\sqrt{\frac{2\pi}{-S''(x_0)}} f(x_0) e^{\lambda S(x_0)} \lambda^{-1/2}\bigl( 1+O(\lambda^{-1/2})\bigr) , 
%$$
%если $a<x_0<b$, $S'(x_0)=0$, $S''(x_0)\ne 0$ (т.е. $S''(x_0)<0$). 

Для решения этой и следующей задачи рекомендуется ознакомиться с книгой Зорич В.А. Математический анализ задач естествознания,-- М.: МЦНМО, 2008.
\end{remark}



\begin{problem}[Изопериметрическое неравенство и принцип концентрации меры; П. Леви, 1919]
\label{levi}
Число $\mu _f $ называют медианой функции $f$, если
$\mu \left( {\vec {x}\in S_1^n :\;\;f\left( {\vec {x}} \right)\ge \mu _f } 
\right)\ge 1 \mathord{\left/ {\vphantom {1 2}} \right. 
\kern-\nulldelimiterspace} 2$ и $\mu \left( {\vec {x}\in S_1^n :\;\;f\left( 
{\vec {x}} \right)\le \mu _f } \right)\ge 1 \mathord{\left/ {\vphantom {1 
2}} \right. \kern-\nulldelimiterspace} 2$,
где $\mu \left( {d\vec {x}} \right)$ -- равномерное мера на единичной сфере 
$S_1^n $ в ${\mathbb R}^n$. Пусть $A$ -- измеримое (борелевское) множество на 
сфере $S_1^n $. Через $A_\delta $ -- будем обозначать $\delta $-окрестность (расстояние определяется по геодезический)
множества $A$ на сфере $S_1^n $. Предположим теперь, что в некотором 
царстве, расположенном на $S_1^n $, царь предложил царице Дидоне построить 
огород с заданной длиной забора. Царица хочет, чтобы её огород при заданном 
периметре имел наибольшую площадь. Таким образом, царице надо решить 
изопериметрическую задачу (такие задачи обычно рассматриваются в курсах 
вариационного исчисления). Решение этой задачи хорошо известно на плоскости -- ``круглый 
огород'', это можно обобщить на наш случай. Для нас же полезно, рассмотрение двойственной задачи, имеющей 
такое же решение: при заданной площади огорода спроектировать его так, чтобы 
он имел наименьшую длину забора, его ограждающего. Используя решение этой 
задачи, покажите, что если $\mu \left( A \right)\ge 1 \mathord{\left/ 
{\vphantom {1 2}} \right. \kern-\nulldelimiterspace} 2$, то
$$
\mu \left( {A_\delta } \right)\ge 1-\sqrt {\frac{\pi}{8}} \exp \left( \frac{-\delta^2n}{2} \right).
$$
Пусть теперь на $S_1^n $ задана функция с модулем непрерывности
\[
\omega _f \left( \delta \right)=\sup \left\{ {\left| {f\left( {\vec {x}} 
\right)-f\left( {\vec {y}} \right)} \right|:\;\;\rho \left( {\vec {x},\vec 
{y}} \right)\le \delta ,\;\vec {x},\vec {y}\in S_1^n } \right\}.
\]
Покажите, что тогда
\[
\mu \left( {\vec {x}\in S_1^n :\;\;\left| {f\left( {\vec {x}} \right)-\mu _f 
} \right|\ge \omega _f \left( \delta \right)} \right)\le \sqrt {\pi 
\mathord{\left/ {\vphantom {\pi 2}} \right. \kern-\nulldelimiterspace} 2} 
\exp \left( {-{\delta ^2n} \mathord{\left/ {\vphantom {{\delta ^2n} 2}} 
\right. \kern-\nulldelimiterspace} 2} \right).
\]
Можно показать, что при весьма естественных условиях медиана асимптотически 
близка к среднему значению (математическому ожиданию). Аналогичное 
неравенство можно получить (М. Талагран, 1994), например, для модели 
случайных графов (Эрдёша - Реньи) исследовать плотную концентрацию около 
среднего значения различные функций на случайных графах: число 
независимости, хроматическое число и т.п.
\end{problem}


\begin{remark}
Изопериметрические неравенства на сфере были обобщены в начале 80-х М.Л. Громовым на римановы многообразия (см. подробнее в \cite{14}).

Пусть $(X,g)$ ~--- компактное связное гладкое риманово многообразие размерности $n>2$ со строго положительной кривизной Риччи и римановой метрикой $g$, наделенное элементом объема $d\mu=\frac{dv}{V}$, где $V$~--- полный объем $X$. 
Кривизна Риччи~--- способ описания изменения многообразия по отношению к евлидовой мере, то есть степени отличия мнообразия  от евклидова пространства. 
Обозначим за $c(X)$ точную нижнюю грань тензора кривизны Риччи по всем единичным касательным векторам. Пусть $c(X)>0$. Тогда 
$$
\mathcal{P}_{\mu}\geq \mathcal{P}_{\sigma^n_{\mathbb{R}}},
$$
где $\sigma^n_{R}$ -- равномерная инвариантная мера, $\mathcal{P}_{\mu}$ -- изопериметрическая функция, т.е. наибольшая функция на $[0,\mu(X)]$, такая что
$$
\mu^{+}(A) \geq \mathcal{P}_{\mu}(\mu(A)) \quad \text{при~}\mu^{+}(A) = \lim_{t\to\infty}\inf\frac{1}{t}\mu(A_t/A),
$$ 
где $A_t = \{x\in X; g(x,A)<t\}$.

Здесь $R>0$ таково, что 
$$
c({S}^n_{R}) = \frac{n-1}{R^2}=c(X),
$$ 
где ${S}^n_{R}$~--- $n$-сфера с радиусом $R$, снабженная нормированной равномерной инвариантной мерой $\sigma^n_{R}$. 
В частности для $(X,g,\mu)$ верно 
\begin{equation*}
\alpha(X;r)\leq \text{e}^{-cr^2/2},\quad r>0, 
\end{equation*}
где концентрационная функция $\alpha(X;r)$ определяется следующим образом
\begin{equation*}
\alpha(X;r) = 1-\inf\biggl\{\mu(A_{r})|\, A \subset X, \mu(A)\geq \frac{1}{2}\biggr\}.
\end{equation*}

\begin{problem}(Концентрация на дискретном кубе) Пусть $E = \{-1, 1\}^{n}$ --- дискретный $n$-мерный куб, на множестве вершин которого задана равномерная вероятностная мера $\mu$. Введем на вершинах куба стандартную Хэммингову метрику. Тогда для всякой $1$-липшицевой (по введенной метрике) действительнозначной функции $f$, заданной на $E$, c медианой $M$ для $\varepsilon \ge 0$ имеет место неравенство
\[
\PR\{\left|f(X) - M\right| \ge \varepsilon\} \le 2\exp\left(\frac{-\varepsilon^{2}}{2n}\right).
\]
а) Пусть $\Exp f(X)$ -- математическое ожидание функции. Докажите, что
\[
\left|\mathbb{E} f(X) - M\right| \le \sqrt{2\pi n}.
\]

б) Покажите, что фактор $\frac{1}{n}$ под экспонентой не может быть 'улучшен'. В частности, неравенство концентрации явно зависит от размерности куба (при условии сохранения гауссовского хвоста по $\varepsilon$).
\end{problem}

\begin{remark}
Используйте тот факт, что для случайной величины $Y > 0$ имеет место равенство $\Exp Y = \int\limits_{0}^{\infty}\PR\{Y \ge x\}dx$.

См.\cite{22} и Barvinok A. Math 710: Measure Concentration. Lecture notes, 2005. http://www.math.lsa.umich.edu/~barvinok/total710.pdf.
\end{remark}

\begin{problem}(Неравенство Талаграна для дискретного куба) Пусть $E = \{-1, 1\}^{n}$ --- дискретный $n$-мерный куб, на множестве вершин которого задана равномерная вероятностная мера $\mu$. Введем на вершинах куба стандартную евклидову метрику. Тогда для всякой выпуклой $1$-липшицевой действительнозначной функции $f$, заданной на $E$, c медианой $M$ для $\varepsilon \ge 0$ имеет место неравенство
\[
\Prob\{\left|f(X) - M\right| \ge \varepsilon\} \le 2\exp\left(\frac{-\varepsilon^{2}}{2n}\right).
\]

а) Покажите, что условие выпуклости функции $f$ нельзя опустить в данном неравенстве.


б) Получите неравенство, аналогичное неравенству Талаграна для концентрации около математического ожидания.
\end{problem}
\begin{remark}
См. Talagrand~M. An Isoperimetric Theorem on the Cube and the Kinitchine-Kahane Inequalities,
Proceedings of the American Mathematical Society, 1988. Pp.\,905-909.

В отличие от предыдущей теоремы в данном неравенстве нет зависимости от размерности куба. Одновременно накладываются два дополнительных требования, во-первых, липшицевость по меньшей -- евклидовой метрике, во-вторых, дополнительно на функцию накладывается условие выпуклости.

Существуют аналогичные неравенства концентрации вокруг математического ожидания с гораздо более точными константами. Тем не менее, даже этот простой способ позволяет получить нужный нам гауссовский хвост, не зависящий от размерности.
\end{remark}

\begin{problem} (Концентрация на сечениях куба) Пусть $E = \{-1, 1\}^{n}$ --- дискретный $n$-мерный куб. Рассмотрим его сечение, состоящее из всех его вершин, содержащих ровно $k$ координат, равных $1$. Введем на вершинах сечения нормированную метрику $d$, равную половине Хэмминговой метрики. При этом расстояние между вершинами, координаты которых отличаются лишь перестановкой пары координат равно единице. На множестве вершин сечения зададим равномерную вероятностную меру $\mu$. Введем также понятие длины дискретного градиента $|\nabla f(X)|$. Обозначим
\[
|\nabla f(X)|^{2} = \sum\limits_{Y : d(X, Y) = 1}|f(X) - f(Y)|^{2},
\]
где суммирование ведется по всем $k(n - k)$ вершинам сечения, удаленным от данной вершины на единицу.

Тогда для всякой действительнозначной функции $f$, заданной на описанном сечении, длина дискретного градиента которой в точках сечения ограничена числом $\sigma$, для $\varepsilon \ge 0$ имеет место неравенство
\[
\PR\{f(X) - \Exp f(X) \ge \varepsilon\} \le \exp\left(\frac{-(n + 2)\varepsilon^{2}}{4\sigma^{2}}\right).
\]
Пусть случайна величина $Y$ имеет гипергеометрическое распределение с параметрами $N, K, n$, то есть для неотрицательного целого $k$
\[
\PR\{Y = k\} = \frac{C_{K}^{k}C_{N - K}^{n - k}}{C_{N}^{n}}.
\]

Получите экспоненциальную оценку на величину $\PR\{Y - \Exp Y \ge \varepsilon\}$.
\end{problem}

\begin{remark}
 Вспомните интерпретацию гипергеометрического распределения и свяжите ее с равномерным распределением на вершинах сечения дискретного куба.
См. Bobkov S.\;G. Concentration of normalized sums and a central limit theorem for noncorrelated random variables, Annals of probability, No.\,4, Pp.\,2884-2907, 2004 и Bobkov S.\;G., Tetali,\;P.
 Modified logarithmic Sobolev inequalities in discrete settings, 
Journal of Theoretical Probability,  No.\,2, Pp.\,289--336, 2006.
\end{remark}

%КАТЯ, ПОСТАРАЙТЕСЬ СДЕЛАТЬ ЭТО ЗАМЕЧАНИЕ ПО ДОСТУПНЕЕ И С КАКОЙ-НИБУДЬ ССЫЛКОЙ

\begin{problem}*
\label{talagran}
В сельском районе, имеющем форму квадрата со стороной $1$, находится $n$ домов $(n\gg 1)$, размерами которых можно пренебречь по сравнению с линейным размером района. Будем считать, что при строительстве домов застройщик случайно (согласно равномерному распределению $R[0,1]^2$)  и независимо выбирал их местоположения. Почтальону необходимо обойти все $n$ домов ровно по одному разу (от любого дома почтальон может направиться к любому другому по прямой). Обозначим через $\ell$ длину наикратчайшего из таких путей (кратчайший гамильтонов путь).
Покажите, что найдется такая константа $c>0$, не зависящая от $n$, что 

\begin{equation*}
\mathbb{P}(\ell - \mathbb{E}\ell \geq t)\leq \exp \biggl(-\frac{t^2}{4c}\biggr). 
\end{equation*}
Можно показать, что $\mathbb{E}\ell\sim\beta\sqrt{n}$, где $\beta$ также не зависит от $n$.

\end{problem}

\begin{remark}
См. книгу Dubhashi D. P., Panconesi A. <<Concentration of measure for the analysis of randomized algorithms>>, Cambridge University Press, 2009.

Приведем несколько неравенств Талаграна. Пусть заданы множества $\Omega_i$, $i=1,\dots,n$, элементарных исходов. На этих множествах заданы вероятностные меры $\PR_i$, $i=1,\dots,n$. Положим 
\begin{equation*}
\Omega= \prod_{i=1}^n\Omega_i,\quad \PR = \prod_{i=1}^n \PR_i.
\end{equation*}
Введем взвешенную метрику Хэмминга:
\begin{equation*}
d_{\alpha}(x,y) = \sum_{x_i\not = y_i} \alpha_i \biggr/ \sqrt{\sum_{i=1}^n \alpha^2_i}
\end{equation*}
и определим $d_{\alpha}(x,A) = \min_{y\in A} d_{\alpha}(x,y)$, $\rho(x,A) = \sup_{\alpha\in \mathbb{R}^n} d_{\alpha}(x,A)$. Пусть $A \in \sigma(\Omega)$. Определим $t$-окрестность ($t\geq$ 0) множества $A$ по формуле 
\begin{equation*}
A_t = \{x\in\Omega: \rho (x,A)\leq t\}.
\end{equation*}
Тогда справедливо неравенство Талаграна:
\begin{equation*}
\mathbb{P}(A)(1-\mathbb{P}(A_t))\leq \exp\biggl(-\frac{t^2}{4}\biggr).
\end{equation*}
\begin{suite}
 %Пусть $X = (X_1,\dots,X_n) $ случайный вектор, значения компонент которого лежат в $[0,1]$. Пусть $F: \mathbb{R}^n\to\mathbb{R}$  выпуклая, липшицева функция с константой $1$ по отношению к метрике Хэмминга ($d(u,v) = \sum_{i=1}^n I(u_i\not=v_i)$,\,\, $u,v \in [0,1]^n$). Пусть $M F(X)$ ~--- медиана $F(X)$, тогда для всех $t>0$ верно
%\begin{equation*}
%\PR (|F(X)-MF(X)|\geq t)\leq 4\mathrm{e}^{-t^2/4}.
%\end{equation*}
%Рассмотрим выпуклую Липшицеву функцию $f$ на ($\mathbb{R}^n$, $\|\cdot\|_2$) с константой Липшица $\sigma$. 

В качестве приложения неравенства Талаграна рассмотрим функцию $h:\; \Omega \to {\rm R}$, $\Omega = \mathbb{R}^n$, удовлетворяющую условию Липшица с константой $\sigma$. Функцию $h$ будем называть проверяемой со сложностью $f$, если при $h(x)\ge s$ существует такое множество $I\subseteq \{1,\ldots ,n\}$ с $\vert I\vert \le f(s)$, что для всех $y\in \Omega $, совпадающих с $x$ в координатах из $I$, выполняется $h(y)\ge s$. Грубо говоря, из выполнения неравенства $h(x)\ge s$ следует, что существует сравнительно небольшое количество 
координат, обеспечивающих выполнение данного неравенства. Тогда из 
неравенства Талаграна можно получить следующее соотношение о плотной 
концентрации случайной величины $h$: для всех $b$ и $t$ 
справедливо 
\[
\PR\left[ {h\le b-t\sqrt {f(b)} } \right]\PR\left[ {h\ge b} \right]\le 
e^{-\frac{t^2}{4}}.
\]
Выбирая либо в качестве $b$, либо в качестве $b-t\sqrt {f(b)} $ медиану случайной величины $h$, получаем результат о плотной концентрации $h$ вокруг своей медианы

\begin{equation*}
\mathbb{P} (|h(X)-M|> t)\leq 4\mathrm{e}^{-t^2/8\sigma^8}.
\end{equation*}
\end{suite}


Неравенство Талаграна для независимых случайных величин. Пусть $X_1,\dots,X_n$ независимые случайные величины в $S$. Для любого класса функций ${\mathcal{F}}$
на $S$ равномерно ограниченного  на $S$ константой $U$ для всех $t>0$ выполнено 
\[
\mathbb{P}\left\{\left\|\sum_{i=1}^n f(X_i)\right\|_{\mathcal{F}} - \mathbb{E}\left\|\sum_{i=1}^n f(X_i)\right\|_{\mathcal{F}}
 \geq t \right\}\leq K\exp\left\{-\frac{t}{UK}\log\left(1+\frac{tU}{V}\right)\right\},
\]
где $K$ - универсальная константа и $V$ удовлетворяет условию 
\[
V\geq \mathbb{E}\sup_{f\in\mathcal{F}}\sum_{i=1}^n f^2(X_i) 
\]
и использованы обозначения  $\|Y\|_{\mathcal{F}} = \sup_{\mathcal{F}}|Y(f)|
$, где $Y: \mathcal{F}\to \mathbb{R}$. 

\end{remark}

%КАТЯ, А ВЫ УВЕРЕНЫ, ЧТО ИМЕННО ТАК? Все как-то странно:)
%КАТЯ ВСЕ ХОРОШО, ТОЛЬКО ЧТО ТАКОЕ ЛИПШИЦЕВА ФУНКЦИЯ ОТНОСИТЕЛЬНО ТОЙ МЕТРИКИ, КОТОРУЮ МЫ ВВЫЕЛИ НЕ ДО КОНЦА ЯСНО, ПОСКОЛЬКУ МЫ ЛИШЬ ОПРЕДЕЛИЛИ РАССТОЯНИЕ ОТ ТОЧКИ ДО МНОЖЕСТВА, НО МНЕ МЕЖДУ ТОЧКАМИ, ЧТО НУЖНО В ОПРЕДЕЛЕНИИ КОНСТАНТЫ ЛИПШИЦА

\begin{problem}[Семейства Леви] 
%Определим для компактного множества $X$ с мерой $\mu$  концентрационную функцию 
%\begin{equation*}
%\alpha(X;\varepsilon) = 1-\inf\biggl\{\mu(A_{\varepsilon})|\, A \subset X, \mu(A)\geq \frac{1}{%2}\biggr\},
%\end{equation*}
%где $A_{\varepsilon} = \bigl\{x\in X | \,\, \rho(s,A) \leq \varepsilon \bigr\}$.
Пусть  $(X_n,\rho_n,\mu_n)$  -- метрическое вероятностное пространство, $X_n$ -- компактное множество с метрикой $\rho_n$, $ \diam X_n\geq 1$ и заданной вероятностной мерой $\mu_n$. Семейство  $(X_n,\rho_n,\mu_n)$ метрических вероятностных пространств называется семейством Леви, если для любого $\varepsilon>0$, $\alpha(X_n,\varepsilon \cdot \diam X_n) \to 0$ для $n\to \infty$ (см. определение концентрационной функции в замечании к задаче \ref{levi}).  Семейство называется нормальным семейством Леви с константами $(c_1,c_2)$, если
\begin{equation*}
\alpha(X_n;\varepsilon) \leq c_1 \exp(-c_2\varepsilon^2 n),
\end{equation*}
Докажите, что следующие семейства будут нормальными семействами Леви.
\begin{enumerate} 
\item \label{first} Пусть на $E^n = \{-1,1\}^n$  задана Хэммингова метрика 
\begin{equation*}
d(s,t) = \frac{1}{n} |\{i:s_i\not=t_i\}|
\end{equation*}
и нормированная считающая мера $\mu$, т.е. $\mu(A) = |A|/2^n$. Докажите неравенство 
\begin{equation*}
\alpha(F_2^n;\varepsilon) \leq \frac{1}{2}\exp(-2\varepsilon^2 n).
\end{equation*}
\item 
Задана группа $\Pi_n$ перестановок $\{1,\dots,n\}$ с заданной нормированной метрикой Хэмминга 
\begin{equation*}
d(\pi_1,\pi_2) = \frac{1}{n} |\{i:\pi_1(i)\not=\pi_2(i)\}|
\end{equation*}
 и нормированной считающей мерой (см. пункт \ref{first}). Докажите неравенство 
\begin{equation*}
\alpha(\Pi_n;\varepsilon) \leq \exp\Bigr(-\varepsilon^2n/64\Bigl).
\end{equation*}
\end{enumerate}
\end{problem}
\begin{remark}
Примеры приведены в статье  Milman V.D. The heritage of P.~Levy in geometrical functional analysis // Asterisques. 1988. V. 157-158. P. 273-302, см. также книгу M. Ledoux <<The Concentration of Measure Phenomenon>>, American Mathematical Soc., 2005, а также теорему Талаграна в замечании к предыдущей задаче.

\end{remark}

\begin{problem}(Кац, Секей)
Рассмотрим полином с вещественными коэффициентами
\begin{equation*}
a_0+a_1t+\ldots+a_{n-1}t^{n-1},
\end{equation*}
где $(a_0,a_1,\dots,a_{n-1})$ точка на единичной сфере $S_n(1)$. 
 Среднее число вещественных корней полинома определим следующим образом:
$$
\mathbb{E} N = \frac{1}{|S_n(1)|}\int_{S_n(1)}N(a)d\sigma,
$$
где  $N(a)$ число вещественных корней полинома, $d\sigma$~--- элемент поверхности единичной сферы площадью
$$|S_n(1)| = \frac{(2\pi)^{n/2} }{ \Gamma\left(\frac{n}{2}\right) }.$$


\begin{enumerate}
\item 
Покажите, что среднее число вещественных корней полинома с коэффициентами на единичной сфере равно среднему числу вещественных корней полинома, коэффициенты которого независимы и распределены стандартно нормально, то есть 
\begin{equation*}
\mathbb{E} N = (2\pi)^{-n/2}\int_{-\infty}^{\infty}\dots\int_{-\infty}^{\infty}N(a)\exp \left(-\frac{1}{2}\|a\|^2\right)\,da_0,\dots,\,da_{n-1}.
\end{equation*}
\item 
Пусть $\mathbb{E}N^{(1)}$, $\mathbb{E}N^{(2)}$, $\mathbb{E}N^{(3)}$, $\mathbb{E}N^{(4)}$~--- средние значения числа вещественных корней, заключенных в интервалах $(-\infty,-1)$, $(-1,0)$, $(0,1)$, $(1,\infty)$ соответственно.
Покажите, что 
\begin{equation*}
\mathbb{E}N^{(1)}=\mathbb{E}N^{(2)}=\mathbb{E}N^{(3)}=\mathbb{E}N^{(4)} 
\end{equation*}
и
\begin{equation*}
\mathbb{E}N^{(i)}\sim (2\pi)^{-1}\ln n, \quad n\to\infty.
\end{equation*}
%\item
\end{enumerate}
\end{problem}
\begin{remark}
Н.Б. Маслова в статье О распределении числа вещественных корней случайных полиномов // ТВП, 1974, Т. 19, В. 3, с. 488–-500 доказала следующую теорему: если коэффициенты $X_i$ случайного алгебраического уравнения 
\[
\sum_{j=1}^n X_jz^j=0
\]
являются независимыми одинаково распределенными случайными величиными с нулевыми математическими ожиданиями и $$\mathbb{E}\left(|X_j|^{2+\epsilon}\right)<\infty$$ для некоторого положительного $\epsilon$, то число действительных корней этого уравнения распределено нормально с математическим ожиданием $\frac{2}{\pi}\ln n$ и стандартным отклонением $2\sqrt{\pi^{-1}(1-2\pi^{-1})\ln n}$.
\end{remark}


\begin{problem}$^{**}$
Дан случайный граф (модель Эрдеша--Реньи, см. задачу \ref{sec:erdRenyi} раздела \ref{hard}) $G\left( {n,\;p} \right)$ с $n$ вершинами и 
вероятностью появления каждого ребра $p$. Пусть $p\ge \sqrt {\frac{2 \ln 
n}{n}} $, причем длины ребер $r_{ij} $ являются независимыми случайными величинами, имеющими равномерное распределение на отрезке 
$\left[ {0,\;2r} \right]$. Покажите, что тогда почти наверное граф $G\left( 
{n,\;p} \right)$ имеет гамильтонов цикл, причём длина почти всех 
гамильтоновых циклов стабилизируется около $nr$.
\end{problem}

\begin{problem}$^{**}$
Дан случайный граф (модель Эрдеша--Реньи, см. задачу \ref{hard}.\ref{sec:erdRenyi}) $G\left( {n,\;p} \right)$ с $n$ вершинами и 
вероятностью появления каждого ребра $p\in \left[ {\varepsilon ,1} \right]$, 
$\varepsilon >0$. Вес каждого появившегося случайного ребра разыгрывается  независимо 
согласно равномерному распределению на отрезке $\left[ {0,2} 
\right]$.  Источник и сток выбираются случайно. Обозначим через $S_n $ значение максимального потока для 
полученного случайного взвешенного графа. Покажите, что 
${S_n } 
\mathord{\left/ {\vphantom {{S_n } {pn}}} \right. \kern-\nulldelimiterspace} 
{pn}\buildrel p \over \longrightarrow 1.$
\end{problem}

\begin{problem}[Cтохастическое агрегирование; В.И. Опойцев]
\begin{enumerate}
\item На рынке имеется $n$ 
продавцов, каждый из которых может продать свой товар в объеме $x_k $ для 
$k$-го товара. Спрос на товары обеспечивают покупатели. Пусть $y_k$ -- спрос на 
товар $k$. Общий объем сделок $L_n=\sum\limits_{k=1}^n {\min 
\left\{ {x_k ,y_k } \right\}} $. Предложите такой естественный способ 
определения вероятностной меры на двух симплексах
\[
S_X =\left\{ {\vec {x}\ge \vec {0}:\;\;\sum\limits_{k=1}^n {x_k } =X} 
\right\},
\quad
S_Y =\left\{ {\vec {y}\ge \vec {0}:\;\;\sum\limits_{k=1}^n {y_k } =Y} 
\right\},
\]
чтобы нашлась функция $f\left( {X,Y} \right)$, удовлетворяющая  $$L_n 
\mathord{\left/ {\vphantom {L n}} \right. \kern-\nulldelimiterspace} 
n\buildrel p \over \longrightarrow f\left( {X,Y} \right).$$

\item Пусть $\vec {y}=A\vec {x}$, $A=\left\| {a_{ij} } 
\right\|_{i,j=1,1}^{l,n} $, $X=\left\langle {\vec {p},\vec {x}} 
\right\rangle $, $Y=\left\langle {\vec {q},\vec {y}} \right\rangle $. 
Матрицы и векторы предполагаются положительными. Легко проверить, что
\[
Y=\lambda \left( {\vec {x}} \right)X,
\quad
\lambda \left( {\vec {x}} \right)=\sum\limits_{i,j} {\frac{q_i a_{ij} }{p_j 
}} \frac{p_j x_j }{X}\mathop =\limits^{def} \sum\limits_{i,j} {b_{ij} } z_j 
.
\]
Считая $z_j >0$ независимыми одинаково распределенными с.в.: $\Exp z_j =m_j $ 
($\sum_{j} m_j  =1)$, $\Var z_j =\sigma _j^2 $ (например, $z_j \in 
\left[ {0,2n^{-1}} \right])$, покажите, что если выражение
\[
\frac{\mathop {\max }\limits_j \sum\limits_i {b_{ij} } \cdot \mathop {\max 
}\limits_j \sigma _j }{\mathop {\min }\limits_j \sum\limits_i {b_{ij} } 
\cdot \mathop {\min }\limits_j m_j }
\]
равномерно ограничено с ростом $n$, то существует такое число $\bar {\lambda 
}$, что с вероятностью стремящейся к единице $Y\simeq \bar {\lambda }X$.

\end{enumerate}
\end{problem}




\begin{problem}[Красносельский--Крейн]
Рассмотрим систему линейных алгебраических уравнений 
\begin{equation*}
x=Ax+b,
\end{equation*}
где $A$ положительно определенная неособенная матрица, собственные числа $\lambda_1\leq\dots\leq\lambda_n$ которой меньше единицы, $b$~--- заданный и  $x$ ~--- искомый векторы $n$-мерного подпространства. Пусть эта система решается при помощи итерационного процесса 
\begin{equation*}
x_{m+1}= Ax_{m}+b,\quad m=1,2,\dots,
\end{equation*}
 который заканчивается на $p$-м шаге, если вектор--невязка $\delta_p = x_{p+1}-x_{p}$ попадает в шар радиуса $\alpha$ с центром в нуле. 
Ошибка итерационного процесса $\varepsilon_m = x^{*} - x_m$, где  $x^{*}$ истинное решение системы уравнений, связана с невязкой  (проверить)
 \begin{equation*}
\varepsilon_m = (I-A)^{-1}\delta_m,
\end{equation*}
поэтому  исходя из значений вектора невязки можно определить вероятностное распределение  ошибок. 

Оказывается, что наиболее вероятными ошибками являются максимальные.
А именно, пусть начальная ошибка равномерно распределена в шаре $T$ радиуса $R$, тогда для любого $\eta<1$ вероятность выполнения следующего неравенства стремится к единице при $R\to\infty$
\begin{equation*}
\eta \frac{\alpha \lambda_n}{1-\lambda_n}\leq \|\varepsilon\| \leq \frac{\alpha}{1-\lambda_n}.
\end{equation*} 

Проверьте это для случая $n=2$.

\end{problem}
\begin{remark}
Пусть итерационный процесс заканчивается на шаге $p$, если вектор-невязка $\delta_p=x_{p+1}-x_p$ попадает в окрестность $G$ нуля. Пусть $G$~--- шар радиуса $\alpha$. Тогда ошибка $\varepsilon_p$ попадет в множество $G_0 = (I-A)^{-1}G$, которое является эллипсоидом с полуосями длины $\frac{\alpha}{1-\lambda_1}$ и $\frac{\alpha}{1-\lambda_2}$.
Обозначим $G_{-1}=AG_0$ ~--- эллипсоид с полуосями $\frac{\alpha\lambda_i}{1-\lambda_i}$, $i=1,2$. 
 
\imgh{100mm}{krein.pdf}{Множества ошибок в случае матрицы $2\times 2$. Закрашенная темно-серым цветом часть соответствует области из утверждения задачи при $\eta$ близком к $1$.}

Обозначим $G_m = A^{-m}G_0$. Процесс заканчивается на $p$-м шаге, если $\varepsilon_0\in G_p$ и $\varepsilon_0\not\in G_p$, те когда $\varepsilon_0$ находится в слое $G_p-G_{p-1}$.
При этом окончательная ошибка будет находиться в слое $A^{p}(G_p-G_{p-1}) = G_0-G_{-1}$.Таким образом окончательная ошибка принадлежит $G_{-1}$ только в случае, если $\varepsilon_0$ принадлежит $G_0$. 
Вероятность нахождения окончательной ошибки в элементе слоя $G_0-G_{-1}$ равна сумме вероятностей нахождения начальной ошибки в элементах $\Delta=A^{-m}\Delta_0$ ($m=0,1,\dots$).

Предположим, что начальная ошибка $\varepsilon_0$ равномерно распределена в шаре $T$ достаточно большого радиуса. В этом случае вероятность $P(\Delta_m)$ нахождения начальной ошибки в элементе $\Delta_m\in T$ пропорциональна объему этого элемента. Подсчитайте вероятность $P(\Delta_0)$ попадания окончательной ошибки в элемент $\Delta_0$ и убедитесь, что вероятность попадания окончательной ошибки в точку слоя $G_0-G_{-1}$ для данной точки тем больше, чем позже эта точка выйдет из $T$ при последовательном применении к ней операции $A^{-1}$. 

Пусть $e_i$~--- собственные векторы матрицы $A$, соответствующие собственным числам $\lambda_i$, $i=1,2$.
Для доказательства утверждения задачи оцените вероятность того, что окончательная ошибка $\varepsilon = \sum_{i=1}^n\xi_ie_i$ не удовлетворяет неравенству (утверждению задачи). Перейдя к пределу по $R\to\infty$ получите, что вероятность невыполнения утверждения задачи стремится к нулю.


\end{remark}

%КАТЯ, НЕОБХОДИМО ТАКЖЕ ДОБАВИТЬ ЗАМЕЧАНИЕ С РИСУНКОМ :)

\begin{problem}[Физическая интерпретация концентрации меры на сфере]
Имеется $n$ частиц массы $m$  со скоростями $v_i$, $i=1,\dots,n$. Известно, что вектор скоростей молекул идеального газа равномерно
распределен по поверхности постоянной энергии. Суммарная кинетическая энергия $E_n$ растет пропорционально $n$, то есть 
\begin{equation*}
\frac{1}{2}mv_1^2+\cdots+\frac{1}{2}m v_n^2 = E_n;\quad \sum_{i=1}^n v^2_i=\frac{2E_n}{m}\asymp n.
\end{equation*}
Получите закон распределения Максвелла скоростей частиц одномерного идеального газа. 
\end{problem}

\begin{ordre}
В решении задачи 1 этого раздела перейдите к термодинамическому пределу, когда $n\to\infty$, $r = \sigma n^{1/2}$, чтобы получить закон распределения Максвелла скоростей частиц.
\end{ordre}

\begin{remark}
Равномерное распределение на поверхности постоянной энергии возникло из-за того, что инвариантной (и предельной, то есть возникающей на больших временах, по эргодической гипотезе) мерой для гамильтоновой системы будет как раз равномерная мера  по теореме Лиувилля (фазовый объем сохраняется). Поскольку выполняется закон сохранения энергии, то система  ``живет'' \mbox{~на} поверхности постоянной энергии. Следовательно, носитель инвариантной меры сосредоточен именно на этой поверхности. 

Приведем для справки результат, полученный  для выпуклых тел с заданной на них равномерной мерой (теорема Б. Клартага в статье Milman V.D. Geometrization of Probability // Progress in Mathematics. 2008. V. 265, http://www.math.tau.ac.il/~milman/, также см. статью Klartag B. A central limit theorem for convex sets // Inventiones mathematicae
April 2007, Volume 168, Issue 1, pp. 91--131). Существует последовательность $\epsilon_n\to 0$, ${n\to\infty}$ для которой выполнено: пусть $K\in \mathbb{R}^n$ выпуклое компактное множество с непустой внутренностью, случайный вектор $X$ распределен равномерно в $K$, тогда существуют вектор $\theta\in\mathbb{R}^n$, $t_0\in\mathbb{R}$ и $\sigma>0$, что выполнено
\[
\sup_{A\in\mathbb{R}}\left|\mathbb{P}\left\{\sum_{i=1}^n X_i\theta_i\in A\right\} - \frac{1}{\sqrt{2\pi}\sigma}\int_{A}{\rm e}^{-\frac{(t-t_0)^2}{2\sigma^2}}\,dt\right|\leq \epsilon_n,
\]
где супремум берется по всем измеримым множествами $A\in\mathbb{R}$. Eсли $\mathbb{E}X_i=1$, $\mathbb{E}X_iX_j = \delta_{ij}$, то $t_0=0$, $\sigma=1$, то можно найти такой единичный вектор  $\theta$, что выполняется приведенное неравенство.

\end{remark}

\begin{problem}[Лемма Пуанкаре]
Пусть $X_n$ -- случайный вектор с равномерным распределением на единичной сфере в ${\mathbb R}^n$. Равномерное распределение 
характеризуется тем, что оно инвариантно относительно группы ортогональных преобразований. Пусть $Y_n$ обозначает первую координату $X_n$. 
Докажите, что $\sqrt{n}\, Y_n \xrightarrow{d}N(0,1)$ при $n\to\infty$. Заметим, что в статистической физике с помощью утверждения 
этой задачи получался закон распределения Максвелла скоростей частиц одномерного идеального газа. 
\end{problem}

\begin{ordre}

См. предыдущую задачу. Решение задачи содержит в себе способ генерирования равномерного распределения. 
Пусть $\xi_1,\ldots, \xi_n$ --- независимые в совокупности с.в., имеющие одинаковое распределение $N(0,1)$. Рассмотрим случайный вектор 
$Z_n=(\xi_1,\xi_2,\ldots,\xi_n)$. Тогда $Z_n\in N(0,I_n)$, $I_n$ --- единичная матрица размера $n$. 

Показажите, что $Z_n$ инвариантно относительно группы ортогональных преобразований. Заметим, что распределения 
$$
X_n \quad\text{ и } \quad \frac{Z_n}{\|Z_n \|_{{\mathbb R}^n}} \quad \text{ совпадают. }
$$
Поэтому имеет место равенство по распределению с.в. 
$$
Y_n=\frac{\xi_1}{\sqrt{\xi_1^2+\ldots+ \xi_n^2}} 
$$
$$
\Rightarrow \quad \sqrt{n}Y_n = \frac{\xi_1}{\sqrt{(\xi_1^2+\ldots+ \xi_n^2)/n}} . 
$$
Применить теорему Колмогорова у.з.б.ч. для $\frac{\xi_1^2+\ldots+ \xi_n^2}{n}$. 

\end{ordre}

\begin{problem}[Геометрическая интерпретация закона больших чисел]
Рассмотрим куб $C^n = [-1,1]^n$ в евклидовом пространстве $\mathbb{R}^n$. Пусть $\xi_i$, $i=1,\dots,n$ независимые случайные величины с равномерным распределением на $[-1,1]$. Приведите геометрическую интерпретацию закона больших чисел.
\end{problem}

\begin{ordre} 
Рассмотреть объем  следующего множества ---   пусть $\mathcal{H}$ часть гиперплоскости, содержащаяся в кубе и перпендикулярная главной диагонали куба, т.е.  $\sum_{i=1}^n x_i = 0$. Необходимо подсчитать объем $\varepsilon\sqrt{n}$-окрестности $\mathcal{H}$. 
\end{ordre}



\begin{problem} [В.И. Опойцев]
\begin{enumerate}
\item[а)] Пусть имеются абсолютно непрерывные (имеющие плотность) независимые случайные величины $X_1,\ldots, X_n$ и пусть 
$Y_n=G_n(X_1,\ldots, X_n)$ --- также случайная величина. Докажите следующее неравенство, описывающее нелинейный закон больших чисел: 
$$
\Var Y_n\leqslant \int_{{\mathbb R}^n} \sum\limits_{i=1}^{n} \Bigl(\frac{\partial G_n(x_1,\ldots, x_n)}{\partial x_i} \Bigr)^2 f_i^*(x_i)
\prod\limits_{j\ne i} f_j(x_j)\, dx_1\ldots dx_n , 
$$
где сопряженные плотности $f_i^*(x_i)$ существуют и определяются следующим образом 
$$
f_i^*(x_i)=\mu_i(\infty)\int\limits_{-\infty}^{x_i} f_i(t)\, dt -\mu_i(x_i), \quad 
\mu_i(x)=\int\limits_{-\infty}^{x} tf_i(t)\, dt . 
$$

\item[б)] Пусть независимые одинаково распределенные случайные величины $X_1,\ldots, X_n$ имеют равномерное распределение на отрезке 
$[0,1]$ (часто пишут $X_i\in R[0,1]$), а 
$$
\max\limits_{x\in [0,1]^n} \|\nabla G_n(x_1,\ldots, x_n) \|\xrightarrow{n\to\infty} 0 . 
$$
Тогда $Y_n\xrightarrow{P}{\mathbb E}Y_n$ при $n\to\infty$. 

\item[в)] Пусть независимые одинаково распределенные случайные величины $X_1,\ldots, X_n$ имеют равномерное распределение на отрезке 
$[0,1]$, а $Y_n=G_n(X_1,\ldots, X_n)=\max\limits_{i=1,\ldots, n} X_i$. Тогда $Y_n\xrightarrow{p}{\mathbb E}Y_n$ при $n\to\infty$. 

\end{enumerate}
\end{problem}

\begin{remark}
См. В. Босс Лекции по математике. Т.4: Вероятность, информация, статистика, 2005.
\end{remark}

%По мотивам лекции Голубева, обзора Лугоши.

%\begin{enumerate}
%\item
\begin{problem}[Неравенство Чернова]
Докажите, что неравенство Чернова для неотрицательной случайной величины $X$
\begin{equation*}
\PR\{ X >t\}\leq \inf_{s>0}\mathbb{E}\exp(sX-st)
\end{equation*}
 дает более завышенную границу по сравнению с моментной границей
\begin{equation*}
\PR\{ X >t\}\leq \min_{q>0}\mathbb{E}[X^q]t^{-q},
\end{equation*}
 то есть 
\begin{equation*}
\min_{q>0}\mathbb{E}[X^q]t^{-q}\leq \inf_{s>0}\mathbb{E}\big[\text{e}^{s(X-t)}\bigl].
\end{equation*}
\end{problem}

\begin{ordre}См. \cite{BLM}. Использовать следствие из неравенства Маркова: для монотонной возрастающей неотрицательной функции $\phi(\cdot)$ и произвольной случайной величины $X$ верно
\begin{equation*}
\PR\{\phi(X)\geq \phi(t)\}\leq \frac{\mathbb{E}\phi(X)}{\phi(t)}.
\end{equation*}
\end{ordre}

%\item 
%\begin{problem}[Неравенство Чернова для суммы случайных величин]

%\end{problem}

%\item


\begin{problem}[Лемма Хёфдинга] Пусть $X$--- случайная величина, такая что $\mathbb{E}X =0$, $a\leq X\leq b$. Покажите, что для $s>0$ верно
\begin{equation*}
\mathbb{E}\exp(s X)\leq \exp\bigg[\frac{s^2(b-a)^2}{8}\biggr].
\end{equation*}
\end{problem}

\begin{ordre}
Используя выпуклость экспоненты, для $a\leq x\leq b$

\begin{equation*}
\text{e}^{sx} \leq \frac{x-a}{b-a} \text{e}^{sb}+\frac{b-x}{b-a}\text{e}^{sa},
\end{equation*}

получите 

\begin{equation*}
\mathbb{E}\text{e}^{sx} \leq \text{e}^{\phi(u)},
\end{equation*}
где $u = s(b-a)$, $\phi(u) = -pu+\log(1-p+p\text{e}^u)$, $p = -a/(b-a)$.
Найдите $\phi^{\prime\prime}(u)$,   $\phi(0)$, $\phi^{\prime}(0)$.
Покажите, что 
\begin{equation*}
\phi^{\prime\prime}(u)\leq \frac{1}{4}.
\end{equation*}

Используя формулу Тейлора, получите 
\begin{equation*}
\phi(u) \leq \frac{u^2}{8}\leq \frac{s^2(b-a)^2}{8}.
\end{equation*}
\end{ordre}

\begin{problem}[Теорема Хёфдинга] Пусть $\xi_t$, $t\in T$ -- независимые случайные величины, такие что $\xi_t\in[a,b]$. Докажите, что 
\begin{equation*}
\PR\bigg\{\bigg|\frac{1}{n}\sum_{t\in T}\big(\xi_t-\mathbb{E}\xi_t\bigr)\biggr|\geq x\biggr\}\leq 2\exp\bigg\{-\frac{2nx^2}{(b-a)^2}\biggr\}.
\end{equation*}
\end{problem}
\begin{ordre}
Введите случайную величину $\xi = \frac{1}{n}\sum_{i=1}^n(\xi_i-\mathbb{E}\xi_i)$.
Воспользуйтесь неравеством Чернова и леммой Хёфдинга для $\xi$ и получите
\begin{equation*}
\PR\{\xi>x\}\leq \exp\bigg\{\min_{\lambda}\bigg[-\lambda x + \frac{\lambda^2}{8}\frac{(b-a)^2}{n}\biggr]\biggr\}.
\end{equation*}
Затем найдите оптимальное $\lambda$.  Аналогичное неравенство справедливо для $-\xi$.
\end{ordre}

\begin{problem}[Неравенство Беннетта]
Пусть $X_1,\dots, X_n$ независимые центрированные ограниченные случайные величины, такие, что с вероятностью $1$ выполнено $|X_i|\leq c$.
Пусть $\sigma^2 = \sum_{i=1}^n\Var\{X_i\}$.
Покажите, что для любого $t>0$ 
\begin{equation*}
\PR\bigg\{\sum_{i=1}^n X_i>t\biggr\}\leq \exp\bigg(-\frac{n\sigma^2}{c^2}h\bigg(\frac{ct}{n\sigma^2}\biggr)\biggr),
\end{equation*}
где $h(u) = (1+u)\log(1+u)-u$ для $u\geq 0$.
\end{problem}
\begin{ordre}
Введем $\sigma_i^2 = \mathbb{E}[X_i^2]$ и $F_i = \sum_{r=2}^{\infty}\frac{s^{r-2}\mathbb{E}[X_i^r]}{r!\sigma_i^2}$.
Используя разложение для ряда Тейлора $\exp(sX)$, показать, что 
\begin{equation*}
\mathbb{E}[e^{sX_i}]\leq \exp(s^2\sigma^2_iF_i).
\end{equation*}

Из ограниченности  $X_i$ получите оценку
\begin{equation*}
F_i\leq \frac{\exp(sc)-1-sc}{(sc)^2}.
\end{equation*} 
Далее воспользуйтесь неравенством Чернова для $X_i$ и минимизируйте правую часть в неравенстве Чернова по $s$.
\end{ordre}

\begin{problem}[Неравенство Бернштейна \cite{BLM}]
\label{bernstain}
Докажите, что при выполнении условий предыдущей задачи для любого  $\varepsilon>0$ верно следующее неравенство
\begin{equation*}
\PR\bigg\{\frac{1}{n}\sum_{i=1}^n X_i>\varepsilon\biggr\}\leq \exp\bigg(-\frac{n\varepsilon^2}{2\sigma^2+2c\varepsilon/3}\biggr).
\end{equation*}
\end{problem}

\begin{ordre} 
Покажите, что верно элементарное неравенство 
\begin{equation*}
h(u)\geq \frac{u^2}{2+2u/3}
\end{equation*}
и используйте неравенство Беннетта.

\begin{comment}
Отметим, что в случае схемы Пуассона, т.е. если рассмотреть последовательность $\xi_1,\dots,\xi_n$ с распределнием Бернулли с вероятностью успеха $\lambda/n$,   оценка в асимптотике по $n$ принимает вид, аналогичный  неравенству больших уклонений.
\end{comment}

\end{ordre}
%\end{enumerate}


\begin{problem}[Неравенство Азумы--Хёфдинга]
Пусть $\{X_i\}_{i=0}^{\infty}$ последовательность со следующим свойством (см. замечание к задаче 3.8)
\begin{equation*}
\mathbb{E}(X_n|X_1,\dots,X_{n-1}) =X_{n-1},
\end{equation*}
и пусть $Y_i = X_i-X_{i-1}$ соответствующая последовательность приращений (мартингальная разность). Покажите, что если существуют такие $c_i>0$, что $|Y_i|\leq c_i$ для всех $i$, то
\begin{equation*}
\PR\Bigl\{\sum_{i=1}^{m}Y_i \geq t\Bigr\}\leq 2\exp\bigg\{\frac{-t^2}{2\sum_{i=1}^{m}c^2_i}\biggl\}.
\end{equation*}
\end{problem}
\begin{ordre}

%\begin{enumerate}
%\item \textit{Использовать теорему Дуба.} 
%%\textbf{TODO}
%\item \textit{Cпособ для доказательства не равномерного варианта теоремы %использует результат задачи 12.}

Вначале необходимо докажите следующее утверждение.
 Пусть $Y$ случайная величина,  $Y\in [-1,+1]$ и $\mathbb{E}[Y]=0$. Тогда для любого $t\geq 0$ верно 
\begin{equation*}
\mathbb{E}[\exp(tY)]\leq \exp(t^2/2).
\end{equation*}
Для этого необходимо использовать выпуклость $\exp(tx)$, а именно для $x\in[-1,1]$ верно
\begin{equation*}
\text{e}^{tx}\leq \frac{1}{2}(1+x)\text{e}^{t} +\frac{1}{2}(1-x)\text{e}^{-t}.
\end{equation*}
Подсчитайте оценку математического ожидания $\mathbb{E}[\text{e}^{tY}]$ используя разложение экспоненты в ряд Тейлора и элементарный факт $(2n)!>2^nn!$. Затем покажите, что 
\begin{equation*}
\mathbb{E}\exp\biggl(s\sum_{j=1}^m Y_j\biggr) = \mathbb{E}\biggl[\exp\biggl(s \sum_{j=1}^{m-1} Y_j\biggr)\mathbb{E}[\exp(sY_m)|X_{1},\dots,X_{m-1}]\biggl]. 
\end{equation*}
Используйте неравенство Чернова
\begin{equation*}
\PR[Y_1+\dots+Y_m>t]\leq \exp\bigg[-st+\sum_{i=1}^mc^2_i s^2/2\biggr].
\end{equation*}
Остается минимизировать правую часть неравенства по $s$.

\end{ordre}


\begin{problem}
Пусть независимые одинаково распределенные невырожденные ($\not \equiv \text{const}$) случайные величины $\xi_1,\xi_2,\dots$ с математическим ожиданием $m$ удовлетворяют \textit{условию Крамера}, то есть существует такая окрестность нуля, что для любого $\lambda$ из этой окрестности 
\begin{equation*}
\mathbb{E}e^{\lambda \xi}<\infty.
\end{equation*}
Пусть 
$$
S_n = \xi_1+\dots+\xi_n, \quad \psi(\lambda) = \ln \mathbb{E}\exp(\lambda\xi)
$$ 
и 
\begin{equation*}
H(a) = \sup_{\lambda}[a\lambda - \psi(\lambda)],\quad a\in \mathbb{R},
\end{equation*}
Покажите, что верно следующее неравенство Дуба
\begin{equation*}
\PR\biggl\{\sup_{k\geq n}\biggr|\frac{S_k}{k}-m\biggl|>\varepsilon\biggl\}\leq 2\exp\biggl(-\min\Big[H(m-\varepsilon),H(m+\varepsilon)\Bigr]n\biggr).
\end{equation*}
\end{problem}

\begin{ordre}
Зафиксируйте $n\geq 1$ и положите 
\begin{equation*}
\kappa  = \inf \biggl\{k\geq n: \frac{S_k}{k}>a\biggr\}, 
\end{equation*}
считая $\kappa = \infty$, если $\frac{S_k}{k}\leq a$, $k\geq n$.
Пусть $\lambda>0$  и $\lambda a - \psi(\lambda)\geq 0$. 
Показать, что 
\begin{equation*}
\begin{split}
&\mathbb{P}\biggl\{\sup_{k\geq n}\frac{S_k}{k}>a\biggr\} = \mathbb{P}\biggl\{\frac{S_{\kappa}}{\kappa}>a,\,\kappa<\infty\biggr\} \\
&\leq \mathbb{P}\biggl\{\exp\Bigl(\lambda S_{\kappa} - \kappa  \psi (\lambda)\Bigr)>\exp\Bigl(n\lambda -n  \psi(\lambda)\Bigr),\kappa<\infty \biggr\}\\
&\leq 
 \mathbb{P}\biggl\{\sup_{k\geq n}\exp\Bigl(\lambda S_{k} - k  \psi (\lambda)\Bigr)>\exp\Big(n\lambda -n  \psi(\lambda)\Bigr)\biggr\}.
\end{split}
\end{equation*}

Затем, необходимо воспользоваться тем фактом, что последовательность случайных величин $Y_k = \exp (\lambda S_k-k \psi(\lambda))$, $k\geq 1$ является мартингалом (см. задачу \ref{sec:doob}  раздела \ref{hard}).

Для момента остановки
$\tau = \inf \{k\leq n: Y_k\geq \lambda \}$, $\tau = n$ если $\max_{k\leq n}Y_k <\lambda$ верна теорема Дуба (см. задачу \ref{sec:doob}  раздела \ref{hard}).
Тогда  из неравенства Маркова для любого $x>0$
\begin{equation*}
x \cdot \mathbb{P}\biggl\{\sup_{k\geq n} Y_k \geq x\biggr\}\leq \mathbb{E}Y_n.
\end{equation*}
Отсюда
\begin{equation*}
\mathbb{P}\biggl\{\sup_{k\geq n}\frac{S_k}{k}>a\biggr\}\leq \exp\biggl\{-n \Bigl(\lambda a -  \psi(\lambda)\Bigr)\biggr\}.
\end{equation*}
Рассмотрите случаи $a>m$ и $a<m$.

\end{ordre}
%\begin{problem}
%Что можно сказать о том, как соотносятся между собой неравенство Бернштейна и Хевдинга? Рассмотреть неравенство Бернштейна в случаях, когда $\sigma^2>\varepsilon$ и когда $\sigma^2<\varepsilon$. Что можно сказать про достижимость неравенства Бернштейна? 
%\begin{remark}
%Рассмотреть предельную теорему Пуассона.
%\end{remark}
%\end{problem}



\begin{problem}
Докажите, что для последовательности независимых одинаково распределенных с.в. $\xi_1,\xi_2,\dots$ с математическими ожиданиями $m = \mathbb{E} \xi_i$, дисперсиями $\Var \xi_i = d$ и функцией распределения $F(x)$ верна следующая оценка вероятности больших отклонений %$\PR\Bigl\{\Bigl|\sum_{i=1}^n\xi_i -n m \Bigr|\geq %n\varepsilon \Bigr\}$: 

\begin{equation*}
\PR\Bigl\{\Bigl|\sum_{i=1}^n \xi_i -n m \Bigr|\geq n\varepsilon \Bigr\} \leq B_n(\phi(t_0))^n \exp\big(-t_0 n\varepsilon \bigr) ,
\end{equation*}
где 
%\begin{equation*}
$\lim_{n\to\infty}B_n=\frac{1}{2},$
%\end{equation*}
%\begin{equation*}
$\phi(t)=\int_{-\infty}^{\infty}\text{e}^{t x}\,d F(x),$
%\end{equation*}
%\begin{equation*}
$m(t) = \frac{\phi^{\prime}(t)}{\phi(t)},$
%\end{equation*}
%\begin{equation*}
$r(\lambda_0) = \text{e}^{-\lambda_0 c}R(\lambda_0),$
%\end{equation*}
значение $t_0$ удовлетворяет условию  $m(t_0) = \varepsilon$.

\end{problem}
\begin{remark}


Если использовать для оценки  $\PR\Bigl\{\Bigl|\sum_{i=1}^n\xi_i - n m\Bigr|\geq s\Bigr\}$ неравенство Чебышева, то при $s = \varepsilon \sqrt{n}$ и $s=\varepsilon n$, где $\varepsilon$~--- некоторая постоянная, получается разный порядок сходимости вероятности. В отличие от первого случая, оценка при $s=\varepsilon n$ является очень грубой. 

Доказательство существования, единственности, а также положительности $t_0$  может быть найдено в учебнике Коралова--Синая.

Воспользуемся \textit{методом Крамера} вычисления асимптотики вероятностей. Покажите, что верно 
\begin{equation*}
\PR\Bigl\{\Bigl|\sum_{i=1}^n \xi_i- n m\Bigr|\geq n \varepsilon \Bigr\} \leq (\phi(t_0)\text{e}^{-t_0\varepsilon})^n \idotsint\limits_{\sum_{i=1}^n x_i>\varepsilon n} \,dF_{t_0}(x_1) \dots dF_{t_0}(x_n),
\end{equation*}
где $F_t(x) = \frac{1}{\phi(t)}\int_{-\infty}^{x} \text{e}^{t u}d F(u)$ -- функция распределения (проверьте это).
Для того, чтобы оценить интеграл, рассмотрите случайные величины $\tilde{\xi}_1,\dots,\tilde{\xi}_n$ с распределением $F_{t_0}$, воспользуйтесь центральной предельной теоремой, чтобы показать, что $B_n\to1/2$ при ${n\to\infty}$.
\end{remark}



\begin{problem}
\label{chernov_th}
 Задана последовательность независимых одинаково распределенных случайных величин $\xi_1,\xi_2,\dots$ и $S_n = \xi_1+\dots+\xi_n$.
Показать, что в бернуллиевском случае ($\mathbb{P}\{\xi_1=1\} = p$, $\mathbb{P}\{\xi_1 = 0\}=1-p$) 
\begin{enumerate}
\item  при  $p<x<1$
\begin{equation*}
\lim\frac{1}{n}\ln\mathbb{P}\{S_n\geq nx\} = -H(x),
\end{equation*}
\begin{equation*}
H(x) = x\ln \frac{x}{p}+(1-x)\ln\frac{1-x}{1-p};
\end{equation*}
\item при $x_n = n(x-p)$ и при  $p<x<1$
\begin{equation*}
\mathbb{P}\{S_n\geq np+x_n\}=\exp\biggl\{-nH\biggl(p+\frac{x_n}{n}\biggr)(1+o(1))\biggr\};
\end{equation*}
\item при $x_n = a_n\sqrt{np(1-p)}$ c $a_n\to\infty$, $\frac{a_n}{\sqrt{n}}\to 0$
\begin{equation*}
\mathbb{P}\{S_n\geq np+x_n\}  = \exp\biggl\{-\frac{x_n^2}{2np(1-p)}(1+o(1))\biggr\}.
\end{equation*}

\item Обобщите предыдущие три пункта на случай, когда вместо $\frac{S_n}{n}$ под знаком вероятности будет стоять $\underset{k\geq n}{\sup}\frac{S_k}{k}$.

\end{enumerate}
\end{problem}
\begin{ordre}
Для доказательства первого пункта используйте следующий результат (теорема Чернова). Пусть $S_n = \sum_{i=1}^n\xi_i$, где $\xi_i$, $i=1,\dots,n$ независимые одинаково распределенные простые случайные величины с 
$$
\mathbb{E}\xi_1\leq 0 \quad \text{и} \quad \mathbb{P}\{\xi_1>0\}>0
,
$$
$$
\inf_{\lambda}\phi(\lambda)=\rho,\quad 0<\rho<1, \quad \phi(\lambda) = \mathbb{E}\text{e}^{\lambda\xi_1}.
$$
Тогда
\begin{equation*}
\lim\frac{1}{n}\ln\mathbb{P}\{S_n\geq 0\} \to \ln\rho\quad \text{при~}n\to\infty.
\end{equation*}
\end{ordre}



\begin{problem} %\begin{enumerate} 
%\item 
\label{KL_EF}
а) Сравнить оценки вероятности отклонений выборочного среднего от теоретического среднего для последовательности одинаково распределенных случайных величин $\xi_1,\dots,\xi_n$ с распределением Бернулли с вероятностью успеха $p$ (не предполагая равномерную отделимость $p$ от нуля, в частности, допуская $p = \lambda/n$, где $\lambda$ постоянна), получаемые с помощью неравенства Хёфдинга, Бернштейна, Спокойного, Буске и неравенства больших уклонений из предыдущих задач.
%\item 

б) В некотором городе прошел второй тур выборов. Выбор был между двумя кандидатами $A$ и $B$ (графы <<против всех>> на этих выборах не было). 
Сколько человек надо опросить на выходе с избирательных участков, чтобы исходя из ответов можно было определить долю проголосовавших 
за кандидата $A$ с точностью $5\%$ и с вероятностью не меньшей $0.99$. %Считайте, что исходя из голосования в первом туре, известно, 
%что каждый из кандидатов наберет не меньше $30\%$ голосов избирателей. 
%
Какой способ решения является более точным: с помощью использования центральной предельной теоремы и неравенства Берри-Эссеена или полученный с использованием неравенств концентрации меры, больших уклонений (см. задачи выше в разделе, неравенства Спокойного, Буске, Бернштейна)?
%\end{enumerate}
\end{problem}
\begin{remark}
{\it Неравенство О. Буске.}
Пусть $X_1,\dots,X_n$ -- последовательность независимых случайных величин с распределением $\PR$, принимающих значения из полного сепарабельного метрического пространства $\mathcal{X}$. Пусть $Z = f(X_1,\dots,X_n)$, где $f:\mathcal{X}^n\to \mathbb{R}$ измеримая функция, обозначим $Z_i = f(X_1,\dots,X_{i-1},X_{i+1},\dots,X_n)$. 

Пусть $Z$ удовлетворяет
$$
\sum_{i=1}^k(Z-Z_k)\leq Z
$$
и существуют такие случайные величины $Y_i$, что 
$$
Y_i\leq Z-Z_i\leq 1,\quad Y_i\leq a\,\, \text{п.н.}
$$
для некоторого $a>0$ и $\mathbb{E}_iY_i \geq 0$, где $\mathbb{E}_iX = \mathbb{E}_i[X|X_1,\dots,X_{i-1},X_{i+1},X_n]$.
Также пусть существует $\sigma,$ такое что п.н. $\sigma^2\geq \frac 1n \mathbb{E}_i Y_i^2$.


%Пусть $\mathcal{F}$ -- счетное семейство функций из $\mathcal{X}$ в $\mathbb{R}$. Предположим, что функции $f$ из $\mathcal{F}$ являются $\PR$-измеримыми, интегрируемыми в квадрате и  удовлетворяют $\mathbb{E}[f(X)]=0$. Если $\sup_{f\in\mathcal{F}}\mathrm{ess}\sup f(x)\leq 1$ тогда обозначим
%\begin{equation*}
%Z = \sup_{f\in\mathcal{F}}\sum_{i=1}^n f(X_i),
%\end{equation*}
%если же $\sup_{f\in\mathcal{F}}\|f\|_{\infty}\leq 1$, то
%\begin{equation*}
%Z = \sup_{f\in\mathcal{F}}\biggl|\sum_{i=1}^n f(X_i)\biggr|.
%\end{equation*}
Тогда для всех $x\geq 0 $ верно
\begin{equation*}
\PR[Z\geq \mathbb{E}[Z]+x]\leq \exp\biggl(-vh\biggl(\frac{x}{v}\biggr)\biggr)
\end{equation*}
при    $v = n\sigma^2+ (1+a)\mathbb{E}[Z]$ и $h(x)=(1+x)\ln(1+x)-x$, а также
\begin{equation*}
\PR\biggl[Z\geq \mathbb{E}[Z]+\sqrt{2vx}+\frac{x}{3}\biggr]\leq \exp(-x).
\end{equation*}

\medskip

См. также книгу St

==> standart/bayes.tex <==
\section{Байесовские методы}
\label{bayes}

\begin{problem}
Охранная система представлена в виде Байесовской модели, изображенной на Рис. \ref{Fig:bayes1.png}. 
\imgh{50mm}{bayes1.png}{Модель охранной системы.}
Пусть $t$ обозначает факт срабатывания тревоги, $v$ -- наличие вора $\in \text{Be}(s)$, $e$ -- было ли землетрясение, $r$ -- наличие радиосообщения. Величины $t$, $v$, $e$, $r$ имеют распределение Бернулли. Переменная $s$ -- статистика по криминогенной активности -- принимает значения из отрезка [0, 1]. Значения $\PR(t = 1|v,e)$, $\PR(r = 1|e)$, $\PR(e = 1)$ и $\PR(v = 1)$ заданы, причем $\PR(t = 1|v=0,e=0) = 0$, $\PR(r = 1|e = 0) = 0$.
Проведите расчет $\PR(v = 1|t = 1, s = s_0)$ и $\PR(v = 1 | t = 1, s=s_0, r = 1)$. 
\end{problem}

\begin{remark}
Генеративные вероятностные модели часто представляются в виде интуитивно понятных  \textit{графических моделей}. Графическая модель -- это граф, определяющий зависимости между случайными величинами. Вершинам соответствуют случайные величины, ребрам -- зависимости между ними.

Наблюдаемые величины (значения которых известны) закрашиваются, скрытые (значения которых надо найти) -- остаются незакрашенными. Стрелка из вершины $A$ в $B$  обозначает зависимость $B$ от $A$ (часто под такого рода зависимостью подразумевается, что $A$ является параметрами распределения с.в. $B$).

Для обозначения повторяющихся величин с одинаковым распределением используются прямоугольники, которые могут быть вложенными. В одном из углов прямоугольника обычно указывается количество повторений случайных величин, расположенных внутри него. 

\end{remark}

\begin{problem}
Радиоактивный источник излучает за одну секунду $n \in \Po(s)$ частиц, где $s$ -- неизвестная интенсивность излучения. Прибор, регистрирующий частицы, имеет погрешность $\theta = 0.9$, т.е. количество зарегистрированных частиц за одну секунду $c \in \mathrm{Bin}(\theta,n)$. Покажите, что 
\[
\PR(c|\theta,s) = \Po(s\theta),
\]
\[
\PR(n-c|c,\theta,s) = \Po(s(1-\theta)). 
\]
Предположим, что за первую секунду прибор зарегистрировал $c_1 = 10$ частиц, а за вторую -- $c_2 = 16$ частиц (см. Рис. \ref{Fig:bayes3.png}). Докажите формулы для условного распределения и математического ожидания $n_1$: 
\[
\PR(n_1 | c_1, c_2, \theta, s) = \int_{0}^{\infty} p(n_1|c_1,\theta,s) p(s|c_1,c_2,\theta) ds = 
\]
\[
= C_{n_1+c_2}^{c_1+c_2} \left(\frac{2\theta}{1+\theta}\right)^{c_1+c_2+1} \left(\frac{1-\theta}{1+\theta}\right)^{n_1 - c_1},  
\]
\[
\Exp(n_1 | c_1, c_2, \theta, s) = \frac{c_1 + c_2 + 1 - \theta}{2\theta} + \frac{c_1 - c_2}{2} = 131.5.
\]
Найдите 90\% доверительный интервал для $n_1 | c_1, c_2, \theta, s$, воспользовавшись соотношением
\[
\PR(|X - \Exp X| > t \sqrt{\Var X}) \leq \frac{1}{t^2}.
\]
\imgh{60mm}{bayes3.png}{Модель радиоактивного источника.}
\end{problem}


\begin{problem}[Распределение Дирихле]
\label{dir}

Ознакомьтесь с распределениями Дирихле, бета и гамма, приведенными в замечании. Покажите, что если $(X_1, \ldots, X_k)$, $X_i \in \text{Г}( \gamma_i, 1)$ -- гамма распределенные независимые с.в. и $S = \sum \limits_{i=1}^k X_i$, то 
\[\tag{1}
(X_1 / S , \ldots, X_k / S) \in \mathrm{Dir}(\gamma_1, \ldots, \gamma_{k}).
\] 
Предложите способ генерации вектора с распределением Дирихле ($\gamma_i \in \mathbb{N}$), имея в распоряжении генератор с.в. с равномерным распределением на отрезке $[0, 1]$. 

Покажите, что каждая компонента вектора с распределением Дирихле имеет бета-распределение $X_i/S \in \mathrm{Beta}(\gamma_i, \sum \limits_{j \neq i} \gamma_j)$. 

Положим, что вектор $(\theta_1,\ldots,\theta_k)$ априорно имеет распределение (1), выборка $Y_1,\ldots, Y_n$ сгенерирована из дискретного распределения $\mathrm{Cat}(\theta_1,\ldots,\theta_k)$, т.е. $\PR(Y_i = m | \theta_1,\ldots,\theta_k) = \theta_m$. Докажите справедливость формулы для плотности апостериорного распределения $\theta_1,\ldots,\theta_k$: 
\[
p(\theta_1,\ldots,\theta_k \vert Y_1,\ldots, Y_n, \gamma_1, \ldots, \gamma_{k}) = 
\]
\[
=\mathrm{Dir}\left(\gamma_1 + \sum_{i=1}^n \delta_1(Y_i), \ldots, \gamma_{k}+ \sum_{i=1}^n \delta_k(Y_i)\right),
\]
где $\delta_k(x) = [x = k]$.
Убедитесь, что данная функция принимает максимальное значение при 
\[\tag{2}
\theta_m \propto \gamma_m - 1 + \sum_{i=1}^n \delta_m(Y_i).
\]

\end{problem}

\begin{remark}

Говорят, что вектор $X$ принадлежит распределению \textit{Дирихле} $\mathrm{Dir}(\gamma_1, \ldots, \gamma_{k})$, если: 
\[
f_{X}(x_1, \ldots, x_k) = \frac{\text{Г}(\gamma_1 +  \ldots + \gamma_{k})}{\text{Г}(\gamma_1)  \ldots  \text{Г}(\gamma_{k})} x_1^{\gamma_1-1} \ldots x_k^{\gamma_k-1},
\] 
\noindent где  $(x_1, \ldots, x_k) \in \{x_i \geq 0, \; \sum x_i  = 1 \}$, $\gamma_i \geq 0$, $\text{Г}$ -- гамма функция. 

Говорят, что вектор $X$ принадлежит \textit{бета} распределению \\  $\mathrm{Beta}(\gamma_1, \gamma_2)$, если: 

\begin{center}
$f_{X}(x) = \frac{\text{Г}(\gamma_1 + \gamma_2)}{\text{Г}(\gamma_1) \text{Г}(\gamma_2)} x^{\gamma_1-1} (1 - x)^{\gamma_2-1}$, где  $x \in [0, 1]$.
\end{center} 


Допускается также обозначение следующего вида \\ $ X \in \mathrm{Dir}(\gamma_1, \ldots, \gamma_{k+1})$, если 
\[
f_{X}(x_1, \ldots, x_k) = \frac{\text{Г}(\gamma_1 +  \ldots + \gamma_{k+1})}{\text{Г}(\gamma_1)  \ldots  \text{Г}(\gamma_{k+1})} x_1^{\gamma_1-1} \ldots x_k^{\gamma_k-1} (1 - x_1 - \ldots - x_k)^{\gamma_{k+1}-1},
\] 


\noindent где  $(x_1, \ldots, x_k) \in \{x_i \geq 0, \; \sum x_i \leq 1 \}$.

Говорят, что с.в. $X$ принадлежит \textit{гамма} распределению
\\  $\text{Г}(\alpha, \lambda)$, если: 
\begin{center}
$f_{X}(x) = \frac{x^{\alpha-1} e^{-x/\lambda}}{\lambda^\alpha\text{Г}(\alpha)}$,  где  $x \geq 0$.
\end{center}

Распределение Дирихле $\Dir(\gamma_1, \ldots, \gamma_{k})$ может быть интерпретировано следующим образом. Его функция плотности возвращает вероятность того, что вероятности $A_1,\ldots,A_K$ -- несовместных  событий равны соответственно $x_1, \ldots, x_K$, $\sum_i x_i = 1$ при условии, что $i$-е событие наблюдалось $\gamma_i-1$ раз. 

Отметим два свойства распределения Дирихле, делающего его удобным для использования в качестве априорного, при оценке параметров дискретного распределения (см. выражение (2)). Первое, семейство распределений Дирихле является сравнительно большим среди всех возможных распределений на симплексе, что является своего рода страховкой от неправильного выбора типа априорного распределения. Второе, имея выборку, сгенерированную из дискретного распределения, апостериорное распределение допускает простое аналитическое вычисление. 

Обратите внимание, что в выражении (2)  при $\gamma_i < 1$, $i = \overline{1,k}$ априорное распределение способствует разреживанию (увеличению количества нулевых компонент) $\theta_1,\ldots,\theta_k$, при  $\gamma_i = 1$, $i = \overline{1,k}$ априорное распределение является равномерным, а при  $\gamma_i > 1$, $i = \overline{1,k}$ распределение способствует сглаживанию $\theta_1,\ldots,\theta_k$.

Распределение Дирихле приобрело широкое практическое применение в области  тематического моделирования текстов (см. задачу \ref{sec:them_modeling}), машинного перевода, построения моделей в экологии, байесовской проверки гипотез, точечного оценивания и оценки доверительных интервалов. 
\end{remark}

\begin{problem}[Упорядоченное распределение Дирихле]
Пусть $X_{(k)}$ является $k$-ой порядковой статистикой в наборе $X_1, \ldots, X_n$ (*) случайных величин с функцией распределения $F_X(x)$. Пусть $U_k = F_X(X_{(k)}).$ Покажите, что $U \in \mathrm{Dir^*}(1, \ldots, 1)$ (см. замечание).

Сравните доказанное утверждение с задачей \ref{sec:ordered_seq} раздела \ref{standart}. 
Покажите, что если $\mathbb{P}(X \in [X_{(i-1)}, X_{(i)}]) = W_i = U_i - U_{i-1}$, где $X_{(0)} = -\infty$, $X_{(n+1)} = +\infty$, то 
$W \in \mathrm{Dir}(1, \ldots, 1)$.
 
Имея в распоряжении набор векторов (*), где $X_i \in \mathbb{R}^m$, эмпирическая оценка плотности распределения в точке $x$ может быть найдена следующим образом:
\[
\widehat{f}_X(x) = \frac{\mathbb{E}U_k}{V_{r_k}},
\]    
где $r_k$ -- расстояние от $x$ до $X_{(k)}$, $V_{r_k}$ -- объем шара радиуса $r_k$ в пространстве $\mathbb{R}^m$. Докажите, что  
\[
U_k \in \mathrm{Beta}(k, n-k+1), 
\]
\[
\widehat{f}_X(x) \xrightarrow{p} f_X(x), \quad
n \to \infty.
\]    


\end{problem}


\begin{remark}

Говорят, что вектор $Y$ принадлежит \textit{упорядоченному распределению Дирихле} $\mathrm{Dir^*}(\gamma_1, \ldots, \gamma_{k+1})$, если: 
\[
f_{Y}(y_1, \ldots, y_k) = \]
\[ \frac{\text{Г}(\gamma_1 +  \ldots + \gamma_{k+1})}{\text{Г}(\gamma_1)  \ldots  \text{Г}(\gamma_{k+1})} y_1^{\gamma_1-1}(y_2 - y_1)^{\gamma_2-1} \ldots (y_k - y_{k-1})^{\gamma_k-1} (1 - y_k)^{\gamma_{k+1}-1},
\] 

\noindent где  $(y_1, \ldots, y_k) \in \{ 0 \leq y_1 \leq \ldots \leq  y_k \leq 1 \}$, $\gamma_i \geq 0$.

Причем, если $X \in \mathrm{Dir}(\gamma_1, \ldots, \gamma_{k+1})$ и $Y_i = \sum \limits_{j=1}^{i} X_j$, $i = \overline{1,k}$ то 
\[
Y \in \mathrm{Dir^*}(\gamma_1, \ldots, \gamma_{k+1}).
\]

\end{remark}


\begin{problem} 
\label{po_dir}
Распределение Пуассона--Дирихле получается из упорядоченного вектора с распределением Дирихле предельным переходом, описанным в замечании. Докажите, что величины $\theta_{(i)}$ с вероятностью 1 убывают с экспоненциальной скоростью:
\[
\theta_{(i)} \propto e^{- i/\lambda}.
\]
Такое распределение часто возникает при моделировании разделения большого числа элементов из $S$ на большое число видов. Предположим, что из $S$, была произведена выборка размера $n$. Докажите, что вероятность того, что все элементы выборки имеют один и тот же вид равна
\[
\frac{\lambda \text{Г}(\lambda) \text{Г}(n) }{\text{Г}(\lambda+n)}.
\]
\end{problem}

\begin{remark}
Пусть $\theta_1,\ldots,\theta_n \in \mathrm{Dir}(\gamma_1,\ldots,\gamma_n)$, при этом
выполнены условия
\[
\max_i\gamma_i \to 0,
\quad n \to \infty,
\] 
\[
\lambda_n = \sum_{i=1}^n \gamma_i \to \lambda. 
\]
Введем обозначения
\[
s_0 = 0, \quad s_j = \gamma_1 + \ldots + \gamma_j, \quad j = \overline{1,n}.
\]
Распределение Дирихле может быть сконструировано из $Y_i \in \text{Г}(\gamma_i, 1)$ по правилу $\theta_i = Y_i/\sum_j Y_j$. Известно, что $Y_i$ безгранично делимы, т.е. могут быть разбиты на сколь угодно большое число гамма распределенных случайных величин $Y_{i1},\ldots,Y_{ip}$. Частичные суммы величин $\sum_j Y_j$ приближаются в пределе к случайному процессу с независимыми приращениями $g$: 
\[
g(s_m) = \sum_{i=1}^{m} Y_i, \quad \theta_j = \frac{g(s_j) - g(s_{j-1})}{g(s_n)}. 
\]       
Из вида характеристической функции 
\[
\phi_{g(s)}(\mu) = \exp \left(  
-s \int_{0}^{\infty} \left(1 - e^{-\mu z} \right) \frac{e^{-z}}{z} dz
\right)
\]
\[
\gamma(dz) = \frac{e^{-z}}{z} dz
\]
заключаем, что $g(s)$ является субординатором на множестве $s \in [0, \lambda]$ (см. задачу \ref{subord} из раздела \ref{geom}). Величины скачков процесса $g(s)$ образуют пуассоновский процесс $J(t)$ на множестве $t \in (0, \infty)$ c переменной интенсивностью
\[
\lambda(z) = \lambda \frac{e^{-z}}{z}.
\]   
Обозначим за $J_{(1)} \geq J_{(2)} \geq J_{(3)} \geq \ldots$ упорядоченные величины скачков. Последовательность $\theta_{(1)} \geq \theta_{(2)} \geq \theta_{(3)} \geq \ldots$, где 
\[
\theta_{(i)}  = \frac{J_{(i)}}{g(\lambda)},
\]
имеет распределение \textit{Пуассона--Дирихле}.

\end{remark}

\begin{problem}[Сопряженные распределения]
\label{bayes_def}
Сформулируем задачу байесовского вывода. Пусть известно распределение $p(X|\theta)$ (\textit{правдоподобие выборки} $X$). Требуется найти: 
\begin{enumerate}
\item $p(\theta|X) = \frac{p(X|\theta)p(\theta)}{p(X)}$ -- апостериорное распределение;
\item $p(x'|X) = \int_\Theta p(x'|\theta)p(\theta|X) d\theta$ -- предсказание нового $x'$.
\end{enumerate} 

Ключевым моментом является выбор наиболее разумного $p(\theta)$ -- \textit{априорного распределения}. Выбор осуществляется, исходя из дополнительной информации о параметре $\theta$ и необходимости введения регуляризации (отдание предпочтения более простым функциям $p(X | \theta)$, которые могут быть построены более точно при ограниченном размере выборки $|X|$). 

Решение  задач Байесовского вывода существенно упрощается при использовании \textit{сопряженных семейств} распределений (см. М. Де Гроот. Оптимальные статистические решения. -- М.: Мир, 1974).  Семейство распределений $\lbrace p(\theta|\alpha), \; \alpha \in \Omega \rbrace$ называется \textit{сопряженным} к семейству правдоподобий $\lbrace p(X|\theta) , \; \theta \in \Theta \rbrace$, если $\forall 
\alpha \; \exists \alpha'$ такой, что апостериорное распределение $p(\theta|X, \alpha) = p(\theta|\alpha')$ (т.е.  апостериорное распределение имеет такой же вид, что и априорное, но с другими параметрами). Именно  сопряженное распределение разумно взять в качестве априорного, что, в частности, упростит вычисление нормировочного интеграла: 
\[
p(X) = \int \limits_{\theta} p(X|\theta)p(\theta) d \theta.
\] 
 

Рассмотрим несколько примеров сопряженных семейств. Покажите, что:

\begin{enumerate}
\item Сопряженным к распределению Бернулли является \textit{бета}  распределение (см. замечание к задаче \ref{dir}).
Если $x_1, \ldots, x_n$ -- реализация выборки из распределения Бернулли, 
априорное распределение есть $\mathrm{Beta}(\alpha, \beta)$, то апостериорное распределение будет иметь параметры:
\[
\alpha + \sum \limits_{i = 1}^n x_i,  \; \; \beta + n - \sum \limits_{i = 1}^n x_i.  
\]


\item Пусть $x_1, \ldots, x_n$ -- реализация одного элемента выборки из мультиномиального  распределения с неизвестным вектором параметров $\theta$ длины $n$. Допустим, что  априорное распределение  $\theta$ есть распределение Дирихле (см. замечание к задаче \ref{dir}) $\mathrm{Dir}(\alpha_1, \ldots, \alpha_n)$. Тогда апостериорное распределение есть  $\mathrm{Dir}(\alpha_1 + x_1, \ldots, \alpha_n + x_n)$.  

\item Если $x_1, \ldots, x_n$ -- реализация выборки из распределения Пуассона с неизвестным значением среднего $\theta$, 
априорное распределение есть гамма-распределение  $\text{Г}(\alpha, \beta)$, то апостериорное распределение будет иметь параметры:
\[
\alpha + \sum \limits_{i = 1}^n x_i,  \; \; \beta + n.  
\]

\item Если $x_1, \ldots, x_n$ -- реализация выборки из экспоненциального распределения  с неизвестным параметром $\theta$, 
априорное распределение есть гамма-распределение  $\text{Г}(\alpha, \beta)$, то апостериорное распределение будет иметь параметры:
\[
\alpha + n,  \; \; \beta + \sum \limits_{i = 1}^n x_i.  
\]


\item Если $x_1, \ldots, x_n$ -- реализация выборки из нормального распределения  с неизвестным  значением среднего $m$ и заданной мерой точности $r = 1/\sigma^2$, 
априорное распределение $m$ есть  $N(\mu, 1/\tau)$, то апостериорное распределение есть $N(\mu', 1/\tau')$, где:
\[
\mu' = \frac{\tau \mu + n r \overline{x}}{\tau + n r},  \; \; 
\tau' = \tau + n r.  
\]

\item Если $x_1, \ldots, x_n$ -- реализация выборки из нормального распределения  c заданным  значением среднего  $m$ и неизвестной мерой точности $r = 1/\sigma^2$. Пусть априорное распределение  $r$ есть гамма-распределение  $\text{Г}(\alpha, \beta)$. Тогда апостериорное распределение будет иметь параметры:
\[
\alpha + \frac{n}{2},  \; \; \beta + \frac{1}{2} \sum \limits_{i = 1}^n (x_i - m)^2.  
\]

\item Если $x_1, \ldots, x_n$ -- реализация выборки из нормального распределения  c неизвестным значением среднего  $m$ и неизвестной мерой точности $r = 1/\sigma^2$ (см. Рис. \ref{Fig:model.pdf}). Пусть условное априорное распределение $m$ при фиксированном $r$ есть  $N(\mu, 1/(\tau r) )$; априорное распределение  $r$ есть гамма-распределение  $\text{Г}(\alpha, \beta)$. Тогда апостериорное совместное распределение $m$ и $r$ имеет  следующий вид:
\[
m \vert r \in N \left( \frac{\tau \mu + n \overline{x}}{\tau + n}, (\tau + n) r  \right),  
\]
\[
r \in \text{Г} \left( \alpha + \frac{n}{2}, \beta + \frac{1}{2} \sum \limits_{i = 1}^n (x_i - \overline{x})^2 + \frac{1}{2} \frac{\tau n (\overline{x} - \mu)^2}{\tau + n} \right),
\]
\[
p(m, r | X, \mu, \tau, \alpha, \beta) = \const \cdot p(r | \alpha, \beta) p(m | r, \mu, \tau) p(X | m, r) =
\]
\[
p(m| r, X, \mu, \tau) p(r | X, \mu, \tau, \alpha, \beta).
\]

\imgh{80mm}{model.pdf}{Графическая модель генерации выборки из нормального распределения с неизвестными параметрами.}

\end{enumerate} 

\end{problem}



\begin{problem}[Экспоненциальное семейство распределений]
\label{EF}
Многие стандартные распределения принадлежат экспоненциальному семейству (см. замечание), например, нормальное, гамма, бета, Бернулли, Дирихле. 
Пусть с.в. $Y \in EF$. Докажите следующие свойства $EF$:

\[
\varphi_{T(x)}(t) = \Exp e^{\langle t, T(x) \rangle} = \frac{Z(\theta + t)}{Z(\theta)};
\]
\[
\nabla \log Z(\theta) = \Exp T(x);
\quad
\nabla^2 \log Z(\theta) = \cov (T(x), T(x));
\]
для выборки $X_1,\ldots,X_n \in p(x|\theta)$ оценка максимума правдоподобия может быть представлена как 
\[
\nabla \log Z(\widehat{\theta}_{ML}) = \frac{1}{n} \sum_{i=1}^{n} T(X_i);
\]
\[
\mathcal{KL}(\nu_2 \Vert \nu_1) = \nabla d(\nu_2) (\nu_2 - \nu_1) - [d(\nu_2) - d(\nu_1)];
\]
сопряженное распределение (см. задачу \ref{bayes_def}) на параметры $\theta$ может быть вычислено по формуле
\[
p(\theta | \alpha_1, \alpha_2) \propto e^{ \langle \theta, \alpha_1 \rangle - \alpha_2 \log Z(\theta)}.
\]

\end{problem}

\begin{remark}
C.в. $X \in EF$, если ее плотность распределения имеет следующий вид (canonical   parametrization):
\[
p(x | \nu) = h(x)e^{\langle x, \nu \rangle - d(\nu)}. 
\]
Возможно также другое представление:
\[
p(x | \theta) = \frac{h(x)}{Z(\theta)} e^{ \langle \theta, T(x) \rangle}, 
\]
где $T(x)$ -- \textit{достаточная статистика} распределения $p(x | \theta)$.
\end{remark}


\begin{problem}[Процесс Дирихле]
\label{DP}
Рассмотрим графическую модель разделения смеси распределений (mixture model). Предполагается, что каждый элемент выборки $X = \{x_1, \ldots, x_n\}$ имеет скрытую компоненту из вектора $Z = \{z_1, \ldots, z_n\}$, обозначающую компоненту смеси, к которой относится элемент. Процесс генерации выборки устроен таким образом (см. Рис. \ref{Fig:DP.pdf}):
генерируется априорное дискретное распределение компонент смеси $(\pi_1, \ldots, \pi_K) \in \mathrm{Dir}(\alpha/K, \ldots, \alpha/K)$; в таком случае $\PR(z_i = m) = \pi_m$; $j$-я ($j \in \overline{1,K}$) компонента смеси имеет параметры $\theta_j$, которые сгенерированы из произвольного распределения $F(\lambda)$; $x_i$ генерируется из распределения $i$-й компоненты с параметрами $\theta_i$. 

Как правило, в таких задачах требуется оценить скрытые переменные $Z$, $\pi$, $\theta$ по известной выборке $X = \{x_1, \ldots, x_n\}$ и заданных значениях параметров $\alpha$, $\lambda$. 

\imgh{60mm}{DP.pdf}{Dirichlet Process Mixture Model.}

В случае, когда $K$ -- число компонент дискретного распределения не задано, вместо распределения Дирихле для конечного $K$ уместно воспользоваться процессом Дирихле DP, где $K = \infty$ (см. замечание).    

Пусть $\theta_1, \ldots, \theta_{n+1}$ -- независимые случайные величины, у которых распределение является случайной мерой $G \in \mathrm{DP}(H, \alpha)$, $A \subset \Theta$. Докажите, что
\[
\PR(\theta_{n+1} \in A | \theta_1, \ldots, \theta_n) = \frac{1}{n+\alpha}\left(\alpha H(A) + \sum \limits_{i=1}^{n} \delta_{\theta_i}(A) \right),
\]
Пусть $m$ -- число уникальных величин среди $\theta_1, \ldots, \theta_n$. Докажите следующие выражения:
\[
\Exp(m | n) = \alpha (\psi(n + \alpha)  - \psi(\alpha)) \simeq \alpha \ln \left(1 + \frac{n}{\alpha} \right) \quad \text{при} \; \alpha, n \gg 0,
\]
\[
\Var(m | n) = \alpha (\psi(n + \alpha)  - \psi(\alpha)) + \alpha^2 (\psi'(n + \alpha)  - \psi'(\alpha)) \simeq \]\[ \alpha \ln \left(1 + \frac{n}{\alpha} \right) \quad \text{при} \; n > \alpha \gg 0,
\]
где $\psi(x) = \frac{\text{Г'(x)}}{\text{Г(x)}}$ -- digamma функция.
\end{problem}

\begin{remark}
Пусть $H$ -- некоторое распределение с носителем $\Theta$, $\alpha$ -- положительное число. $G$, случайная вероятностная мера (распределение), называется   \textit{процессом Дирихле} $\mathrm{DP}(H, \alpha)$ с базовым распределением $H$ и параметром концентрации $\alpha$, если для любого конечного измеримого разбиения пространства элементарных исходов $\Theta$: $A_1, \ldots, A_r$ выполнено
\[
(G(A_1), \ldots, G(A_r)) \in \mathrm{Dir}(\alpha H(A_1), \ldots, \alpha H(A_r)).
\]

Процесс Дирихле обладает следующими свойствами:
\begin{enumerate}
\item $\forall A \subset \Theta$: $\Exp \left[G(A)\right] = H(A)$;
\item $\forall A \subset \Theta$: $\Var \left[G(A)\right] = \frac{H(A)(1-H(A))}{\alpha+1}$;
\item Пусть $\theta_1, \ldots, \theta_n$ -- независимые случайные величины со случайным распределением $G \in \mathrm{DP}(H, \alpha)$, тогда
\[
\PR(G(A_1), \ldots, G(A_r) | \theta_1, \ldots, \theta_n) \in \mathrm{Dir}(\alpha H(A_1) + n_1, \ldots, \alpha H(A_r) + n_r),
\]
где $n_j = | i: \theta_i \in A_j |$. 
Что также можно записать в другом виде:
\[
G | \theta_1, \ldots, \theta_n \in \mathrm{DP} \left(\alpha + n, \frac{\alpha}{\alpha+n} H + \frac{n}{\alpha+n} \cdot \frac{\sum \delta_{\theta_i}}{n} \right),
\]
где $\frac{\sum \delta_{\theta_i}}{n}$ -- смесь распределений $\delta_{\theta_1}, \ldots, \delta_{\theta_n}$, в котором $\PR(\theta = \theta_i) = 1$ при $\theta \in \delta_{\theta_i}$.   
\end{enumerate}

\end{remark}

\begin{problem}[Stick-breaking construction]
\label{stick}

Рассмотрим альтернативное определение процесса Дирихле (см. замечание к задаче \ref{DP}). Пусть $J_k$ -- $k$-й по счету скачек гамма процесса $g(s)$, $s \in [0,\alpha]$ (см. замечание к задаче \ref{po_dir}), нормированное значение скачка обозначим как $\pi_k = J_k/g(\alpha)$. Введем также последовательность с.в. $v_k: \Theta \to \Theta$ с вероятностной мерой $H: \mathcal{B}(\Theta) \to [0,1]$, где $\mathcal{B}(\Theta)$ -- все измеримые подмножества $\Theta$. Докажите, что случайная мера $G: \mathcal{B}(\Theta) \to [0,1]$, такая что
\[
\forall A \in \mathcal{B}(\Theta): \; G(A) = \sum_{k = 1}^{\infty} \pi_k \delta_{v_k}(A),
\]
является процессом Дирихле $DP(H, \alpha)$.

Для программной реализации процесса Дирихле, как правило, используется генеративная модель ``ломания палки'':
\[
\beta_k \in \mathrm{Beta}(\alpha, 1),
\quad
\pi_k = \beta_k \prod \limits_{l=1}^{k-1} (1-\beta_l), 
\quad
\theta_k \in F(\lambda) = H,
\]
\[
G \in \sum \limits_{k = 1}^{\infty} \pi_k \delta_{\theta_k}.
\]
Докажите, что $G \in \mathrm{DP}(H, \alpha)$.

\end{problem}

\begin{ordre}
См. статью T. Ferguson. A Bayesian analysis of some nonparametric problems. 1973. 
\end{ordre}

\begin{problem}
Для процесса Дирихле $G \in DP(H, \alpha)$ (см. альтернативное определение в задаче \ref{stick}) и измеримой функции $Z: \Theta \to \mathbb{R}$ докажите справедливость следующего утверждения. Если $\int_{\Theta} |Z(\theta)| dH (\theta) < \infty$, то с вероятностью единица 
$\int_{\Theta} |Z(\theta)| dG (\theta) < \infty$ и 
\[
\Exp \int_{\Theta} Z(\theta) dG (\theta)  = \int_{\Theta} Z(\theta) d \Exp G (\theta) =  \int_{\Theta} Z(\theta) dH (\theta).
\]
\end{problem}

\begin{problem}
\label{Fx_bayes}
Требуется по выборке $X_1,\ldots,X_n \in \mathbb{R}$ оценить функцию распределения $F_X(t)$. Априорно предполагается, что $F_X$ соответствует вероятностной мере $H: \mathcal{\mathbb{R}} \to [0,1]$. Предлагается оценивать функцию $F_X$ как 
\[
\widehat{F}_X(t) = \Exp G((-\infty, t) | X_1,\ldots,X_n),
\]
где $G((-\infty, t) | X_1,\ldots,X_n)$ -- с.в., соответствующая условной случайной мере $G | X_1,\ldots,X_n$ (см. замечание к задаче \ref{DP}).
Покажите, что
\[
\widehat{F}_X(t) = \frac{\alpha}{\alpha+n} H((-\infty, t)) + \frac{n}{\alpha+n}\frac{1}{n} \sum_{i=1}^{n} [X_i < t].
\]
Аналогично, для оценки $\Exp X$ предлагается использовать оценку
\[
\widehat{m}_X = \Exp \int_{-\infty}^{+\infty} x dG(x).
\]
Покажите, что
\[
\widehat{m}_X = \frac{\alpha}{\alpha+n} \Exp_{H} X + \frac{n}{\alpha+n}\frac{1}{n} \sum_{i=1}^{n} X_i.
\]

\end{problem}


\begin{problem}
Требуется по выборкам $X_1,\ldots,X_n \in \mathbb{R}$ и $Y_1,\ldots,Y_m \in \mathbb{R}$ оценить вероятность
\[
\bigtriangleup = \PR(X_1 < Y_1) = \int_{-\infty}^{+\infty} F_X(t)dF_Y(t).
\]
Априорно предполагается, что $F_X$ соответствует вероятностной мере $H_X: \mathcal{\mathbb{R}} \to [0,1]$, $F_Y$ -- вероятностной мере $H_Y$. Предлагается оценивать $\bigtriangleup$ как (см. задачу \ref{Fx_bayes}) 
\[
\widehat{\bigtriangleup} = \int_{-\infty}^{+\infty} \widehat{F}_X(t)d\widehat{F}_Y(t).
\]
Покажите, что
\[
\widehat{\bigtriangleup} = p_x p_y \bigtriangleup_0 + p_x(1-p_y)\frac{1}{m} \sum_{i=1}^m H_X(Y_i) + (1-p_x)p_y\frac{1}{n} \sum_{i=1}^n H_Y(X_i) + 
\]
\[
+(1-p_x)(1-p_y) \frac{1}{m n} \sum_{i,j} [X_i < Y_i],
\]
где
\[
p_x = \frac{\alpha_x}{\alpha_x+n},
\quad
p_y = \frac{\alpha_y}{\alpha_y+m},
\quad
\bigtriangleup_0 = \int_{-\infty}^{+\infty} H_X(t)dH_Y(t).
\]
\end{problem}

\begin{problem}[Вариационный вывод для DP]
Для поиска максимума функции правдоподобия $\log p(X | Z, \theta, \pi, \alpha, \lambda)$ в задаче \ref{DP} можно воспользоваться вариационным выводом (см. задачу \ref{varinf} из раздела \ref{CS}), введя более простую параметрическую модель распределения скрытых переменных $q(Z, \theta, \pi)$ и приближая $q(Z, \theta, \pi)$ к $p(Z, \theta, \pi| X, \alpha, \lambda)$ в смысле расстояния $\KL(q \Vert p)$.   

Приведем генеративную модель из задачи \ref{DP}, в которой в качестве процесса Дирихле используется Stick-breaking construction (см. задачу \ref{stick}), а также конкретный пример распределения $F(\lambda) = \mathrm{Dir}(\lambda_1,\ldots,\lambda_M)$: 
\[
\beta_k \in \mathrm{Beta}(\alpha, 1),
\;
\pi_k = \beta_k \prod \limits_{l=1}^{k-1} (1 - \beta_l), 
\;
z_i \in \mathrm{Cat}(\pi),
\;
\theta_k \in \mathrm{Dir}(\lambda_1,\ldots,\lambda_M),
\]
\[
\beta = \Vert \beta_k \Vert_{K \times 1}, \quad
Z = \Vert z_i \Vert_{n \times 1}, \quad
\theta = \Vert \theta_{km} \Vert_{K \times M}.
\]


В качестве примера распределения $x$ в каждой из компонент смеси расмматривается дискретное распределение с параметрами $\theta_k$, т.е.
\[
x_i|z_i \in \mathrm{Cat}(\theta_{z_i}) \quad 
\Leftrightarrow 
\quad
\PR(x_i = m | z_i = k) = \theta_{k m},  
\]
\[
m = \overline{1,M}, \quad k = \overline{1,K}, \quad
i = \overline{1,n}.
\]
Будем искать $q(Z, \beta, \theta)$ в следующем факторизованном виде
\[
q(Z, \beta, \theta) = \prod \limits_{k=1}^K q(\beta_k | \gamma_k) \prod \limits_{k=1}^K q(\theta_k | \tau_k) \prod \limits_{i=1}^n q(z_i | \phi_i),
\]
$\gamma_k$ -- Beta параметры для распределений с.в. $\beta_k$, $\tau_k$ -- параметры распределения $F$ аналогичные $\lambda$, $\phi_i$ -- параметры дискретного распределения с.в. $z_i$, $K \sim \alpha \ln n$. 
Покажите, что параметры $q$, соответствующие минимуму $\KL(q \Vert p)$, удовлетворяет следующей системе уравнений:
\[
\gamma_{k1} = \alpha + \sum_{i = 1}^n q(z_i = k), \quad
\gamma_{k2} = 1 + \sum_{i = 1}^n q(z_i > k), 
\]
\[
\tau_{km} = \lambda_m + \sum_{i = 1}^n [x_i = m] q(z_i = k),
\]
\[
\phi_{ik} \propto \exp \left( \Exp_q \log (\beta_k) + \sum_{l < k} \Exp_q \log (1 - \beta_l) + \sum_{i = 1}^n \Exp_q \log (\theta_{kx_i}) 
\right),
\]
где
$$
q(z_i = k) = \phi_{i,k}, \quad q(z_i > k) = \sum \limits_{j = k+1}^K \phi_{i,j},
$$
$$
\Exp_q \log (\beta_k) = \psi(\gamma_{k1}) - \psi(\gamma_{k1} + \gamma_{k2}), 
$$
$$
\Exp_q \log (1- \beta_k) = \psi(\gamma_{k2}) - \psi(\gamma_{k1} + \gamma_{k2}), 
$$
$$
\Exp_q \log (\theta_{km}) = \psi(\tau_{km}) - \psi\left(\sum_{j}\tau_{kj}\right). 
$$

\end{problem}






\begin{problem}[Тематическое моделирование]
\label{sec:them_modeling}
Вероятностная тематическая модель представляет собой средство для выявления тем в коллекции текстовых документов, описывая каждую тему $z \in Z$ дискретным распределением на множестве терминов $W$, a каждый документ $d \in D$  — дискретным распределением на множестве тем. Предполагается, что порядок терминов в документах не важен, и коллекция является  выборкой из дискретного распределения $\PR(d, w, z)$, где  $\Omega = D \times W \times Z$,  $z$ -- скрытая переменная темы термина $w$ в документе $d$. Коллекция представляется матрицей частот $F  
 = \Vert \widehat{p}_{wd} \Vert_{W\times D}$. Предполагается также, что
\[
\PR(d, w, z) = \PR(w|d,z)\PR(z|d)\PR(d) = \PR(w|z)\PR(z|d)  \PR(d) 
= \phi_{wz} \theta_{zd} \; \PR(d), 
\]  
\[
 \PR(d, w) = \PR(d) \sum_z \phi_{wz} \theta_{zd} . 
\]
Обозначим за $n_{dw}$ число слов $w$ в документе $d$.
Поиск максимума правдоподобия модели для заданной выборки $X = \{(d,w, n_{dw}): d \in D, w \in W\}$  
\[
 L(\Phi, \Theta) = \log  \prod_{d,w} \bigg[\PR(d, w)\bigg]^{n_{dw}}
\] 
 равносилен минимизации расстояния $\mathcal{KL}(F \Vert \Phi \Theta)$, где стохастическое матричное разложение $\Phi \Theta$ не единственно и определено с точностью до невырожденного преобразования $\Phi S^{-1}  S \Theta$.
Ввиду наличия неопределенности в выборе решения, наряду с правдоподобием имеет смысл максимизировать одновременно набор критериев $R_i(\Phi, \Theta)$, выражающих априорные предположения на счет $\phi_z$ и $\theta_d$ как столбцов матриц $\Phi, \Theta^T$ и называемых \textit{регуляризаторами}. Предлагается в качестве решения задачи многокритериальной  оптимизации максимизировать
\[
L(\Phi, \Theta) + R(\Phi, \Theta) = L(\Phi, \Theta) + \sum_i \tau_i R_i(\Phi, \Theta).
\]
Покажите, что шагами EM-алгоритма (см. задачу \ref{em} в разделе \ref{CS}) для решения данной задачи будут

Expectation step: вычислить распределение по темам для каждого термина в документе  
\[
q_{dw}(z) = \frac{\phi_{wz} \theta_{zd}}{\sum_s \phi_{ws} \theta_{sd}};
\]
Maximization step:  найти оптимальные  $\Phi, \Theta$

\[
\phi_{wz} \propto \left( 
\sum_d n_{dw} q_{dw}(z)  + \phi_{wz}\frac{\partial R}{\partial \phi_{wz}}
\right)_{+}, \;
\theta_{zd} \propto \left( 
\sum_w n_{dw} q_{dw}(z)  + \theta_{zd}\frac{\partial R}{\partial \theta_{zd}}
\right)_{+}.
\]
Докажите, что регуляризатор вида
\[
R(\Theta) = - \sum_{d=1}^{D}\sum_{k=1}^{K} \alpha_k \log(\theta_{dk})
\]
соответствует следующему априорному предположению на счет распределения $\theta_d$
\[
\theta_d \in \mathrm{Dir}(\alpha_1 + 1,\ldots,\alpha_K + 1),
\quad
d \in \overline{1,D}, \; K = |T|.
\]
При каком значении $\alpha_1,\ldots,\alpha_K$ данный регуляризатор будет способствовать увеличению количества нулевых компонент $\theta_d$?
\end{problem}

\begin{problem}[PAC-Байесовские неравенства]
Ознакомьтесь с постановкой задачи классификации. 
Для правила (алгоритма) классификации $h \in H$ и набора классифицируемых объектов $X_1, \ldots, X_n$ пусть выборка $X_1^h, \ldots, X_n^h$ есть значения функции потерь  с $X_i^h \in [0,1]$ и $\Exp[X_1^h] = \mu^h$, $\Var[X_1^h]=(\sigma^h)^2$. 

Воспользовавшись неравенством Хефдинга и указанием к задаче, докажите следующее утверждение.
Для любого не зависящего от выборок распределения $p$ на $H$ ($h \sim p$), $\lambda \geq 0$, $\delta \in (0, 1)$ и произвольного априорного распределения $q$ на $H$ с вероятностью не меньше $1 - \delta$  справедливо:
\[\tag{1}
\Exp_q \left( 
\frac{1}{n} \sum_{i=1}^n X_i^h - \mu^h
\right) \leq
\frac{\mathcal{KL} (q \Vert p) + \ln \frac{1}{\delta}  }{n \lambda} + \frac{\lambda}{8}.
 \]
Воспользовавшись неравенством Бернштейна, докажите утверждение, аналогичное предыдущему.
 \[\tag{2}
\Exp_q \left( 
\frac{1}{n} \sum_{i=1}^n X_i^h - \mu^h
\right) \leq
\frac{\mathcal{KL} (q \Vert p) + \ln \frac{1}{\delta}  }{n \lambda} + \lambda (e-2) \Exp_p (\sigma^h)^2.
 \]


\end{problem}

\begin{ordre}
Докажите следующие утверждения.

Для любого измеримого отображения $f : H \to \mathbb{R}$ и любых пар распределений $q$ и $p$ на $H$ справедливо:
\[
\Exp_q f(h) \leq  \mathcal{KL} (q \Vert p)  + \ln \left( \Exp_p e^{f(h)} \right).
\]

Случайная величина $X$ определена на множестве $D$.  Рассмотрим c.в.  $h \sim p$, $h \in H$, не зависящую от $X$,   измеримое отображения $f : H \times D \to \mathbb{R}$. Тогда $\forall \delta \in (0, 1)$ и произвольного распределения $q$ на $H$   с вероятностью не меньше $1 - \delta$ справедливо следующее:
\[
\Exp_q f(h, X) \leq \mathcal{KL} (q \Vert p) + \ln \frac{1}{\delta} + \ln \left( \Exp_p \Exp_X e^{f(h,X)} \right).
\]

\end{ordre}

\begin{remark}
Минимизация по $\lambda$, фигурирующем в выражениях (1) и (2), приводит к зависимости вида $\lambda = \lambda(q)$. Для получения оценки, выполняющейся одновременно для всех $q$, рассмотрим конечный набор значений $\lambda_i$, и для каждого $q$ будем брать $i$, соответствующее минимуму в выражениях (1) и (2). Т.о., если определить $\lambda_i$ как $c^i \lambda_{\min}$, где $\lambda_{\min}$ соответствует $\mathcal{KL} (q \Vert p) = 0$, то получим следующие \textit{PAC-Байесовские неравенства} Хефдинга и Бернштейна.
\[
\Exp_q \left( 
\frac{1}{n} \sum_{i=1}^n X_i^h - \mu^h
\right) \leq
\frac{1+c}{2}
\sqrt{
\frac{\mathcal{KL} (q \Vert p) + \ln \frac{1}{\delta} + \varepsilon(q) }{2 n} 
},
\]
\[
\varepsilon(q) = \frac{\ln 2}{2 \ln c} \left(
1 + \frac{\mathcal{KL} (q \Vert p) }{\ln (1/\delta) }
\right);
\]
при условии
$\mathcal{KL} (q \Vert p) \leq n  (e-2) \Exp_p (\sigma^h)^2  -  \ln \frac{\nu}{\delta}$ выполнено неравенство
\[
\Exp_q \left( 
\frac{1}{n} \sum_{i=1}^n X_i^h - \mu^h
\right) \leq
(1 + c)
\sqrt{
\frac{ (e-2) \Exp_p (\sigma^h)^2 (\mathcal{KL} (q \Vert p) + \ln \frac{\nu}{\delta})  }{n} 
},
 \]
 \[
 \nu  = \left\lceil \frac{1}{\ln c} \ln \left( \frac{(e-2)n}{4\ln(1/\delta)} \right) \right\rceil + 1.
 \]   
   
Данные неравенства позволяют с хорошей точностью оценить отличие среднего риска от эмпирического риска, по сравнению с $VC$-оцениванием. Оптимизация  по $q$ позволяет настраивать гиперпараметры алгоритма классификации.     
\end{remark}





==> standart/bernully.tex <==

%\subsection{Схема испытаний Бернулли}

\begin{problem}
Опыт состоит в подбрасывании симметричной монеты до тех пор, пока два раза подряд она не выпадет одной и той же стороной. Подбрасывания независимы в совокупности. 
Постройте пространство элементарных событий и найдите вероятности следующих событий: 
\begin{enumerate}
\item опыт окончится до шестого бросания; 
\item для завершения опыта потребуется четное число бросаний. 
\end{enumerate}
\end{problem}

\begin{problem}(Pаспределение Паскаля или отрицательно биномиальное распределение.)
Найдите распределение дискретной случайной величины, равной количеству произошедших неудач в последовательности испытаний Бернулли с вероятностью успеха $p$, проводимой до $r$-го успеха.

\end{problem}

\begin{problem}
При каждом подбрасывании монета падает вверх орлом с вероятностью $p>0$. Пусть $\pi _{n} $ -- вероятность того, что число орлов после $n\in {\mathbb N}$ независимых подбрасываний будет чётно. Показав, что $\pi _{n+1} =\left(1-p\right)\cdot \pi _{n} +p\cdot \left(1-\pi _{n} \right)$, $n\in {\mathbb N}$, или иным способом найдите~$\pi _{n} $. 
\end{problem}

\begin{comment}
\begin{problem}
Симметричную монету независимо бросили $n$ раз. Результат бросания записали в виде последовательности нулей и единиц. Покажите, что с вероятностью стремящейся к единице при $n\to \infty $ длина максимальной подпоследовательности из подряд идущих единиц лежит в промежутке
\[\left(\log \sqrt{n} ,\; \log n^{2} \right).\] 
\end{problem}
\end{comment}

\begin{problem}

В так называемой ``безобидной игре'' с повторениями участвуют два игрока. Начальный капитал первого игрока равен $z$ руб, второго равен $\infty$. В каждой партии первый игрок выигрывает или проигрывает 1 руб с вероятностью $0.5$, независимо от предшествующих партий. Обозначим за $z + s_k$ капитал первого игрока после $k$-й итерации, $\eta(z)$ -- число шагов до разорения:
\[
\eta(z) = \min \{k: z + s_k = 0 \}.
\]     
Покажите, что с вероятностью 1 первый игрок разорится, т.е. \linebreak что $\PR(\eta(z)<\infty) = 1,$ но при этом $\Exp \eta(z) = \infty$.  

\end{problem}

\begin{ordre}
Получите рекуррентные соотношения для вероятности разорения и  $\Exp \eta(z)$. Допустив  $\Exp \eta(z) < \infty$, придите к противоречию, доказав $\Exp \eta(z) < 0$ при больших $z$.
\end{ordre}

\begin{problem}
Сколько раз в среднем нужно подбросить монету, чтобы решка выпала два раза подряд?
\end{problem}



\begin{problem} (Честная игра \cite{book2012}.)
Два человека играют в {\it орлянку} (кидают симметричную монету, и ставят по рублю: один на орла, другой на решку). У каждого есть своя монетка, и каждый подозревает партнера в несимметричности его монетки. Предложите правила (как, имея эти две монеты, ``сгенерировать'' симметричную монету), по которым игра будет гарантированно честной?
\end{problem}


==> standart/combinatorica.tex <==
%\subsection{Дискретное равномерное распределение}


\begin{problem}
Некто имеет $N$ ключей, из которых только один от его двери. Какова вероятность того, что, используя ключи в случайном порядке, 
он откроет дверь 
\begin{enumerate}
\item[а)] первым ключом; 
\item[б)] последним ключом? 
\end{enumerate}
Требуется найти вероятность того, что потребуется не менее $k$ попыток, чтобы открыть дверь, если ключи, которые не подошли 
\begin{enumerate}
\item[в)] откладываются; 
\item[г)] не откладываются. 
\end{enumerate}

\begin{ordre}
В пункте в) воспользоваться заменой вероятности бинарной величины на математическое ожидание.
\end{ordre}

\end{problem}


\begin{problem}
Ребенок играет с десятью буквами разрезной азбуки: А, А, А, Е, И, К, М, М, Т, Т. 
Какова вероятность того, что при случайном расположении букв в ряд он получит слово << МАТЕМАТИКА >>? 
\end{problem}


\begin{problem}
Казалось бы, при бросании двух игральных костей как 9, так и 10 можно получить двумя разными способами: $9 = 3+6 = 4+5$, $10 = 4+6 = 5+5$. В случае бросания трех костей 9 и 10 получаются 6 различными способами. Почему тогда 9 появляется чаще, когда бросают две кости, а 10, когда бросают три? 
\end{problem}



\begin{problem}(Парадокс раздела ставки \cite{2013}, \cite{book12}.)
Два игрока играют в безобидную игру (с вероятностью победы в каждой из партий 1/2). Они договорились, что тот, кто первым выиграет 6 партий, получит  весь приз. Предположим, что игроки не успели доиграть: первый выиграл 5 партий, а второй -- 3. Как следует разделить приз?   
\end{problem}

\begin{problem}(Вероятностный парадокс лжеца \cite{book2012}.)
Если Вы выберете ответ на этот вопрос случайно, какова вероятность правильного ответа:

а) 25{\%}; б) 50{\%}; в) 60{\%}; г) 25{\%}?
\end{problem}

\begin{problem}
Из урны, содержащей $a$ белых, $b$ черных и $c$ красных шаров, последовательно извлекаются три шара. Найдите 
вероятность следующих событий: 
\begin{enumerate}
\item[а)] все три шара разного цвета; 
\item[б)] шары извлечены в последовательности белый, черный, красный; 
\item[в)] шары извлечены в обратной последовательности. 
\end{enumerate}
\end{problem}



\begin{problem}
Из урны, содержащей $a$ белых и $b$ черных шаров, извлекается наугад один шар и откладывается в сторону. Какова вероятность 
того, что извлеченный наугад второй шар окажется белым, если: 
\begin{enumerate}
\item[а)] первый извлеченный шар белый; 
\item[б)] цвет  первого извлеченного шара остается неизвестным? 
\end{enumerate}
\end{problem}


\begin{problem}(Задача Стефана Банаха \cite{2013}, \cite{29}.)
В двух спичечных коробках имеется по $n$ спичек. На каждом шаге наугад выбирается коробок, и из него удаляется (используется) 
одна спичка. Найдите вероятность того, что в момент, когда один из коробков опустеет, в другом останется $k$ спичек. 
\end{problem}

\begin{ordre}
Событие, удовлетворяющее условию задачи: из выбранного коробка взяли последнюю спичку, а в другом коробке имеется $k$ спичек. 
\end{ordre}

\begin{problem}
Партия продукции состоит из десяти изделий, среди которых два изделия дефектные. Какова вероятность того, что из пяти отобранных 
наугад и проверенных изделий: 
\begin{enumerate}
\item[а)] ровно одно изделие дефектное; 
\item[б)] ровно два изделия дефектные; 
\item[в)] хотя бы одно изделие дефектное? 
\end{enumerate} 

\begin{ordre}
В пункте в) удобнее искать вероятность противоположного события.
\end{ordre}

\end{problem}

\begin{problem}
Известно, что в результате бросания десяти игральных костей выпала  по крайней мере одна «шестерка». Какова вероятность того, что число выпавших «шестерок» больше единицы?
\end{problem}

\begin{problem}
Найдите вероятность того, что из $50$ студентов, присутствующих на лекции по теории вероятностей, хотя бы двое имеют одну и ту же дату рождения. 

\begin{remark}
См. Мостеллер~Ф. Пятьдесят занимательных вероятностных задач с решениями. М.: Едиториал УРСС, 2009.
\end{remark}

\end{problem}


\begin{problem}
В урне находится $m$ шаров, из которых $m_1$ белых и $m_2$ черных $(m_1 + m_2 = m)$. 
Производится $n$ извлечений одного шара с возвращением его (после определения его цвета) обратно в урну. Найдите вероятность того, 
что ровно $r$ раз из $n$ будет извлечен белый шар. 
\end{problem}


\begin{problem}
Найдите вероятность того, что при размещении $n$ различных шаров по $N$ различимым ящикам заданный ящик будет содержать ровно 
$k$: $0\leqslant k\leqslant n$, шаров (все различимые размещения равновероятны). 
\end{problem}


\begin{problem}
В урне находится $m$ шаров, из которых $m_1$ -- первого цвета, $m_2$ -- второго цвета, $\ldots$, $m_s$ -- $s$-го цвета 
$(m_1+m_2+\ldots +m_s=m)$. 
Производится $n$ извлечений одного шара с возвращением его (после определения его цвета) обратно в урну. Найдите вероятность того, 
что $r_1$ раз будет извлечен шар первого цвета, $r_2$ раз -- шар второго цвета, $\ldots$, $r_s$ раз -- шар $s$-го цвета 
$(r_1+r_2+\ldots +r_s=n)$. 
\end{problem}


\begin{problem}
\label{sec:clubok}
Из клубка с $n$ разноцветными веревочками выходит $2n$ концов. Свяжем их попарно в случайном порядке (все возможные варианты связок равновероятны); получится несколько (зацепленных друг за друга) веревочных колец разной длины. Найдите математическое ожидание числа колец.
\end{problem}

\begin{ordre}
Задача (взятая из \cite{book2012}) легко сводится к подсчету математического ожидания числа циклов в случайной перестановке \linebreak(см.~задачу~\ref{cycle} из раздела~\ref{genF}). 
\end{ordre}


\begin{problem}
\label{vkl_iskl}
Пусть $A_1,\ldots,A_n$ -- последовательность событий и $J\subset \{1,\ldots,n\}$:
\begin{align*}
&\PR_1(J) = \sum\limits_{i\in J} \PR(A_i),\\
&\PR_2(J) = \underset{i < j, (i,j)\in J}{\sum} \PR(A_i \cap A_j),\\
&\PR_k(J) = \underset{i_1 < \ldots < i_k, i_{s}\in J}{\sum} \PR(A_{i_1} \cap \ldots \cap A_{i_k}).
\end{align*}

 Покажите, что для всех нечетных $k$ справедливо неравенство
 \[
 \PR(A_{i_1} \cup \ldots \cup A_{i_k}) \leq \underset{j = 1}{\overset{k}{\sum}} (-1)^{j+1}\PR_j(i_1,i_2,..,i_k),    
 \]
  а для всех четных $k$
 
 \[
 \PR(A_{i_1} \cup \ldots \cup A_{i_k}) \geq \underset{j = 1}{\overset{k}{\sum}} (-1)^{j+1}\PR_j(i_1,i_2,..,i_k).	
 \]

 
\end{problem}

\begin{remark}
При $k=n$ получим равенство, известное как \textit{формула включений-исключений}.
\end{remark}

\begin{problem}
В гардеробе случайным образом перепутались $N$ одинаковых шляп посетителей. Какова вероятность того, что хотя бы один посетитель получит свою шляпу (рассмотреть случаи $N=4, \, N=10\,000$)?  
\end{problem}

\begin{ordre}
Воспользоваться формулой включений-исключений \linebreak(см.~задачу~\ref{vkl_iskl}). См.~также задачу~\ref{permloop} из раздела~\ref{genF}.
\end{ordre}

\begin{problem}
Несколько раз бросается игральная кость. Какое событие более вероятно: 
\begin{enumerate}
\item[а)] сумма выпавших очков четна; 
\item[б)] сумма выпавших очков нечетна? 
\end{enumerate}
\end{problem}


\begin{problem}
Для уменьшения общего количества игр $2n$ команд спортсменов разбиваются на две подгруппы. Определите вероятности того, что 
две наиболее сильные команды окажутся: 
\begin{enumerate}
\item[а)] в одной подгруппе; 
\item[б)] в разных подгруппах. 
\end{enumerate}
\end{problem}


\begin{problem}
В урне находятся $a$ белых и $b$ черных шаров, которые наугад по одному без возвращения извлекаются из урны до тех пор, пока урна не опустеет. 
Какое событие более вероятно: 
\begin{enumerate}
\item[а)] первый извлеченный шар белый; 
\item[б)] последний извлеченный шар белый?
\end{enumerate}
\end{problem}



\begin{problem}
В урне находятся $a$ белых и $b$ черных шаров. Шары наугад по одному извлекаются из урны без возвращения. Найдите вероятность того, 
что $k$-й вынутый шар оказался белым. 
\end{problem}


\begin{problem}
$30$ шаров размещаются по $8$ ящикам так, что для каждого шара вероятности попадания в каждый ящик одинаковы. Найдите вероятность 
размещения, при котором будет $3$ пустых ящика, $2$ ящика -- с~тремя, $2$ ящика -- с~шестью и $1$ ящик -- с~двенадцатью шарами. 
\end{problem}


\begin{problem}(Вероятностная формулировка Большой Теоремы Ферма.)
Две урны содержат одинаковое количество шаров. Шары окрашены в белый и черный цвета. Из каждой урны вынимают по $n$ шаров с возвращением, $n\geq 3$. Найдите $n$ и ``состав'' каждой урны, если вероятность того, что все шары, взятые из 1-й урны белые, равна вероятности того, что все шары, взятые из 2-й урны либо белые, либо черные.
\end{problem}

\begin{problem}
$N$ частиц случайно и независимо друг от друга размещаются в $k$ ячейках так, что каждая из них попадает 
в $i$-ю ячейку с вероятностью $p_i$ $(i=1,\ldots,k, \sum\limits_{i=1}^{k} p_i=1)$. Найдите вероятность того, что число частиц в ячейках 
примет заданные значения $n_1$, $\ldots$, $n_i$, $\ldots$, $n_k$ (полиномиальное распределение). 
\end{problem}

\begin{problem}
Из $n$ лотерейных билетов $k$ -- выигрышные $(n\geqslant 2k)$. Какова вероятность, что среди $k$ купленных билетов по крайней мере 
один будет выигрышным? 
\end{problem}


\begin{comment}
\begin{problem}
Из совокупности всех подмножеств множества $\{1,2,\ldots,N\}$ по схеме выбора с возвращением выбираются множества $A$ и $B$. 
Найти вероятность, что $A$ и $B$ не пересекаются. 
\end{problem}
\end{comment}





\begin{comment}
\begin{problem}
В самолете $n$ мест. Есть $n$ пассажиров, выстроившихся друг за другом в очередь. Во главе очереди -- <<заяц>>. У всех, 
кроме <<зайца>>, есть билет, на котором указан номер посадочного места. Так как <<заяц>> входит первым, он случайным образом занимает 
некоторое место. Каждый следующий пассажир, входящий в салон самолета, действует по такому принципу: если его место свободно, то 
садится на него, если занято, то занимает с равной вероятностью любое свободное. Найдите вероятность того, что последний пассажир 
сядет на свое место. 
\end{problem}
\end{comment}


\begin{problem}(Какие автобусы переполнены? \cite{book2012}.) Двое заканчивают рабочий день 
одновременно и идут к автобусной остановке вместе. Каждый уезжает на первом 
подъехавшем автобусе: одному нужен 24-й автобус, другому 25-й. При этом 
первый считает, что в среднем 24-е автобусы более полные, а второй -- что 
25-е. Почему так может быть?
\end{problem}

\begin{problem}(Задача Кавалера де Мере.) 
Что более вероятно: при одновременном бросании четырех игральных костей получить хотя бы одну единицу или при $24$ бросаниях 
 по две игральные кости одновременно получить хотя бы один раз две единицы? Найдите вероятности указанных событий. 
\end{problem}


\begin{problem}
Из $2^N$ множеств: совокупности всех подмножеств множества $\{1,2,\ldots,N\}$ случайно и независимо выбираются два множества $A$ и $B$. Найти вероятность, что $A$ и $B$ не пересекаются.
\end{problem}

\begin{problem}(Н.Н. Константинов \cite{book2012}.)
В самолете $n$ мест. Есть $n$ пассажиров, выстроившихся друг за другом в очередь. Во главе очереди -- ``заяц''. У всех, 
кроме ``зайца'', есть билет, на котором указан номер посадочного места. Так как ``заяц'' входит первым, он случайным образом занимает 
некоторое место. Каждый следующий пассажир, входящий в салон самолета, действует по такому принципу: если его место свободно, то 
садится на него, если занято, то занимает с равной вероятностью любое свободное. Найдите вероятность того, что последний пассажир 
сядет на свое место. 
\end{problem}




==> standart/condition.tex <==
%\subsection{Независимость и условные вероятности}

\begin{problem}
Приведите пример вероятностного пространства и трёх событий на этом пространстве, которые попарно независимы, но зависимы в совокупности. Предложите обобщение полученной конструкции, в котором любые $n$ из $(n+1)$ событий независимы в совокупности, а все $(n+1)$ -- зависимы в совокупности.
\end{problem}

\begin{ordre}
См. задачу \ref{bernshtein}, а также источники \cite{book12}, \cite{stoianov}.
\end{ordre}

\begin{problem}
Покажите, что из независимости событий $A$ и $B$ следует независимость событий $A$ и $\overline B$, $\overline A$ и $B$, 
$\overline A$ и $\overline B$. 
\end{problem}


\begin{problem}
Покажите, что из равенства ${\mathbb P}(A\, |\, B)={\mathbb P}(A\, |\, \overline B)$ для ненулевых событий $A$ и $B$ следует 
равенство ${\mathbb P}(AB)={\mathbb P}(A){\mathbb P}(B)$, т.е. их независимость. 
\end{problem}


\begin{problem}(Пример Бернштейна \cite{stoianov}.)
\label{bernshtein}
Подбрасываются три игральные кости. События $A$, $B$ и $C$ означают выпадение одинакового числа очков (соответственно) на первой и 
второй, на второй и третьей, на первой и третьей костях. Являются ли эти события независимыми 
\begin{enumerate}
\item[а)] попарно, 
\item[б)] в совокупности? 
\end{enumerate}
\end{problem}


\begin{problem} (См. \cite{book2012}, \cite{2013}.)
Имеется три картонки. На одной с обеих сторон нарисована буква $A$, на другой -- $B$, а на третьей с одной стороны -- $A$,\linebreak с другой -- $B$. Одна из картонок выбирается наугад и кладется на стол. Предположим, что на видимой стороне картонки оказывается буква $A$. Какова вероятность, что на второй стороне тоже $A$?
\end{problem}




\begin{problem}
Пусть $A$, $B$, $C$ -- заданные события. Доказажите справедливость неравенств 
\begin{enumerate}
\item ${\mathbb P}(AB)+{\mathbb P}(AC)+{\mathbb P}(BC)\geqslant {\mathbb P}(A)+{\mathbb P}(B)+{\mathbb P}(C)-1$; 
\item ${\mathbb P}(AB)+{\mathbb P}(AC)-{\mathbb P}(BC)\leqslant {\mathbb P}(A)$; 
\item ${\mathbb P}(A\bigtriangleup B)\leqslant {\mathbb P}(A\bigtriangleup C)+{\mathbb P}(C\bigtriangleup B).$ 
\end{enumerate}
\end{problem}

\begin{problem}(Задача A.A. Натана \cite{5}.)
Вероятности конъюнкций событий $A$, $B$ и $C$ приведены в таблице истинности: 
\vspace{0.3cm}

\begin{tabular}{|c|c|c|c|}
\hline
$\quad A\quad$ & $\quad B\quad$ & $\quad C\quad$ & $\quad {\mathbb P}(ABC)\quad$ \\
\hline
$0$ & $0$ & $0$ & $20/36$ \\
\hline
$0$ & $0$ & $1$ & $5/36$ \\
\hline
$0$ & $1$ & $0$ & $5/36$ \\
\hline
$0$ & $1$ & $1$ & $0$ \\
\hline
$1$ & $0$ & $0$ & $5/36$ \\
\hline
$1$ & $0$ & $1$ & $0$ \\
\hline
$1$ & $1$ & $0$ & $0$ \\
\hline
$1$ & $1$ & $1$ & $1/36$ \\
\hline
\end{tabular}

\vspace{0.3cm}

Можно ли наблюдаемые события $A$ и $B$ использовать как признаки, используемые для обнаружения события $C$? 
\end{problem}

\begin{problem}
Юноша собирается сыграть три теннисных матча со своими родителями, и для выигрыша он должен победить два раза подряд. 
Порядок матчей может быть следующим: отец--мать--отец, мать--отец--мать. Юноше нужно решить, какой порядок для него предпочтительней, 
учитывая, что отец играет лучше матери. 

\end{problem}


\begin{problem}
Имеются две урны. В одной из них находится один белый шар, в другой -- один черный шар (других шаров урны не содержат). Выбирается 
наугад одна урна. В нее добавляется один белый шар и после перемешивания один из шаров извлекается. Извлеченный шар оказался белым. 
Определите апостериорную вероятность того, что выбранной оказалась урна, которая первоначально содержала белый шар. 
\end{problem}


\begin{problem}
В первой урне содержится $a$ белых и $b$ черных шаров (и только они), во второй -- $c$  белых и $d$ черных шаров 
(и только они). Из выбранной наугад урны извлекается один шар, который обратно не возвращается. Извлеченный шар оказался белым. 
Найдите вероятность того, что и второй шар, извлеченный из той же урны, окажется белым. 
\end{problem}

\begin{problem}(Парадокс Монти Холла \cite{book12}.)
Представьте, что вы стали участником игры, в которой находитесь перед тремя дверями. Ведущий поместил за одной из трех 
пронумерованных дверей автомобиль, а за двумя другими дверями -- по козе (козы тоже пронумерованы) случайным образом -- это значит, 
что все $3! = 6$ вариантов расположения автомобиля и коз за пронумерованными дверями равновероятны. У~вас нет никакой информации 
о том, что за какой дверью находится. Ведущий говорит: <<Сначала вы должны выбрать одну из дверей. После этого я открою одну из 
оставшихся дверей (при этом если вы выберете дверь, за которой находится автомобиль, то я с вероятностью $1/2$ выберу дверь, 
за которой находится коза номер $1$, и с вероятностью $1-1/2=1/2$ дверь, за которой находится коза номер $2$). Затем я предложу 
вам изменить свой первоначальный выбор и выбрать оставшуюся закрытую дверь вместо той, которую вы выбрали сначала. Вы можете 
последовать моему совету и выбрать другую дверь либо подтвердить свой первоначальный выбор. После этого я открою дверь, 
которую вы выбрали, и вы выиграете то, что находится за этой дверью.>> Вы выбираете дверь номер $3$. Ведущий открывает дверь номер $1$ 
и показывает, что за ней находится коза. Затем ведущий предлагает вам выбрать дверь номер $2$. Увеличатся ли ваши шансы 
выиграть автомобиль, если вы последуете его совету? 
\end{problem}


\begin{problem}
Известно, что $96\%$ выпускаемой продукции соответствует стандарту. Упрощенная схема контроля признает годным с вероятностью 
$0.98$ каждый стандартный экземпляр аппаратуры и с вероятностью $0.05$ -- каждый нестандартный экземпляр аппаратуры. Найдите вероятность того, 
что изделие, прошедшее контроль, соответствует стандарту. 
\end{problem}


\begin{problem}
Пусть отличник правильно решает задачу с вероятностью 0.95, а двоечник с вероятностью 0.15. Сколько задач нужно дать на зачете и сколько требовать решить, чтобы отличник не сдал зачет с вероятностью, не большей 0.01, а двоечник сдал зачет с вероятностью, не большей 0.1?
\end{problem}


\begin{problem}(Задача про мужика.)
Пусть некоторый мужик говорит правду с вероятностью 75\% и лжет с 
вероятностью 25\%. Он подбрасывает симметричную кость и говорит, 
что ``выпала 6''. C какой вероятностью выпала 6?
\end{problem}

\begin{problem}
\label{exp_eps}
Пусть с.в. $X$ имеет показательное распределение $\mathrm{Exp}(\lambda)$. Покажите, что имеет место ``отсутствие последействия'': 
$$
{\mathbb P}(X>x+y\,|\, X>x)={\mathbb P}(X>y) . 
$$
Верно ли обратное утверждение? Приведите пример дискретной с.в. со свойством ``отсуствия последействия''.
\end{problem}
\begin{remark}
Следует также обратить внимание на задачу~\ref{sec:poisson} раздела~\ref{zb4}.
\end{remark}



\begin{problem}
В $(m+1)$ урне содержится по $m$ шаров, причем урна с номером $n$ содержит $n$ белых и $(m-n)$ черных шаров $(n = 0,1,\ldots,m)$. 
Случайным образом выбирается урна и из нее $k$ раз с возвращением извлекаются шары. Найдите: 
\begin{enumerate}
\item[а)] вероятность того, что следующим также будет извлечен белый шар при условии, что все $k$ шаров оказались белыми, 
\item[б)] ее предел при $m\to\infty$. 
\end{enumerate}
\end{problem}

\begin{ordre}
Применить \textit{формулу полной вероятности} в следующем виде: 
$$
{\mathbb P}(B\, |\, A)=\sum\limits_{n=1} {\mathbb P}(B\, |\, H_n A){\mathbb P}(H_n\, |\, A).
$$
\end{ordre}


\begin{problem}
    Береговая охрана замечает вражеский корабль на расстоянии 1~км от побережья и начинает его обстреливать, делая 1 выстрел в минуту. После первого же выстрела корабль разворачивается и движется в сторону от побережья со скоростью 60 км/ч. Вероятность попадания обратно пропорциональна квадрату расстояния от побережья до корабля (если цель находится на расстоянии $x$, тогда вероятность попадания $0.75x^{-2}$). Вероятность того, что корабль выдержит $n$ попаданий и не утонет, равна $4^{-n}$. Посчитайте вероятность того, что кораблю удастся уйти.
\end{problem}

\begin{problem}
Параметр $p$ (вероятность выпадаения <<орла>>) в схеме испытаний Бернулли является равномерно распределенной случайной величиной на отрезке $[0.1, 0.9]$ и разыгрывается до начала испытаний, причем $p$ не изменяется от опыта к опыту. В серии из $n=1000$ бросаний было подсчитано число успехов $r=777$.  Найдите условную плотность распределения $p(x|r=777)$. Оцените, как изменится ответ, если известно, что точное значение числа успехов $r\in[750, 790]$.
\end{problem}


\begin{comment}
\begin{problem}
\begin{enumerate}
\item Имеется монетка (несимметричная). Несимметричность монетки заключается в том, что либо орел выпадает в два раза чаще решки; 
либо наоборот (априорно (до проведения опытов) оба варианта считаются равновероятными). Монетку бросили $10$ раз. Орел выпал $7$ раз. 
Определите апостериорную вероятность того, что орел выпадает в два раза чаще решки (апостериорная вероятность считается с учетом 
проведенных опытов (иначе говоря, это просто условная вероятность)). 

\item Определите апостериорную вероятность того, что орел выпадает не менее чем в два раза чаще решки. Если несимметричность 
монетки заключается в том, что либо орел выпадает не менее чем в два раза чаще решки; либо наоборот (априорно оба варианта считаются 
равновероятными). 
\end{enumerate}
\end{problem}
\end{comment}

\begin{problem}
Пусть $X$ и $Y$ -– независимые случайные величины,  имеющие распределение Пуассона. 
Доказать, что случайная величина $Z = X + Y$ имеет распределение Пуассона. 
Найдите вид условного распределения случайной величины $X$ при фиксированном значении случайной величины $Z$.
\end{problem}


==> standart/continuousDist.tex <==

%\subsection{Примеры непрерывных распределений}

\begin{problem}
Допустим, что вероятность столкновения молекулы с другими молекулами в промежутке времени $[t,t + \Delta t)$ 
равна $p = \lambda\Delta t + o(\Delta t)$ и не зависит от времени, прошедшего после предыдущего столкновения $(\lambda = \const)$. 
Найдите распределение времени свободного пробега молекулы и вероятность того, что это время превысит заданную \linebreak величину $t^*$. 
\end{problem}

\begin{ordre}
Разобьем интервал $\Delta=[0,t)$ на $n$ отрезков равной длины.
Пусть $A_i$ -- событие, означающее, что на отрезке $\Delta_i$  молекула претерпит столкновение с другими молекулами. Можно представить вероятность отсутствия столкновения в виде произведения вероятностей событий $\overline{A_i}$.
\end{ordre}

\begin{problem}(Задача об оптимальном моменте замены оборудования.)
Пусть некоторая система состоит из $n$ элементов, выходящих из строя независимо друг от друга через случайное время $\tau _{i} $, имеющее показательное распределение с параметром $\lambda _{i} $ ($i$ -- номер элемента, $1\le i\le n$). Вышедший из строя элемент немедленно заменяется новым. Пусть $c_{i} $ -- убытки, связанные с выходом из строя и заменой элемента $i$-го типа. Через промежуток времени $T$ разрешается провести профилактический ремонт, при котором все $n$ элементов заменяются новыми. Пусть $D$ -- стоимость профилактического ремонта. Найдите оптимальное время $T$, минимизирующее средние убытки в единицу времени.
\end{problem}

\begin{remark} 
Примите в учет ``отсутствие последействия'' для показательного распределения из задачи \ref{exp_eps}.
Согласуется ли Ваш результат со здравым смыслом: не стоит проводить профилактический ремонт, если выход оборудования из строя не связан с его старением? Детали см. в книге Афанасьева~Л.Г. Очерк исследования операций. М.: Изд-во МГУ, 2007.  176~с. 
\end{remark}



\begin{problem}
Приведите пример таких с.в. $X$ и $Y$, что $X=-Y$, но $F_X=F_Y$  (имеют одинаковые  функции распределения).
\end{problem}

\begin{problem}
Случайная величина $X$ имеет функцию распределения $F_X$ и функцию плотности распределения $f_X$. Найти функции распределения и плотности распределения (если последние существуют) для случайных величин:\\
\indent а) $Y = aX+b$,\\
\indentб) $Z =e^X$,\\
\indent в) $V = X^2$ ($a$ и $b$ -- неслучайные величины).\\
Конкретизировать решения при $X \in \N(0,1)$.
\end{problem}

\begin{problem}
Пусть случайные величины $X$ и $Y$ связаны соотношением $Y =$\linebreak $= \phi(X)$ ($\phi^{-1}(X)$ -- непрерывная вещественнозначная функция). Найдите распределение случайной величины $Y$, если случайная величина $X$ равномерно распределена на отрезке $[0,1]$.
\end{problem}

\begin{problem}
С.в. $X$, $Y$, $Z$ независимы и равномерно распределены на $(0,1)$. Докажите равенство распределений  $(XY)^{Z}$  и $X$.
\end{problem}

\begin{ordre}
Докажите, что величина $-Z(\ln X + \ln Y)$ показательно распределена на $[0,\infty)$. Для этого удобно воспользоваться заменой $U = Z W$, $V = W/Z$, где $W = - \ln X - \ln Y$, $f_W(w) = w e^{-w} [w>0]$. 
\end{ordre}

\begin{problem}
Случайные величины $X_1,\ldots,X_n$ независимы и имеют показательное распределение с параметром $\lambda$.
Докажите равенство распределений $(X_1+  \frac{1}{2} X_2 + \ldots+ \frac{1}{n} X_n)$ и  $\max\{X_1,\ldots,X_n\}$.
\end{problem}

\begin{problem}
Рассмотрим лампочку, которая может ломаться, и устройство, которое чинит лампочку мгновенно, когда та выходит из строя. При этом считается, что времена работы лампочки от поломки до поломки распределены как $\xi \in \text{Exp}(\lambda)$ и не зависят друг от друга. Чинящее устройство, в свою очередь, тоже может ломаться. Распределение времени работы этого устройства $\eta \in \text{Exp}(\mu)$ и не зависит от времени работы лампочки. Найти распределение времени работы всей системы в целом. Рассмотреть случаи, когда $\lambda = \mu$ и $\lambda \neq \mu$.
\end{problem}
\begin{remark}
См. задачу \ref{exp_eps}. 
\end{remark}



\begin{problem}(А.Н. Соболевский.)
Пусть плотность $p(x,y)$ задает равномерное распределение на единичном квадрате $(0, 1)^2$. Проверьте, что $p(x | X =$\linebreak $= Y )$, понимаемая как предел при $\delta \to 0$ условной плотности $p(x | -\delta <$\linebreak $< X - Y <  \delta)$, постоянна и равна~1, в то время как аналогичный предел для $p (x | 1 - \delta < X/Y < 1 + \delta)$ равен $2x$. 
\end{problem}



\begin{comment}
\begin{problem}[распределение Коши]
Радиоактивный источник испускает 
частицы в случайном направлении (при этом все направления равновероятны). 
Источник находится на расстоянии $d$ от фотопластины, которая представляет 
собой бесконечную вертикальную плоскость.

\begin{enumerate}
\item При условии, что частица попадает в плоскость, покажите, что 
горизонтальная координата точки попадания (если начало координат выбирается 
в точке, ближайшей к источнику) имеет плотность распределения:
\[
p\left( x \right)=\frac{d}{\pi \left( {d^2+x^2} \right)}.
\]
Это распределение известно как \textit{распределение Коши}.

\item Можно ли вычислить среднее (математическое ожидание) этого 
распределения?
\end{enumerate}
\end{problem}
\end{comment}


==> standart/graphs.tex <==
\section{Случайные модели графов}

\begin{problem}

На некоторой реке имеется 6 островов, соединенных между собой системой мостов. Во время летнего наводнения часть мостов была разрушена. При этом каждый мост разрушается с вероятностью ${1\mathord{\left/ {\vphantom {1 2}} \right. \kern-\nulldelimiterspace} 2} $, независимо от других мостов. Какова вероятность того, что после наводнения можно будет перейти с одного берега на другой, используя не разрушенные мосты?

\imgh{70mm}{graphs_bridges.pdf}{Схема мостов}

\end{problem}

\begin{problem}

(Модель Эрдёша-Реньи).

 Пусть есть конечное множество (в дальнейшем множество вершин) $V$. $\xi _{vv'} $ - независимые с.в., занумерованные парами $\left\{v,v'\right\}\in V\times V$, $\vert V \vert = N$.
\[\xi _{vv'} =\left\{\begin{array}{cc} {1,} & {p} \\ {0,} & {1-p} \end{array}\right. .\] 
Таким образом, можно задать абстрактный случайный граф на фиксированном множестве вершин. Покажите, что 

\begin{enumerate}
\item  При $p=\frac{1}{N^{1+\varepsilon } } $, $\varepsilon >0$ среднее число не изолированных вершин в случайном графе $o\left(N\right)$.

\item  При $p=\frac{1}{N^{1-\varepsilon } } $, $\varepsilon >0$ с вероятностью близкой к единице ($N \gg 1$) существует связная компонента порядка $N$.
\end{enumerate}



\end{problem}

\begin{problem} 
Рассматривается конфигурация спинов $\omega =\left\{x_{mn} \right\}$ (где $x_{mn} $ - независимые бернуллиевские с.в. с параметром $p$) на двумерной решетке $\left\{(m,n)\right\}\in {\mathbb Z}^{2} $. Вершину $(m,n)$ назовем занятой, если $x_{mn} =1$. Соединим ребром все соседние (находящиеся на расстоянии 1) занятые вершины. Получится случайный граф $G=G\left(\omega \right)$. Назовем кластером графа $G$ максимальное подмножество $A$ вершин решетки такое, что для любых двух $v,v'\in A$ существует связывающий их путь по ребрам графа $G$. Докажите, что существует такое $0<\bar{p}<1$, что при $p<\bar{p}$ все кластеры конечны с вероятностью 1, а при $p>\bar{p}$ с положительной вероятностью есть хотя бы один бесконечный кластер.


\begin{ordre}
Покажите, что при достаточно малых значения $p$ вероятность события, что все кластеры конечны, равна 1. Покажите, что вероятность того, что кластер, содержащий начало координат и имеющий не менее $N$ вершин, не превосходит $\left(Cp\right)^{N} \mathop{\to }\limits_{N\to \infty } 0$, где $C$ - некоторая константа. А значит и событие: бесконечный кластер содержит начало координат - имеет нулевую вероятность.
\end{ordre}

\end{problem}


\begin{problem}
Найти математическое ожидание числа вершин, принадлежащих древесным компонентам.
\begin{ordre}
Число возможных деревьев на $k$ вершинах равно $k^{k-2}$. 
\end{ordre}
\end{problem}

\begin{problem}
Докажите, что количество лесов на $n$~вершинах с $r$~компонентами, каждая из которых содержит ровно по одной вершине из множества $ \{1, \ldots, r\} $, в точности $rn^{n-1-r}$~штук.
\end{problem}

\begin{problem}
Покажите, что число попарно неизоморфных деревьев на $n$ вершинах не меньше, чем $ c_n n^{-2.5} e^n $, где $ c_n \to \frac{1}{\sqrt{2\pi}}$.
\end{problem}

==> standart/limit.tex <==
%\subsection{Сходимость случайных величин}



\begin{problem}
Пусть $X_n \overset{\text{ п.н. }}{\longrightarrow} X$, $Y_n \overset{\text{ п.н. }}{\longrightarrow} Y$. Докажите справедливость соотношений
\begin{enumerate}
\item $a X_n + b Y_n \overset{\text{ п.н. }}{\longrightarrow} a X + b Y$, где  $a, b = {\rm const}$;
\item $|X_n| \overset{\text{ п.н. }}{\longrightarrow} |X|$;
\item $X_n Y_n \overset{\text{ п.н. }}{\longrightarrow} XY$;
\item верны ли предыдущие пункты для других типов сходимостей (см. \cite{stoianov})? 
\end{enumerate}

\end{problem}

\begin{problem}
Докажите, что из сходимости по вероятности всегда следует сходимость по распределению. Обратное -- не всегда верно. Приведите контрпример.
\end{problem}

\begin{problem}
Пусть $X_n \overset{d}{\longrightarrow} a$, где $a = {\rm const}$. Докажите, что $X_n \overset{p}{\longrightarrow} a$.
\end{problem}

\begin{problem}
Приведите пример, показывающий, что из сходимости по вероятности не следует сходимость в среднем порядка $p>0$ $(\Exp (\xi_n - \xi)^p \to$\linebreak $\to 0)$ (см. \cite{stoianov}).
\end{problem}



\begin{problem}
Пусть в вероятностном пространстве  $(\Omega, \mathcal{F},\PR)$  $\Omega = [0,1)$, $\mathcal{F}$  -- $\sigma$-алгебра, содержащая полуинтервалы вида $\Omega _{in} =[(i-1)/n,\; i/n)$,  $i = \overline{1,n}$, $n \in \mathbb{N}$  и $\PR$ -- мера  Лебега $(\forall i,n:\PR\{ \omega \in \Omega _{in} \} =1/n)$.

Исследуйте сходимость следующих последовательностей случайных величин: 

$X_{1}^{(1)}  (\omega ),\; \; X_{2}^{(1)}  (\omega ),\; \; X_{2}^{(2)}  (\omega ),\; \; X_{3}^{(1)}  (\omega ),\; \; X_{3}^{(2)}  (\omega ),\; \; X_{3}^{(3)}  (\omega ),\ldots $

в случаях:

\textit{а}) $X_{n}^{(i)} \; (\omega )=n\; \; \text{при}\; \; \omega \in \Omega _{in} ,\; X_{n}^{(i)} (\omega )=0\; \; \text{при}\; \; \omega \in \Omega \backslash \Omega _{in} ;$

\textit{б}) $X_{n}^{(i)} \; (\omega )=n^{-1} \; \; \text{при} \; \omega \in \Omega _{in} ,\; X_{n}^{(i)} (\omega )=0\; \; \text{при} \; \; \omega \in \Omega \backslash \Omega _{in} ;$

\textit{в}) $X_{n}^{(i)} (\omega )=n\; \; \text{при}\; \; \omega \in \Omega _{in} ,\; \, X_{n}^{(i)} \; (\omega )=n^{-1} \; \text{при}\; \; \omega \in \Omega \backslash \Omega _{in} ;$

\textit{г}) $X_{n}^{(i)} \; (\omega )=n^{-1} \; \; \text{при}\; \; \omega \in \Omega _{in} ,\; X_{n}^{(i)} \; (\omega )=1-n^{-1} \; \text{при}$ $\omega \in \Omega \backslash \Omega _{in} ;$

\textit{д}) $X_{n}^{(i)} \; (\omega )\in N(m_{in} ,\; \sigma _{in}^{2} ),\; \, \text{где}\; \mathop{\lim }\limits_{in\to \infty } \; m_{in} =3,\; \mathop{\lim }\limits_{in\to \infty } \sigma _{in}^{2} =1.$
\end{problem}


\begin{problem}(Лемма Бореля--Кантелли.)
\label{bor_kant}
Для последовательности с.в. $\{X_k\}_{k=1}^{\infty}$  $\exists X$, что $\forall\,\varepsilon >0$: 
\[
\sum \limits_{k=1}^{\infty} \PR(|X_k - X| > \varepsilon) < \infty.
\] 
Докажите, что в этом случае $X_1, X_2, \ldots$ сходится к $X$ с вероятностью единица (п.н.). Справедливо также обратное утверждение для последовательности независимых в совокупности с.в. $\{X_k\}_{k=1}^{\infty}$.
\end{problem}

\begin{ordre}
Введите вспомогательное событие $A_n^m$ -- найдется такоe $k > n$, что $|X_k - X| > 1/m$. Покажите, что 
\[
\PR(A^m) = \PR(\mathop{\cap} \limits_{n=1}^{\infty} A_n^m) = 0.
\] 
Пусть событие  $A$ заключается в том, что  
$$
\exists m: \forall\,n \exists k(n): \; |X_{n+k(n)} - X| > 1/m \, \text{(отрицание сходимости п.н.)}.
$$
Убедитесь в равенстве событий  $A$ и $\cup_{m=1}^{\infty} A^m$.
\end{ordre}

\begin{problem}
\label{limsubseq}
Докажите следующее утверждение: если последовательность $\{\xi_n\}$ сходится  по вероятности, то из нее можно извлечь подпоследовательность  $\{\xi_{n_k}\}$, сходящуюся с вероятностью единица.   
\end{problem}

\begin{ordre}
Выберите $n_k$ в соответствии со свойством
\[
\PR(|\xi_{n_{k+1}} - \xi_{n_k}| > 2^{-k}) < 2^{-k}. 
\]
При помощи леммы  Бореля--Кантелли установите, что ряд \[\sum_k |\xi_{n_{k+1}} - \xi_{n_k}| \] сходится на множестве с вероятностной мерой 1. Предельное значение случайной величины в точках расхождения ряда можно определить равным $0$.
Детали доказательства можно найти в книге Ширяева~А.Н. Т.~1 [12].  %\cite{21}. 
\end{ordre}


\begin{problem}\Star
\label{limpnnero}
Докажите, что не существует метрики, определенной на парах случайных величин, сходимость в которой равносильна сходимости почти наверное.
\end{problem}

\begin{ordre}
Используя результат задачи \ref{limsubseq}, придите к противоречию для последовательности, сходящейся по вероятности, но расходящейся с вероятностью 1. См. также \cite{stoianov}.
\end{ordre}

\begin{problem}
Число $\alpha$ из отрезка $[0, 1]$ назовем нормально приближаемым рациональными числами, если найдутся $c,\varepsilon>0$ такие, что 
при любом натуральном $q$ 
\begin{equation*}
\label{BorelKantel}
\min\limits_{p\in {\mathbb Z}} \Bigl|\alpha-\frac{p}{q} \Bigr|\geqslant \frac{c}{q^{2+\varepsilon}} . 
\end{equation*}
Используя лемму Бореля--Кантелли (см. задачу \ref{bor_kant}), докажите, что множество нормально приближаемых чисел на отрезке $[0, 1]$ имеет лебегову меру единица. 

\end{problem}
\begin{ordre}

Зафиксируем $c$, $\varepsilon >0$ и рассмотрим множество
\[A_{q} =\left\{\left. \alpha \in \left[0,\; 1\right]\; \right|\; \mathop{\min }\limits_{p\in {\mathbb Z}} \left|\alpha -\frac{p}{q} \right|<\frac{c}{q^{2+\varepsilon } } \right\}.\] 
Покажите, что $\mu \left(A_{q} \right)\le {2c\mathord{\left/ {\vphantom {2c q^{1+\varepsilon } }} \right. \kern-\nulldelimiterspace} q^{1+\varepsilon } } $. Таким образом, ряд $\sum_{q=1}^{\infty} \mu \left(A_{q} \right) $ сходится. В силу леммы Бореля--Кантелли (см. задачу \ref{bor_kant}) отсюда следует нужное утверждение.

\end{ordre}

\begin{remark}

В связи с полученным результатом будет интересно заметить, что $\forall\,\alpha \in [0, 1]$ существует такая бесконечная последовательность $q_{k} $ и соответствующая ей последовательность $p_{k} $, что
\[\left|\alpha -\frac{p_{k} }{q_{k} } \right|<\frac{1}{\sqrt{5} } \frac{1}{q_{k} ^{2} } .\] 
В теории цепных дробей показывается, что последовательность ${p_{k} \mathord{\left/ {\vphantom {p_{k}  q_{k} }} \right. \kern-\nulldelimiterspace} q_{k} } $  будет подпоследовательностью последовательности подходящих дробей для числа $\alpha $. Заметим также, что константу ${1\mathord{\left/ {\vphantom {1 \sqrt{5} }} \right. \kern-\nulldelimiterspace} \sqrt{5} } $ в неравенстве уменьшить нельзя.

Отметим также, что данная задача возникает в КАМ-теории (см.~Синай~Я.Г. Введение в эргодическую теорию.  М.: Фазис, 1996.  144~с.; Treschev~D., Zubelevich~O. Introduction to the perturbation theory of Hamiltonian systems. Berlin: Springer-Verlag,  2010.  211~p.).
\end{remark}


\begin{comment}
\begin{problem}
Докажите, что при $n\to\infty$ 
$$
X_n\xrightarrow{L_2} X \,\Rightarrow\, X_n\xrightarrow{L_1}X \, \Rightarrow\, X_n\xrightarrow{P}X 
\, \Leftarrow\, X_n\xrightarrow{\text{ п.н. }}X , 
$$
$$
X_n\xrightarrow{P}X \, \Rightarrow\, X_n\xrightarrow{d}X . 
$$
С помощью контрпримеров покажите, что никакие другие стрелки импликации в эту схему в общем случае добавить нельзя. 
При каких дополнительных условиях можно утверждать, что 
$$
X_n\xrightarrow{\text{ п.н. }}X  \, \Rightarrow\, X_n\xrightarrow{L_1}X ?
$$
Кроме того, показать, что 
$$
X_n\xrightarrow{P} X \; (n\to\infty) \,\Leftrightarrow\, \rho_P(X_n,X)={\mathbb E}\Bigl( \frac{|X_n-X|}{1+|X_n-X|}\Bigr)
\xrightarrow{n\to\infty} 0 . 
$$
Также показать, что 
$$
X_n \xrightarrow{d}c\quad \Rightarrow \quad X_n \xrightarrow{P}c, \text{ где } c=\const \text{ (не с.в.) }
$$
\end{problem}

\begin{ordre}
$ $
\begin{enumerate}

\item Из сходимости по распределению не следует сходимость по вероятности, а также сходимость в $L_1$, $L_2$ и почти наверное. Проанализируйте следующий контр пример.  

\[
X,Y,X,Y,\ldots
\]

 где  случайные величины $X(\omega)=\omega$ и $Y(\omega)=1-\omega$ имеют одну и ту же функцию распределения 
$$
F_X(x)=F_Y(x)=x\cdot {\mathbb I}_{\{ x\in[0,1]\}} . 
$$

\item Из сходимости по вероятности не следует сходимость почти наверное. Проанализируйте в качестве контр примера серию бегущих импульсов.
 
$$
X_1={\mathbb I}_{[0,1/2]},\, X_2={\mathbb I}_{[1/2,1]},\, X_3={\mathbb I}_{[0,1/4]},\, X_4={\mathbb I}_{[1/4,1/2]}, \ldots, 
$$

\item Выполнена импликация 
$$
X_n\xrightarrow{\text{ п.н. }}X  \, \Rightarrow\, X_n\xrightarrow{L_1}X , 
$$
т.е. возможен предельный переход под знаком математического ожидания, если семейство с.в. $\{ X_n\}$ является равномерно интегрируемым: 
$$
\sup\limits_n {\mathbb E}\bigl[ |X_n|\cdot {\mathbb I}_{\{ |X_n|>c\}} \bigr]\xrightarrow{c\to +\infty}0 . 
$$

\item 


$\frac{|X_n-X|}{1+|X_n-X|}<1$, $\frac{|X_n-X|}{1+|X_n-X|}\leqslant |X_n-X|$. 


\begin{multline*}
{\mathbb E}\Bigl( \frac{|X_n-X|}{1+|X_n-X|}\Bigr)=\int\limits_{|X_n-X|\leqslant\varepsilon} 
\frac{|X_n(\omega)-X(\omega)|}{1+|X_n(\omega)-X(\omega)|}\, P(d\omega)+\\
+\int\limits_{|X_n-X|>\varepsilon}
\frac{|X_n(\omega)-X(\omega)|}{1+|X_n(\omega)-X(\omega)|}\, P(d\omega)
\leqslant \varepsilon+{\mathbb P}(|X_n-X|>\varepsilon) . 
\end{multline*}

\end{enumerate}

\end{ordre}
\end{comment}


==> standart/moments.tex <==
%\subsection{Моментные характеристики}


\begin{problem}(Обобщённое неравенство Чебышёва.)
\label{mark_cheb}
Пусть $g$ -- неотрицательная и неубывающая функция такая, что $\Exp g(|\xi|) < \infty$. Покажите, что для всех $x$, удовлетворяющих условию $g(x) > 0$,
\[
\PR(|\xi| \geq x) \leq \frac{ \Exp g(|\xi|) }{ g(x)}.
\]
Докажите следующие следствия (см. \cite{21}):
\begin{enumerate}
\item (Неравенство Маркова) $\Exp |\xi|^p < \infty$, $p > 0$, $x > 0$:
\[
\PR(|\xi| \geq x) \leq \frac{ \Exp |\xi|^p }{ x^p}.
\]
\item (Неравенство Чебышёва) $\Var \xi < \infty$, $x > 0$:
\[
\PR(|\xi - \Exp \xi| \geq x) \leq \frac{ \Var \xi }{ x^2}.
\]
\item (Экспоненциальное неравенство Чебышёва) $\Exp \left[e^{t \xi}\right] < \infty$, $t > 0$:
\[
\PR(\xi \geq x) \leq \frac{ \Exp \left[e^{t \xi}\right] }{ e^{t x} }.
\]
\item (Неравенство Кантелли) $\Var \xi < \infty$, $x > 0$:
\[
\PR( \xi - \Exp \xi \geq x) \leq \frac{ \Var \xi }{ x^2 + \Var \xi}.
\]
\end{enumerate}

\end{problem}

\begin{problem}
Докажите \textit{неравенство Ляпунова}: $0 < p < q$: 
\[
(\Exp |\xi|^p)^{1/p} \leq (\Exp |\xi|^q)^{1/q}. 
\]
\end{problem}

\begin{ordre}
Воспользуйтесь неравенством Йенсена: $\Exp |\xi| < \infty$, $g$ -- выпуклая функция:
\[
g(\Exp \xi) \leq \Exp g(\xi). 
\]

\end{ordre}

\begin{problem}
Докажите \textit{неравенство Гёльдера}: $1 < p < \infty$, $1/p + 1/q = 1$, $\Exp |\xi|^p < \infty$, $\Exp |\eta|^q < \infty$:  
\[
\Exp |\xi \eta | \leq (\Exp |\xi|^p)^{1/p} (\Exp |\eta|^q)^{1/q}. 
\]
\end{problem}

\begin{ordre}
Воспользуйтесь неравенством Юнга: $x > 0$, $y > 0$: 
\[
x y \leq \frac{x^p}{p} + \frac{y^q}{q}.  
\]

\end{ordre}

\begin{problem}
Докажите \textit{неравенство Минковского}: $1 \geq p < \infty$, $\Exp |\xi|^p < \infty$, $\Exp |\eta|^p < \infty$:  
\[
(\Exp |\xi + \eta |^p)^{1/p} \leq (\Exp |\xi|^p)^{1/p} + (\Exp |\eta|^p)^{1/p}. 
\]
\end{problem}

\begin{ordre}
Воспользуйтесь неравенством $p > 0$: 
\[
\left| \sum \limits_{k=1}^n x_i \right|^p \leq \max\{1, n^{p-1}\} \sum \limits_{k=1}^n |x_i|^p  
\]
и неравенством Гёльдера.
\end{ordre}

\begin{problem}
Покажите, что неравенство Чебышёва:
\[P\left(\left|X-EX\right|>\varepsilon \right)\le \frac{DX}{\varepsilon ^{2} } \] 
принципиально не улучшаемо.

\begin{ordre} 
Рассмотрите с.в. 
\[X=\left\{\begin{array}{cc} {a,} & {{\raise0.7ex\hbox{$ p $}\!\mathord{\left/ {\vphantom {p 2}} \right. \kern-\nulldelimiterspace}\!\lower0.7ex\hbox{$ 2 $}} } \\ {0,} & {1-p} \\ {-a,} & {{\raise0.7ex\hbox{$ p $}\!\mathord{\left/ {\vphantom {p 2}} \right. \kern-\nulldelimiterspace}\!\lower0.7ex\hbox{$ 2 $}} } \end{array}.\right.\] 
Положите $\varepsilon =a-\delta $, где $\delta \to 0+$. См. также Червоненкис~А.Я. Компьютерный анализ данных. М.: Яндекс, 2009.
\end{ordre}

\begin{remark}
В частности, данное неравенство не улучшаемо в классе $X \in L_2$. 
\end{remark}

\end{problem}


\begin{problem}
Существует ли случайная величина с конечным вторым моментом и бесконечным первым моментом?
\end{problem}

\begin{problem}
В начале карточной игры принято с помощью жребия определять первого сдающего. Для этого колода хорошо тасуется, и игрокам сдается по одной карте до появления первого туза. Кому выпал туз, тот и сдает в первой игре. На каком месте в среднем появляется первый туз, если в колоде 32 карты (то есть нужно найти математическое ожидание случайной величины «Число карт, сданных до первого туза»)?
\end{problem}



\begin{problem}(А. Шень \cite{book2012}.)
 В лотерее на выигрыш уходит 40\% от стоимости проданных билетов. Каждый билет стоит 100 рублей. Докажите, что вероятность выиграть 5000 рублей (или больше) меньше 1\%.

Искомая вероятность зависит, конечно, от правил лотереи, но ни при каких условиях она не превосходит $1\%$.
Приведите пример правил лотереи, где искомая вероятность минимальна и максимальна.

\begin{ordre} 
Воспользуйтесь неравенством Маркова (см. задачу \ref{mark_cheb}).
\end{ordre}

\end{problem}

\begin{comment}
\begin{problem}

Покажите, что все моменты распределения

 $p_{\lambda } \left(x\right)=\frac{1}{24} e^{-x^{{1\mathord{\left/ {\vphantom {1 4}} \right. \kern-\nulldelimiterspace} 4} } } \left(1-\lambda \sin x^{{1\mathord{\left/ {\vphantom {1 4}} \right. \kern-\nulldelimiterspace} 4} } \right)$, $x\ge 0$ при любом значении параметра $\lambda \in \left[0,1\right]$ совпадают.

\begin{remark}

Необходимое и достаточное условие того, чтобы моменты однозначно определяли распределение, вообще говоря, комплексной случайной величины $x$, имеет вид:

\noindent $\sum _{n=0}^{\infty }\left(M\left(\left|x\right|^{2n} \right)\right)^{{-1\mathord{\left/ {\vphantom {-1 \left(2n\right)}} \right. \kern-\nulldelimiterspace} \left(2n\right)} } =\infty  $ (условие Карлемана).
\end{remark}

\end{problem} 
\end{comment}

\begin{comment}
\begin{problem}
В каждую $i$-ую единицу времени живая клетка получает случайную дозу облучения $X_i$, причем $\{ X_i\}_{i=1}^{t}$ имеют 
одинаковую функцию распределения $F_X(x)$ и независимы в совокупности $\forall t$. Получив интегральную дозу облучения, 
равную $\nu$, клетка погибает. Оценить среднее время жизни клетки ${\mathbb E}T$. 
\end{problem}

\begin{ordre}

Показать тождество Вальда: 
$$
{\mathbb E}S_T={\mathbb E}X\cdot {\mathbb E}T, 
$$

введя вспомогательную случайную величину

$$
Y_j=\begin{cases}
1, &\text{ если }\quad X_1+\ldots +X_{j-1}=S_{j-1}<\nu, \\
0, &\text{ в остальных случаях }. 
\end{cases}
$$
 

\end{ordre}

\end{comment}


\begin{problem}
Восемь мальчиков и семь девочек купили билеты в кинотеатр на $15$ подряд идущих мест. Все $15!$ возможных способов рассадки равновероятны. Вычислите среднее число пар рядом сидящих мальчика и девочки. Например, (\mars, \female, \mars, \female) содержит три такие пары. 
\end{problem}


\begin{problem}
На первом этаже семнадцатиэтажного общежития в лифт вошли десять человек. Предполагая, что каждый из вошедших (независимо от остальных) может с равной вероятностью жить на любом из шестнадцати этажей (со 2-го по 17-й), найдите математическое ожидание числа остановок лифта.
\end{problem}



\begin{problem}
\label{sec:latters}
Имеется $n$ пронумерованных писем и $n$ пронумерованных конвертов. Письма случайным образом раскладываются по конвертам (все $n!$ 
способов равновероятны). 
Найдите математическое ожидание числа совпадений номеров письма и конверта (письмо лежит в конверте с тем же номером). 
\end{problem}

\begin{problem}
\label{mom_ineq}
С.в. $\xi$ имеет ограничение $\PR(\xi \geq h(x)) \leq e^{-x}$ при $x \geq x_0$, $h(x)$ -- абсолютно непрерывная функция. Докажите следующие неравенства для первого и второго моментов $\xi$:
\[
\Exp \xi \leq h(x_0) + \int_{x_0}^{\infty}h'(x)e^{-x}dx,
\]
\[
\Exp \xi^2 \leq h^2(x_0) +  2\int_{x_0}^{\infty}h(x) h'(x)e^{-x}dx.
\]
\end{problem}

\begin{ordre}
Удобно воспользоваться следующей формулой для подсчета математического ожидания: 
\[
\Exp \xi = \int\limits_{0}^{+\infty} \PR(\xi \geq x)dx - 
    \int\limits_{-\infty}^{0}\PR(\xi < x)dx.
\]
\end{ordre}





\begin{comment}

\begin{problem}

Требуется определить начиная с какого этажа брошенный с балкона 100-этажного здания стеклянный шар разбивается. В наличии имеется два таких шара. Предложить метод нахождения граничного этажа, минимизирующий математическое ожидание числа бросков. Рассмотреть случай большего числа шаров.  

\end{problem}

\begin{problem}
На подоконнике лежат $N$ помидоров. У каждого из них предначертана своя судьба - сгнить вечером $i$-го дня ($1 \leqslant i \leqslant N$, причем ни у каких двух помидоров судьба не совпадает). Утром каждого дня приходит человек и случайным образом съедает один свежий помидор из оставшихся. Таким образом, каждый помидор либо сгнивает в свой предначертанный день, либо употребляется ранее в качестве пищи.

\begin{enumerate}
\item Получите рекуррентную формулу для математического ожидания съеденных помидоров от числа $N$.
\item Найдите асимптотическую оценку количества съеденных помидоров при $N \rightarrow \infty$.
\end{enumerate}

\end{problem}

\end{comment}


==> standart/order.tex <==


%\subsection{Порядковые статистики}

\begin{problem}
Случайным образом выстраиваются в шеренгу  $n$ человек разного роста. Найдите вероятность того, что
\begin{enumerate}
\item[а)] самый низкий окажется $i$-м слева; 
\item[б)] самый высокий окажется первым слева, а самый низкий --- последним слева; 
\item[в)] самый высокий и самый низкий окажутся рядом; 
\item[г)] между самым высоким и самым низким расположатся более $k$ человек. 
\end{enumerate}
\end{problem}


\begin{problem}
Урна содержит $N$ шаров с номерами от $1$ до $N$. Пусть $K$ -- наибольший номер, полученный при $n$ их поштучных извлечениях 
с возвращением. Найдите: 
\begin{enumerate}
\item распределение $K$;
\item асимптотику математического ожидания ${\mathbb E}K$ при $N\to\infty$. 
\end{enumerate}
\end{problem}

\begin{ordre}
\[
{\mathbb E}K=\sum\limits_{j=0}^{N} {\mathbb P}(K>j).
\]
\end{ordre}

\begin{problem}
Найдите математическое ожидание ${\mathbb E}Z$, где $Z$ -- $k$-я по величине из координат $n$ точек, взятых наудачу на отрезке 
$[0, 1]$ $(k \leqslant n)$. 
\end{problem}

\begin{comment}
\begin{problem}[рекорды]
Пусть $X_1 ,X_2 ,\ldots $ -- независимые 
случайные величины с одной и той же плотностью распределения вероятностей 
$p(x)$. Будем говорить, что наблюдается рекордное значение в момент времени 
n$>$1, если $X_n >\max \left[ {X_1 ,\ldots,X_{n-1} } \right]$. Докажите 
следующие утверждения.

\begin{enumerate}
\item Вероятность того, что рекорд зафиксирован в момент времени $n$, 
равна $1/n$.

\item Математическое ожидание числа рекордов до момента времени $n$ 
равно 
\[
\sum\limits_{1<i\le n} {\frac{1}{i}} \sim \ln n.
\]

\item Пусть $Y_n $ --- случайная величина, принимающая значение $1$, если 
в момент времени $n$ зафиксирован рекорд, и значение $0$ -- в противном случае. 
Тогда случайные величины $Y_1 ,Y_2 ,\ldots$ независимы в совокупности.

\item Дисперсия числа рекордов до момента времени $n$ равна
\[
\sum\limits_{1<i\le n} {\frac{i-1}{i^2}} \sim \ln n.
\]

\item Если $T$ -- момент появления первого рекорда после момента времени $1$, то $ET=\infty $.
\end{enumerate}
\end{problem}

\end{comment}

\begin{problem}
Покажите, что если независимые с.в. $X_1,\dots,X_n$ имеют   
\textit{показательное распределение}, т.е. 
$$
f_{X_i}(x)=\begin{cases}
\lambda_i\exp(-\lambda_i x), \; x\geqslant 0, \\
0,\; x<0
\end{cases}
$$
(часто пишут $X_i\in \mathrm{Exp}(\lambda_i)$), то 
$$
\min\{ X_1,\ldots, X_n\}\in \mathrm{Exp}\Bigl( \sum\limits_{i=1}^{n}\lambda_i\Bigr) . 
$$
\end{problem}


\begin{problem}
В некотором вузе проходит экзамен. Количество экзаменационных билетов $N$. Перед экзаменационной аудиторией выстроилась очередь из 
студентов, которые не знают, чему равно $N$. Согласно этой очереди студенты вызываются на экзамен (второй студент заходит в аудиторию 
после того, как из нее выйдет первый, и т.д.). Каждый студент с равной вероятностью может выбрать любой из $N$ билетов (в независимости 
от других студентов). Проэкзаменованные студенты, выходя из аудитории, сообщают оставшейся очереди номера своих билетов. 
Оцените (сверху), сколько студентов должно быть проэкзаменовано, чтобы оставшаяся к этому моменту очередь смогла оценить число 
экзаменационных билетов с точностью $10\%$ с вероятностью, не меньшей $0.95$. 
\end{problem}



==> standart/sigmaAlgebra.tex <==
%\subsection{Вероятностное пространство, $\sigma$–алгебра}

\begin{problem}
Покажите, что борелевская $\sigma$-алгебра в ${\mathbb R}^1$, содержащая все числовые промежутки вида $[a,b)$, 
содержит все промежутки вида $(a,b)$, $(a,b]$, $[a,b]$ и отдельные точки прямой. 

\begin{ordre}
Учесть свойство замкнутости $\sigma$-алгебры относительно операций 
объединения, пересечения и вычитания. 
\end{ordre}

\end{problem}


\begin{problem}
Пусть $\Omega = [a,b]\times...\times[a,b]$, $\mathcal{F}$ -- $\sigma$–алгебра, содержащая все отрезки 
$[\alpha_1,\beta_1]\times...\times[\alpha_n,\beta_n]$ $(a \leqslant \alpha_1 < \beta_1 \leqslant b, \ldots, a \leqslant \alpha_n < \beta_n \leqslant b)$ с вероятностной мерой 
\[
{\mathbb P}\left(\omega_1  \in [\alpha_1,\beta_1], ..., \omega_n  \in [\alpha_n,\beta_n]  \right)=\dfrac{\mes[\alpha_1, \beta_1]}{\mes[a,b]}  \ldots  \dfrac{\mes[\alpha_n, \beta_n]}{\mes[a,b]}.
\]
Покажите, что 
\begin{enumerate}
\item ${\mathbb P}\left( \omega_1=c=\const\right)=0$; 
\item ${\mathbb P}\left( \omega_1=\omega_2\right)=0$.
\end{enumerate}
Найдите вероятность ${\mathbb P}\left( \omega_1 \leq \omega_3 \leq \omega_2\right)$. 

\end{problem}


\begin{problem}
Число элементарных событий некоторого вероятностного пространства равно $n$. Укажите минимальное и максимальное возможные значения 
для числа событий. 
\end{problem}

\begin{problem}
Может ли число всех событий какого-либо вероятностного пространства быть равным $128$; $129$; $130$? 
\end{problem}


\begin{problem}(Задача о встрече \cite{2}.)
\label{L_extension}
Два лыжника условились о встрече между $10$ и $11$ часами утра у подножия тягуна, причем договорились ждать друг друга не более $10$ минут, чтобы не замерзнуть. Считая, что момент прихода на встречу каждым выбирается ``наудачу'' в пределах указанного часа, найдите вероятность того, что встреча состоится. 
\end{problem}

\begin{remark}
В подобного рода задачах, где явно не определена вероятностная тройка $( \Omega, \mathcal{F}, \PR )$, в общем случае следует придерживаться такой последовательности действий: 
\begin{enumerate}
\item задать вероятностную меру на множествах простой структуры;
\item продолжить вероятностную меру на множества более сложной структуры, рассматриваемые в задаче;  
\item проверить условия, гарантирующие $\sigma$-аддитивность продолженной меры ($\PR(\bigcup_{i=1}^{n} A_i) \to \PR(A)$, при условии $\bigcup_{i=1}^{\infty} A_i = A$).   
\end{enumerate}
Рассмотрим каждый из этапов в отдельности, придерживаясь контекста задачи о встрече. Возьмем $\Omega = [0,1] \times [0,1]$. В качестве множеств простой структуры $\text{П}$ удобно воспользоваться \textit{полукольцом с единицей} $\Leftrightarrow$ $C_i, A, B \in \text{П}$, $C_i \cap C_j  = \emptyset$:
\[
\Omega \in \text{П},  \quad A\cap B \in \text{П}, \quad A_{\supset B} \setminus B = \bigcup \limits_{i=1}^n C_i.
\]
Зададим меру $\PR$ на $\text{П}$, $\Omega \subseteq \mathbb{R}^n$ при помощи формулы 
\[
\PR\left( [x_1^{(0)}, x_1^{(1)})\times \ldots \times [x_n^{(0)},  x_n^{(1)})  \right) = 
\]
\[\tag{1} =
\begin{cases}
\sum \limits_{\alpha_1, \ldots, \alpha_n} (-1)^{\sum \alpha_i} F\left(x_1^{(\alpha_1)} ,\ldots, x_n^{(\alpha_n)}\right),  \; n \; \text{четно}, \\
\sum \limits_{\alpha_1, \ldots, \alpha_n} (-1)^{\sum \alpha_i - 1} F\left(x_1^{(\alpha_1)} ,\ldots, x_n^{(\alpha_n)} \right) ,  \; n \; \text{нечетно}.\\
\end{cases}
\]
Тогда выполнимость свойств аддитивной вероятностной меры $\PR$ равносильна  выполнимости свойств (1--5) для функции $F$, а $\sigma$-аддитивность равносильна свойству 6: 

\begin{enumerate}
\item[1.] Неотрицательность;
\item[2.] Монотонность по каждому аргументу;
\item[3.] $F(x_1, \ldots, x_n) \to 0$, если хотя бы один аргумент $x_i \to -\infty$;
\item[4.] $F(x_1, \ldots, x_n) \to 1$, если все $x_1, \ldots, x_n  \to \infty$;
\item[5.] $F(x_1, \ldots, x_n) \to  F(x_1, \ldots x_{i-1}, x_{i+1}  \ldots , x_n)$ при $x_i \to \infty$;
\item[6.] Непрерывность справа в точках разрыва, существование предела слева (cadlag -- функция).
\end{enumerate} 

Заметим также, что если $F$ абсолютно непрерывна, то существует функция плотности распределения  $f(x_1 ,\ldots, x_n ) \geq 0$, что гарантирует выполнение свойств (1--6), т.е. $\PR$ является  $\sigma$–аддитивной вероятностной мерой на  $\text{П}$.
Продолжим вероятностную меру на класс множеств 
\[\mu \tilde{A} \supset \{t_1, t_2 \in \Omega: |t_1 - t_2| =\tau \}\]
посредством \textit{пополнения по Лебегу} (см. Константинов Р.В. Лекции по функциональному анализу.   Долгопрудный, 2007.  156~с.):
\[
\PR^{*}(B) = \inf \limits_{B \subseteq \bigcup \limits_{i=1}^{\infty} A_i} \sum \limits_{i=1}^{\infty} \PR(A_i),
\]
 \[
 A \in \mu \tilde{A} \Leftrightarrow  \forall \varepsilon >0 \; \exists A_\varepsilon \in \tilde{A}:  \PR^{*}(A_\varepsilon \triangle A) < \varepsilon,
 \] 
где $\tilde{A}$ --  минимальная по мощности алгебра, содержащая $\text{П}$ ($B \in \tilde{A} \Leftrightarrow$\linebreak $\Leftrightarrow B = \bigcup \limits_{i=1}^n C_i, \; C_i \cap C_j  = \emptyset$).

Предложенное продолжение сохраняет $\sigma$-аддитивность и другие свойства меры.  

\end{remark}

\begin{problem}
Имеется монетка с вероятностью выпадение орла $p=1/2$. Покажите, что событие $A$, заключающееся в том, что отношение числа успехов к
общему числу бросаний $n$ стремится к $1/2$ при $n \to \infty$, принадлежит $\mu \tilde{A}$ (см. замечание к задаче \ref{L_extension}). Считать бросания независимыми.
\end{problem}

\begin{ordre}
Воспользуйтесь вспомогательными событиями 
\[
A_n^\varepsilon = \Bigg\{ (x_1, x_2, x_3, \ldots):\Bigg| \frac{1}{n}\sum \limits_{i=1}^n x_i -\frac{1}{2} \Bigg| \geq \varepsilon \Bigg\}.
\]
\end{ordre}

\begin{remark}
При $\Omega = \mathbb{R}^\infty$ аналогом выражения (1) в задаче \ref{L_extension} будет
\[
\PR\left( [x_{k_1}^{(0)}, x_{k_1}^{(1)})\times \ldots \times [x_{k_n}^{(0)},  x_{k_n}^{(1)} )\times \prod \limits_{k \in \mathbb{N} \setminus \{k_1, \ldots, k_n\} }  \mathbb{R}_k  \right) = 
\]
\[
=\begin{cases}
\sum \limits_{\alpha_1, \ldots, \alpha_n} (-1)^{\sum \alpha_i} F_{k_1 \ldots k_n}\left(x_{k_1}^{(\alpha_1)} ,\ldots, x_{k_n}^{(\alpha_n)} \right) ,  \; n \; \text{четно}, \\
\sum \limits_{\alpha_1, \ldots, \alpha_n} (-1)^{\sum \alpha_i - 1} F_{k_1 \ldots k_n}\left( x_{k_1}^{(\alpha_1)} ,\ldots, x_{k_n}^{(\alpha_n)} \right)  ,  \; n \; \text{нечетно},\\
\end{cases}
\]
где $\mathbb{R}_k$ -- множество значений $k$-й координаты. 
К свойствам (1--7) в этом случае необходимо добавить еще одно свойство:
 для любой перестановки  $\pi$ 
\[
 F_{\pi(k_1) \ldots \pi(k_n)} \left(x_{\pi(k_1)} ,\ldots, x_{\pi(k_n)} \right) =  F_{k_1 \ldots k_n}\left(x_{k_1} ,\ldots, x_{k_n}\right). 
\]

\end{remark}


\begin{problem} (Случайное направление \cite{book2012}.) 
Вы приходите на станцию метро в случайный момент времени $T$ (например, $T$ имеет равномерное распределение на интервале между 10 и 11 часами) и садитесь в первый пришедший поезд (в ту или другую сторону). Будем считать, что поезда в обе стороны ходят одинаково часто (например, каждые 10 минут) согласно расписанию. Одинаковы ли вероятности событий, что Вы поедете в одну или в другую сторону? Рассмотрите случай, когда в одну сторону поезда идут в 10:00, 10:10, 10:20,\dots , а в другую -- в 10:02, 10:12, 10:22,\dots 
\end{problem}


\begin{remark} Казалось бы, интуиция подсказывает, что оба направления ``равноправны'' -- ведь мы приходим в ``случайный'' момент времени. ``Парадокс'' легко разрешается введением вероятностного пространства (конкретизацией ``случайности'' времени прихода на станцию).
\end{remark}

\begin{problem}
В урне находится $3$ белых и $2$ черных шара. 
Эксперимент состоит в последовательном извлечении из урны всех шаров по одному наугад без возвращения. Постройте вероятностное пространство. 
Описать $\sigma$-алгебру, порожденную случайной величиной $X$, если: 
\begin{enumerate}
\item $X$ -- число белых шаров, предшествующих первому черному шару; 
\item $X$ -- число черных шаров среди извлеченных; 
\item $X=X_1+X_2$, где $X_1$ -- число белых шаров, предшествующих первому черному шару, 
$X_2$ -- число черных шаров, предшествующих белому шару. 
\end{enumerate}
\end{problem}


\begin{problem}\Star
\label{SigmaAlgebra}
Пусть $(\Omega,\mathcal{F},{\mathbb P})$ -- некоторое вероятностное пространство и $A$ -- алгебра подмножеств $\Omega$ такая, что 
$\sigma(A)=\mathcal{F}$\quad $(\sigma(A)$ -- наименьшая \mbox{$\sigma$-алгебра}, содержащая алгебру $A)$. Докажите, что 
$$
\forall\,\varepsilon>0,\, B\in\mathcal{F}\quad \exists A_{\varepsilon}\in A:\quad {\mathbb P}(A_{\varepsilon}\bigtriangleup B)
\leqslant\varepsilon . 
$$
\end{problem}

\begin{ordre}
Рассмотрите совокупность множеств (см. детали в \cite{21} Т.~2): 
$$
{\mathcal B}=\bigl\{ B\in\Sigma\, | \, \forall\varepsilon>0 \; \exists A_B\in A:\; {\mathbb P}(A_B\bigtriangleup B)
\leqslant\varepsilon \bigr\} . 
$$

\noindent Покажите, что ${\mathcal B}$ является минимальной $\sigma$-алгеброй (см. \cite{22}, \cite{220}).

\end{ordre}



 \begin{problem}
 \begin{enumerate}
 
 \item Может ли приведенная ниже функция
\[
F\left( {x_1 ,x_2 } \right)=\left\{ {\begin{array}{l}
 1,\quad \min \left( {x_1 ,x_2 } \right)>1, \\ 
 0,\quad \min \left( {x_1 ,x_2 } \right)\le 1 \\ 
 \end{array}} \right.
\]
быть функцией распределения некоторого двумерного случайного вектора? 
Приведите необходимое и достаточное условие того, чтобы $F\left( {x_1 
,...,x_n } \right)$ была функцией распределения некоторого случайного 
вектора.

\item На ${\mathbb R}^n$ задана функция $F\left( {x_1,\ldots,x_n } \right)$, 
неубывающая по каждому аргументу, такая, что $F\left( {x_1 ,\ldots,-\infty 
,\ldots, x_n } \right)=0$, $F\left( {\infty,\ldots,\infty } \right)=1$. Что еще 
надо потребовать от этой функции, чтобы с ее помощью  можно было бы 
естественным образом задать счетно-аддитивную вероятностную меру на 
минимальной $\sigma $-алгебре, содержащей всевозможные прямоугольные 
параллелепипеды в ${\mathbb R}^n$?

\item Может ли функция распределения $F_X \left( x \right)$ с.в. $X$ 
иметь более чем счетное множество точек разрыва?

\end{enumerate}
\end{problem}

\begin{comment}
\begin{problem}(Пример о сходимости ряда.)
Пусть $(\Omega,\Xi,{\mathbb P})$ --- вероятностное пространство, $\xi_1,\xi_2,\ldots$ --- некоторая последовательность с.в.. 
Обозначим $\Xi_n^{\infty}=\sigma(\xi_{n},\xi_{n+1},\ldots)$ --- $\sigma$-алгебру, порожденную с.в. $\xi_{n},\xi_{n+1},\ldots$ и пусть 
$$
{\mathcal X}=\bigcap\limits_{n=1}^{\infty} \Xi_{n}^{\infty}. 
$$
Поскольку пересечение $\sigma$-алгебр есть снова $\sigma$-алгебра, то ${\mathcal X}$ -- есть $\sigma$-алгебра. Эту $\sigma$-алгебру 
будем называть <<хвостовой>> или <<остаточной>>, в связи с тем, что всякое событие $A\in{\mathcal X}$ не зависит от значений с.в. 
$\xi_1,\xi_2,\ldots,\xi_n$ при любом конечном $n$, а определяется лишь <<поведением бесконечно далеких значений последовательности 
$\xi_1,\xi_2,\ldots$ >>. 

С помощью задачи $\ref{SigmaAlgebra}$ докажите справедливость следующего утверждения: 

Пусть $\xi_1,\xi_2,\ldots$ -- последовательность независимых в совокупности с.в. и $A\in{\mathcal X}$ 
(событие $A$ принадлежит <<хвостовой>> $\sigma$-алгебре). Тогда ${\mathbb P}(A)$ может принимать лишь два значения $0$ или $1$. 
\end{problem}

\begin{ordre}
Идея доказательства состоит в том, чтобы показать, что каждое <<хвостовое>> событие $A$ не зависит от самого себя и, значит, 
${\mathbb P}(A\cap A)={\mathbb P}(A)\cdot {\mathbb P}(A)$, т.е. ${\mathbb P}(A)={\mathbb P}^2(A)$, откуда 
${\mathbb P}(A)=0$ или $1$. 
\end{ordre}
\end{comment}


==> standart/vector.tex <==
%\subsection{Случайный вектор}



\begin{problem}
Пусть $X$ и $Y$ --- независимые случайные величины, равномерно распределенные на $(-b,b)$. 
Найдите вероятность $q_b$ того, что уравнение $t^2+tX+Y=0$ имеет действительные корни. Докажите, что 
существует $\lim\limits_{b\to\infty} q_b=q$. Найдите $q$. 
\end{problem}


\begin{problem}
Пусть $X=(X_1,...,X_n)$ -- случайный вектор, компоненты которого имеют нормальное распределение, т.е. $X_i \sim \mathcal{N}(\mu_i,\sigma^2_i)$. Следует ли из этого, что вектор $X$ имеет многомерное нормальное распределение?
\end{problem}

\begin{problem}
Двумерный случайный вектор $X=(X_1,X_2)$  имеет следующую функцию плотности распределения: 
$$
f(x_1,x_2)=\begin{cases}
\dfrac{c}{\sqrt{x_1^2+x_2^2}} \text{ при } x_1^2+x_2^2\leqslant 1 , \\
\quad 0 \quad\text{ иначе}. 
\end{cases}
$$
\begin{enumerate}
\item Найдите $c$.
\item Найдите частные и условные распределения его компонент. 
\item Являются ли они 
\begin{enumerate}
\item стохастически зависимыми; 
\item коррелированными? 
\end{enumerate}
\end{enumerate}
\end{problem}

\begin{problem}
Попарно некоррелированные с.в. $\xi, \eta, \zeta$ обладают одинаковыми математическими ожиданиями и дисперсиями $\Exp\xi = \Exp\eta = \Exp\zeta = 0$, $\Var\xi = \Var\eta = \Var\zeta = \sigma^2$. Найдите $\max \Exp(\xi\eta\zeta)$ и $\min \Exp(\xi\eta\zeta)$.
\end{problem}

\begin{problem}
\label{scalar_prod}
Будем говорить, что  с.в. $\xi$ принадлежит классу $L_2$, если  выполнено ${\mathbb E}\xi^2<\infty$. $L_2$ является линейным пространством, в котором можно задать скалярное произведение следующим образом:
\[
\langle \xi_1, \xi_2 \rangle = \Exp\left[\xi_1 \xi_2\right].
\]
Для величин в $L_2$ введем среднеквадратичное расстояние
\[
\Vert \xi_1 - \xi_2 \Vert_2 = (\Exp{|\xi_1 - \xi_2|^2})^{1/2}.
\]
Пусть $H$ -- конечномерное  подпространство пространства  $L_2$ и $\widehat{\xi}$ -- проекция с.в. $\xi$ на подпространство $H$.

\begin{enumerate}

\item Покажите, что если $H$ является совокупностью всех постоянных, то 
$\widehat{\xi}  = \Exp{\xi}$ и как следствие 
\[
\Vert \xi - \Exp{\xi} \Vert_2 = \underset{\lambda \in H}{\min} \Vert \xi - \lambda \Vert_2.
\] 

\item Рассмотрим  последовательности с.в. $\xi_n \overset{L_2}{\longrightarrow} \xi$, $\eta_n \overset{L_2}{\longrightarrow} \eta$. Докажите, что в этом случае  $\Exp(\xi_n \eta_n) \rightarrow \Exp(\xi \eta)$. 

\end{enumerate}

\end{problem}

\begin{remark}
Рекомендуем также ознакомиться с аналогичными задачами \ref{condExp1}--\ref{condExp3} из раздела \ref{hard}. 
\end{remark}

\begin{problem}
\label{scalar_prod_1}
Пусть  $\xi_1$, $\xi_2$ $\in L_2$ (см. предыдущую задачу) со средними значениями $a_1$ и $a_2$, дисперсиями $\sigma_1^2$ и $\sigma_2^2$ 
и коэффициентом корреляции~$r$. Покажите, что наилучшая линейная оценка
$\widehat{\xi_1}  = c_1 + c_2 \xi_2$ для~$\xi_1$ с точки зрения расстояния в $L_2$ дается формулой 
\[
\widehat{\xi_1}  = a_1 + r \frac{\sigma_1}{\sigma_2} (\xi_2 - a_2).
\]
\end{problem}
\begin{remark}
Коэффициент корреляции определяется как  
\[
r = \frac{\Exp (\xi_1 - a_1) (\xi_2 - a_2)}{\sigma_1 \sigma_2}.
\]
\end{remark}

\begin{comment}
\begin{problem}
Предположим, что с.в. $X\in L_2$, это означает ${\mathbb E}X^2<\infty$. Докажите, что 
\begin{equation}
\label{UMO}
\| X-{\mathbb E}(X|Y_1,\ldots,Y_n)\|_{L_2}=\min\limits_{\varphi\in H} \| X-\varphi(Y_1,\ldots,Y_n)\|_{L_2} , 
\end{equation}
где $H$ --- подпространство пространства $L_2$ всевозможных борелевских функций $\varphi(Y_1,\ldots,Y_n)\in L_2$; 
${\mathbb E}(X|Y_1,\ldots,Y_n)$ --- условное математическое ожидание с.в. $X$ относительно $\sigma$-алгебры, порожденной с.в. 
$Y_1,\ldots,Y_n$, часто говорят просто относительно с.в. $Y_1,\ldots,Y_n$; 
$$
\| X\|_{L_2}=\sqrt{\langle X,X\rangle_{L_2}}=\sqrt{{\mathbb E}(X\cdot X)}=\sqrt{{\mathbb E}(X^2)} . 
$$
\end{problem}

\begin{ordre}
Покажите, что $X-{\mathbb E}^{\mathcal A}X \bot \xi,\quad \forall\xi\in H$, т.е. ${\mathbb E}^{\mathcal A}$ 
является проектором на подпространство $H$ в $L_2$. 
\end{ordre}


\begin{problem}
Докажите, что если в условиях предыдущей задачи $(X,Y_1,\ldots,Y_n)^T$ --- является нормальным случайным вектором (без ограничения 
общности можно также считать, что $(Y_1,\ldots,Y_n)^T$  --- невырожденный нормальный случайный вектор), то в качестве $H$ можно взять 
подпространство всевозможных линейных комбинаций с.в. $Y_1,\ldots,Y_n$. Т.е. мы можем более конкретно сказать, на каком именно 
классе борелевских функций достигается минимум в $(\ref{UMO})$. 
\end{problem}

\begin{ordre}
Будем искать 
${\mathbb E}(X|Y_1,\ldots,Y_n)$ в виде 
\begin{equation}
\label{Gauss}
{\mathbb E}(X|Y_1,\ldots,Y_n)=c_1 Y_1+\ldots +c_n Y_n . 
\end{equation}

Докажите следующие утверждения:

\begin{enumerate}
\item $X-c_1 Y_1-\ldots-c_n Y_n, Y_1,\ldots, Y_n$ - независимы.
\item $X-c_1 Y_1-\ldots-c_n Y_n$ ортогонален подпространству $H$ пространства $L_2$ всевозможных борелевских функций $\varphi(Y_1,\ldots,Y_n)\in L_2$.
\end{enumerate}
 
\end{ordre}

\end{comment}

\begin{problem} Пусть
$$
X=\begin{pmatrix}
X_1\\
X_2\\
X_3
\end{pmatrix}
\in \N\left(
\begin{pmatrix}
2\\
3\\
1
\end{pmatrix}, 
\begin{Vmatrix}
5 & 2 & 7\\
2 & 5 & 7\\
7 & 7 & 14
\end{Vmatrix}
\right) . 
$$
\begin{enumerate}
\item Найдите распределение случайной величины $Y_1=X_1+X_2-X_3$. 
\item Найдите распределение случайной величины $Y_2=X_1+X_2+X_3$. 
\item Найдите ${\mathbb E}(Y_2\, |\, X_1=5, X_2=3)$. 
\item Найдите ${\mathbb E}(Y_2\, |\, X_1=5, X_2<3)$. 
\item Найдите ${\mathbb P}(Y_2<10\, |\, X_1=5, X_2<3)$.

\item Пусть $X \in \N\left(m, R\right)$, где матрица $R$ -- неотрицательно определена (это означает, что характеристическая функция вектора $X$ представима в виде \[
\phi_{X}(t) = \Exp e^{it^TX} = \exp\left( it^{T}m-(1/2)t^{T}Rt \right)),
\] где верхний индекс $T$ означает транспонирование. Найдите распределение случайного вектора $Y = AX + b$. 

\end{enumerate}
\end{problem}

\begin{ordre}
Покажите, что
$\phi_{AX+b}(t) = e^{ib}\phi_{X}(A^{T}t)$.
\end{ordre}



\begin{problem}
\label{sec:ordered_seq}
Случайный вектор $W=(W_1, W_2, \ldots, W_n)^T$ имеет плотность распределения 
$$
f_W(w)=\begin{cases}
n! , & \text{ если } 0\leqslant w_1\leqslant w_2\leqslant \ldots \leqslant w_n\leqslant 1, \\
0 & \text{в остальных случаях}. 
\end{cases}
$$
Найдите распределение вектора $U=(U_1, U_2, \ldots, U_n)^T$, если 
$$
U_1=W_1, \quad U_2=W_2-W_1, \ldots, U_n=W_n-W_{n-1} . 
$$
\end{problem}

\begin{ordre}
В общем случае: 
$$
U=\varphi(W) \,\Rightarrow\, f_U(u)=f_W\bigl(\varphi^{-1}(u)\bigr) \Bigl| J\Bigl( \frac{\partial W}{\partial U}\Bigr)\Bigr|,$$
$$
J(\cdot)=\det\Bigl( \frac{\partial \varphi_i^{-1}(u)}{\partial u_j}\Bigr) . 
$$
\end{ordre}


\begin{problem}(См. \cite{4}.)
Спортсмен стреляет по круговой мишени. Вертикальная и горизонтальная 
координаты точки попадания пули (при условии, что центр мишени -- начало 
координат) -- независимые случайные величины, каждая с распределением 
$\N(0,1)$. Покажите, что расстояние от точки попадания до центра имеет 
плотность распределения вероятностей $r\exp \left( {-{r^2} \mathord{\left/ 
{\vphantom {{r^2} 2}} \right. \kern-\nulldelimiterspace} 2} \right)$ для 
$r\ge 0$. Найдите медиану этого распределения.
\end{problem}


==> standart/zb4.tex <==
%\subsection{Закон больших чисел}

\begin{problem}
Пусть случайная величина $X_n$ принимает значения 
\begin{enumerate}
\item $(2^n, -2^n)$ с вероятностями $(1/2, 1/2)$;
\item $(-\sqrt{n}$, $\sqrt{n})$ с вероятностями $(1/2, 1/2)$;
\item $(n, 0, -n)$ с вероятностями $(1/4, 1/2, 1/4)$.
\end{enumerate}
Выполняется ли для последовательности независимых случайных величин 
$X_1$, $X_2$, $\ldots$ \textit{закон больших чисел}? 
\end{problem}

\begin{ordre}
 Воспользуйтесь тем, что
\[
S_n\xrightarrow{p}0 \,\Leftrightarrow\, S_n\xrightarrow{d}0 \,\Leftrightarrow\, \forall t \; \varphi_{S_n}(t) \to 1,   
\]
\noindent где $S_n=\frac{X_1+\ldots +X_n}{n}$, $\varphi_{S_n}(t)$ -- характеристическая функция. В общем случае соответствие между сходимостью функций распределения $F_n(x)$ и сходимостью соответствующих $\varphi_n(t)$ такое (см.~также задачу~\ref{levi_kramer} раздела~\ref{zb4}):
\begin{enumerate}
\item Если $F_n(x) \to F(x)$ в точках непрерывности $F(x)$ и $F(x)$ удовлетворяет свойствам функции распределения, то $\forall\,t \; \varphi_n(t) \to \varphi(t)$, где $\varphi(t)$ х.ф. $F(x)$.
\item Если $\forall\,t \; \varphi_n(t) \to \varphi(t)$ и $\varphi(t)$ непрерывна в точке $t = 0$, то $\varphi(t)$ является х.ф. некоторого распределения $F(x)$  и $F_n(x) \to F(x)$ в точках непрерывности $F(x)$.

\end{enumerate}

\end{ordre}


\begin{problem}
При каких значениях $\alpha > 0$ к последовательности независимых случайных величин $\{ X_n\}_{n=1}^{\infty}$, 
таких что ${\mathbb P}\left( X_n=n^{\alpha}\right)={\mathbb P}\left( X_n=\right.$\linebreak $\left.=-n^{\alpha}\right)=1/2$, применим усиленный закон больших чисел? 
\end{problem}

\begin{comment}
\begin{ordre}
Докажите достаточное условие выполнения ЗБЧ:
 \[
Var S_n \xrightarrow {n\to\infty}0
\] 
\end{ordre}
\end{comment}

\begin{problem}
Пусть $\{ X_n\}_{n=1}^{\infty}$ -- последовательность случайных величин с дисперсиями $\sigma_i^2$. Докажите, что если все 
корреляционные моменты (корреляции) $R_{ij}$ случайных величин $X_i$ и $X_j$ неположительны и при  
$\frac{1}{n^2}\sum\limits_{i=1}^{n} \sigma_i^2\to 0$, $n\to\infty$, то для последовательности $\{ X_n\}_{n=1}^{\infty}$ выполняется закон больших чисел. 
\end{problem}

\begin{problem}
Пусть $\{ X_n\}_{n=1}^{\infty}$ -- последовательность случайных величин с равномерно ограниченными дисперсиями, причем каждая 
случайная величина $X_n$ зависит только от $X_{n-1}$ и $X_{n+1}$, но не зависит от остальных $X_i$. Докажите выполнение для этой 
последовательности закона больших чисел.
\end{problem}

\begin{problem} Следует ли из УЗБЧ для схемы испытаний Бернулли, что с 
вероятностью 1 для любых, сколь угодно маленьких $\varepsilon >0$ и $\delta 
>0$, можно подобрать такое $n\left( {\varepsilon ,\delta } \right)\in {\mathbb N}$, что с вероятностью, не меньшей $1-\delta $ для всех $n\ge n\left( 
{\varepsilon ,\delta } \right)$, частота выпадения герба $\nu _n $ отличается 
от вероятности выпадения герба $p$ не больше, чем на $\varepsilon $? Следует 
ли это из обычного ЗБЧ?
\end{problem}

\begin{problem} Приведите пример последовательности независимых с.в. 
$\left\{ {\xi _n } \right\}_{n\in {\mathbb N}} $ таких, что предел $\mathop 
{\lim }\limits_{n\to \infty } \frac{\xi _1 +...+\xi _n }{n}$ существует по 
вероятности, но не существует с вероятностью 1 (cм. \cite{stoianov}).
\end{problem}





\begin{problem} Докажите \textit{локальную теорему Муавра--Лапласа} в общем случае:
\[
C_n^k p^k\left( {1-p} \right)^{n-k}\sim \left( {2\pi np\left( {1-p} \right)} 
\right)^{-1 \mathord{\left/ {\vphantom {1 2}} \right. 
\kern-\nulldelimiterspace} 2}\exp \left( {-\frac{1}{2}\frac{\left( {k-np} 
\right)^2}{np\left( {1-p} \right)}} \right)
\]
равномерно по таким $k$, что $\left| {k-np} \right|\le \varepsilon \left( n 
\right)$, $\varepsilon \left( n \right)=o\left( {n^{2 \mathord{\left/ 
{\vphantom {2 3}} \right. \kern-\nulldelimiterspace} 3}} \right)$, $n\to 
\infty $, $p$ -- фиксировано.
\end{problem}

\begin{ordre}
См. книгу  Гнеденко~Б.В. \cite{2}. 
\end{ordre}

\begin{problem}
Докажите, что для с.в. $X_i \in \text{Be}(p)$, $p > 0$ выполнена локальная теорема Муавра--Лапласа:
\[
\PR\left(\sum_{i = 1}^n X_i = k \right) \sim
\left( {2\pi np\left( {1-p} \right)} 
\right)^{-1 \mathord{\left/ {\vphantom {1 2}} \right. 
\kern-\nulldelimiterspace} 2}\exp \left( {-\frac{1}{2}\frac{\left( {k-np} 
\right)^2}{np\left( {1-p} \right)}} \right).
\]
Если же $X_1,\ldots,X_n \in \text{Be}(1/n)$, то $\sum_{i = 1}^n X_i \mathop{\longrightarrow}\limits^{d} \text{Po}(1)$. Будет ли иметь место сходимость по вероятности  $\sum_{i = 1}^n X_i \mathop{\longrightarrow}\limits^{p} \text{Po}(1)$?

\end{problem}

\begin{problem}
Рассмотрим прибор, называемый ``доска Гальтона'' (см.~рис.~\ref{Fig:gam_scheme.JPG}).
\imgh{30mm}{gam_scheme.JPG}{\smallДоска Гальтона}    
Принцип работы этого устройства таков: металлические шарики поступают в самый верхний канал. Наткнувшись на первое острие, они «выбирают» путь направо или налево. Затем происходит второй такой выбор и т.д. При хорошей подгонке деталей выбор оказывается случайным. Как видно, попадание шариков в нижние лунки не равновероятно. В этом случае мы имеем дело с нормальным распределением. Объясните почему?
\end{problem}

\begin{problem}
Книга объемом $500$ страниц содержит $50$ опечаток. Оцените вероятность того, что на случайно выбранной странице 
имеется не менее трех опечаток, используя нормальное и пуассоновское приближения, сравнить результаты. 
\end{problem}

\begin{problem}
В тесто для выпечки булок с изюмом замешано $N$ изюмин. Всего из данного теста выпечено $K$ булок. Оцените вероятность того, 
что в случайно выбранной булке число изюмин находится в пределах от $a$ до $b$. 
\end{problem}

\begin{problem}
В поселке $N$ жителей, каждый из которых в среднем $n$ раз в месяц ездит в город, выбирая дни поездки независимо от остальных. 
Поезд из поселка в город идет один раз в сутки. Какова должна быть вместимость поезда для того, чтобы он переполнился с вероятностью, 
не превышающей заданного числа $\beta$? 
\end{problem}

\begin{problem}\label{cauchy_gen}
Случайные величины $X_1,\ldots,X_n$ независимы и имеют распределение Коши, т.е. 
\[
f(x) = \frac{d}{\pi(d^2 + x^2)}, 
\quad
x \in \mathbb{R}.
\]
Докажите равенство распределений $(X_1+\ldots+X_n)/n$ и  $X_1$. Противоречит ли это ЗБЧ или ЦПТ?
\end{problem}




==> title.tex <==


\thispagestyle{empty} 
\begin{center}

МИНИСТЕРСТВО ОБРАЗОВАНИЯ И НАУКИ \\
РОССИЙСКОЙ ФЕДЕРАЦИИ \\

 $ $ \\

Московский физико-технический институт \\
(государственный университет) \\
 
  $ $ \\ $ $ \\ $ $ \\
  $ $ \\
  $ $  \\
\smallskip
\smallskip
%\premierAuthors, \\
%\autresAuthors \\
 
 $ $ \\ $ $ \\
 
\textbf{СТОХАСТИЧЕСКИЙ АНАЛИЗ \\ В ЗАДАЧАХ} \\
$ $ \\
\textbf{Часть 1}
 
 $ $ \\
  $ $ \\
  $ $ \\
  $ $ \\
Учебно-методическое пособие \\
 

 
Москва -- Долгопрудный 2015


\end{center}

\newpage
